Logic Explained Networks

The large and still increasing popularity of deep learning clashes with a major limit of neural network architectures, that consists in their lack of capability in providing human-understandable motivations of their decisions. In situations in which the machine is expected to support the decision of human experts, providing a comprehensible explanation is a feature of crucial importance. The language used to communicate the explanations must be formal enough to be implementable in a machine and friendly enough to be understandable by a wide audience. In this paper, we propose a general approach to Explainable Artificial Intelligence in the case of neural architectures, showing how a mindful design of the networks leads to a family of interpretable deep learning models called Logic Explained Networks (LENs). LENs only require their inputs to be human-understandable predicates, and they provide explanations in terms of simple First-Order Logic (FOL) formulas involving such predicates. LENs are general enough to cover a large number of scenarios. Amongst them, we consider the case in which LENs are directly used as special classifiers with the capability of being explainable, or when they act as additional networks with the role of creating the conditions for making a black-box classifier explainable by FOL formulas. Despite supervised learning problems are mostly emphasized, we also show that LENs can learn and provide explanations in unsupervised learning settings. Experimental results on several datasets and tasks show that LENs may yield better classifications than established white-box models, such as decision trees and Bayesian rule lists, while providing more compact and meaningful explanations.

==> main_july_19_backup.tex <==

% \usepackage{icml2021}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[pagebackref=true,
    breaklinks=true,
    colorlinks,
    linkcolor=blue,
    citecolor=blue,
    filecolor=black,
    urlcolor=blue,
    bookmarks=false]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{caption}
\usepackage{subcaption}

\setcounter{secnumdepth}{6}


\usepackage{tikz}
% \usetikzlibrary{decorations}
\usetikzlibrary{decorations.text}
\usetikzlibrary{arrows.meta,bending,decorations.markings}


\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}

\lstset{style=mystyle}

\usepackage{pifont}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{float}
\usepackage{fontawesome}
\usepackage{makecell}

\def\UrlFont{\rmfamily}
\usepackage{fancyhdr}
\usepackage{mathrsfs}
\usepackage{color}
\usepackage{hyperref}
\usepackage{longtable}
\hypersetup{colorlinks=true}
% \usepackage[linesnumbered, ruled]{algorithm2e}


\newtheorem{definition}{Definition}[]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{example}{Example}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\graphicspath{ {./images/} }


\def\[#1\]{$$#1$$}

\def\frac#1#2{{#1\over#2}}
\def\eps{\varepsilon}

\def\bbR{{\bf R}}
\def\X{{\bf X}}
\def\meno{\medskip\noindent}

\newcommand{\draft}[1]{\textcolor{violet}{#1}}

\newcommand{\fg}[1]{\textcolor{red}{F: #1}}
\newcommand{\gc}[1]{\textcolor{red}{G: #1}}
\newcommand{\sm}[1]{\textcolor{blue}{#1}}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.5}


\title{Logic Explained Networks}

\author{Gabriele Ciravegna\thanks{Equal contribution}\hspace{1.2mm}$^{1,2}$\hspace{1.2mm}\href{https://orcid.org/0000-0002-6799-1043}{\includegraphics[scale=0.06]{orcid.png}},
Pietro Barbiero$^{*3}$\hspace{1mm}\href{https://orcid.org/0000-0003-3155-2564}{\includegraphics[scale=0.06]{orcid.png}},
Francesco Giannini$^{*2}$, \\
\textbf{
Marco Gori$^{2,4}$\hspace{1mm}\href{https://orcid.org/0000-0001-6337-5430}{\includegraphics[scale=0.06]{orcid.png}},
Pietro Li\'o$^{3}$,
Marco Maggini$^{2}$,
Stefano Melacci$^{2}$\hspace{1mm}\href{https://orcid.org/0000-0002-0415-0888}{\includegraphics[scale=0.06]{orcid.png}}
}\\
$^{1}$Università di Firenze (Italy), $^{2}$Università di Siena (Italy), \\ $^{3}$University of Cambridge (UK), $^{4}$Universitè Côte d’Azur (France)\\
\texttt{gabriele.ciravegna@unifi.it, pb737@cam.ac.uk, francesco.giannini@unisi.it}\\
\texttt{marco.gori@unisi.it, pl219@cam.ac.uk, marco.maggini@unisi.it, mela@diism.unisi.it}
}

\begin{document}
\maketitle
\begin{abstract}
The large and still increasing popularity of deep learning clashes with a major limit of neural network architectures, that consists in their lack of capability in providing human-understandable motivations of their decisions.
%Despite the increasing popularity of deep networks in real-world application, in real wold domains the employment of deep neural networks is still limited and strongly criticized due to their lack of interpretability.
In situations in which the machine is expected to support the decision of human experts, providing a comprehensible explanation is feature of crucial importance.
%providing a comprehensible explanation for a certain classification task can be crucial in decision support contexts.
The language used to communicate the explanations must be formal enough to be implementable in a machine and friendly enough to be understandable by a wide audience.
%To this aim, rule-based explanations expressed in a high-level language are particularly relevant.
In this paper, we propose a general approach to Explainable Artificial Intelligence in the case of neural architectures, showing how a mindful design of the networks leads to interpretable deep learning models called Logic Explained Networks (LENs).
LENs only require their inputs to be semantically meaningful and human understandable predicates, and they provide explanations in terms of simple First-Order Logic (FOL) formulas involving such predicates. LENs are general enough to cover a large number of scenarios. Amongst them, we consider the case in which LENs are directly used as special classifiers with the capability of being explainable, or when they act as additional networks with the role of creating the conditions for making a black-box classifier explainable by FOL formulas.
Explanations can be either local (single-example level) or global (problem level), and,
despite supervised learning problems are mostly emphasized,
%and are given as first-order logic formulas expressed in terms of input concepts.
we also show that LENs can learn to provide explanations in unsupervised learning settings.
%to provide explanations of the predictions made either by a black-box model or by the LEN itself.
We describe and evaluate three different use-cases of the LEN framework, based on multiple out-of-the-box LEN models. Experimental results on several datasets and tasks show that LENs not only yield better classifications than established white-box models, such as decision trees and Bayesian rule lists, but they also provide more compact and meaningful explanations.
\end{abstract}


\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/vis_abs.png}
\caption{Logic Explained Networks (LENs) are neural networks capable of making predictions and providing First-Order Logic explanations. In detail, A LEN (blue box -- function $f$) provides FOL explanations (purple box -- formula $\rho$\fg{replace FOL explanation with logic explanation in pink box}) of a set of output concepts (rightmost yellow-box -- output concepts belong to set $E$) in function of the LEN inputs, that might be other concepts (mid yellow box -- input concepts belong to $C$) computed by a neural network (gray box -- function $g$) and/or concepts provided within the available data (leftmost yellow box -- data belong to $X$), following the dotted connection).  %Colors are used in all figures to identify different parts of the framework: yellow boxes contain input data and concepts, output predictions and labels; grey boxes represent the black box classifier $g$ that can either provide final classification or extract low-level concepts; the blue box represents the LEN $f$; t
There are several different ways of instantiating this generic model into real-world problems, that are described in Section~\ref{sec:basics}.
Within the blue box, the key components of LENs are listed, that are the main subject of Section~\ref{sec:methods}:  Learning Criteria (Section~\ref{sec:learncrit}), FOL Rule Extractor (Section~\ref{sec:logic_rule_extr}), and the Parsimony Criteria (Section~\ref{sec:parsimony}).
}
    \label{fig:framework}
\end{figure}

\begin{figure}[h]
    \centering

     \includegraphics[width=1.\textwidth]{figs/abstract.pdf}
         \caption{An example of a possible instance of the generic model of Fig.~\ref{fig:framework}, inspired by the CUB 200-2011 fine-grained classification dataset. Classes are divided into a two-level hierarchy. {\color{red}[Add a citation to the dataset.]} A LEN is placed on top of a convolutional neural network $g(\cdot)$ in order to \textit{(i)} classify the species of the bird in input and \textit{(ii)} provide an explanation on why it belongs to this class. 
         \gc{Prendere la figura di NIPS e cambiare i colori e la figura iniziale in modo da non essere troppo simili all'altro paper.\\}
         {\color{red}[Add at least another output concept (no need to show its explanation). Avoid being to strictly close to the CUB dataset, otherwise the example is not clear. In other words, make black-footed-albatross the name of the output concept (instead of 'bird') and also add another one. Rename the input concepts with the names that are in the purple box. If they are too long, you can shorten them by renaming them in a more simple manner (hooked-bill, solid-wing, medium-size, white-throat, black-bill). Moreover, user the lower-case $x$ instead of $X$.]}\\
         \fg{da cambiare un po' l'img perchè è la stessa img di NIPS.. cambierei esempio}
         \fg{forse metterei $\forall c, billShapeHooked(c)\wedge...$}}
         \label{fig:len}

\end{figure}


\section{Introduction}
The application of deep neural networks in safety-critical domains has been strongly limited \cite{chander2018working}, since they are generally considered as black-boxes whose decision processes are opaque and too complex to understand for their users. 
%\fg{tolto perchè era identito a quello mandato a NIPS} The lack of transparency in the decision process of some machine learning models, such as neural networks, limits their application in many safety-critical domains \cite{chander2018working}. 
Employing black-box\footnote{In the context of this paper, a black-box classifier is any classifier that cannot provide human understandable explanations about its decisions} models may be unacceptable in contexts such as industry, medicine or courts, where the potential economical or ethical repercussions are calling for lawmakers to discourage from a reckless application of non-interpretable models \cite{gdpr2017,law10code,goddard2017eu,gunning2017explainable}. As a consequence, research in Explainable Artificial Intelligence (XAI) has become strategic and has been massively encouraged, leading to the development of a variety of techniques that aim at explaining black-box models \cite{das2020opportunities,brundage2020toward} or at developing effective interpretable models \cite{carvalho2019machine,rudin2019stop}.
% Some of the latter case, like decision rules, provide one of the best forms of explanations as they were originally developed for decision support systems \cite{sprague1980framework}.

The notions of \emph{interpretability} and \emph{explainability} were historically used as synonyms, however nowadays the distinction between interpretable models and models providing explanations has become more evident, as recently discussed by different authors \cite{gilpin2018explaining,lipton2018mythos,marcinkevivcs2020interpretability}.
Even if there are no common accepted formal definitions, a model is considered interpretable when its decision process is generally transparent and can be understood directly by its structure and parameters, such as \emph{linear models} or \emph{decision trees}. On the other hand, the way an existing (black-box) model makes predictions can be explained by a surrogate interpretable model or by means of techniques based on providing intelligible descriptions of the model behaviour by e.g. formal rules, saliency maps, question-answering. 
% {\color{red}[Say something on the definitions of interpretability and explainability, connected to what follows (we need to define what we mean with these terms).]}
In some contexts, the use of a black-box model may be unnecessary or even not preferable \cite{rudin2019stop}. For instance, a proof of concept, a prototype, or the solution to a simple classification problem can be easily based on standard out-of-the-box AI solutions which are interpretable by design.
However, interpretable models may generally miss to capture complex relationships among data. Hence, in order to achieve state-of-the-art performance in more challenging problems, it may be necessary to exploit black-box models that, in turn, may require an additional explanatory model to gain the trust of the user.

In the literature, there is a wide consensus on the necessity of having an explanation for machine learning models that are employed in safety-critical domains, while there is not even agreement on what an \emph{explanation} actually is, nor if it could be formally defined \cite{doshi2017towards,lipton2018mythos}.
An explanation should serve cognitive-behavioral purposes such as engendering trust, aiding bias identification, or taking actions/decisions \cite{srinivasanexplanation}. An explanation may help humans understand the black box, may allow for a deeper human-machine interaction \cite{koh2020concept}, and may engender trust on fully automated tasks. All of this is possible as long as the explanations are useful from a human perspective.
% and take into account how humans think and make decisions
In a nutshell, an explanation is an answer to a ``why'' question %\cite{miller2019explanation}.
%But what is that characterize a good explanation?
and what makes an explanation good or bad depends on ``the degree to which a human can understand the cause of a decision'' \cite{miller2019explanation}. The goodness of an explanation is intimately connected to how humans collect evidences and eventually make decisions.
In Herbert Simon's words we may say that a good explanation is \textit{satisficing} \cite{simon1956rational}, i.e. \textit{it either gives an optimal description of a simplified version of the black box (e.g. a surrogate model) or a satisfactory description for the black box itself}
% \footnote{"Decision makers can satisfice either by finding optimum solutions for a simplified world, or by finding satisfactory solutions for a more realistic world".}
\cite{simon1979rational}. However, the notion itself of explanation generally depends on both the domain of the application and who it is aimed at \cite{carvalho2019machine}.
% This is the reason why, different criteria and taxonomies
% such as the \textit{scope}, the \textit{usage} and the \textit{methodology} have been identified as key-properties to define a XAI technique \cite{das2020opportunities}.


The need for high-quality evidences is one of the main reasons why concept-based explanations are receiving ever-growing consideration. Explanations are given in terms of human-understandable symbols (the \textit{concepts}) rather than raw features such as pixels or characters \cite{kim2018tcav,ghorbani2019towards,koh2020concept}. As a consequence, they seem more suitable to serve many strategic human purposes such as decision making tasks. For instance, a concept-based explanation may describe a high-level category through its attributes as in ``a \textit{human} has \textit{hands} and a \textit{head}''.
% However, many concept-based explanations still look ambiguous, it is not obvious how to \textit{quantitatively} assess their generality, and may not be suitable for effective decision making at all.
% How much effort requires analyzing a pairwise dependence plot \cite{friedman2008predictive} or a ranking of SHAP values \cite{NIPS2017_7062} or a decision tree with depth 10 \cite{breiman1984classification} for domain experts? How much for laypeople?
% If you are looking for a quick and comprehensible answer these methodologies will not suit your needs.
While collecting high-quality evidences for an explanation is a common feature of concept-based techniques, there are very few approaches formulating hypothesis and even less providing synthetic descriptions whose validity can be quantitatively assessed \cite{das2020opportunities}.
A possible solution is to rely on a formal language that is
% synthetic but also
very expressive and closely related to natural language and reasoning, such as First-Order Logic (FOL). A FOL explanation can be considered a special kind of a concept-based explanation, where the description is given in terms of logical predicates, connectives and quantifiers, such as ``$\forall x:\ \textit{is\_human}(x) \rightarrow \textit{has\_hands}(x) \wedge \textit{has\_head}(x)$''. However, FOL formulas generally express much more complex relationships among the concepts %that are
involved in a certain explanation. Compared to other concept-based techniques, logic-based explanations provide many key advantages, that we briefly described in what follows.
% \begin{itemize}
% CLARITY
An explanation reported in FOL is a rigorous and unambiguous statement (\textsc{clarity}). This formal clarity may serve cognitive-behavioral purposes such as engendering trust, aiding bias identification, or taking actions/decisions. For instance, dropping quantifiers and variables for simplicity, the formula ``\textit{snow} $\wedge$ \textit{tree} $\leftrightarrow$ \textit{wolf}'' may easily outline the presence of a bias in the collection of training data.
% MODULARITY
Different logic-based explanations can be combined to describe groups of observations or global phenomena (\textsc{modularity}). %Different observations of the same phenomenon may have completely different %logic-based
%explanations according to their characteristics.
For instance, for an image showing only the face of a person, an explanation could be ``(\textit{nose} $\wedge$ \textit{lips}) $\rightarrow$ \textit{human}'', while for another image showing a person from behind a valid explanation could be ``(\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})  $\rightarrow$ \textit{human}''. The two local explanations can be combined into ``(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears}) $\rightarrow$ \textit{human}''.
% MEASURABILITY
The quality of logic-based explanations can be quantitatively measured
    % on independent data sets
to check their correctness and completeness (\textsc{measurability}). For instance, once the explanation ``(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})'' is extracted for the class \textit{human}, this logic formula can be applied on a test set to check its generality in terms of quantitative metrics like accuracy, fidelity and consistency.
% SIMPLIFIABILITY
Finally, FOL-based explanations can be rewritten in
    different equivalent forms such as in \emph{Disjunctive Normal Form} (DNF) and \emph{Conjunctive Normal Form} (CNF)  (\textsc{simplifiability}). Further, techniques such as the Quine–McCluskey algorithm can be used to compact and simplify logic explanations \cite{mccoll1878calculus,quine1952problem,mccluskey1956minimization}. For instance, the explanation ``(\textit{person} $\wedge$ \textit{nose}) $\vee$ ($\neg$\textit{person} $\wedge$ \textit{nose})'' can be easily simplified in ``\textit{nose}''.
% \end{itemize}


This paper presents a unified framework for XAI where a neural network, the \emph{Logic Explained Network} (LEN), is trained to \textit{solve-and-explain} a categorical learning problem integrating elements from deep learning and logic.
Differently from vanilla neural architectures, LENs can be directly interpreted by means of a set of FOL formulas. In order to implement such a property, LENs require their inputs to represent the activation scores of human-understandable concepts. Then, specifically designed learning objectives allow LENs to make predictions in a way that is well suited for providing FOL-based explanations that involve the input concepts. In order to reach this goal, LENs exploit parsimony criteria aimed at keeping their structure simple.
% learn a set of explanations of its classification results, or for the class-assignments of another classifier.
%(eventually another neural network).
There are several different computational pipelines in which a LEN can be configured, depending on the properties  of the considered problem and on other potential experimental constraints. For example, LENs can be used to directly classify data in an explainable manner, or to explain another black-box neural classifier. Moreover, according to the user expectations, different kinds of logic rules may be provided.
Due to this intrinsic versatility of LENs, what we propose can also be taught as a generic framework that encompasses a large variety of use cases.

%This versatility makes the proposed framework
%and in particular LENs
%applicable to a wide range of learning tasks and in different use cases. % by providing logic-based explanations in different use cases. % and according to different user preferences.
Fig.~\ref{fig:framework} depicts a generic view on LENs, in which the main components are reported. A LEN (blue box -- function $f$) provides FOL explanations (purple box) of a set of output concepts (rightmost yellow-box) in function of the LEN inputs. Inputs might be other concepts (mid yellow box) computed by a neural network classifier (gray box -- function $g$) and/or concepts provided within the available data (leftmost yellow box). %The output concepts are the ones that are the main subject of the explanations (e.g., they could be the classes of a classification problem). Explanations involve the inputs of the LEN.
This generic structure can be instantiated in multiple ways, depending on the final goal of the user and on the properties of the considered problem. In order to provide the reader with an initial example/use-case (different configurations are explored in the paper), we consider an image classification problem with concepts organized into a two level hierarchy. In Fig.~\ref{fig:len} we report an instance of Fig.~\ref{fig:framework} in which a CNN-based neural classifier gets an input image $X$, predicting the activations of a number of low-level concepts (organized in a vertical manner). The LEN $f$ processes such concepts, and it predicts the activation of higher-level output concepts. The LEN can provide a FOL description of each (high-level) output concept with respect to the (low-level) input ones. Another possible instance of the proposed framework consists in using the LEN to directly classify and explain some input data (that is basically the case in which the input concepts are immediately available in the data themselves, and not the output of another neural model), thus the LEN itself becomes an interpretable machine. Moreover, LENs can be paired with a black-box classifier operating on the same input data, and forced to mimic as much as possible the behaviour of the black-box, basically implementing an additional  explanation-oriented module. At a first glance, since the internal structure of LENs is subject to a number of constraints, LENs might not be as powerful as a black-box classifier. However, the versatility of LENs allows the user to customize his approach to the considered classification problem in order to find a satisfactory compromise between interpretability and accuracy.

We investigate three different use-cases that are inspired by the aforementioned instances, comparing different ways of implementing the LEN models. 
While most of the emphasis of this paper is on supervised classification, we also show how LEN can be exploited in fully unsupervised settings.
Additional human priors could be eventually incorporated into the learning process \cite{ciravegna2020constraint}, in the architecture \cite{koh2020concept}, and, following \cite{ciravegna2020constraint,ciravegna2020human}, what we propose can be trivially extended to semi-supervised learning (out of the scope of this paper).


%Furthermore, LENs can also be integrated with existing black-box classifiers to extract low-level concepts or to explain their classification results.




%The overall problem configuration of how a Logically Explained Network can be integrated with an existing classifier is shown in Fig. \ref{fig:framework} and further described in Sec. \ref{sec:use_cases}. A configuration example is reported in Fig. \ref{fig:len}.




%Out-of-the-box neural networks based on this framework span a wide range of flavors, from fully interpretable models to black-boxes providing different interpretability-VS-accuracy trade-off.
%high-quality explanations and state-of-the-art classification performance.

%Further, human priors expressed by FOL formulas can be naturally incorporated with LENs both in the learning process \cite{ciravegna2020constraint} and in the architecture \cite{koh2020concept}.

Our work contributes to the XAI research field in the following ways.
\begin{itemize}
    \item It provides a unifying framework for solving and explaining categorical learning problems with neural networks. We designed the LEN framework inspired by our previous experiences \cite{ciravegna2020human,ciravegna2020constraint}.
    \item It allows users to decide how to interconnect LENs in the classification task under investigation, and to express a set of preferences to get one or more customized explanations. We provide and experimentally evaluate three out-of-the-box preset models.
    % \item Supporting a wide range of logic-based explanations from \textit{local explanations} and \textit{node-level explanations}, explaining the prediction for an individual sample or a hidden neuron, to \textit{cluster explanations} up to \textit{class-level explanations} and \textit{global explanations}.
    \item It offers a wide range of logic-based explanations at different level of granularity, such as \textit{example}, \textit{local} and \textit{global} explanations, aiming at explaining a single sample, a subset of the available data or the whole dataset, respectively.
    \item It reports experimental results confirming how LENs generalize better in terms of model accuracy than established white-box models such as decision trees on complex boolean tasks (as observed in \cite{tavares2020understanding}).
    \item It advertises our public implementation of LENs through a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on out-of-the-box LENs, implementing different trade-offs between intepretability, explainability and accuracy. {\color{red}[This goes back to my previous comment on better defining these terms.]}
\end{itemize}

% \paragraph{Reading path}
The paper is organized as follows. Related works are described in Section \ref{sec:related}. Section \ref{sec:basics} gives a formal definition of a LEN and it describes its underlying assumptions, key paradigms and design principles. The methods used to extract logic formulas and to effectively train LENs are described in Section \ref{sec:methods}. Three out-of-the-box LENs, presented in Section \ref{sec:outofthebox}, are compared on a wide range of benchmarks in terms of classification performance and quality of the explanations, in Section \ref{sec:experiments}.
% A coding example showing how to use LENs with the associated python library is shown in Section \ref{sec:tool}.
Finally, Section \ref{sec:conclusion} outlines the social and economical impact of this work as well as future research directions.


\section{Related work}
\label{sec:related}


In the last few years, the demand for human-comprehensible models has significantly increased in safety-critical and data-sensible contexts. This popularity is justified by the emerging need for unveiling the decision process of pitch-black models like deep neural networks. To this aim, the scientific community has developed an important variety of XAI techniques, with different properties and goals. Several taxonomies have been proposed to categorize the XAI models, with partial overlapping and some ambiguities on the referred terminology. Without pretending to be exhaustive, in the following we only focus on some key-properties that are relevant to compare LENs with other existing approaches. In particular, we will describe related works considering the type of \textsc{result} they provide (feature-scoring vs. rule-based),
their specific \textsc{role} (interpretable models vs. explanation methods),
and the \textsc{scope} of the provided explanations (local vs. global). A brief summary of a few XAI works in terms of these features is reported in Tab.~\ref{tab:related_work} -- for more details on existing taxonomies we refer, e.g., to the following surveys \cite{adadi2018peeking,carvalho2019machine,marcinkevivcs2020interpretability,molnar2020interpretable}.

%\textsc{Results of Explanation Methods. }
XAI models can be differentiated according to the \textsc{result} of the produced explanation.
Most of the methods in literature usually focus on scoring or providing summary statistics of features. However, \textit{feature-scoring} methods
%
can be of scarce utility in decision support cases, whereas a comprehensible language may bring light on the black-box behaviour by identifying concept-based correlations.
% do not consider how concepts are interconnected, therefore, these explanations may not live up to the expectations.
On the other hand, \emph{rule-based} explanations are generally more comprehensible, since they usually rely on a formal language, such as FOL. Further, the learned rules can be directly applied to perform the learning task in place of the explained model.
%\textsc{Explanation Usage. }
Existing approaches has different \textsc{roles} in the XAI landscape, acting as intrinsically \emph{interpretable models} or as \emph{explanation methods}. 
As a matter of fact, the interpretability of a model can be achieved either by constraining the model to be interpretable per se (\emph{interpretable models}) or by applying some methods to get an explanation of an existing model (\emph{explanation methods}). Interpretable models are by definition {model specific}, while explanation methods can rely on a single model or be, as more commonly happens, {model agnostic}. In principle, interpretable models are the best suited to be employed as decision support systems. However, their decision function often is not smooth which makes them quite sensible to data distribution shifts and impairs their generalization ability on unseen observations \cite{tavares2020understanding,molnar2020interpretable}.
On the other hand, explanation methods can be applied to get approximated interpretation of state-of-the-art models. These methods are generally {``post hoc''}, since the explanations are produced when the training procedure is concluded.
%\textsc{Scope of Interpretability. }
A fundamental feature to distinguish among explainable methods is the \textsc{scope} of the provided explanations. \textit{Local} explanations are valid for a single given sample, while \textit{global} explanations {hold} on the whole input space. However, several models consider local explanations together with aggregating heuristics to get a global explanation.

% {\bf Methodology. }
% The algorithms employed by most XAI models can be roughly categorized into two main categories. \textit{Backpropagation}-based techniques analyze the gradients of the activation up to the input features, in order to identify the most relevant ones for the classification task. \textit{Perturbation}-based techniques, instead, observe how the machine output changes when altering a given input data. The aim of these methods is to understand which %are the most discriminative
% features (when altered) may drive the model to take different decisions.
% Nonetheless, not all algorithms belong to these two categories. In particular, \textit{Model-intrinsic} explanation methods significantly differ according to the training algorithms.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
                                    & \multicolumn{2}{c|}{\textbf{Result Type}} & \multicolumn{2}{c|}{\textbf{Scope}} & \multicolumn{2}{c}{\textbf{Role}} \\
                        & feature-scoring & rule-based & local & global & interpretable model & explanation method \\
\hline
LIME &\faCheckCircle & & \faCheckCircle            & & & \faCheckCircle  \\
SHAP &\faCheckCircle & & \faCheckCircle & & & \faCheckCircle  \\
% DeConv \cite{zeiler2014visualizing}                     &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           & \faCheckCircle         &               &                  \\
Activation Maximization & \faCheckCircle & & \faCheckCircle  &  &  & \faCheckCircle  \\
Saliency Maps &\faCheckCircle&& \faCheckCircle &      &              & \faCheckCircle \\
% Grad-CAM \cite{selvaraju2017grad}                       &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
SP-LIME &\faCheckCircle&& & \faCheckCircle &              & \faCheckCircle  \\
Class Model Visualization &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle                 \\
% TCAV \cite{kim2018tcav}                                 &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
LORE &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle \\
Anchors &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle  \\
DeepRED   &&\faCheckCircle& \faCheckCircle & \faCheckCircle &  & \faCheckCircle \\
GAM  &\faCheckCircle&&              & \faCheckCircle          & \faCheckCircle            &   \\
Decision Trees       &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
BRL                   &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
\hline
\textbf{LENs}                                           &&\faCheckCircle& \textbf{\faCheckCircle}    & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle} \\
\end{tabular}
}
\vspace{0.3cm}
\caption{Summary of related work. The first column lists a number of approaches in the context of XAI. The other columns are about different properties. See the paper text for more details and for a description of all the approaches. }
\label{tab:related_work}
\end{table}

Some of the most famous XAI techniques share the characteristics of being feature-scoring, local, post hoc methods.

Sometimes indeed, the easiest way to solve the explanation problem is simply to treat the model as a black-box and, sample-by-sample, determine which are the most important features for a prediction.
Prominent examples of algorithms falling in this area %are Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should}, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} and DeConvolution Neural Network (DeConv) \cite{zeiler2014visualizing}, which
accomplish this task by perturbing the input data.
Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should} trains a white-box model (e.g., a logistic regression) to mimic the predictions of a given model in the neighbourhood of the sample to explain. By analyzing the weights of the white-box model it identifies the most important group of pixels (superpixel).
Differently, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} computes the Shapley value of each feature by removing each of them in an iterative manner. %provides for local explanations by computing each input feature contributions in a certain prediction. In the Kernel SHAP version, the Shapley values of each feature are calculated by iteratively removing features in a similar way to what is done in LIME.
% Deconvolutional Network were initially introduce in \cite{zeiler2011adaptive} for unsupervised learning.
% Firstly introduced in \cite{zeiler2011adaptive}, DeConvolution Neural Network (DeConv) are used in \cite{zeiler2014visualizing} to %visualize the activation of a convolutional layer. In particular, they
%visually determine pixel importance for a certain prediction by analyzing how the classification output changes when part of the input image is masked.
Other important techniques %such as Activation Maximization \cite{erhan2010understanding}, Saliency Maps \cite{simonyan2013deep} and Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad}
provide the same type of explanations through gradient analysis. %Differently from the previous one, however, they determine feature importance  %in the context of Convolutional Neural Network (CNN).
Authors of Activation Maximization \cite{erhan2010understanding} firstly introduced this idea as an optimization problem. They explain the behaviour of a hidden/output unit by slightly modifying a given input data such that it maximizes its activation. An easier way to identify features causing a certain output has been found with Saliency Maps \cite{simonyan2013deep}, which project the classification loss until the input image.
% A further improvement has been introduced with Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} which allows to identify both class-specific image area and counterfactual explanations.
%They achieved this by modifying global average pooling with class activation mapping which allows to identify important image area with a single forward pass.
%
Other post hoc methods have been devised to extract global feature-scoring explanations, often starting from local explanations. %like LIME for Global Explanations \cite{ribeiro2016should} based on perturbation and Class Model Visualization \cite{simonyan2013deep} or Testing with Concept Activation Vectors \cite{kim2018interpretability} based on Backpropagation.
A submodular-pick algorithm extends the LIME module (SP-LIME) in %LIME for Global Explanations
\cite{ribeiro2016should} to provide global explanations. SP-LIME first finds superpixels of all input samples with the standard LIME module. Successively, it finds the minimum number of common superpixels that covers most of the images.
Starting from the idea of Activation Maximization, Class Model Visualization \cite{simonyan2013deep} finds the input sample that maximizes a certain class probability score in the whole input space. %Differently from Activation Maximization, here the input sample is not searched in the neighbourhood of a given sample, but in the whole input space.
Differently, LENs take a quite different perspective with respect to these methods, still inheriting several of their properties (see Tab.~\ref{tab:related_work}). A LEN aims at providing human comprehensible decision support in terms of a set of FOL rules.


Explanation methods, indeed, can also supply FOL explanations.
LOcal Rule-based Explanations of black-box decision systems (LORE) \cite{guidotti2018local} extracts FOL explanations via tree induction. The authors of \cite{guidotti2018local} focus on local rules extracted through input perturbation. For each sample to explain, a simple decision tree is trained to mimic the behaviour of the black-box model in the neighbourhood of the sample. Both standard and counterfactual explanations can then be extracted  following the branches of the tree.
Again based on LIME, Anchors \cite{ribeiro2018anchors}  also provides local rules of black-box model prediction via input perturbation. In this case, rules are not extracted from a decision tree but are generated by solving a Multi-Armed-Bandit beam search problem.
Extending the CRED algorithm \cite{sato2001rule}, DeepRED  \cite{zilke2016deepred} employs a decomposition strategy to globally explain neural networks. Starting from the output nodes, each node in a layer is explained in terms of the activations of the previous ones through a decision tree. In the end, all rules for each class are merged in a single global rule in terms of input nodes only. For a single example a single local rule can be extracted following the firing path.
The approach proposed in this paper is in some sense similar to the DeepRED algorithm. Indeed, as it will become clear in the following sections, LENs can explain the behaviour of a neural network both end-to-end and layer by layer. However, LENs can be used to explain any black-box model as far as its input and output are interpretable (Section~\ref{sec:basics}). Furthermore, LENs support different forms of FOL rules, with different scopes and goals.

Interpretable models are generally capable of providing both local and global explanations. These explanations may be based again on feature-scoring as in Generalized Additive Models (GAM) \cite{hastie1987generalized} or on FOL rules as in Decision Tree \cite{breiman1984classification} and Bayesian Rule Lists (BRL) \cite{letham2015interpretable}. Meant to overcome the non-linearity assumptions of Linear regression, GAM learns to predict the given class for each feature via decision tree. In \cite{caruana2015intelligible}, authors proposed GA$^2$M where attribute interaction is allowed at a pair level. Recently a further extension employing neural network as non-linear function has been proposed in \cite{agarwal2020neural}, which, however, lose interpretability at feature-level.
Decision trees are a greedy learning algorithm which iteratively divides input data into smaller subsets until they only contain elements belonging to the same class. Different pruning algorithms have been also proposed to simplify the resulting structure and therefore the explanations \cite{quinlan1987simplifying}. Each path of a decision tree may be seen as a decision rule, i.e., an \textit{IF-THEN} statement.
Many algorithms also focus on exactly generating set of decision rules in different ways, either with sequential covering as in \cite{cohen1995fast} or by selecting the best rules from a pre-mined set via Bayesian statistics as in BRL.
%
Interestingly, LENs can be directly used to solve a learning task, being almost interpretable per se.
Employing an interpretable by-design neural network as classifier has the advantage that the extracted explanations will perfectly match the classifier predictions.
In addition, relying on a neural network, LEN generalization performance can be much better than standard interpretable-by-design methods, that generally have a very limited representation capacity.

Summing up, the proposed approach can be used both as interpretable model and explanation method. Indeed, the flexibility of LENs allows the user to find an appropriate trade-off between interpretability and accuracy that is well suited for the task at hand.
The explanation type of LENs is in terms of FOL rules and different explanation styles, corresponding to different types of logic formulas. Such explanations are extracted with different scopes, from local rules valid on a single sample to global rules that hold for an entire class.





\section{Logic Explained Networks}
\label{sec:basics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%O
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTATION REMINDER
%\fg{mettere in tabella es alla fine del 2.1?}
% {\color{red}
% \textbf{Notation}
% X = input space (non-interpretable)\\
% Y = symbolic output space (interpretable)\\
% C = symbolic "concept" space (interpretable)\\
% E = symbolic "rule" space (interpretable)\\

% n = \# samples\\
% d = \# features of X\\
% q = \# categories of Y\\
% k = \# categories of C\\
% r = \# categories of E\\
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DISCORSINO intro su cosa è il nostro modello, cosa fa, a cosa si appoggia.. caratteristiche generali


% Differently from several existing XAI models,
We consider a general framework in which a special kind of neural network, referred to as Logic Explained Network (LEN), is used to make predictions and provide explanations about them, or it is used to  explain the behaviour of another classifier, being it another neural network or another generic black-box model. Moreover, a LEN might also be used to explain relationships among some given data.
%LENs can be defined according to different criteria and exploited in different use cases.
In this section we will formally introduce LENs and the notation used throughout the paper. Then, instead of immediately diving into the internals of LENs (Section~\ref{sec:methods}), we will focus on
the different ways in which LENs can be set up. In particular, we consider how LENs can be instantiated in the framework of Fig.~\ref{fig:len}, discussing a variety of computational pipelines (Section~\ref{sec:use_cases}), and on the type of explanations that we can ask the LEN to generate in function of our precise objectives (Section~\ref{sec:explanation_styles}). %Fig.~\ref{fig:scheme1} provides an overview of the main topics covered in this section.
In Fig.~\ref{fig:visual} (left) we provide an overview of the contents of this section.

\begin{figure}[h]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme1.png}
    \includegraphics[width=0.98\textwidth]{figs/LEN.pdf}
    % \input{tikz/framework}
    \caption{Visual overview of the organization of the paper for those sections that are about describing the whole LEN framework and the specific use-cases we selected. Starting from the nodes on the left, each path that ends to one of the nodes on the right creates a specific instance of the LEN framework. The proposed framework is generic enough to create several other instances than the ones we studied in this paper. \fg{Switch Learning criteria with FOL Rule extraction in the scheme.}} 
    \label{fig:visual}
\end{figure}

\iffalse
\begin{figure}[h]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme1.png}
    \includegraphics[width=0.6\textwidth]{figs/lens_1.pdf}
    % \input{tikz/framework}
    \caption{Basics of LENs (Section~\ref{sec:basics}). In order to setup a LEN-based model, first, the way the LENs communicate with a black-box classifier or directly with the data must be defined (what we refer to as computational \textsc{pipeline} Section~\ref{sec:use_cases}). The type of expected explanations has a direct consequence in the objective that drives the learning of the LENs parameters (\textsc{learning and explanations}, Section \ref{sec:explanation_styles}). {\color{red}[Remove the word 'explainer' from the 3 points in Pipeline.
    Remove the word 'explanations' from the white box on the right.]} 
    }
    \label{fig:scheme1}
\end{figure}
\fi

%There are different ways of letting LENs communicate with a black-box classifier

%and for which
%the main aspects on what LENs can be used for and which kind of explanation we may get with
%learning problems it applies (see Fig. \ref{fig:scheme1}).

%Let us consider a standard classification problem where a classifier f defines the membership values of

A LEN is a function $f$, implemented with a neural network, that map data falling within a $k$-dimensional boolean hypercube onto data that fall within another $r$-dimensional boolean hypercube. Each dimension is about the activation strength of what we refer to as \textit{concept}, with the strict requirement of having a human-understandable description of each \textit{input} dimension/concept.
Formally, a LEN is a mapping $f: C \rightarrow E$, where $C = [0,1]^{k}$ is the \textit{input concept space}, and $E = [0,1]^{r}$ is the so called 
\textit{output concept space} \draft{(or also \textit{explanation space})}. 
% Explanations are given in terms of the input concepts, while the $r$ output concept activations are about the truth degrees of $r$ FOL rules. Whenever a LEN has been trained, the $i$-th output concept can be directly translated into a FOL rule $\rho_i$ such as the one shown in Fig.~\ref{fig:len}. Rules can be then aggregated to different extents, altering their granularity level from a local to a more global coverage of the available data.
Explanations are given in terms of the input concepts, while the $r$ output 
% concept activations
\draft{predictions are about the validity of $r$ explanations that correspond to the}
truth degrees of $r$ logic rules. Whenever a LEN has been trained, the $i$-th output 
\draft{$f_i$}
% concept
can be directly translated into a logic rule $\varphi_i$ and \draft{eventually}
explained by a FOL formula $\rho_i$, such as the one shown in Fig.~\ref{fig:len}. Logic rules can be aggregated to different extents, altering their granularity level from a local to a more global coverage of the available data.


In order to provide a concrete meaning to the LEN model, we have to define the source of the input concept activations and how to learn the criteria that allow LENs to predict the output concepts/rules. Amongst a variety of possible configurations that are instance of Fig.~\ref{fig:framework}, we will focus on a limited set of computational pipelines in which the input and output concept spaces are defined with respect to real-world use-cases. In some of them, LENs communicate with a black-box classifier, with the goal of providing explanations of its predictions, or with the goal of exploiting its predictions to model the LEN input concept activations.
In all the cases, for each input sample, LENs provide $r$ logic explanations that might be directly associated to $r$ categories of a classification problem or they could be interpreted as $r$ generic different explanations of the input data. In the former case, LENs are trained in a supervised manner, while in the latter case they are trained in an unsupervised setting.

Before going into further details, we introduce the entities and the notation that will be used throughout the paper.
\begin{itemize}
\item We consider a scenario in which we have the use of a finite collection $\mathcal{X}$ of data samples belonging to $X\subseteq\mathbb{R}^d$ to train LENs.
\item The notation $\mathcal{C}$ indicates a finite set of samples belonging to the space $C$ of the input concepts. The data in $\mathcal{C}$ are  associated to the data in $\mathcal{X}$, i.e., \draft{there is a mapping from} each element in $\mathcal{X}$ \draft{onto} a corresponding element in $\mathcal{C}$.
    \item We use the notation $q$ to indicate the total number of classes in a classification problem. Each data sample can be associated with one or more classes. No strict conditions are posed on the potential mutual exclusivity of the different classes, thus we consider the most generic setting that spans from multi-label to single-label classification. Moreover, classes could also be organized in a structured manner, such as in hierarchy. Classes are encoded with binary targets belonging to $\bar{Y} = \{0,1\}^{q}$. We will use the notation $\bar{Y}_{(a:b)}$ to indicate a projection of $\bar{Y}$ limited to the dimensions going from index $a$ to index $b$ -- included. The function $\bar{y}(\cdot)$ returns the binary target vector associated to the data sample passed as its argument, while $\bar{y}_i(\cdot)$ returns the binary label restricted to the $i$-th class. %The classification problem might also be structured in a hierarchical manner. In this case, at each level $\ell$ of the hierarchy we have $q^{(\ell)}$ classes, $\ell \in [1,h]$.
%In the case of hierarchically organized classes, the higher-level classes are predicted in function of the ones activated at the lower levels, $g^{(\ell)}: Y^{(\ell-1)} \rightarrow Y^{(\ell)}$, $\ell \in [1,h]$, where $Y^{(0)} = X$.
\item The function $g$ is about a generic black-box neural classifier,
%\footnote{With "black box classifier" we mean that there are no assumptions on the classifier structure. The classifier architecture could be totally unknown to the logically explained network, that only requires a $[0,1]$-valued I/O.}
 where $g: X \rightarrow Y^{(u)}$ defines the membership scores of $x$ to $u$ categories, i.e.,  $g(x)=(g_1(x),\ldots,g_u(x))\in Y^{(u)}$, $Y^{(u)} = [0,1]^{u}$, $u\leq q$, with $g_i(x)=1$ (resp. $g_i(x)=0$) when $x$ belongs (does not belong) to class $i$. The $u$ categories could be exactly the ones of the considered classification problem ($u = q$) or a subset of them ($u < q$). No special conditions are enforced in the definition of $g$.
 \item The notation $\bar{f}$ is about a boolean instance of function $f$, in which each output of $f$ is projected to either $0$ or $1$.\footnote{When not directly specified, we will assume $0.5$ to be used as threshold value to compute the projection.} In order to refer to a single output of the vector function $f$ (or $\bar{f}$), the subscript will be used, e.g., $f_i$ (or $\bar{f}_i$). Similarly, for a vector $c \in \mathcal{C}$ with activation scores of concepts, $c_i$ is the $i$-th score, while $\bar{c}_i$ is the boolean instance of it.
 \item Any dimension of space $C$ includes a human-readable label. Logic rules generated by LENs will exploit such labels to give understandable name to predicates. In order to simplify the notation, whenever we provide the rule associated to a sample $c \in \mathcal{C}$, we will use the already introduced symbol $\bar{c}_i$ also to refer to the label of the $i$-th dimension. \draft{Similarly, in any FOL rule, $\bar{y}_i$ will refer to the human-understandable name of the logic predicate corresponding to the $i$-th output class.}
 \item \draft{Any output $f_i$ is associated with a human-understandable logic formula denoted by $\varphi_i$. For any $i=1,\ldots,r$,  a FOL formula related to $\varphi_i$, and eventually to a class $\bar{y}_i$, is denoted by $\rho_i$.}
\end{itemize}
The listed elements will play a precise role in different portions of the LEN framework.




\iffalse
such that:
\begin{itemize}
    \item Any input $c\in C$ consists in a $[0,1]$-valued feature or concept vector, i.e. $C \subseteq [0,1]^k$. $C$ is also said the \emph{concept space}. Concepts need to be semantically meaningful since they will be exploited to provide explanations. Many times $X=C$ if $X$ is already semantically meaningful; otherwise a mapping is required.
    \item $f$ can be any neural model, but it is required that $E\subseteq[0,1]^r$ where, for any $c\in C$, $i=1,\ldots,r$, $f_i(c)=1$   means that the $i$-th explanation holds for $c$, viceversa if $f_i(c)=0$. $f_i$ is sometimes called the $i$-th output of the LEN $f$. We refer to $E$ as the \emph{explanation space}. In standard supervised problems $E=Y$, however, LENs can also be employed in other contexts.
    % \item there is no pair $c^i,c^j\in C$, such that $\bar{f}(c^i) \neq \bar{f}(c^j)$ and $\bar{c}^i=\bar{c}^j$, where the overline notation denotes the boolean discretization (thresholded at $0.5$) of values from $[0,1]$ to $\{0,1\}$ values.
\end{itemize}



In a broad sense, a LEN for the classifier $g$ can be simply thought of as any neural model $f$ aiming at explaining the decision processes taken by $g$.

The explanations will generally hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrences or global principles among different classes.




% One of the main advantage of the proposed framework is its versatility, indeed a LEN can be defined according to different user-preferences by serving different purposes.
%In particular, the layout of a XAI pipeline based on LENs follows the definition of a few aspects concerning the classification problem under investigation and the properties of the required explanations. Setting these points allows the correct definition of a LEN in a learning problem. For clear, this is also schematized in Fig. \ref{fig:scheme1}.
LENs can be integrated in different learning problems with different classifier architectures. How the integration will take place depends on the nature of the input data and the presence of one or more concept bottlenecks among the classes under investigation. LENs can provide different kind of explanations both in supervised and unsupervised learning settings, according to user needs.
%In particular, we may be interested in individual explanation, i.e. the explanation of the decision taken by the classifier on a specific sample. However, we may also look for more general explanations, such as explaining the decisions taken for a whole class predictions, or even looking for more abstract relations among the classes.
Indeed, by now, we referred to LENs as neural networks aiming to accomplish a classification task.
%(either to explain the behaviour of a black box or to solve the classification problem itself).
However, LENs can also be used in unsupervised learning task.
In the latter case, the output of the LEN denotes the cluster-assignment.
\fi


\begin{figure}[t]
    \centering
    %\includegraphics[width=0.55\textwidth]{figs/E2E.pdf}
    $\vcenter{\hbox{\includegraphics[width=.40\textwidth]{figs/E2E.pdf}}}$ \quad %\\ \bigskip
    $\vcenter{\hbox{\includegraphics[width=.56\textwidth]{figs/e2e_explaining.pdf}}}$
    \caption{End-to-end (E2E) LENs directly work on input data that are interpretable per se and treated as concepts ($C=X$), while the output concepts are the activation scores of the classes of the dataset ($r = q$). This is a real-world example from the MIMIC II dataset (see the experimental section), where patient features are used to classify if the patient will survive 28 days after hospital recovery. Left: the LEN solves the classification problem and provides explanation, also referred to as \textit{interpretable classification}. Right: the LEN \textit{provides explanations} of a black-box classifier. {\color{red}[Replace $X=C$ with $X$ (twice). Replace $C$ with $C=X$ (twice). Add $E=[0,1]^{q}$ in place of $f(C)$ (left only). Add $E=Y^{(q)}$ in place of $f(C)$ (right only). Replace $g(C)$ with $Y^{(q)}$. Replace $Y$ (twice) with $\bar{Y}$.]}}
    \label{fig:E2EExplainer}
\end{figure}

\subsection{Computational Pipelines}
\label{sec:use_cases}
% In general, we can state that the above assumptions about the input data and the classifier are not always valid. However, in the following we will see how we can apply the LEN framework in different use cases where these conditions hold.
%Roughly speaking, a logically explained network $f$ is simply a function mapping $[0,1]$-values to $[0,1]$-values.
%, with the aim of providing itself the final classifications or to provide explanations for a classifier $g$.
%This very general definition allows the application of LENs to different contexts that can be made consistent with real-unit I/O.
%The most straightforward way of designing a computational pipeline involving LENs is to let the black-box classifier $g$ predict the activation scores of the $q$ classes and provide them to the LEN. In this way, we have $C = Y$, i.e., the LEN outpt concept space collides with $Y$. This is indeed feasible since $Y$ is bounded by a Boolean hypercube. %However, if the available data are already encoded in a symbolic manner in which the $d$ input features are actually  scores in $[0,1]$ (or in $\{0,1\}$ in the most extreme case) that can be considered the activation scores of $d$ concepts, then we can set $C = X$, and directly provide the data to the LEN.
%The output space of the LEN can be designed in multiple ways, depending on what is the final goal of the whole system. For example, it could collide with $Y$, i.e., the output space of the black-box $g$, $E=Y$, or it could be a totally new concept space.}

Amongst a large set of feasible input/output configurations of the LEN block, here we consider three different computational pipelines that are about three concrete scenarios/use-cases where LENs may be applied, that consist in what we refer to as \textsc{end-to-end}, \textsc{concept bottleneck}, and \textsc{cascading} pipelines.

%directly working on structured data; in a concept bottleneck-scenario where low-level concepts are first extracted from unstructured data (e.g. images); as a cascade of LENs providing explanations at different level of granularity.

%{\color{magenta}******* TBC ******}

% \paragraph{End-to-end explainer}
\textsc{End-to-end. } The most immediate instance of the LEN framework is the one in which the LEN block aims at directly explain, and eventually solve, a supervised categorical learning problem. In this case, we have $C = X$, and $r = q$, as shown in Fig.~\ref{fig:E2EExplainer}. In order to make the first equality valid with respect to the LEN requirements, the $d$ input features of the data in $X$ must score in $[0,1]$ (or in $\{0,1\}$ in the most extreme case), so that they can be considered as activations of $d$ human-interpretable concepts. 
%, i.e., $X=C \xrightarrow[]{f} E$.
%An E2E LEN assumes that the features of the input space are meaningful individually, i.e. they correspond to human-interpretable concepts.
%Structured datasets usually fall into this category.
Of course, in order to create these conditions in different types of datasets, generic continuous features can be either discretized into different bins or booleanized by comparing them to a reference ground truth (e.g., for gene expression data, the gene signature obtained from control groups can be used as a reference).
An End-to-End (E2E) LEN can perform a fully \textit{interpretable classification} task, having the double role of main classifier and explanation provider (Fig.~\ref{fig:E2EExplainer}, left) with $E=\bar{Y}$, or it can work in parallel with another neural black-box classifier $g$, thus {providing explanations} of the predictions of $g$ (Fig.~\ref{fig:E2EExplainer}, right) with $E = Y^{(q)}$ -- what we refer to as \textit{explaining a black-box}.
%used to explain the predictions of any black box model $g:X\rightarrow Y$,
%as shown in Fig. \ref{fig:E2EExplainer}.
The first solution is preferred when it is of fundamental importance to have a white-box classifier, while we can accept some drawbacks in terms of classification performances, due to the constrained nature of the LENs.
The second solution is instead useful in those context where the classification performance plays a key role, and we may accept approximate explanations of the decision taken.

\begin{figure}[t]
\centering
    %\includegraphics[width=0.55\textwidth]{figs/E2E.pdf}
    $\vcenter{\hbox{\includegraphics[width=.48\textwidth]{figs/CBM.pdf}}}$ \quad %\\ \bigskip
    $\vcenter{\hbox{\includegraphics[width=.48\textwidth]{figs/concept_relations.pdf}}}$
    \caption{Concept-bottleneck (CB) LEN. Left: the LEN is placed on top of a black box model $g$ which maps the input data into a first set of interpretable concepts. An MNIST-based experiments is shown (see the experimental section). Handwritten digits are first classified by $g$. A LEN is then employed to classify and explain whether the digit is even or odd -- \textit{interpretable classification}. {\color{red}[Replace $g^{(1)}(X)$ on top of the blue column of concepts with $C=Y^{(z)}$. Replace $f(g^{(1)})(X)$ with $E=[0,1]^{(q-z)}$. Remove the superscript $(1)$ everywhere here. Replace the $Y$ on the right with $\bar{Y}_{(z+1:q)}$. Replace $C$ on top with $\bar{Y}_{(1:z)}$.]} Right: MNIST digits are classified as belonging to one of the 10 classes and whether they are even of odd by a black-box $g$ (see the experimental section).  %in a Concept-bottleneck pipeline
     A LEN groups these predictions in an unsupervised manner, and analyzes the relations within each cluster -- \textit{interpretable clustering}. Supervision labels are not provided for the LEN output. {\color{red}[Replace $g(X)$ on top of the blue column of concepts with $C=Y^{(z)}$. Replace  $f(g(X))$ with $E=[0,1]^{r}$. Fix FOL Explanation of Cluster 2 (not 1).]}}
    \label{fig:CMBExplainer}
\end{figure}

% \paragraph{Concept-bottleneck explainer}
\textsc{Concept-bottleneck. }
A Concept-Bottleneck (CB) LEN is a computational pipeline in which the LEN $f$ aims at explaining, and eventually solving, a categorical learning problem in which the data in $X$ are not readily exploitable as LEN inputs, and a black-box model $g$ computes the activations of an initial set of $z$ concepts out of the available data. The LEN solves the problem of predicting $r$ new concepts from the activations of the $z$ ones, as shown in Fig.~\ref{fig:CMBExplainer} (left/right). Differently from the E2E case, there is always a neural network $g$ processing the data, and the outcome of such processing is the input of the LEN. Formally, we have $g: X \rightarrow Y^{(z)}$, while $f: (C=Y^{(z)}) \rightarrow E$.
This two-level scenario can be implemented in a way that is coherent with the already discussed example of Fig.~\ref{fig:len}, that is what we also show in Fig.~\ref{fig:CMBExplainer} (left). In this case, each example is labeled with $q$ binary targets divided into two disjoint sets, where the black-box network predicts the first $z < q$ ones, and the LEN predicts the remaining $r = q-z$.
The LEN will be both responsible of predicting the higher level concepts and of explaining them in function of the lower level concepts yielded by the black-box model, thus still falling withing the context of \textit{interpretable classification}.
 We also consider the case in which the outcome of the LEN is not associated to any known classes, thus the LEN is trained in an unsupervised manner, as shown in  Fig.~\ref{fig:CMBExplainer} (right), thus implementing a form of \textit{interpretable clustering}. In both the cases, the black-box classifier $g$ is trained in a supervised manner.\footnote{The extraction process can be either implicit, through the analysis of the latent spaces learnt by the black-box \cite{kazhdan2020now}, or explicit by training a black-box to classify specific concepts \cite{koh2020concept}.}

%in which the features of the data in $X$ are not interpretable as activations of human-understandable concepts or they are too low-level to be directly involved into compact explanations (e.g., all the pixels of an image \cite{koh2020concept}). In this case, we assume to have information to process the data in order to extract an initial set of concepts that will be provided to the LEN.
%Then, given


%In this latter setting, a model $g$ can be used to extract high-level concepts $C$ from raw features in $X$, and then producing the final classification $Y$. In this case, we may assume $g=g^{(2)}\circ g^{(1)}$ with $X\xrightarrow[]{g^{(1)}}C\xrightarrow[]{g^{(2)}}Y$.
%Given the concepts extracted from $g$, a LEN $f$ may be exploited to produce a set of explanations $X \xrightarrow[]{g^{(1)}} C\xrightarrow[]{f}E$,
% and eventually solve the classification task (if $E=Y$)
%classify and explain the categorical learning problem at a higher level of abstraction, i.e. $X \xrightarrow[]{g} C\xrightarrow[]{f}E$ %$C \xrightarrow[]{f} E$
%as shown in Fig. \ref{fig:CMBExplainer} where $E=Y$.
% or even producing itself a solution by assuming $E=Y$.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.58\textwidth]{figs/cascade.png}

      \caption{Cascading LENs, an example taken from the V-Dem classification dataset (see the experimental section). The final classification on the status of the democracy is divided into two steps.
    %   $X=C^{(1)} \xrightarrow[]{f^{(1)}} C^{(2)}\xrightarrow[]{f^{(2)}} E$.
    First, the input data/concepts $C_1$ are mapped into high-level concepts $C_2$. %$= f_1(X)$.
    High-level concepts are then used to compute the final classification. %$= f_2(f_1(X))$.
    Cascading LENs can provide explanations at different levels of granularity, implementing multiple \textit{interpretable classifications}. {\color{red}[Replace $X=C_1$ with $X$. Add $C_1$ on top of the first column of blue concepts. Replace $f_1(X)$ with $E_1 = C_2$. Replace $f_2(f_1(X))$ with $E_2$. Replace $C_2$ on top with $\bar{Y}_{(1:z)}$. Replace $Y$ on the right with $\bar{Y}_{(z+1:q)}$.]}}
    \label{fig:CascadeExplainer}
\end{figure}

% \paragraph{Cascading explainers}
\textsc{Cascading. }
Cascading LENs can be used to provide explanations by means of a hierarchy of concept layers. In particular, multiple LENs are used to map concepts into a higher-abstraction level (without the need of any black-box $g$), %Each model is trained on a concept space to predict concepts at a higher level of abstraction which will feed the next LENs $C^{(i)} \xrightarrow[]{f^{(i)}} C^{(i+1)}$.
%The final model solves and explains the more abstract classification task $C^{(m)} \xrightarrow[]{f^{(m)}} E$
as shown in Fig.~\ref{fig:CascadeExplainer}. Each LEN provides explanations of its outputs with respect to its inputs, thus cascading LENs handle multiple levels of granularity. This structure provides a hierarchy of explanations and upholds human interventions at different levels of abstraction, providing a far deeper support for human-machine interactions. We indicate with $(C_1, E_1), (C_2, E_2), \ldots, (C_m, E_m)$ the input/output concept spaces of the $m$ cascading LENs, with $C_{j} = E_{j-1}$, $j > 1$. We will consider the case in which LENs are trained in a supervised manner, thus implementing multiple \textit{interpretable classifications}.



\subsection{Learning \& Explanations}
\label{sec:explanation_styles}
%Different pipelines may be employed to solve different learning problems while (eventually) producing different explanations.
%In addition,
Each LEN module can be trained in a supervised or an unsupervised fashion, according to the preference of the user with respect to the type of explanations generated by the LEN. %The user might be interested in finding explanations that hold whenever specific categories of the considered problem are predicted, 
% that hold on a certain portion of data
%or in letting the LEN autonomously discover a set of regularities among the input concepts.
In Section~\ref{sec:use_cases}, when describing the selected computational pipelines, we made a precise distinction among \textit{interpretable classification}, \textit{explaining a black-box}, and \textit{interpretable clustering}, that represent three different preferences that the user might have in the problem at hand. These preferences impose precise constraints in the selection of the learning criteria and on the form of the FOL rules that can be obtained by the LENs. In addition to this choice, the user can select the granularity level of the logic rules, moving from \textit{example} to \textit{set}-level rules. The former are about single examples, while the latter covers more aggregated samples. While all the formal details on the learning criteria and the rule types will be provided in  Section~\ref{sec:learncrit}, here we contextualize their role with respect to the properties of the previously described computational pipelines.

Whenever LENs are exploited to both solve the classification problem and provide explanations, i.e., in \textit{interpretable classification},  they become white-box classifiers. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CMBExplainer} (left), Fig.~\ref{fig:CascadeExplainer} are all about this case. Learning is driven by supervised criteria that exploit the available supervised data in order to create the conditions for extracting different types of FOL rules. Each output concept of the LEN is associated to a target category of the considered learning problem, and LENs can provide a FOL explanation of each prediction, e.g., explanation of the target class \textit{person} with respect to the input concepts/attributes \textit{head, hands, body}.
%
In the case in which the user aim at \textit{explaining a black-box}, a LEN acts in parallel to a black-box classifier with the only goal of providing explanations, and it is forced to yield outputs that are as close as possible to the ones of the black-box, i.e., $f$ is forced to be close to $g$ on the available data samples. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right) and it does not require any supervision, since learning is driven by a coherence criterion between the outputs of $g$ and those of $f$ when processing the same data.
%
%
%For instance, in the selected computational pipelines of Section~\ref{sec:use_cases}, while most of the focus is on supervised learning, the Concept-bottleneck case is also about unsupervised learning of LENs (Fig.~\ref{fig:CMBExplainer} right).
%
%
%
%In the former case, each output concept of the LEN is associated to a target category of the considered learning problem, and LENs are developed by learning criteria that exploit the available supervisions (ection~\ref{sec:learncrit}). The rationale behind this approach it that LENs implicitly learn to predict each target class with respect to the input concepts, that are lower-level attributes. Then, LENs can provide a FOL explanation of such prediction, e.g., explanation of the target class \textit{person} with respect to the input concepts/attributes \textit{head, hands, body}. %We refer to this context as \textsc{targeted explanations}, and the learning process is driven by supervised criteria (Section~\ref{sec:learncrit}).
%Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations, i.e., in \textit{interpretable classification}, then it becomes a white-box classifier. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CascadeExplainer} (left), Fig.~\ref{fig:CMBExplainer} are all about this case.
%
%In the E2E case when $g$ is present or, more generally, whenever LENs act in parallel to a black-box classifier with the only goal of providing explanations, then LENs are forced to yield outputs that are as close as possible to the black-box, so $f$ is forced to be close to $g$. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right).
%
A user may be interested in discovering relations among different input concepts without posing any preferences on any pre-defined class.
For example, the user might be interested in discovering  co-occurrences of certain input concept activations in not-defined-before subsets of the dataset, such as $soccer\_ball \wedge foot$ for some samples in a collection of miscellaneous images.
In the case of \textit{interpretable clustering}, each output concept of the LEN is associated to a symbol that is not defined in advance, as in Fig.~\ref{fig:CMBExplainer} (right), and the activation score can be tough as a cluster membership score.
LENs yield an explanation for each of these symbols, that is about discovering relations among the input concepts. In this context, no supervisions are exploited, and the learning criterion is designed in order to cluster the input concepts into $r$ groups.

 %For instance, by analyzing the output of a multi-label classifier $C=g_1(X)$ in a CB pipeline, %with eventually several output classes,
%it could be interesting to get an explanation of the holding relationships among different classification outputs.
%For example, the user might be interested in discovering  co-occurrences of certain input concept activations, like $soccer\_ball \wedge foot$ for a set of football images.

Independently on what has been described so far, the user might decide to automatically discover regularities that are about single examples, groups of data points, an entire class, or, more generally, the whole dataset, moving from \textit{local} to \textit{global} explanations. %On the other hand, the user may also look for unbiased global explanations, like $zero\oplus one\oplus\ldots\oplus nine$, in a digit classification task.
%In both the cases, learning is driven by unsupervised criteria.
%Each output concept activation of the LEN module can be tough as a cluster membership score. Thus, another view of \textsc{untargeted explanations} can be directly related to the notion of \textit{interpretable clustering}, where LEN can provide explanation of each cluster, as shown in Fig.~\ref{fig:concept_relations} for the case of MNIST digits.
%As another example, consider the case of gene expression analysis, where neural networks are usually employed to group similar patients according to their genes activations. LENs can be used not only to perform such grouping (E2E), but also understand why such groups have been formed and in particular which are the most relevant gene activations in each group. 


%In the following we provide further insights for \textsc{targeted} and \textsc{untargeted explanations}.

%For this reason, we distinguish between the case in which LENs are trained in a supervised manner or with unsupervised criteria.

%A supervised task consists in learning and explaining a target \textit{class} with respect to a set of lower-level attributes, e.g. explanation of the class \textit{person} with respect to the attributes \textit{head, hands, body}. In this scenario LENs generate \textit{Supervised Explanations}.
%Alternatively, an unsupervised task consists in explaining hidden relations among \textit{concepts}, e.g. the classification outputs of another classifier or categorical attributes. In this scenario LENs yield \textit{Unsupervised Explanations}.
% Further, the explanation could have a global, local or even example-level validity. For instance, we may be interested in explaining a certain decision for a specific input, but also in universally valid regularities or simply most frequent co-occurrences among classes.
%In the following, we briefly discuss these two logical explanation styles %that are currently supported by the LENs framework
%which we respectively referred as \textit{Supervised Explanations} and \textit{Unsupervised Explanations}.
%In order to train a LEN to produce these %one or more of the following explanation styles, we can make use of ad hoc learning criteria, as successively discussed in Sec.\ref{sec:learncrit}


% \paragraph{Class-driven explanations}
%\textsc{Targeted explanations. }
% (local or global); \fg{richiederebbe spiegare, che mentre la LEN è vera esattamente dove la classe che spiega, la formula logica è soddisfatta dovunque.}
%Targeted explanations aim at providing a valid explanation for all the samples of a specific class.
%This may be achieved by training a LEN to provide \textit{interpretable classification} or to \textit{explain a black-box model}.
%represent different kinds of causalities for a selected class with respect to the other ones, or a set of lower-level concepts.
%Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations (E2E when no black-box is considered, CB, Cascading), then it becomes a white-box classifier.
%Learning of the LEN module is simply driven by a supervised objective function, in which $f$ is forced to be as close as possible to the corresponding $\bar{Y}$ on the available data. Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations (E2E when no black-box is considered, CB, Cascading), then it becomes a white-box classifier. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CascadeExplainer}, Fig.~\ref{fig:CMBExplainer} are all about targeted explanations. In the E2E case when $g$ is present or, more generally, whenever LENs act in parallel to a black-box classifier with the only goal of providing explanations, then LENs are forced to yield outputs that are as close as possible to the black-box, so $f$ is forced to be close to $g$. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right)., and that we refer to as \textit{explaining a black-box}

%One possibility is to use a LEN to directly accomplish a classification task. Indeed, it can provide an interpretable classification by training a LEN $f$ to satisfy $f_i\simeq Y_i$ for some $i\in\{1,\ldots,q\}$, i.e. to have $f_i(c)$ as close as possible to $Y_i(c)$ for any $c\in C$, where $Y_i(c)$ denotes the label of the $i$-th class on the input $c$, that the LEN is meant to both learn and explain. This solution is preferred when it is of fundamental importance to have a white-box classifier, while we can accept some drawbacks in terms of classification performances.
%However, we may also train a LEN $f$ to explain a black-box model $g$. Therefore, to satisfy $f_i\simeq g_i$ for some $i\in\{1,\ldots,d\}$, i.e. to have $f_i(c)$ as close as possible to $g_i(c)$ for any $c\in C$. This other solution is instead useful in those context where the classification performances play a key role and we may accept approximate explanations of the decision taken.
%It is worth noticing that when explaining a black-box model $g$, a LEN may also take into account the classifier predictions on unlabeled data, e.g. in a semi-supervised learning setting. This allows the LEN to produce explanations covering a larger set of data, but also possibly inaccurate.
%On the other hand, in the interpretable classification case the LEN learns explanations directly from (limited to) the labeled data.
% \begin{itemize}
%     \item
%     \textit{IF-Rules. } This kind of explanation provides a superset of a specific class assignment. For instance, an upper bound containing the class $flies$ can be defined according to the explanation "$flies\rightarrow bird\vee airplane$".
%     \item
%     \textit{Only IF-Rules. } In this case an explanation is required to provide a subset of a specific class assignment. A lower bound contained in the class $flies$ may be obtained with the explanation "$has\_wings \ \wedge \ has\_engine\rightarrow flies$".
%     \item
%     \textit{IFF-Rules. } An explanation  can completely characterize a certain class. For instance, the class $airplane$ can be defined according to the explanation "$airplane \leftrightarrow has\_wings\wedge has\_engine$".
% \end{itemize}
% We note that only with IFF-Rules explanations a LEN can be used for interpretable classification. Indeed, not any bird or plane can fly, so as a seagull can fly without having an engine. Hence, IF and Only IF-Rules are not suitable to correctly predict a specific class behaviour.
\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figs/E2E.pdf} \quad %\\ \bigskip
    \includegraphics[width=.48\textwidth]{figs/e2e_explaining.pdf}
    \caption{LENs Supervised Explanations: interpretable classification, where the LEN directly provides the final classification (left), or explaining a black-box model $g$ (right).}
    % Classification style: Explaining an existing classifier. Differently from the previous examples, here a LEN is used to explain the predictions made by an existing classifier $g(x)$ on the MIMIC classification task.}
    
    \label{fig:explainablevsexplanation}
\end{figure}
\fi

% \paragraph{Relations among concepts}
%\textsc{Untargeted explanations. }
%  (local or global): MI, Conversion to CNF
%A user may be interested in discovering relations among different input concepts without posing any preferences on any specific class. %For instance, by analyzing the output of a multi-label classifier $C=g_1(X)$ in a CB pipeline, %with eventually several output classes,
%it could be interesting to get an explanation of the holding relationships among different classification outputs.
%For example, the user might be interested in discovering  co-occurrences of certain input concept activations, like $soccer\_ball \wedge foot$ for a set of football images.
%Differently from the case of \textsc{targeted explanations}, the user might decide to automatically discover regularities that are not about the whole dataset, but that may hold only for a portion of the available data. On the other hand, the user may also look for unbiased global explanations, like $zero\oplus one\oplus\ldots\oplus nine$, in a digit classification task. In both the cases, learning is driven by unsupervised criteria.
%Each output concept activation of the LEN module can be tough as a cluster membership score. Thus, another view of \textsc{untargeted explanations} can be directly related to the notion of \textit{interpretable clustering}, where LEN can provide explanation of each cluster, as shown in Fig.~\ref{fig:concept_relations} for the case of MNIST digits.
%As another example, consider the case of gene expression analysis, where neural networks are usually employed to group similar patients according to their genes activations. LENs can be used not only to perform such grouping (E2E), but also understand why such groups have been formed and in particular which are the most relevant gene activations in each group. 

\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=0.58\textwidth]{figs/concept_relations.pdf}
    \caption{Automatic explanations. MNIST digits are classified as belonging to one of the 10 classes and whether they are even of odd by a black-box $g$.  %in a Concept-bottleneck pipeline
     A LEN groups these predictions in an unsupervised manner, and analyzes the relations within each cluster. Supervision labels are not provided for the LEN output. {\color{red}[Remove $g(X)$ and $f(g(X))$. FOL Explanation of Cluster 2 (not 1).]}}
    \label{fig:concept_relations}
\end{figure}
\fi

% \paragraph{Explanation Ranges}
% \textsc{Explanation Ranges. }
% As already mentioned, the explanations may hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrencies or global principles among different classes.
%\fg{aggiungere qualche esempio?}



\section{Methods}
% \section{Formulas, Criteria and Pruning}
\label{sec:methods}
This section presents the fundamental methods that are used to implement the ideas of LENs. 
% We start with the formal definition of the learning objectives (Section~\ref{sec:learncrit}), followed by the procedure that is used to extract FOL rules out of LENs for an individual observation  or in an aggregated manner (Section~\ref{sec:logic_rule_extr}). Finally, we discuss how to constraint LENs to avoid developing complex logic formulas by means of precise parsimony criteria (Section~\ref{sec:parsimony}). In Fig.~\ref{fig:visual} (middle) we provide an overview of the contents of this section.
\draft{We start by describing the procedure that is used to extract logic rules out of LENs for an individual observation  or in an aggregated manner (Section~\ref{sec:logic_rule_extr}). This procedure is common to any LEN use case. Then, we provide the formal definition of the learning objectives that may ensure LENs output to provide required types of logic explanations  (Section~\ref{sec:learncrit}).}
Finally, we discuss how to constraint LENs to avoid developing complex logic formulas by means of precise parsimony criteria (Section~\ref{sec:parsimony}). In Fig.~\ref{fig:visual} (middle) we provide an overview of the contents of this section.



\iffalse
\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme2.png}
    \includegraphics[width=0.85\textwidth]{figs/lens_2.pdf}
    % \input{tikz/methods}
    \caption{Inside the LEN block (Section~\ref{sec:methods}). We distinguish among three categories of methods that implement the principles behind LENs: learning criteria (Section~\ref{sec:learncrit}), FOL rule extraction (Section~\ref{sec:logic_rule_extr}), and parsimony criteria (Section~\ref{sec:parsimony}). {\color{red}[Swap cluster-level and class-level explanations. Rename example-level explanations with 'Example-level (local)'. Rename 'Class-level explanations' with 'Class-level (global). Do the same for 'cluster-level expl.']}}
    \label{fig:scheme2}
\end{figure}
\fi







% \subsection{FOL Rule Extraction}
\subsection{\draft{Extraction of Logic Explanations}}
\label{sec:logic_rule_extr}



Once a LEN has been trained, it can be associated one logic formula to each output concept $f_i$. As it will become clear shortly, extracting logic formulas out of a trained LEN can be done by inspecting its inputs/outputs accordingly to a boolean interpretation of them. 
We indicate with $\varphi_{i,\cdot}$ the logic explanation of the output concept $i$, where the second subscript can index either a single data sample $c$, $\varphi_{i,c}$, or a \draft{set} $S$ of data samples, $\varphi_{i,S}$. 
% Whenever this is independently done for each single input sample, we get back \textsc{example-level explanations}, that we also refer to as \textit{local explanations}. Differently, whenever the explanations covers an entire category of examples, we talk about \textit{global explanations}, distinguishing between \textsc{class-level explanations} and \textsc{cluster-level explanations}. {\color{red}[I still don't understand what kind of explanations we can provide]}
\draft{In practice, $S$ denotes the sub-portion of the concept space that is covered by the $i$-th explanation, i.e. the set of concept tuples for which the corresponding formula $\varphi_{i,S}$ is true. By aggregating over multiple samples we may vary the scope of the logic formula from strictly local \textsc{example-level explanations} ($S=\{c\}$) to \textsc{set-level explanations} ($S\subseteq \mathcal{C}$), where eventually $S=\mathcal{C}$ in case of global logic formulas holding on the whole sampled concept space $\mathcal{C}$.}
%%%Old pieces
% Whenever this is independently done for each single input sample, we get back \textsc{example-level explanations}, that can be aggregated into \draft{\textsc{set-level explanations}}. 
% We refer to such explanations as \textit{local}, since their corresponding formulas only hold on a sub-portion of the concept space. However, local explanations can be combined and reformulated as \textit{global} explanations according to Eq. \ref{eq:dnf2cnf}.
%%%

 %As already mentioned, the explanations may hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrences or global principles among different classes.

% The logic formula becomes human understandable whenever concepts appearing in such a formula are replaced with human-interpretable strings that represent their name (similar consideration holds for $\hat{f}^i$, in what follows)

In detail, any LEN $f=(f_1,\ldots,f_r)$ requires both its inputs and outputs to belong to the real-unit interval. 
This apparent limitation allows any $f_i$, for $i=1,\ldots,r$, to be easily \draft{associated with a logic formula according to the following procedure.
First,  its I/O are thresholded, e.g., with respect to $0.5$, to obtain a set of boolean values. Then we build an \textit{empirical truth-table} $\mathcal{T}^i$ by concatenating the $k$-columns of booleanized input concept tuples $\bar{c}$, for $c\in\mathcal{C}$, with the column of the corresponding outcomes $\bar{f}_i(c)$ (left-side of Fig. \ref{fig:tt2form_freq}). 
The truth-table $\mathcal{T}^i$ can be converted into a logic formula $\varphi_i$ in Disjunctive Normal Form (DNF) as usually done in literature \cite{mendelson2009introduction}.
However, since any $f_i$ will depend only on a proper subset of $m_i < k$ concepts, according to a certain parsimony index (Section \ref{sec:parsimony}), the formula $\varphi_i$ will be built according to the restriction of $\mathcal{T}^i$ to the columns $1,\ldots,m_i$, see e.g. Fig.~\ref{fig:tt2form}.}
In order to better point out the described procedure, 
we define the set $O_i = \{c\in \mathcal{C}:\ \bar{f}_i(c)=1\}$ as the set of all the sampled concept tuples that make true the $i$-th output explanation, i.e., the \emph{support} of $\bar{f}_i$. %For instance, if we are interested in targeted explanations only, any $O_i$ will generally consist in the set of inputs that are classified as belonging to the $i$-th class by the LEN.
% \paragraph{Local Explanation}
% \paragraph{Example-Level Explanation}

%Each output concept $i$ is associated to one of more explanations $\varphi_i,\cdot$, depending on its granularity level. In what follows, we described the case 

\textsc{Example-level explanations. }
Given $c\in O_i$, the booleanization of its continuous features may provide a natural way to get a logical explanation at example-level $\varphi_{i,c}$ as a logic formula. To make logic formulas more human understandable, the overline notation over concepts denotes here human-interpretable strings (or their negation) that represent their name.
\begin{equation}
    \varphi_{i,c} = \tilde{c}_1\wedge\ldots\wedge\tilde{c}_{m_i} \qquad\mbox{where } \tilde{c}_j:=
    \begin{cases}
        \bar{c}_j, & \mbox{if }c_j \geq 0.5\\
        \neg \bar{c}_j, &\mbox{if } c_j < 0.5\\
    \end{cases}\ ,
    \mbox{ for $j=1,\ldots,m_i$.}
    \label{eq:locexp}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/truth-table-counter.png}
    \caption{Aggregation of concept tuples with the same booleanization yields a common example-level explanation, and do not complicate the class-level explanation. For any example-level explanation, we may count how many samples it explains. Infrequent explanations may then be pruned to avoid explanation overfitting.}
    \label{fig:tt2form_freq}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=0.8\textwidth]{figs/truth-table.png}
    \caption{Extracting a logic formula from the truth-table of a binary boolean function $\bar{f}$. \fg{change figure: remove <->, ->, $\bar{f}$ and equality symbols, from the explanations.}}
    \label{fig:tt2form}
\end{figure}



% \paragraph{Aggregated Explanation}
\textsc{Set-level explanations. }
By considering Eq. \ref{eq:locexp} for any $c\in S$, with $S\subseteq O_i$, and aggregating all the example-level explanations, we may easily provide an explanation for a set of samples.
\begin{equation}
    \varphi_{i,S} = \displaystyle\bigvee_{c \in S}\varphi_{i,c} = \displaystyle\bigvee_{c \in S}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_{m_i}
\label{eq:agg_exp}
\end{equation}
\draft{In case $S=O_i$, we simply write $\varphi_i$ in place of $\varphi_{i,S}$ and we refer to it as the \textsc{class-level explanation} of the $i$-th output concept $f_i$.}
% \textsc{Class-level explanation. }
% By considering Eq. \ref{eq:agg_exp} with $S=O_i$, i.e., aggregating all the example-level explanations of class $i$, we get an overall explanation $\varphi_i$ for the LEN output $f_i$.
% \begin{equation}
%     \varphi_i = \displaystyle\bigvee_{c \in O_i}\varphi_{i,c} = \displaystyle\bigvee_{c \in O_i}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_{m_i}.
% \label{eq:glo_exp}
% \end{equation}


%%%%tolto pezzo regole messo in sec learning criteria
%%%%

\begin{example}
\label{ex:xor}
Let's consider the boolean $xor$ function, defined by $xor(0,0)=xor(1,1)=0$, $xor(1,0)=xor(0,1)=1$.
Let $f$ be a LEN that has been trained to approximate the $xor$ function in the input space $C=[0,1]^2$. Then, if we consider e.g. the inputs $c^1=(0.2,0.7)$, $c^2=(0.6, 0.3)$, we get $\bar{c}^1=(0,1)$, $\bar{c}^2=(1,0)$, and therefore $\bar{f}_1(c^1)=\bar{f}_1(c^2)=1$. These examples yield respectively the example-level explanations $\varphi_{1,c^1}=\neg \bar{c}_1\wedge \bar{c}_2$ and $\varphi_{1,c^2}=\bar{c}_1\wedge\neg \bar{c}_2$, and the class-level explanation for $f_1$ is given by $\varphi_1=(\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)$. In the same way, we may get the class-level explanation for the output $f_0$. 
% In the end, the following formulas represent the supervised explanations of the false and true classes, respectively:
% \[
% \forall c:\ \bar{f}_0(c)\leftrightarrow (\neg \bar{c}_1\wedge\neg \bar{c}_2)\vee(\bar{c}_1\wedge \bar{c}_2)\qquad\mbox{and}\qquad
% \forall c:\ \bar{f}_1(c)\leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)
% \]
The two class-level explanations correctly match the truth-table of the boolean $xor$ function.





% If we then consider that $f$ is composed of two hidden and one output neurons, we may want to explain the behaviour of each node. In particular, we may get that the first hidden neuron is represented by $ \tilde{h}_1^1  \leftrightarrow \neg \textit{c}_1\wedge \textit{c}_2$
% while the second $ \tilde{h}_2^1  \leftrightarrow \textit{c}_1\wedge \neg \textit{c}_2$. The output neurons $h^2 = f$ can be also represented in terms of the hidden neurons $f \leftrightarrow h_1^1 \vee h_2^1$ which in turns can be described again in terms of input concepts $f \leftrightarrow (\neg \textit{c}_1\wedge \textit{c}_2) \vee ( \textit{c}_1\wedge \neg\textit{c}_2)$.

\end{example}





Finally we mention that both example and set-level explanations can be recursively applied in case a cascading LEN or a single LEN with multiple $[0,1]$-valued layers are considered. For instance, given a cascading LEN as the one of Fig.~\ref{fig:CascadeExplainer}, we may get both example and class-level explanations of the concepts in $E_1 = C_2$ with respect to the ones in $C_1$, so as the concepts in $E_2$ with respect to the ones in $C_2$ and, in turn, in $C_1$. The modularity of logic formulas allows the composition of concepts at different levels that may express arbitrary complex relationships among them.



\draft{Logic explanations $\varphi_{i,S}$ generally hold only on a sub-portion $S$ of the sampled concept space $\mathcal{C}$.
% In the case in which the maximum MI criterion (Eq. \ref{eq:MI}) is used to drive the learning problem, each $\varphi_i$ will generally hold on a sub-portion of the concept space $O_i\subseteq C$. {\color{red}[This is also true for the supervised case, what is the difference?]}
However, we may get a logic formula providing an explanation holding everywhere by means of the disjunction
$\varphi = \varphi_1\vee\ldots\vee\varphi_r$, if we assume $O_1\cup\ldots\cup O_r=\mathcal{C}$.} Since $\varphi$ can turn out to be of little significance, if we are interested in simpler (and clearer) global explanations we may  convert $\varphi$ into an equivalent $\varphi'$ in \emph{Conjunctive Normal Form} (CNF). In particular, will there exist $r'$ and some clauses $\varphi'_1,\ldots,\varphi'_{r'}$ such that:
\begin{equation}
    \varphi=\bigvee_{i=1}^r\varphi_i \equiv \bigwedge_{i=1}^{r'}\varphi'_i=\varphi'.
\label{eq:dnf2cnf}
\end{equation}
As a result, we get a set of $r'$ explanations holding on the whole $\mathcal{C}$, indeed  $\varphi'_i(c)=1$ for every $c\in \mathcal{C}$, $i=1,\ldots,r'$.
Unfortunately, converting a boolean formula from DNF into CNF can lead to an exponential explosion of the formula.
% \fg{in che senso?}; in the following, we will see how to address this problem.
However, after having converted each $\varphi_i$ in CNF, the conversion can be computed in polynomial time with respect to the number of minterms in each $\varphi_i$ \cite{russell2016artificial}.



% \paragraph{Remarks}
The methodologies described so far illustrate how logic-based explanations can be aggregated to produce a range of explanations, from the characterization of individual observations to formulas explaining the model predictions for all the samples producing the same output concept.
The formula for a whole class can be obtained by aggregating all the minterms corresponding to example-level explanations of all the observations having the same concept output.
In theory, this procedure may lead to overly long formulas as each minterm may increase the complexity of the explanation. In practice, we observe that many observations share the same logic explanation, hence their aggregation does not change the complexity of the class-level formula (right-side Fig. \ref{fig:tt2form_freq}). In general, class-level explanations can be provided by aggregating just the most common explanations extracted from samples with the same output concept, avoiding a sort of "explanation overfitting" with the inclusion of noisy minterms which may correspond to outliers. To summing up, a possible limitation of this approach can be the readability of the logical rules, for instance in case (i) the number of input \draft{concepts} (the length of any minterm) $k \gg 1$, (ii) the size of the support $|O_i|$ is very large (possibly getting too many different minterms for any $f_i$). For these reasons, possible approaches to maintain an easy-to-understand set of very concise logical rules are fundamental to provide an useful explanation, e.g. as decision support. More details on how to select the most meaningful explanation terms are provided in Section \ref{sec:parsimony}.



\subsection{Learning Criteria}
\label{sec:learncrit}

\draft{We just saw how a logic rule $\varphi_i$ can be associated to an output concept $f_i$. However to improve the expressiveness of logic explanations, in what follows any formula $\varphi_i$ will be considered as a FOL formula, where any $\bar{c}_j$ is thought of as a logic predicate defined on the concept space $C$, and such that $\bar{c}_j(c)=1$ if and only if $c_j>0.5$, for any $c\in C$. In addition, if for instance $\varphi_i=\bar{c}_2\wedge\neg \bar{c}_5$, we will write $\varphi_i(c)$ for $\bar{c}_2(c)\wedge\neg \bar{c}_5(c)$. 
}
Following the distinction among the user preferences introduced in Section~\ref{sec:explanation_styles}, this subsection focuses on the loss functions that are optimized to train a LEN to develop the capability of providing explanations accordingly to such preferences, that are the outcome of our previous experiences in \cite{ciravegna2020constraint,ciravegna2020human}.
For simplicity, here we will not distinguish among the different computational pipelines, thus referring to a single generic LEN block with $r$ output units in all the cases of \textsc{interpretable classification}, \textsc{explaining a black-box} and \textsc{interpretable clustering}.







\textsc{Interpretable classification. }
%In the case of \emph{Supervised Explanations}, we aim at providing explanations of certain classes. In this sense, we want our model $f$ to be active whenever the class we aim to explain is also active.
% (i.e. $f_i(c) = Y_i(c) = 1$)
% We do not distinguish here whether the LEN is performing an \textit{interpretable classification} ($f_i\simeq Y_i$) or it is \textit{explaining an existing classifier} ($f_i \simeq g_i$), since for what concerns the optimization function it does not make any difference.
%Let us assume the interpretable classification case. The case of explaining a black-box model $g$ can be obtained by replacing $Y_i(c)$ with $g_i(c)$ in the loss unctions. The only difference in the two cases is that while $Y_i(c) \in \{0, 1\}$ is a discrete membership function, $g_i(c) \in [0,1]$ provides the probability of class assignment.
%Further, for sake of simplicity, in what follows we will assume $f: C=X\rightarrow E=Y$.
\draft{Training a LEN by supervised learning is what is needed in order to create the conditions to extract explanations for specific categories, i.e. to bind a logic explanation provided by $\varphi_i$ to a specific output class of a classification problem. By denoting with $\bar{y}_i$ the binary predicate associated to the name of the output class $i$, we will consider three kind of FOL explanations $\rho_i$ (as reported by the equations (\ref{eq:FOLexplIF})-(\ref{eq:FOLexplIFF})) expressed as the universal closure of an IF, Only IF or IFF rule, between $\varphi_i$ and $\bar{y}_i$.
%
These rules can be enforced in case of interpretable classification according to the following learning criteria.
% $\varphi_i$ can be related to the class $i$, by training the corresponding output $f_i$ of a LEN with supervised learning. 
}

IF rules mean that, in the extreme case, for each example of class $i$ we want the $i$-th output of the LEN to score one (and not necessarily vice-versa). In other words, \draft{the set of concept tuples $c$ belonging to the $i$-th class, i.e. such that $\bar{y}_i(c)=1$ has to be included in the support of $\bar{f}_i$.}
This behavior can be achieved by minimizing a hinge loss,
\begin{equation}
L_{\rightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \max\{0, \bar{y}_i(c) - f_i(c)\}\qquad  i \in [1,  r].\label{eq:IF}
\end{equation}
 Following a symmetric approach, in Only IF rules it may be the case of a class to be explained in terms of some lower-level concepts. This principle is easily enforced by switching the two terms of the loss function in Eq. \ref{eq:IF},
\begin{equation}
L_{\leftarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \max\{0, f_i(c) - \bar{y}_i(c)\}\qquad  i \in [1,  r].\label{eq:IF2}
\end{equation}
Both in IF and Only IF rule, in order to make the learning problem well posed, further conditions on $f$ must be included, to define its behaviour in the space areas not covered by the data and to avoid trivial solutions with constant $f$.

At last, LEN can learn double implication rules (IFF) in which an explanation can completely characterize a certain class. %These rules require the support of the LEN and the support of the class to be strictly equal.
%For this reason,
Any function penalizing points for which $f_i(c)\neq \bar{y}_i(c)$ may be employed in this scenario, such as the the classic Cross-Entropy loss,
\begin{equation}
L_{\leftrightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \bar{y}_i(c)*log(f_i(c)) + \left( 1-\bar{y}_i(c) \right) *log \left( 1-(f_i(c)) \right)
% L_{\leftrightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} |f_i(c) - \bar{y}_i(c)|^2 \qquad  i \in [1,  r], 
\label{eq:IFF}
\end{equation}
%IFF loss function is preferred when a LEN performs E2E \textit{interpretable classification}, since we want the output of $f$ to be as close as possible to $\bar{Y}$ in order to maximize the classification accuracy.
% In this latter case if we want the same LEN to explain different, mutually exclusive classes, a Softmax activation function can be also employed.
\draft{
In any of these cases (equations (\ref{eq:IF})-(\ref{eq:IFF})), we provide a logic explanation in First-Order Logic by means of the following equations, by introducing the FOL formulas $\rho_i$ for $i=1,\ldots,r$, ranging on the whole concept space $C$. 
\begin{align}
\text{IF-rule}: \qquad &  \rho_i = \forall c\in C:\ \bar{y}_i(c)\rightarrow\varphi_i(c). \label{eq:FOLexplIF}\\ 
     \text{Only IF-rule}: \qquad  & \rho_i = \forall c\in C:\ \varphi_i(c) \rightarrow  \bar{y}_i(c) \label{eq:FOLexplFI}\\
     \text{IFF-rule}: \qquad & \rho_i = \forall c\in C:\  \bar{y}_i(c) \leftrightarrow \varphi_i(c)\label{eq:FOLexplIFF}
\end{align}
In the same way, in case of a concept-bottleneck pipeline, we may still derive a FOL explanation according to a certain function $g:X\to C$ extracting LEN input concepts from raw features. For instance for the IFF-rule, we will get
\begin{equation}
\rho_i=\forall x \in X:\ \bar{y}_i(g(x))\leftrightarrow\varphi_i(g(x))
\label{eq:FOLexplCB}
\end{equation}
To be precise, the logic predicate $\bar{y}_i$ appearing in the equations (\ref{eq:FOLexplIF})-(\ref{eq:FOLexplCB})
should be thought of as a \textit{virtual} predicate denoting the membership of a certain concept tuple $c\in C$ to the $i$-th output class. However, assuming it coincides with the available class labels of concept in $\mathcal{C}$, then the previous FOL formulas are correctly verified for any $c\in\mathcal{C}$.
%
% In particular, any $f_i$ will be related to class labels $\bar{y}_i$ or class predictions $g_i$ for the interpretable classication and explaining a black-box cases, respectively. 
Despite the correspondence between $f_i$ and $\bar{y}_i$ can be enforced only on the sampled concept  space $\mathcal{C}$, we assume that any $\rho_i$ can generalize to unseen concept tuples in the whole concept space $C$.
}

















%%%%%%%%%%%%%%CUT

\textsc{Explaining a black-box. } In this case, the output of the LEN is forced to mimic the one of a black-box \draft{$g:C\rightarrow Y$}. A coherence loss can be exploited to reach this goal,
\begin{equation}
L_{\leftrightarrow}(g_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} g_i(c)*log(f_i(c)) + \left( 1-g_i(c) \right) *log \left( 1-(f_i(c)) \right)
 \label{eq:coher}
\end{equation}
\draft{As in the interpretable classification case, IF, Only IF and IFF rules can be expressed according to the equations (\ref{eq:FOLexplIF})-(\ref{eq:FOLexplCB}). However, now the FOL explanations will be guaranteed to hold assuming that $\bar{y}_i$  coincides with the black box predictions $g_i(c)$ for $c\in\mathcal{C}$.
}
%
% In particular, any $f_i$ will be related to class labels $\bar{y}_i$ or class predictions $g_i$ for the interpretable classication and explaining a black-box cases, respectively. 

%the explanations provided by LENs are first-order logic formulas, and this newly devised pieces of knowledge can be reused and enforced on the output of the classifier $g$. This is commonly considered in the generic \emph{learning from constraints} framework \cite{gnecco2015foundations}, and it may be of particular interest, especially for semi-supervised settings. A similar strategy has already been considered e.g. in \cite{ciravegna2020constraint}, where a set of FOL formulas have been, at first extracted from data, and then converted into continuous loss functions to be injected in the learning objective.
%At last, the extracted formulas can also be used to check the behaviour of the classifier on test data, e.g. to detect adversarial samples as done in \cite{melacci2020domain}.

\textsc{Interpretable clustering. }
% \paragraph{Mutual Information Criterion}
% \paragraph{Relations among Concepts.}
Generic explanations can be achieved by means of fully unsupervised  principles from Information Theory. As a matter of fact, the maximization of the Mutual Information (MI) index between the input concept space $C$ and the output concept space $E$ allows the LEN to
be trained in a fully unsupervised way \cite{ciravegna2020constraint}. More specifically, a max-MI criterion (see \cite{melacci2012unsupervised} for further details) leads to the development of a LEN that has the tendency of producing 1-hot activation scores, such that $\forall c \in \mathcal{C}$ only one $f_i(c) \simeq 1$, while the others are close to zero. In a sense, it enforces the LEN to cluster the data in a way that each input sample belongs to a single cluster.
In order to define the MI index, we have to model the probability distribution $P_{i|c}(f)$, that is the probability of $f_i$ to be active (close to 1) on sample $c$ -- we implemented it using the softmax operator on the LEN output. %Following the classic notation of discrete MI,
%$E$ is a discrete random variable associated to the output of the LEN functions while $C$ is the variable related to the data in the concept space.
The penalty term to minimize to train the LEN is minus the MI index,
\begin{equation}
    L_{MI}(f,\mathcal{C}) = - H_{E}(f,\mathcal{C}) + H_{E|C}(f,\mathcal{C}) \ ,
	\label{eq:MI}
\end{equation}
where $ H_{E}$ and $ H_{E|C} $ denote  the entropy and the conditional entropy functions associated to the aforementioned probability distribution, respectively, and measured over the whole $C$, as in  \cite{ciravegna2020constraint}. \fg{ma non sarebbero solo su $\mathcal{C}$?}
%An outcome of the maximization of the MI index is that the supports of the explaining functions will tend to partition the input space $X$, i.e., $X=\bigcup_{j=1}^mX_j$ and $X_j\cap X_k=\emptyset$, for $j\neq k$ (see \cite{melacci2012unsupervised,betti2019cognitive} for further details).
\draft{
In this case, the support $O_i$ of $\bar{f}_i$ is exactly the cluster of data points where the $i$-th output of the LEN is active. Leaving $\varphi_i$ free to relate concepts in a pure unsupervised manner, we simply get the FOL explanation
\begin{equation}
\rho_i=\forall c \in O_i:\ \varphi_i(c)
\label{eq:FOLexplMI}
\end{equation}
}

Of course, in all the computational pipelines in which a classifier $g$ is also employed,
%In the particular case of a LEN providing explanations for an existing classifier $g$,
the available supervision is enforced on $g$ as well, e.g., by means of the Cross-Entropy loss. As a side note, we remark that what we are describing in a fully supervised setting can be trivially extended to the semi-supervised one, as we already investigated in \cite{ciravegna2020constraint,ciravegna2020human}.






\subsection{Parsimony criteria} \label{sec:parsimony}
When humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one \cite{aristotlePosterior,mackay2003information}. Over the years, researchers have proposed many approaches to integrate "\textit{the law of parsimony}" into learning machines.
Here we describe a few fundamental parsimony criteria which may help in developing and implementing a variety of Logically Explained Networks. A specific combination of the following methodologies may be adopted or ignored depending on end-user requirements on the explanations and on the classification performance.
% \subsubsection{Occam's razors}
% \paragraph{Occam's razors}
% \textsc{Occam's Razors. }
Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous techniques to put in practice the Occam's razor principles in the fields of statistics and machine learning.
Among such techniques, $L1$-regularization \cite{santosa1986linear} has been recently shown quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages weight sparsity \cite{tibshirani1996regression}:
% \begin{equation}
    $\lambda ||W||_1$.
% \end{equation}
By shrinking the less important weights %'s values
to zero, this regularization technique completely removes some weights %altogether in the limit,
leading to sparse configurations. This allows to ignore the associated input features and, therefore, to provide simpler explanations. For this reason, all out-of-the-box LENs presented in the next section are trained using this parsimony criterion.

\subsubsection{Pruning strategies}
\label{sec:pruning}
The action of parsimony criteria, such as regularizers or human priors, influences the learning process %of learning machines
towards specific local minima. Once the model has finally converged to the desired region of the optimization space, the effort can be speed up and finalized by pruning the neural network \cite{lecun1989optimal,hassibi1993second}. The pruning strategy has a profound impact both on the quality of the explanations but also on the learning capacity model and, as a result, on the classification performance as well \cite{frankle2018lottery}. Here we present three effective pruning strategies specifically devised for LENs.

% \paragraph{Node-level pruning}
\textsc{Node-level pruning. }
A straightforward approach to pruning consists in defining the maximum \textit{fan-in} (number of non-pruned connections) for each neuron of a feed-forward neural network. We refer to this strategy as \textit{Node-level pruning}.
%A fan-in pruning strategy generates a feed-forward graph where each neuron has the same number of incoming non-pruned connections.
At the end of the training process, the absolute value of the weight matrix $W_i$ is computed for each layer $i=1,\dots,L$.
The node-level approach prunes one by one the weights with the smallest absolute value, such that each neuron in the network has a fixed number of incoming non-pruned weights $q \geq 2$. The parameter $q$ must be decided a priori and determines the learning capacity of the pruned model as well as the complexity of the logic formulas which can be extracted. To get reasonably simple explanations, the parameter $q$ may range between $2$ and $9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Recent work on explainer networks has shown how node-level pruning strategies may lead to fully explainable models  \cite{ciravegna2020constraint}. However, we will show in the experimental section that this pruning strategy strongly reduce the classification performances.

% \paragraph{Network-level pruning}
\textsc{Network-level pruning. }
In order to overcome the heavy reduction of the learning capacity of the node-level pruned models, we introduce here the \textit{Network-level pruning}.
Indeed, the main aim of pruning is to only reduce the number of input terms involved in the final explanations. By directly limiting the number of input features considered by the network, we can achieve this result with a lighter impact on the overall model.
At each iteration step, the Frobenius norm of the first-layer weight matrix $W_1$ is computed: $w_1 = ||W_1||_2$. The vector $w_1$ is then re-scaled in the interval $[0,1]$:
\begin{equation}
    w_1' = \frac{w_1}{\max w_1}
\end{equation}
In this way, $w_1'$ gives a normalized score to rank input feature by importance. The \textit{Network-level strategy} consists in pruning all the input features where $w_1' < \tau$, where $\tau$ is a threshold set a priori (usually $\tau = 0.5$). Alternatively, %the $\mu$ approach may
we can also retain the $q$ most important input features and prune the others for the entire first layer, as done in the \textit{Node-level pruning} for each single node. %The parameter $q$ is user-defined and may range between $2$ and $9$ to get sensibly compact explanations \cite{miller1956magical,cowan2001magical,ma2014changing}.
This pruning strategy is far less stringent compared to the node-level pruning as it affects only the first layer and it does not prescribe a fixed fan-in for each neuron.

% \paragraph{ReLU pruning}
% \paragraph{Example-level Pruning}
\textsc{Example-level pruning. }
Example-level pruning is a particular strategy exploiting the well-studied local linearity property of neural networks whose activation functions in all hidden layers are Rectified Linear Units (ReLu Networks) \cite{hahnloser2000digital}.
% \paragraph{Local Linearity}
For any input $x \in \mathbb{R}^d$, the initial Directed Acyclic Graph (DAG) ${\cal G}$ describing the structure of a ReLu Network, is reduced to ${\cal G}_{x}$,
which only keeps the units corresponding to active neurons and the corresponding arcs (firing path).
Since all neurons operate in ``linear regime'' (affine functions), as stated in the following,
the transformation $z: X \rightarrow Y$, which  is the composition of affine functions, corresponds to a single affine function $f^*(x) = W x + b$.
\begin{theorem}
	Let $\{h_1,\ldots,h_L \}$ a collection of affine functions, where
% 	\[
		$h_{i}: X_{i} \mapsto Y_{i}: x \mapsto W_{i} x + b_{i}$
% 	\]
	and $\forall i=1,\ldots, L-1: \ \ X_{i+1} \subset Y_{i}$, then,
% 	\[
		$z(x) = h_{L} \circ h_{L-1} \circ \dots \circ h_{2} \circ h_{1} x.$
% 	\]
	is affine and we have $f^*(x) = W x + b$, where
	\begin{equation}
	    W(L) = \prod_{\kappa=1}^{L} W_{\kappa}, \qquad
		b(L) = \sum_{\kappa=0}^{L-1}  b_{L-\kappa} \prod_{h=0}^{\kappa} W_{L-h+1}
	\end{equation}
	and $W_{L+1}:=I$.
	\label{theorem:affine}
\end{theorem}

Therefore, for a given input $x$ an affine function $f^*(x)$ can be devised. Notice that Theorem \ref{theorem:affine} only requires hidden layers node to be equipped with a ReLU activation function: nor the input nor the output nodes needs to employ it. %On the contrary, output nodes may be equipped with a sigmoid activation for binary or multi-label classification or a softmax activation function in case of multiclass.
Since the function $f^*(x)$ is affine, its interpretation is already much easier than considering the initial deep network $f(x) = h_{L} \circ h_{L-1} \circ \dots \circ h_{2} \circ h_{1} x$. Indeed, for each sample we can calculate the Frobenius norm of the corresponding weight matrix $w_L = ||W(L)||_2$. At last, similarly to what is done in the network-level pruning, we can retain the most important input features which satisfy $w'_L > \tau$, where again $w'_L = \frac{w_L}{\max w_L}$ and $\tau$ is set to 0.5.


\section{Out-of-the-box LENs}\label{sec:outofthebox}


Crafting state-of-the-art fully interpretable models is not an easy task; rather, there is a trade-off between interpretability and performances.
The proposed framework is designed to provide the building-blocks to create a wide range of models having different interpretability-VS-accuracy
% interpretability-VS-explainability-VS-performance
trade-offs.
Here, we show how to combine the methods presented in the previous section to design three different out-of-the-box LENs (Fig. \ref{fig:out-of-the-box}): a) the $\psi$ network, as proposed in \cite{ciravegna2020constraint} which is a fully interpretable model with limited learning capacity and providing mediocre explanations; b) the $\mu$ network, a neural model providing high-quality explanations, great learning performances and modest interpretability;  c) the ReLU network, a black box model ensuring state-of-the-art learning performance and good explanations at the cost of very low interpretability. The characteristics of these three LENs are also resumed in Tab. \ref{tab:LENs}, and in Fig.~\ref{fig:visual} (right).


\begin{table}[ht]
\centering
\caption{Out-of-the-box LENs summary.}
\label{tab:LENs}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{LEN}                            & \textbf{Pruning} & \textbf{Activation}  & \textbf{Learning}  & \textbf{Explanation}   & \textbf{Interpretability}\\
\midrule

$\psi$ Network (Fig. \ref{fig:psi_net}) & Node-level        & Sigmoid                       & Low                           & Low                               & Very high     \\
$\mu$ Network (Fig. \ref{fig:mu_net})   & Network-level     & Any                           & High                          & Very high                         & High          \\
ReLU Network (Fig. \ref{fig:relu_net})  & Example-level     & ReLU                          & Very high                     & High                              & Low           \\

\bottomrule
\end{tabular}
}
\end{table}


\begin{figure}[ht]
    \centering

     \begin{subfigure}{1\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth]{figs/psi_nn.png}
         \caption{$\psi$ network (Subsection \ref{subsec:psi}).}
         \label{fig:psi_net}
     \end{subfigure}\\

     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/mu_nn.png}
         \caption{$\mu$ network (Subsection \ref{subsec:mu}).}
         \label{fig:mu_net}
     \end{subfigure}
     \qquad
     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/relu_nn.png}
         \caption{ReLU network (Subsection \ref{subsec:relu}).}
         \label{fig:relu_net}
     \end{subfigure}

    \caption{Out-of-the-box LENs. (a) $\psi$ networks
    %(Subsection \ref{subsec:psi})
    only admit $[0,1]$-valued neurons with low fan-in, hence we can associate a boolean formula to each neuron by analysing its I/O truth-table. (b) $\mu$ networks
    %(Subsection \ref{subsec:mu})
    do not have interpretable hidden neurons but the input concepts are drastically pruned which allows to provide simple network-level explanations. (c) ReLU networks
    %(Subsection \ref{subsec:relu})
    supply explanations for each sample by means of the equivalent affine transformation. However, nor the nodes, nor the network can be logically interpreted.}
    \label{fig:out-of-the-box}
\end{figure}

\subsection{The $\psi$ network} \label{subsec:psi}
A $\psi$ network is a Logically Explained Network already proposed by \cite{ciravegna2020constraint,ciravegna2020human}. A $\psi$ network is based on three design principles:
(i) all activation functions for all neurons (including hidden units) should be Sigmoid;
(ii) a strong L1-regularization is used in all layers to shrink the less important weight's values towards zero;
(iii) a Node-level pruning strategy, where each neuron of the network must have the same number of incoming non-pruned weights (suggested values are between 2 and 9). This number is directly proportional to the number of terms involved in the explanations.
Also the number of hidden layers in the network needs to be set carefully, since the number of terms exponentially grows with the number of layers.
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.24]{figs/psi_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
The typical use case presented in the original work is a concept-bottleneck scenario. A black-box model $g$ (e.g. a convolutional neural network) is used to predict a set of categories $C$ from an unstructured data set $X$ (e.g. images). The authors used a $\psi$ network to explain the behaviour of a classifier $g$, i.e. $C \xrightarrow[]{f} E=g(X)$. The $\psi$ network is specifically designed to be a fully interpretable neural network, therefore, here we also show its performances as a classifier in different contexts. It can provide the whole set of logic-based explanations: example-level, aggregated, class-level, and it is the only LEN providing also compounding node by node explanations. As a matter of fact, thanks to the node-level pruning strategy, the $\psi$ network allows to interpret (and extract a corresponding logic formulas) from each node.
Recalling Example \ref{ex:xor}, a $\psi$ network with two hidden nodes may learn the logic formula:
\begin{equation}
\forall c:\ \bar{f}_1(c)\leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2),
\label{eq:xor}
\end{equation}
with hidden nodes learning $h_1(c) \leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)$, $h_2(c) \leftrightarrow ( \bar{c}_1\wedge \neg\bar{c}_2)$ and output node $f_1 \leftrightarrow h_1 \vee h_2$.
A $\psi$ network can be seen as a Cascading LEN where each layer corresponds to a new level of LEN. However, the network is always trained as a whole since no symbolic concept is provided at each level. Furthermore, also the explanations are always given in terms of input features for this reason.
As reported in Fig. \ref{fig:psi_net}, this network provides the highest level of interpretability since the $\psi$ network provides for an explanation of the behaviour of each neuron.
On the contrary, the strong regularization and the restrictive pruning strategy lead to poor classification accuracy making $\psi$ networks hard to train and not suitable for solving complex categorical learning problems. Besides, the provided explanations can be very expressive but they can be not outstanding as expected, due to the limited learning performance.

\subsection{The $\mu$ network}  \label{subsec:mu}
A $\mu$ network is a LEN based on a standard multi-layer perceptron. A $\mu$ network is based on two design principles:
    (i) a strong L1-regularization is used only in the first layer of the network;
    (ii) a Network-level pruning strategy, which only prune the  neurons (features).
After the pruning step, the $\mu$ network can be fine-tuned to adjust to the new configuration. No assumption need to be made nor on the hidden layers nor on the activation functions. However, by applying a Network-level strategy, the same set of retained features is used for the whole network. On the one side, this allows to logically-interpret the network and, therefore, to provide explanations. On the other side, this may represent a severe limitations for multi-class classification since each class may rely on few features, but these may be very different between each class. Therefore, in the multi-class experiments of Section \ref{sec:experiments}, we train a set of light binary $\mu$ networks, one for each class.

%This LEN can provide a wide range of logic-based explanations (i.e. local, cluster, and class-level).
%For each $\mu$ network, an explanation is provided in terms of the input concepts.
Recalling Ex. \ref{ex:xor}, a $\mu$ network with variable number of hidden layers, may learn the logic formula in \ref{eq:xor}.
The Network-level strategy in this case should not prune any input features since both $c_1$ and $c_2$ are important for the final classification. In case instead also some redundant features are present, they are discard in favor of $c_1$ and $c_2$ as shown in Fig. \ref{fig:mu_net}.
%As described in Sec. \ref{sec:logic_rule_extr}
For some points the network will learn the aggregated explanations:
\begin{equation}
\forall c \in S_1: \neg c_1 \wedge c_2 \rightarrow f_1(c) \quad \text{and} \quad \forall c \in S_2: c_1 \wedge \neg c_2 \rightarrow f_1(c).
\end{equation}
The two explanations can be then considered altogether to explain the class $C_1$:
\begin{equation}
\forall c\in C:\ \bar{f}_1(c)\leftrightarrow\varphi_1(c) = \bigvee_{c \in C_i}\varphi_{i,c} =
 (\neg \bar{c}_1\wedge \bar{c}_2) \vee ( \bar{c}_1\wedge \neg\bar{c}_2).
 \label{eq:mu}
\end{equation}

Thanks to the permissive pruning strategy, the learning capacity of the network remains intact for the most part. As a consequence, $\mu$ networks are suitable for solving and explaining more complex categorical learning problems. The quality of the explanations provided by the $mu$ networks are among the higher between the proposed models. At last, a mild-level of interpretability is also guaranteed since it can be logically interpreted at a network-level.

\subsection{The ReLU network}  \label{subsec:relu}
Another example of LEN which provides a different accuracy-vs-interpretability trade-off is the ReLU network. %is a special case of a $\mu$ network sharing most of its characteristics but with a few different properties.
It is based on three design principles:
    (i) all activation functions for all \emph{hidden} neurons are rectified linear units;
    (ii) a mild L1-regularization in all layers of the network;
    (iii) an Example-level pruning strategy, i.e. a specialized pruning strategy for each sample.
The pruning employed in this LEN is an example-level pruning, which is available since it employs rectified linear units activation functions. %, i.e. a pruning strategy which is applied for each sample.
This is not a limitations since it is one of the most widely used and efficient activation functions employed in deep learning \cite{glorot2011deep,ramachandran2017searching}.
On the contrary, this pruning strategy, does not cut the connections of the LEN $f$ as it is applied on the affine function $f^*$ directly to get a custom explanation for each observation. This means that the original capacity of the model is fully preserved, eventually leading to state-of-the-art classification performances. However, this type of pruning does not provide any insights of the model behaviour and may not always lead to optimum explanations.

Recalling again Example \ref{ex:xor}, a ReLu network with variable number of hidden layers, may learn the correct logic formula by aggregating local examples as it is done in \ref{eq:mu}. However, the local explanations of a certain point $c$ may not be as correct as the ones provided by the $\mu$ networks. Indeed, it can be demonstrated that the corresponding affine function $f*$, actually corresponds to the nearest decision boundary to the points.
% On the other hand, an example-based pruning strategy may be provide more unstable explanations as the pruning may be negatively affected by the presence of outliers.
Therefore, the corresponding weights may miss some important features to explain $c$. A Relu network sometimes may explain the XOR problems with the wrong formula:
\begin{equation}
\forall c\in C:\ \bar{f}_1(c)\leftrightarrow\varphi_1(c) = \bigvee_{c \in C_i}\varphi_{i,c} =
 (\neg \bar{c}_1) \vee (\neg\bar{c}_2).
\end{equation}
Summing up, this LEN does provide the best performances in terms of classification accuracy thanks to the example-level pruning strategy. However, this comes at the cost of poor model interpretability and mild explanation capacity.

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figs/relu_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


\section{Benchmarking out-of-the-box LENs} \label{sec:experiments}
In this section, we quantitatively assess the quality of the explanations and the performance of Logically Explained Networks compared to state-of-the-art white-box models. Each task is uniquely defined by the tuple "pipeline / explanation style". The summary of each task is reported in Table \ref{tab:datasets}.
A brief description of each task, the corresponding dataset and all the related experimental details are exposed in Subsection \ref{sec:exp_details}. In Subsection \ref{sec:exp_metrics} six quantitative metrics are defined and used to compare LENs with state-of-the-art methods.

\begin{table}[ht]
\centering
\caption{Experiments.}
\label{tab:datasets}
\resizebox{\textwidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Dataset} & \textbf{Description} & \textbf{Explanation Style} & \textbf{Pipeline}\\
\midrule

MIMIC-II (Fig. \ref{fig:E2EExplainer})                      & \small{Predict patient survival from clinical data}       & Interpretable classification  & E2E \\
MNIST E/O (Fig. \ref{fig:CMBExplainer})                         & \small{Predict parity from digit images}                  & Interpretable classification  & CB\\
CUB (Fig. \ref{fig:len})                                    & \small{Predict bird species from bird images}             & Interpretable classification  & CB\\
V-Dem (Fig. \ref{fig:CascadeExplainer})                     & \small{Predict electoral democracy from social indexes}   & Interpretable classification  & Cascading \\
MIMIC-II (EBB) (Fig. \ref{fig:explainablevsexplanation})    & \small{Predict patient survival from clinical data}       & Explaining black box       & E2E\\
MNIST E/O (IC) (Fig. \ref{fig:concept_relations})                    & \small{Cluster digit properties from digit images}        & Interpretable clustering      & CB\\
\bottomrule
\end{tabular}
}
\end{table}


% \subsection{Software tool and usability}
% \label{sec:tool}
In order to make the LENs framework accessible to the whole community, we released of a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on methods and out-of-the-box LENs. The Python code and the scripts used for the experiments, including parameter values and documentation, is freely available under Apache 2.0 Public License from a GitHub repository\footnote{\url{https://github.com/pietrobarbiero/deep-logic}}.

The Deep Logic library is designed to make out-of-the-box LENs accessible to researchers and neophytes by means of intuitive APIs requiring only a few lines of code to train and get explanations from a LEN (as shown in the code example \ref{code:example}).

\begin{lstlisting}[language=Python, label=code:example, caption=Example on how to use the Deep Logic library.]
import deep_logic as dl

# import train, validation and test data loaders
[...]

# instantiate a mu network
model = dl.models.MuNN(n_classes=n_classes, n_features=n_features,
                       hidden_neurons=[200], loss=torch.nn.CrossEntropyLoss(),
                       l1_weight=0.001, fan_in=10)

# fit the model
model.fit(train_data, val_data, epochs=100, l_r=0.0001)

# get predictions on test samples
outputs, labels = model.predict(test_data)

# get first-order logic explanations for a specific target class
target_class = 1
formula = model.get_global_explanation(x_val, y_val, target_class)
# compute explanation accuracy
accuracy = dl.logic.test_explanation(formula, target_class, x_test, y_test)
\end{lstlisting}

% \textbf{Unless required by applicable law or agreed to in writing, software is distributed on an "as is" basis, without warranties or conditions of any kind, either express or implied.}

\subsection{Dataset and classification task details}
\label{sec:exp_details}
For the experimental analysis, we consider five categorical learning problems ranging from computer vision to medicine and democracy. Some datasets (e.g. CUB) were already annotated with high-level concepts (e.g. bird attributes) which can be exploited to train a concept bottleneck pipeline. For datasets without annotations for high-level concepts, we transform the input space into a predicate space (i.e. $\mathbb{R}^d \rightarrow [0,1]^d$) to make it suitable for training LENs. According to the considered data type, we evaluate and discuss the usage of  different LEN pipeline, classification and explanation style (see Tab. \ref{tab:datasets}).
For the sake of consistency, in all supervised experiments LENs were trained by optimizing Eq. \ref{eq:IFF}, therefore extracting IFF rules. However also Eq. \ref{eq:IF} \ref{eq.IF2} could be optimized, above all when explaining a black-box model.


\textsc{MIMIC-II - E2E Interpretable classification. }
The Multiparameter Intelligent Monitoring in Intensive Care II (MIMIC-II, \cite{saeed2011multiparameter,goldberger2000physiobank}) is a public-access intensive care unit (ICU) database consisting of 32,536 subjects (with 40,426 ICU admissions) admitted to
%medical, surgical, cardiovascular and neonatal ICUs, surgical recovery units, and coronary care units
ICUs at a single tertiary care hospital. The dataset contains detailed description of a variety of clinical data classes: general,
%(e.g. patient demographics, hospital admission and discharge dates, hospital death dates, etc),
physiological, % (e.g.	nurse-verified vital signs, blood pressure, heart rate, etc),
results of clinical laboratory tests, % (e.g. hematology, blood chemistries, urinalysis, microbiology, etc),
records of medications, fluid balance, %(e.g. solutions, urine, estimated blood loss, etc),
and free text notes and reports of imaging studies (e.g. x-ray, CT, MRI, etc). In our experiments, we remove the text-based input features and
%discretize some of the continuous features into a set of categories in order to get a one-hot encoded representation. For instance,
we discretize blood pressure (BP) into five different categories (one-hot encoded): very low BP, low BP, normal BP, high BP, and very high BP. After such preprocessing step, we obtain an input space $X=C \subset [0,1]^d$ composed of $d=90$ key features.
The task consists in training a classifier function to identify recovering ($Y=1$) or dying ($Y=0$) patients, after 28 days from ICU admission. In particular, we consider the case of
% {\bf Interpretable classification. }
\textit{Interpretable classification} where an End-to-End LEN $X=C \rightarrow E=Y$ is employed to carry out the classification task.
But we also considered the case of

\textsc{MIMIC-II (EBB) - {E2E Explaining a black-box model}. } On the same dataset, a second task is set up. A black-box model $g$ $X=C \rightarrow Y$ is employed to solve the classification task, with predictions $g(C) \approx Y$. The end-to-end model $f$ $X=C \rightarrow E=g(C)$ instead is trained to mimic the behaviour of the black box $g$.

% \subsubsection{Concept bottleneck explainers}
% \label{sec:exp_cbm}

% \paragraph{MNIST Even/Odd}
\textsc{MNIST Even/Odd - {CB Interpretable classifications}. }
The Modified National Institute of Standards and Technology database (MNIST, \cite{lecun1998mnist}) contains a large collection of images representing handwritten digits. The input space $X \subset \mathbb{R}^{28\times 28}$ is composed of 28x28 pixel images while the concept space $C \subset [0,1]^{10}$ is represented by digits from $0$ to $9$.
However, the task we aim to solve is slightly different from the common digit-classification. In the case of
% {\bf Interpretable classification}
\textit{interpretable classification}, indeed, assuming $Y \subset [0,1]^2$, we are interested in determining if a digit is either odd or even, and explain the assignment to one of these classes in terms of the high-level concepts $C$ (digits). The mapping $X \rightarrow C$ is learned by a ResNet10 classifier $g$ \cite{he2016deep}  trained from scratch, while a LEN $f$ is used to learn both the mapping and the explanation as a function $C=g(X) \rightarrow E=Y$.

% The $\mu$ network is equipped with a single hidden layer with 10 neurons and the $L_1$ loss weight $\lambda = 10^{-2}$.
% The $ReLU$ network is equipped with two hidden layers composed of 30, 10 hidden neurons respectively and $\lambda = 10^{-3}$.
% The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^-3$ and fan-in = 5.
% All networks have been trained for 200 epochs with learning rate = $10^ {-3}$.

\textsc{MNIST E/O (IC) - {CB Interpretable clustering}. }
 The same dataset has been used to perform
% {\bf Interpretable Clustering}
\textit{Interpretable clustering}.  We consider a concept space $C \subset [0,1]^{12}$ which comprise both the digits and the even/odd labels. The mapping $X \rightarrow C$ is learned again by a Resnet10 model $g$ trained as a multi-label classifier, while the LEN $f$ performs clustering from $C=g(X) \rightarrow E$, where $E \subset [0,1]^{2}$ space, in order two extract two clusters.
% In this case,
% the $\mu$ network is equipped with two hidden layer with 20, 10 neurons respectively and the $L_1$ loss weight $\lambda = 10^{-3}$.
% The $ReLU$ network is equipped with two hidden layers composed of 50, 30 hidden neurons and $\lambda = 10^{-4}$.
% The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^{-2}$ and fan-in = 2.
% The $\mu$ and the $ReLU$ networks have been trained for 100 epochs with learning rate = $10^{-3}$ while for the $\psi$ network is equal to $10^{-2}$.

%Quantitative results are reported in Table \ref{tab:exp_metrics_mnist_cbm} while Table \ref{tab:exp_formula_mnist_cbm} shows for each fold the explanation extracted from trained explainers.
\textsc{CUB - CB Interpretable Classification .}
The Caltech-UCSD Birds-200-2011 dataset (CUB, \cite{wah2011caltech}) is a fine-grained classification dataset. It includes 11,788 images representing $r = 200$ ($Y \subset [0,1]^{200}$) different bird species. 312 binary attributes have been also collected for each image representing visual characteristics (color, pattern, shape) of particular parts (beak, wings, tail, etc.). Attributes annotations, however, is quite noisy. Similarly to \cite{koh2020concept}, we denoised attributes by considering class-level annotations, i.e. a certain attribute is set as present only if it is also present in at least 50\% of the images of the same class. Furthermore we only considered attributes present in at least 10 classes after this refinement. In the end, a total of $d = 108$ attributes ($C \subset [0,1]^{108}$) have been retained. The mapping $X \rightarrow C$ from images to attribute concepts is performed again with a ResNet10 model $g$ trained from scratch while a LEN $f$ learns the final function $C = g(X) \rightarrow E=Y$.


\textsc{V-Dem - Cascade Interpretable classification. }
Varieties of Democracy (V-Dem, \cite{pemstein2018v,coppedge2021v}) is a dataset containing a collection of indicators of latent regime characteristics over 202 countries from 1789 to 2020. The database include $d_1 = 483$ low-level indicators $C_1 \subset [0,1]^{d_1}$ (e.g. media bias, party ban, high-court independence, initiatives permitted, etc), $d_2 = 82$ mid-level indices $C_1 \subset [0,1]^{d_2}$ (e.g. freedom of expression, freedom of association, equality before the law, etc), and 5 high-level indices of democracy principles (i.e. electoral, liberal, participatory, deliberative, and egalitarian). In the experiments a binary classification problem is considered to identify electoral democracies ($Y=1$) from non-electoral democracies ($Y=0$). Cascading LENs $f_1$ and $f_2$ are trained to learn the map $C_1 \rightarrow C_2 \rightarrow E=Y$.



\subsection{Quantitative metrics for model and explanations}
\label{sec:exp_metrics}
Seven metrics are used to compare the performance of LENs with respect to state-of-the-art approaches.
While measuring classification metrics is necessary for models to be viable in practice to perform interpretable classification tasks, assessing the quality of the explanations is required to justify their use for explainability. In contrast with other kind of explanations, logic-based formulas can be evaluated quantitatively. Given a classification problem, first we extract a set of rules from a trained model and then we test each explanation on an unseen set of samples.
The results for each metric are reported in terms of the mean and the standard error of the mean, computed over a 10-fold cross validation \cite{krzywinski2013error}. Only in the CUB experiments a 5-fold cross validation is performed due to timing issues related to BRL (each training of BRL on CUB lasts about 3 hours).
For each experiment we measure:
% (1) the test accuracy of the classifier, (2) the test accuracy of the explanation, (3) the complexity of the explanation, (4) the fidelity of the explanation with respect to the classifier, (5) the elapsed time required to extract the explanations, (6) the consistency of the explanation over different runs, and (7) the normalized mutual information (for unsupervised tasks only).
% \cite{andrews1995survey}.

\begin{itemize}
\item The \textsc{model accuracy} measures how well the classifier correctly identifies the target class (see Table. \ref{tab:model-accuracy}). When the model is the classifier itself (i.e. interpretable classification), this metric represents the accuracy of the model. Instead, when the model explain the predictions of a black box classifier, this metric represents the accuracy of the black box classifier.
\item The \textsc{explanation accuracy} measures how well the extracted logic formula correctly identifies the target  class (see Table. \ref{tab:explanation-accuracy}).
\item The \textsc{complexity of an explanation} measures how hard would it be for a human being to understand the logic formula (see Table. \ref{tab:complexity}). This metric is computed by standardizing the explanations in disjunctive normal form and then by counting the number of terms of the standardized formula.
\item The \textsc{fidelity of an explanation} measures how well the predictions obtained using the extracted explanation match the predictions obtained using the classifier (see Table. \ref{tab:fidelity}). When the model is the classifier itself (i.e. interpretable classification), this metric represents the match between the extracted explanation and the model. Instead, when the model is explaining the predictions of a black box classifier, this metric represents the match between the extracted explanation and the black box classifier.
\item The \textsc{rule extraction} measures the time required to obtain an explanation from scratch. It is computed as the sum of the time required to train the (see Table. \ref{tab:extraction}) model and the time required to extract the formula from a trained model. This is justified by the fact that for some models, like BRL, training and rule extraction consist of just one simultaneous process.
\item The \textsc{consistency of an explanation} measures the similarity of the extracted explanations over different runs (see Table. \ref{tab:consistency}). It is computed by counting how many times the same concepts appear in the logic formulas over different folds of a cross-validation or over different initialization seeds.
% \item The \textsc{normalized mutual information} measures the quality of the clusters obtained in the interpretable clustering experiments. It is calculated as the mutual information of Eq. \ref{eq:MI}, divided by the Entropy $H_E$ so that it reports a number always comprehended between $[0,1]$.
\end{itemize}




\subsection{Results and Discussion}
% \textsc{Interpretable classification. }
Experiments show how LENs generalize better than decision trees on complex boolean functions (e.g. CUB and MIMIC-II) as already observed in \cite{tavares2020understanding} (Table. \ref{tab:model-accuracy}). For most experiments the formulas extracted from LENs are either better or almost as accurate as the formulas found by decision trees or mined by BRL (Table. \ref{tab:explanation-accuracy}). The complexity of LEN explanations is usually lower than the complexity of the rules extracted from a decision tree or mined by BRL. The complexity of decision tree formulas is never below 100 terms, making them useless for quick decision making (Table. \ref{tab:complexity}). White-box models like decision trees and BRL outperform LENs in terms of fidelity. Their predictions is directly based on the explanation therefore fidelity is always 100\%. However, the fidelity of the formulas extracted by the $\mu$ and the ReLU network is often higher than $90\%$. This means that almost any prediction has been correctly explained, making these networks very close to white boxes (Table. \ref{tab:fidelity}). BRL is the slowest rule extractor over all the experiments by one order of magnitude, while the decision tree is the fastest overall (Table. \ref{tab:extraction}). In terms of consistency there is not a dominant method (Table. \ref{tab:consistency}).

Fig. \ref{fig:multi-objective} shows the Pareto frontiers \cite{marler2004survey} for each experiment in terms of the complexity of the explanation and its classification error ($100 -$ classification accuracy). The simplest and most accurate formulas are found by the LENs, whose complexity is almost always below the maximum complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Across all the experiments, there is at least one set of formulas extracted from out-of-the-box LEN dominating both BRL and decision trees.

For each dataset and for each method Table \ref{tab:best-rules} reports some compact FOL formula extracted.


\textsc{Interpretable Clustering. }
As introduced in the MNIST E/O dataset explanation we performed clustering starting from a Concept space composed of the 10 digits and the even/odd labels. The LEN are instructed two extract 2 clusters possibly respecting the even/odd division of digits. In Table \ref{tab:exp_metrics_mnist_mi} the metrics regarding this task are reported. We can see that all methods are capable to maximize the normalized mutual information. However only the $\psi$ network is capable to consistently explain the two clusters in terms of the important labels (even and odd), as we can see from the complexity of the rules (higher than 2 for the $\mu$ and ReLu net) and for the consistency of terms used in the explanation (100\% for the $\psi$ network).
Other examples and application of Interpretable Clustering has been performed in \cite{ciravegna2020constraint, ciravegna2020human} employing the $\psi$ network only.

% \subsection{Other experiences}

% \textsc{Explanation as a defense}



\begin{table}
\centering
\caption{Model's accuracy (\%)}
\label{tab:model-accuracy}
\begin{tabular}{llllll}
\toprule
{} &              Tree &               BRL &        $\psi$ net &          Relu net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $77.53 \pm 1.45$ &  $76.40 \pm 1.22$ &  $77.19 \pm 1.09$ &  $\bf{80.11} \pm 1.87$ &  $80.00 \pm 0.95$ \\
\textbf{vDem    } &  $85.61 \pm 0.57$ &  $91.23 \pm 0.75$ &  $89.78 \pm 1.64$ &  $\bf{92.08} \pm 0.37$ &  $90.40 \pm 0.51$ \\
\textbf{MNIST   } &  $99.75 \pm 0.01$ &  $99.80 \pm 0.02$ &  $99.80 \pm 0.03$ &  $\bf{99.88} \pm 0.02$ &  $99.83 \pm 0.01$ \\
\textbf{CUB     } &  $81.62 \pm 1.17$ &  $90.79 \pm 0.34$ &  $91.92 \pm 0.27$ &  $\bf{92.29} \pm 0.40$ &  $92.21 \pm 0.33$ \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Model's accuracy (\%)}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lllllll}
% \toprule
% {} &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL & Black box \\
% \midrule
% \textbf{MIMIC-II     }  &  ${\bf 86.60 \pm 0.30}$ &  $85.36 \pm 0.78$ &  $84.01 \pm 0.09$ &  $79.56 \pm 0.80$ &  $86.15 \pm 0.51$ & N/A \\
% \textbf{MIMIC-II (EBB)}  &  N/A &  N/A &  N/A &  N/A &  N/A  & $85.13 \pm 0.70$\\
% \textbf{V-Dem         } &  $91.96 \pm 0.42$ &  $91.88 \pm 0.37$ &  $79.23 \pm 2.20$ &  $92.11 \pm 0.38$ &  ${\bf 92.23 \pm 0.38}$ & N/A \\
% \textbf{MNIST}          &  $99.75 \pm 0.02$ &  $99.81 \pm 0.01$ &  $99.80 \pm 0.01$ &  ${\bf 99.96 \pm 0.01}$ &  $99.80 \pm 0.01$ & N/A \\
% \textbf{CUB          }  &  ${\bf 92.26 \pm 0.28}$ &  $92.19 \pm 0.27$ &  $91.72 \pm 0.56$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ & N/A \\

% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}
\centering
\caption{Explanation's accuracy (\%)}
\label{tab:explanation-accuracy}
\begin{tabular}{llllll}
\toprule
{} &              Tree &               BRL &        $\psi$ net &          Relu net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $69.15 \pm 2.24$ &  $70.59 \pm 2.17$ &  $49.51 \pm 3.92$ &  $70.28 \pm 1.67$ &  $71.84 \pm 1.82$ \\
\textbf{vDem    } &  $85.45 \pm 0.58$ &  $91.21 \pm 0.75$ &  $67.08 \pm 9.68$ &  $90.21 \pm 0.55$ &  $88.18 \pm 1.07$ \\
\textbf{MNIST   } &  $99.74 \pm 0.01$ &  $99.79 \pm 0.02$ &  $65.64 \pm 5.05$ &  $99.74 \pm 0.02$ &  $99.74 \pm 0.02$ \\
\textbf{CUB     } &  $89.36 \pm 0.92$ &  $96.02 \pm 0.17$ &  $76.10 \pm 0.56$ &  $87.96 \pm 2.81$ &  $93.69 \pm 0.27$ \\
\textbf{MIMIC-II (EBB)} &  ${\bf85.75 \pm 0.51}$ &  $81.07 \pm 3.33$ &  $83.90 \pm 1.25$ &  $85.53 \pm 0.61$ &  $85.70 \pm 0.48$ \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Explanation's accuracy (\%)}
% \label{tab:explanation-accuracy}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $85.08 \pm 0.48$ &  $82.09 \pm 1.38$ &  $82.83 \pm 0.66$ &  $79.56 \pm 0.80$ &   ${\bf86.15 \pm 0.51}$ \\
% \textbf{MIMIC-II (EBB)} &  ${\bf85.75 \pm 0.51}$ &  $81.07 \pm 3.33$ &  $83.90 \pm 1.25$ &  $85.53 \pm 0.61$ &  $85.70 \pm 0.48$ \\
% \textbf{V-Dem         } &  $90.81 \pm 1.24$ & ${\bf94.65 \pm 0.32}$ &  $80.29 \pm 2.99$ &  $92.11 \pm 0.38$ &  $92.23 \pm 0.38$ \\
% \textbf{MNIST}         &  $99.67 \pm 0.01$ &  $98.04 \pm 1.60$ &  $75.47 \pm 0.46$ &  ${\bf99.96 \pm 0.01}$  &  $99.80 \pm 0.01$ \\
% \textbf{CUB*         } &  ${\bf96.15 \pm 0.16}$ &  $93.98 \pm 1.97$ &  $80.41 \pm 2.31$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ \\

% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}
\centering
\caption{Complexity}
\label{tab:complexity}
\begin{tabular}{llllll}
\toprule
{} &              Tree &                   BRL &         $\psi$ net &           Relu net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $66.60 \pm 1.45$ &     $57.70 \pm 35.58$ &   $20.60 \pm 5.36$ &  $39.50 \pm 11.62$ &  $15.80 \pm 1.37$ \\
\textbf{vDem    } &  $30.20 \pm 1.20$ &    $145.70 \pm 57.93$ &    $5.40 \pm 2.70$ &   $18.40 \pm 2.17$ &   $9.10 \pm 0.94$ \\
\textbf{MNIST   } &  $47.50 \pm 0.72$ &  $1352.30 \pm 292.62$ &  $96.90 \pm 10.01$ &   $73.30 \pm 5.77$ &  $80.50 \pm 4.85$ \\
\textbf{CUB     } &  $45.92 \pm 1.16$ &       $8.87 \pm 0.11$ &   $15.96 \pm 0.96$ &   $60.57 \pm 6.95$ &  $14.65 \pm 0.16$ \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Complexity}
% \label{tab:complexity}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {}                     &        $\mu$ net &         ReLU net &       $\psi$ net &                 Tree &               BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $5.10 \pm 0.35$ &  $23.40 \pm 11.20$ &  ${\bf2.60 \pm 0.16}$ &  $1342.60 \pm 16.94$ &  $20.70 \pm 4.08$ \\
% \textbf{MIMIC-II (EBB)} &  $7.00 \pm 0.70$ &    $6.40 \pm 0.95$ &  ${\bf1.30 \pm 0.15}$ &   $432.10 \pm 16.46$ &  $22.90 \pm 4.13$ \\
% \textbf{V-Dem         } &  $9.60 \pm 1.17$ &    $4.90 \pm 0.10$ &  ${\bf2.00 \pm 0.49}$ &    $294.10 \pm 7.88$ &   $8.70 \pm 0.97$ \\
% \textbf{MNIST}         &  ${\bf22.00 \pm 4.67}$ &  $48.10 \pm 1.43$ &  $24.85 \pm 2.89$ &  $632.35 \pm 5.01$ &  $1291.05 \pm 234.40$ \\
% \textbf{CUB          } &  $10.53 \pm 0.08$ &  $29.25 \pm 3.26$ &  $28.36 \pm 2.75$ &  $138.83 \pm 5.31$ &  ${\bf4.10 \pm 0.09}$ \\


% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}
\centering
\caption{Fidelity (\%)}
\label{tab:fidelity}
\begin{tabular}{llllll}
\toprule
{} &               Tree &                BRL &         $\psi$ net &          Relu net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &   $51.63 \pm 6.68$ &  $75.62 \pm 2.07$ &  $88.37 \pm 2.73$ \\
\textbf{vDem    } &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &  $69.67 \pm 10.43$ &  $96.36 \pm 0.64$ &  $94.73 \pm 2.16$ \\
\textbf{MNIST   } &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &   $65.68 \pm 5.05$ &  $99.85 \pm 0.02$ &  $99.83 \pm 0.02$ \\
\textbf{CUB     } &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &   $77.34 \pm 0.52$ &  $89.28 \pm 2.90$ &  $95.21 \pm 0.25$ \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[!h]
% \centering
% \caption{Fidelity (\%)}
% \label{tab:fidelity}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $96.23 \pm 0.81$ &  $87.84 \pm 2.12$ &  $84.63 \pm 0.67$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
% \textbf{MIMIC-II (EBB)} &  $92.28 \pm 0.90$ &  $86.58 \pm 4.00$ &  $90.32 \pm 1.27$ &   $93.07 \pm 0.53$ &   ${\bf94.82 \pm 0.50}$ \\
% \textbf{V-Dem         } &  $91.52 \pm 1.13$ &  $94.62 \pm 0.37$ &  $82.45 \pm 1.80$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
% \textbf{MNIST}         &  $99.90 \pm 0.03$ &  $98.14 \pm 1.60$ &  $75.53 \pm 0.46$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
% \textbf{CUB*         } &  $97.82 \pm 0.15$ &  $95.37 \pm 2.06$ &  $81.89 \pm 2.35$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\

% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}
\centering
\caption{Rule extraction time(s)}
\label{tab:extraction}
\begin{tabular}{llllll}
\toprule
{} &             Tree &                       BRL &             $\psi$ net &            Relu net &             $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $0.06 \pm 0.00$ &         $440.24 \pm 9.75$ &       $36.69 \pm 6.11$ &    $87.51 \pm 8.44$ &      $44.22 \pm 3.38$ \\
\textbf{vDem    } &  $0.49 \pm 0.07$ &     $22843.21 \pm 194.49$ &       $49.27 \pm 1.13$ &    $47.41 \pm 5.94$ &     $100.96 \pm 4.42$ \\
\textbf{MNIST   } &  $2.72 \pm 0.02$ &      $2594.79 \pm 177.34$ &     $385.58 \pm 17.82$ &  $907.18 \pm 67.75$ &     $414.21 \pm 7.48$ \\
\textbf{CUB     } &  $8.11 \pm 0.65$ &  $264678.29 \pm 56521.40$ &  $3707.29 \pm 1006.54$ &  $305.19 \pm 30.42$ &  $1173.87 \pm 146.42$ \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Rule extraction time (s)}
% \label{tab:extraction}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {} &        $\mu$ net &         ReLU net &       $\psi$ net &             Tree &              BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $13.32 \pm 0.30$ &  $266.22 \pm 166.90$ &   $8.81 \pm 0.15$ &  ${\bf0.02 \pm 0.00}$ &  $495.59 \pm 7.13$ \\
% \textbf{MIMIC-II (EBB)} &  $15.30 \pm 0.19$ &     $18.46 \pm 1.00$ &  $10.14 \pm 0.03$ &  ${\bf0.01 \pm 0.00}$ &  $543.43 \pm 3.39$ \\
% \textbf{V-Dem         } &  $34.40 \pm 0.78$ &     $34.24 \pm 0.32$ &  $20.83 \pm 0.04$ &  ${\bf0.06 \pm 0.00}$ &   $53.69 \pm 0.41$ \\
% \textbf{MNIST}         &  $173.24 \pm 6.77$ &  $221.07 \pm 4.06$ &  $236.71 \pm 3.36$ &  ${\bf2.04 \pm 0.04}$ &  $836.14 \pm 3.15$ \\
% \textbf{CUB          } &  $726.19 \pm 2.43$ &  $660.30 \pm 121.16$ &  $2094.49 \pm 730.50$ &  ${\bf4.17 \pm 0.07}$ &  $9863.52 \pm 147.57$ \\

% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}
\centering
\caption{Rule consistency (\%)}
\label{tab:consistency}
\begin{tabular}{llllll}
\toprule
{} &     Tree &       BRL & $\psi$ net &  Relu net & $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $40.49$ &   $30.48$ &    $27.62$ &   $53.75$ &   $71.43$ \\
\textbf{vDem    } &  $72.00$ &   $73.33$ &    $38.00$ &   $64.62$ &   $41.67$ \\
\textbf{MNIST   } &  $41.67$ &  $100.00$ &    $96.00$ &  $100.00$ &  $100.00$ \\
\textbf{CUB     } &  $21.47$ &   $42.86$ &    $41.43$ &   $44.17$ &   $76.92$ \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Rule consistency (\%)}
% \label{tab:consistency}
% \begin{tabular}{llllll}
% \toprule
% {} & $\mu$ net & ReLU net & $\psi$ net &     Tree &      BRL \\
% \midrule
% \textbf{MIMIC-II     } &   $51.00$ &  $26.00$ &    $37.14$ &  ${\bf81.50}$ &  $28.33$ \\
% \textbf{MIMIC-II (EBB)} &   $41.18$ &  $35.56$ &    $43.33$ &  ${\bf60.36}$ &  $22.22$ \\
% \textbf{V-Dem         }&   $71.67$ &  ${\bf98.00}$ &    $15.83$ &  $36.86$ &  $76.25$ \\
% \textbf{MNIST}         &   $60.00$ &  ${\bf100.00}$ &    $50.00$ &  $50.95$ &  ${\bf100.00}$ \\
% \textbf{CUB          } &   ${\bf58.82}$ &  $58.40$ &    $43.08$ &  $21.79$ &  $30.00$ \\
% \bottomrule
% \end{tabular}
% \end{table}



\begin{figure}[!h]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/mimic.pdf}
    \includegraphics[width=0.49\textwidth]{figs/mimic_explain_classifier.pdf}\\
    \includegraphics[width=0.49\textwidth]{figs/mnist.pdf}
    \includegraphics[width=0.49\textwidth]{figs/cub.pdf}\\
    \includegraphics[width=0.49\textwidth]{figs/vDem.pdf}
    \\
    \includegraphics[width=0.9\textwidth]{figs/legend.pdf}
    \\
    \caption{Pareto frontiers (dotted black line) in terms of average test error and average complexity of the explanations. Formulas out-of-the-box extracted from out-of-the-box LENs are reported as circles while BRL and decision trees as crosses. The vertical dotted red line marks the maximum explanation complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}).}
    \label{fig:multi-objective}
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=.9\textwidth,trim=0 15 0 0,clip]{figs/elapsed_time_plot.pdf}
    \caption{Time required to train models and to extract the explanations. Our models compare favorably with the competitors, with the exception of Decision Trees. BRL is by one to three order of magnitude slower than our approaches. Error bars show the 95\% confidence interval of the mean.}
    \label{fig:time}
\end{figure}

\begin{table}[!h]
\centering
\caption{MNIST Mutual Information}
\label{tab:exp_metrics_mnist_mi}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
     Method & Model's accuracy (\%) & Exp. accuracy (\%) &       Complexity & Extraction time (s) & Rule consistency (\%) \\
\midrule
 $\psi$  net &     $99.90 \pm 0.01$ &           $99.90 \pm 0.01$ &  $2.00 \pm 0.00$ &     $0.33 \pm 0.15$ &             $100.00$ \\
 $\mu$ net &     $94.91 \pm 4.99$ &           $95.41 \pm 4.50$ &  $2.30 \pm 0.64$ &     $2.36 \pm 0.75$ &              $35.00$ \\
   ReLU net &     $96.87 \pm 3.04$ &           $95.97 \pm 3.94$ &  $2.15 \pm 0.39$ &     $4.15 \pm 1.62$ &              $45.00$ \\
\bottomrule
\end{tabular}
}
\end{table}





% \subsection{Rules Extracted}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
{\renewcommand{\arraystretch}{1.5}
\begin{table}[!h]
\centering
\caption{A selection of some of the best rules extracted for each experiment.}
\label{tab:best-rules}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
\multicolumn{1}{l}{\textbf{Dataset}}    & \textbf{Model}  & \textbf{Rule} \\ \hline
\multirow{5}{*}{MIMIC-II}      & $\mu$ net  & $Death \leftarrow stroke \wedge age\_HIGH  \wedge \neg atrial\_fibrillation $  \\
                               & ReLU net   & $Death \leftarrow stroke \wedge age\_HIGH \wedge \neg atrial_fibrillation \wedge \neg sapsi\_first\_LOW \wedge \neg sapsi\_first\_HIGH $  \\
                               & $\psi$ net & $Death \leftarrow stroke \vee bun\_first\_NORMAL \vee sapsi\_first\_HIGH $  \\
                               & Tree       & $Death \leftarrow \quad ^*$formula is too long (1000+ terms) \\
                               & BRL        & $Death \leftarrow \makecell[l]{(stroke \wedge resp \wedge \neg age\_LOW \wedge \neg sapsi\_first\_LOW) \\
                               \vee (stroke  \wedge age\_HIGH \wedge \neg age\_LOW  \wedge  \neg sapsi\_first\_LOW) }$  \\ \hline
\multirow{5}{*}{MIMIC-II (EBB)} & $\mu$ net  & $Death \leftarrow atrial_fibrillation \wedge stroke \wedge \neg sapsi\_first\_HIGH \wedge \neg weight\_first\_NORMAL $  \\
                               & ReLU net   & $Death \leftarrow stroke \wedge \neg sapsi\_first\_LOW  \wedge  \neg sapsi\_first\_HIGH \wedge \neg sodium\_first\_LOW $  \\
                               & $\psi$ net & $Death \leftarrow stroke \wedge age\_HIGH $  \\
                               & Tree       & $Death \leftarrow  \quad ^*$formula is too long (100+ terms)  \\
                               & BRL        & $Death \leftarrow \makecell[l]{stroke \wedge age\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW) \\ \vee  (stroke \wedge platelet\_first\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW } $  \\  \hline
\multirow{5}{*}{MNIST}         & $\mu$ net  & $Even \leftarrow \neg One \wedge \neg Three \wedge \neg Five \wedge \neg Seven \wedge \neg Nine $  \\
                              & ReLU net   & $Even \leftarrow \makecell[l]{(Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Two \wedge \neg Zero \wedge \neg One \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Four \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Six \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Eight \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Nine) } $ \\
                              & $\psi$ net & $Even \leftarrow \makecell[l]{(Six \wedge Zero \wedge \neg One \wedge \neg Seven)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Three)  \\
                              \vee (Six \wedge Zero \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge \neg One \wedge \neg Seven \wedge \neg Three) \\
                              \vee (Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)}$  \\
                              & Tree       & $Even \leftarrow \quad ^*$formula is too long \\
                              & BRL        & $Even \leftarrow  \makecell[l]{(Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two)) \vee (Eight \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two))
                              \\ \vee (Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Seven \wedge \neg Two)) \\
                              \vee (Two \wedge \neg One \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \\ \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two)) \\
                              \vee (Four \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \\ \wedge  \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One)) \\
                              \vee (Zero \wedge \neg Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \\
                              \wedge \neg (Nine \wedge \neg Zero) \wedge \neg (One \wedge \neg Two) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One))
                              }$  \\ \hline
\multirow{5}{*}{CUB}          & $\mu$ net  & $ Black\ foot\ albatross \leftarrow \makecell[l]{  bill \ shape \ hooked \ seabird \ \wedge \  size \ medium \wedge \ wing \ pattern \ solid \\
                              \wedge \neg wing color \ black \wedge \neg  underparts\ color\ white \wedge \neg upper\ tail\ color\ grey \\
                              \wedge \neg breast\ color\ white \wedge \neg  throat\ color\ white \wedge \neg tail\ pattern\ solid \wedge \neg  crown\ color\ white} $  \\
                              & ReLU net   & $ Black\ foot\ albatross \leftarrow  \makecell[l]{ size\  medium  \wedge \neg  bill\  shape\  allpurpose  \\
                              \wedge \neg  upperparts\  color\  black  \wedge \neg  head\  pattern\  plain  \wedge \neg  under\  tail\  color\  yellow \\  \wedge \neg  under\  tail\  color\  black  \wedge \neg  nape\  color\  buff  \\
                              \wedge \neg  wing\  shape\  roundedwings  \wedge \neg  shape\  perchinglike  \\
                              \wedge \neg  leg\  color\  grey  \wedge \neg  leg\  color\  black  \wedge \neg  bill\  color\  grey  \\
                              \wedge \neg  bill\  color\  black  \wedge \neg  wing\  pattern\  multicolored }$\\
                              & $\psi$ net & $ Black\ foot\ albatross \leftarrow  \makecell[l]{(bill \ shape \ hooked\ seabird \wedge tail \ pattern \ solid \wedge \neg underparts \ color \ white \\
                              \wedge ( \neg  \ breast \ color \ white \vee \neg   \ wing \ color \ grey)) }$  \\
                              & Tree       & $ Black\ foot\ albatross \leftarrow  ^*$formula is too long (1000+ terms)  \\
                              & BRL        & $ Black\ foot\ albatross \leftarrow  \makecell[l]{( bill\  shape\  hooked\  seabird \wedge forehead\ color\ blue \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white) \\
                              \vee ( bill\  shape\  hooked\  seabird \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white \wedge  \neg  tail\  pattern\  solid)}$ \\
\hline
\multirow{5}{*}{V-Dem}         & $\mu$ net  & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & ReLU net   & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & $\psi$ net & $Elect\_ Dem \leftarrow v2x\_frassoc\_thick \wedge v2xeg\_eqaccess $  \\
                               & Tree       & $Elect\_ Dem \leftarrow \quad ^*$formula is too long (1000+ terms)  \\
                               & BRL        & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\ \hline
\end{tabular}%
}
\end{table}}



% These challenging or product-oriented contexts are the actual targets of XAI research. This great research effort have produced a variety of quite interesting and efficient approaches to unveil the decision process of black-box models. Some of the most common taxonomies are based on a few discriminative criteria (intrinsic interpretability VS post-hoc, model-specific VS model-agnostic, local VS global explanations), but the most important characteristic, i.e. the \textit{form} of the explanation, is often overlooked.

% include white-box models, model-agnostic approaches \cite{ribeiro2016model} and example-based explanations \cite{aamodt1994case,kim2016examples,barbiero2020uncovering}.


% decision trees \cite{breiman1984classification}, or decision rules: oneR \cite{holte1993very}, RIPPER \cite{cohen1995fast}, Bayesian Rule Lists \cite{letham2015interpretable}).

% \begin{itemize}
%     \item many interesting works around explainability, from fully interpretable models (LR, DT, DR), to surrogates (LIME, Anchors, SHAP, etc) to example-based
%     \item great effort on scoring/ranking features/concepts
%     \item that's NOT the whole point
%     \item what matters (even more?) is how concepts are related (PDP? mah...)
%     \item what is the effort for the end user for analyzing a pairwise dependence plot or a ranking or a decision tree with depth 5?
%     \item good explanations must be simple
%     \item simple <-> few concepts involved? well yes, but...
%     \item traditional methods tend to assume: simplicity -> simple relationships among concepts (linear, max PDP)
%     \item we argue: why??
% \end{itemize}

% % -idee generali su che tipo di bestie c'è per fare expl..
% % -s'è già detto che i sistemi a regole sono più utili per fare supporto a umani.. che robe c'è in giro, perchè il nostro è più fiho
% % - il survey congnitivo dice che regole buone devono essere semplici.. -> pruning! che tipi di pruning usa sta gente che fa expl?

% What Is an Explanation? An explanation is the answer to a why-question (Miller 2017).


% to mention: (Bayesian Rule Lists: \cite{letham2015interpretable} tipo decision trees)

% \begin{itemize}
%     \item taxonomy
%     \begin{itemize}
%         \item intrinsic or post-hoc? LENs support both!
%         \item result of the interpretation:
%         \begin{itemize}
%             \item Feature summary statistic (feature importance or pairwise feature interactions or rank visualization)
%             \item Model internals (weights in linear models or the learned tree structure)
%             \item Data point (counterfactual explanations or identification of prototypes of predicted classes)
%             \item Intrinsically interpretable model
%         \end{itemize}
%         \item Model-specific or model-agnostic?
%         \item Local or global?
%     \end{itemize}
%     \item Properties of Explanation Methods
%     \begin{itemize}
%         \item Expressive Power is the "language" or structure of the explanations (IF-THEN rules, decision trees, a weighted sum, natural language or something else)
%         \item Translucency describes how much the explanation method relies on looking into the machine learning model
%         \item Portability
%         \item Algorithmic Complexity
%     \end{itemize}
%     \item Properties of Individual Explanations
%     \begin{itemize}
%         \item Accuracy: How well does an explanation predict unseen data?
%         \item Fidelity: How well does the explanation approximate the prediction of the black box model?
%         \item Consistency: How much does an explanation differ between models that have been trained on the same task and that produce similar predictions?
%         \item Stability: How similar are the explanations for similar instances?
%         \item Comprehensibility: How well do humans understand the explanations?
%         \item Certainty: Does the explanation reflect the certainty of the machine learning model?
%         \item Degree of Importance: How well does the explanation reflect the importance of features or parts of the explanation?
%         \item Novelty: Does the explanation reflect whether a data instance to be explained comes from a "new" region far removed from the distribution of training data?
%         \item Representativeness: How many instances does an explanation cover?
%     \end{itemize}
%     \item good explanations
%     \begin{itemize}
%         \item Explanations are contrastive (Lipton 1990)
%         \item Explanations are selected (simple)
%         \item Explanations are social. They are part of a conversation
%         \item Explanations focus on the abnormal. People focus more on abnormal causes to explain events (Kahnemann and Tversky, 1981).
%         \item Explanations are truthful. Good explanations prove to be true in reality
%         \item Good explanations are consistent with prior beliefs of the explainee
%         \item Good explanations are general
%     \end{itemize}
%     \item interpretable models: logistic regression, decision trees, decision rules and the RuleFit algorithm
%     \item model agnostic:
%     \begin{itemize}
%         \item plots: Accumulated local effects, Partial Dependence Plot, Individual Conditional Expectation
%         \item surrogates: Global Surrogate, Local Surrogate (LIME), \textbf{Scoped Rules (Anchors)} (many scenarios require discretization, many calls to the ML model), \textbf{SHAP} (SHapley Additive exPlanations)
%     \end{itemize}
%     \item example based: Counterfactual explanations, Prototypes
%     \item neural networks: Feature Visualization, Concepts, Modell Distillation (How can we explain a neural network with a simpler model?)
% \end{itemize}

% \paragraph{Occam's razors}
% In his Posterior Analytics, Aristotle stated: "We may assume the superiority ceteris paribus [other things being equal] of the demonstration which derives from fewer postulates or hypotheses" \cite{aristotlePosterior}. The \textit{law of parsimony} presented by the Greek philosopher has deeply influenced researchers and scientists across the centuries. In other words, when humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one. Researchers have proposed many approaches to integrate this parsimony principle into learning machines over the years. Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous approaches. Among such techniques, $L1$-regularization \cite{santosa1986linear,tibshirani1996regression} has been recently shown quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages sparsity by shrinking the less important weight's values to zero thus removing some weights altogether in the limit. Following \cite{ciravegna2020human}, the models analyzed in this work are mainly based on $L1$-regularization. However, in future works it may also worth exploring the integration of LENs with concept-based parsimony criteria \cite{chen2020concept} or with fuzzy-logic regularizers which have recently been used to combine deductive reasoning and human priors with deep learning \cite{marra2019lyrics}.






\subsection{Application of LENs to Adversarial Attacks}
The explanations provided by LENs are first-order logic formulas, and this newly devised pieces of knowledge can be reused and enforced on the output of the classifier $g$. This is commonly considered in the generic \emph{learning from constraints} framework \cite{gnecco2015foundations}, and it may be of particular interest, especially for semi-supervised settings. A similar strategy has already been considered e.g. in \cite{ciravegna2020constraint}, where a set of FOL formulas have been, at first extracted from data, and then converted into continuous loss functions to be injected in the learning objective.
Furthermore, the extracted formulas can also be used to check the behaviour of the classifier on test data, e.g. to detect adversarial samples as done in \cite{melacci2020domain}.
In the following, we consider this last scenario in the context of the bird-identification task (CUB 200), where a convolutional neural network (ResNet18) is trained from scratch to classify both the main classes and the 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.6\textwidth]{figs/cub_adv_plot.pdf}
    \caption{Quality of the explanations extracted by the LENs in terms of robust accuracy when used to defend a model. In purple, the accuracy of the model when facing a white box attack without any defense. Error bars show the 95\% confidence interval of the mean. }
    \label{fig:time}
\end{figure}




%At last, the extracted formulas can also be used to check the behaviour of the classifier on test data, e.g. to detect adversarial samples as done in \cite{melacci2020domain}.


% The experiments show how this framework can be used to aid bias identification and to make black boxes more robust to adversarial attacks by giving an explanation for the attack itself.

\section{Conclusion} \label{sec:conclusion}

\subsection{Limitations and future research directions}
The extraction of a first-order logic explanation requires symbolic input and output spaces. This constraint is the main limitation of our framework, as narrows the range of applications down to symbolic I/O problems. In some contexts, such as computer vision, the use of LENs may require additional annotations and attribute labels to get a consistent symbolic layer of concepts. However, recent work on automatic concept extraction may partially solve this issue leading to more cost-effective concept annotations \cite{ghorbani2019towards,kazhdan2020now}.

Another area to focus on might be the improvement of out-of-the-box LENs. The efficiency and the classification performances of fully interpretable LENs, i.e. $\psi$ network, is still quite limited due to the extreme pruning strategy. Even more flexible approaches, like $\mu$ networks, are not as efficient as standard neural models when tackling multi-class or multi-label classification problems, as they require a bigger architecture to provide a disentangled explanation for each class.

In our vision this framework would thrive and express its full potential by interacting with the external world and especially with humans in a dynamic way. In this case, logic formulas might be rewritten as sentences to allow for a more natural interaction with end users. Moreover, a dynamic interaction may call for an extended expressivity leading to higher-order or temporal logic explanations. Finally, in some contexts different neural architectures as graph neural networks might be worth exploring as they may be more suitable to solve the classification problem.


\subsection{Broader impact}
Current legislation in US and Europe binds AI to provide explanations especially when the economical, ethical, or financial impact is significant \cite{gdpr2017,law10code}. This work contributes to a lawful and safer adoption of some of the most powerful AI technologies allowing deep neural networks to have a greater impact on society. Extracting first-order logic explanations from deep neural networks enables satisficing knowledge distillation while achieving performances comparable with the state of the art. The formal language of logic provides clear and synthetic explanations, suitable for laypeople, managers, and in general for decision makers outside the AI research field.

The experiments show how this framework can be used to aid bias identification and to make black boxes more robust to adversarial attacks by giving an explanation for the attack itself. As out-of-the-box LENs are easy to use even for neophytes and can be effectively used to understand the behavior of an existing algorithm, our approach might be used to reverse engineer competitor products, to find vulnerabilities, or to improve system design. From a scientific perspective, formal knowledge distillation from state-of-the-art networks may enable scientific discoveries or confirmation of existing theories.


\section*{Acknowledgments and Disclosure of Funding}
We thank ... for useful feedback and suggestions.

This work was partially supported by the European Union’s Horizon 2020 research and innovation programme under grant agreement No 848077.




\bibliographystyle{apalike}  % Sry Pietro, just had to
\bibliography{references}  %%% Remove comment to use the external .bib file (using bibtex).
%%% and comment out the ``thebibliography'' section.

\end{document}


==> main_july_22_backup.tex <==

% \usepackage{icml2021}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[pagebackref=true,
    breaklinks=true,
    colorlinks,
    linkcolor=blue,
    citecolor=blue,
    filecolor=black,
    urlcolor=blue,
    bookmarks=false]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{caption}
\usepackage{subcaption}

\setcounter{secnumdepth}{6}


\usepackage{tikz}
% \usetikzlibrary{decorations}
\usetikzlibrary{decorations.text}
\usetikzlibrary{arrows.meta,bending,decorations.markings}


\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}

\lstset{style=mystyle}

\usepackage{pifont}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{float}
\usepackage{fontawesome}
\usepackage{makecell}

\def\UrlFont{\rmfamily}
\usepackage{fancyhdr}
\usepackage{mathrsfs}
\usepackage{color}
\usepackage{hyperref}
\usepackage{longtable}
\hypersetup{colorlinks=true}
% \usepackage[linesnumbered, ruled]{algorithm2e}


\newtheorem{definition}{Definition}[]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{example}{Example}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\graphicspath{ {./images/} }


\def\[#1\]{$$#1$$}

\def\frac#1#2{{#1\over#2}}
\def\eps{\varepsilon}

\def\bbR{{\bf R}}
\def\X{{\bf X}}
\def\meno{\medskip\noindent}

\newcommand{\draft}[1]{\textcolor{violet}{#1}}

\newcommand{\fg}[1]{\textcolor{red}{F: #1}}
\newcommand{\gc}[1]{\textcolor{red}{G: #1}}
\newcommand{\sm}[1]{\textcolor{blue}{#1}}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.5}


\title{Logic Explained Networks}

\author{Gabriele Ciravegna\thanks{Equal contribution}\hspace{1.2mm}$^{1,2}$\hspace{1.2mm}\href{https://orcid.org/0000-0002-6799-1043}{\includegraphics[scale=0.06]{orcid.png}},
Pietro Barbiero$^{*3}$\hspace{1mm}\href{https://orcid.org/0000-0003-3155-2564}{\includegraphics[scale=0.06]{orcid.png}},
Francesco Giannini$^{*2}$, \\
\textbf{
Marco Gori$^{2,4}$\hspace{1mm}\href{https://orcid.org/0000-0001-6337-5430}{\includegraphics[scale=0.06]{orcid.png}},
Pietro Li\'o$^{3}$,
Marco Maggini$^{2}$,
Stefano Melacci$^{2}$\hspace{1mm}\href{https://orcid.org/0000-0002-0415-0888}{\includegraphics[scale=0.06]{orcid.png}}
}\\
$^{1}$Università di Firenze (Italy), $^{2}$Università di Siena (Italy), \\ $^{3}$University of Cambridge (UK), $^{4}$Universitè Côte d’Azur (France)\\
\texttt{gabriele.ciravegna@unifi.it, pb737@cam.ac.uk, francesco.giannini@unisi.it}\\
\texttt{marco.gori@unisi.it, pl219@cam.ac.uk, marco.maggini@unisi.it, mela@diism.unisi.it}
}

\begin{document}
\maketitle
\begin{abstract}
The large and still increasing popularity of deep learning clashes with a major limit of neural network architectures, that consists in their lack of capability in providing human-understandable motivations of their decisions.
%Despite the increasing popularity of deep networks in real-world application, in real wold domains the employment of deep neural networks is still limited and strongly criticized due to their lack of interpretability.
In situations in which the machine is expected to support the decision of human experts, providing a comprehensible explanation is feature of crucial importance.
%providing a comprehensible explanation for a certain classification task can be crucial in decision support contexts.
The language used to communicate the explanations must be formal enough to be implementable in a machine and friendly enough to be understandable by a wide audience.
%To this aim, rule-based explanations expressed in a high-level language are particularly relevant.
In this paper, we propose a general approach to Explainable Artificial Intelligence in the case of neural architectures, showing how a mindful design of the networks leads to interpretable deep learning models called Logic Explained Networks (LENs).
LENs only require their inputs to be semantically meaningful and human-understandable predicates, and they provide explanations in terms of simple First-Order Logic (FOL) formulas involving such predicates. LENs are general enough to cover a large number of scenarios. Amongst them, we consider the case in which LENs are directly used as special classifiers with the capability of being explainable, or when they act as additional networks with the role of creating the conditions for making a black-box classifier explainable by FOL formulas.
%Explanations can be either local (single-example level) or global (problem level), and,
Despite supervised learning problems are mostly emphasized,
%and are given as first-order logic formulas expressed in terms of input concepts.
we also show that LENs can learn to provide explanations in unsupervised learning settings.
%to provide explanations of the predictions made either by a black-box model or by the LEN itself.
We describe and evaluate three different use-cases of the LEN framework, based on multiple out-of-the-box LEN models. Experimental results on several datasets and tasks show that LENs not only yield better classifications than established white-box models, such as decision trees and Bayesian rule lists, but they also provide more compact and meaningful explanations.
\end{abstract}


\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/general_schema_stefano.pdf}
\caption{Logic Explained Networks (LENs) are neural networks capable of making predictions and providing First-Order Logic explanations. In detail, A LEN (blue box -- function $f$) provides FOL explanations (purple box -- formulas belong to $P$) of a set of output concepts (rightmost yellow-box -- output concepts belong to set $E$) in function of the LEN inputs, that might be other concepts (mid yellow box -- input concepts belong to $C$) computed by a neural network (gray box -- function $g$) and/or concepts provided within the available data (leftmost yellow box -- data belong to $X$), following the dotted connection).  %Colors are used in all figures to identify different parts of the framework: yellow boxes contain input data and concepts, output predictions and labels; grey boxes represent the black box classifier $g$ that can either provide final classification or extract low-level concepts; the blue box represents the LEN $f$; t
There are several different ways of instantiating this generic model into real-world problems, that are described in Section~\ref{sec:basics}.
Within the blue box, the key components of LENs are listed, that are the main subject of Section~\ref{sec:methods}:  Learning Criteria (Section~\ref{sec:learncrit}), FOL Rule Extractor (Section~\ref{sec:logic_rule_extr}), and the Parsimony Criteria (Section~\ref{sec:parsimony}).
}
    \label{fig:framework}
\end{figure}

\begin{figure}[h]
    \centering

     \includegraphics[width=1.\textwidth]{figs/abstract.pdf}
         \caption{An example of a possible instance of the generic model of Fig.~\ref{fig:framework}, inspired by the CUB 200-2011 fine-grained classification dataset. Classes are divided into a two-level hierarchy. A LEN is placed on top of a convolutional neural network $g(\cdot)$ in order to \textit{(i)} classify the species of the bird in input and \textit{(ii)} provide an explanation on why it belongs to this class. The logic explanation in the example showcases a sample output class (all the output concepts can be explained).
         %\gc{Prendere la figura di NIPS e cambiare i colori e la figura iniziale in modo da non essere troppo simili all'altro paper.\\}
         %{\color{red}[Add at least another output concept (no need to show its explanation). Avoid being to strictly close to the CUB dataset, otherwise the example is not clear. In other words, make black-footed-albatross the name of the output concept (instead of 'bird') and also add another one. Rename the input concepts with the names that are in the purple box. If they are too long, you can shorten them by renaming them in a more simple manner (hooked-bill, solid-wing, medium-size, white-throat, black-bill). Moreover, user the lower-case $x$ instead of $X$.]}\\
         %\fg{da cambiare un po' l'img perchè è la stessa img di NIPS.. cambierei esempio}
         %\fg{forse metterei $\forall c, billShapeHooked(c)\wedge...$}
         {\color{red}offuscare un po' per evitare similitudine forte con NeurIPS; al posto di LOGIC EXPLANATIONS scrivere LOGIC EXPLANATION $\rho \in P$ OF Black Footed Albatross}}
         \label{fig:len}

\end{figure}


\section{Introduction}
The application of deep neural networks in safety-critical domains has been strongly limited \cite{chander2018working}, since neural networks are generally considered black-boxes whose decision processes are opaque or too complex to be  understood by users. 
%\fg{tolto perchè era identito a quello mandato a NIPS} The lack of transparency in the decision process of some machine learning models, such as neural networks, limits their application in many safety-critical domains \cite{chander2018working}. 
Employing black-box\footnote{In the context of this paper, a black-box classifier is any classifier that cannot provide human understandable explanations about its decision.} models may be unacceptable in contexts such as industry, medicine or courts, where the potential economical or ethical repercussions are calling for lawmakers to discourage from a reckless application of non-interpretable models \cite{gdpr2017,law10code,goddard2017eu,gunning2017explainable}. As a consequence, research in Explainable Artificial Intelligence (XAI) has become strategic and has been massively encouraged, leading to the development of a variety of techniques that aim at explaining black-box models \cite{das2020opportunities,brundage2020toward} or at developing effective interpretable models \cite{carvalho2019machine,rudin2019stop}.
% Some of the latter case, like decision rules, provide one of the best forms of explanations as they were originally developed for decision support systems \cite{sprague1980framework}.

The notions of \emph{interpretability} and \emph{explainability} were historically used as synonyms, however nowadays the distinction between interpretable models and models providing explanations has become more evident, as recently discussed by different authors \cite{gilpin2018explaining,lipton2018mythos,marcinkevivcs2020interpretability}.
Even if there are no common accepted formal definitions, a model is considered interpretable when its decision process is generally transparent and can be understood directly by its structure and parameters, such as \emph{linear models} or \emph{decision trees}. On the other hand, the way an existing (black-box) model makes predictions can be explained by a surrogate interpretable model or by means of techniques based on providing intelligible descriptions of the model behaviour by e.g. formal rules, saliency maps, question-answering. 
% {\color{red}[Say something on the definitions of interpretability and explainability, connected to what follows (we need to define what we mean with these terms).]}
In some contexts, the use of a black-box model may be unnecessary or even not preferable \cite{rudin2019stop}. For instance, a proof of concept, a prototype, or the solution to a simple classification problem can be easily based on standard out-of-the-box AI solutions which are interpretable by design.
However, interpretable models may generally miss to capture complex relationships among data. Hence, in order to achieve state-of-the-art performance in more challenging problems, it may be necessary to exploit black-box models that, in turn, may require an additional explanatory model to gain the trust of the user.

In the literature, there is a wide consensus on the necessity of having an explanation for machine learning models that are employed in safety-critical domains, while there is not even agreement on what an \emph{explanation} actually is, nor if it could be formally defined \cite{doshi2017towards,lipton2018mythos}.
An explanation should serve cognitive-behavioral purposes such as engendering trust, aiding bias identification, or taking actions/decisions \cite{srinivasanexplanation}. An explanation may help humans understand the black box, may allow for a deeper human-machine interaction \cite{koh2020concept}, and may lead to more trustworthy fully automated tasks. All of this is possible as long as the explanations are useful from a human perspective.
% and take into account how humans think and make decisions
In a nutshell, an explanation is an answer to a ``why'' question %\cite{miller2019explanation}.
%But what is that characterize a good explanation?
and what makes an explanation good or bad depends on ``the degree to which a human can understand the cause of a decision'' \cite{miller2019explanation}. The goodness of an explanation is intimately connected to how humans collect evidences and eventually make decisions.
In Herbert Simon's words we may say that a good explanation is \textit{satisficing} \cite{simon1956rational}, i.e. \textit{it either gives an optimal description of a simplified version of the black box (e.g. a surrogate model) or a satisfactory description for the black box itself}
% \footnote{"Decision makers can satisfice either by finding optimum solutions for a simplified world, or by finding satisfactory solutions for a more realistic world".}
\cite{simon1979rational}. However, the notion itself of explanation generally depends on both the domain of the application and who it is aimed at \cite{carvalho2019machine}.
% This is the reason why, different criteria and taxonomies
% such as the \textit{scope}, the \textit{usage} and the \textit{methodology} have been identified as key-properties to define a XAI technique \cite{das2020opportunities}.


The need for high-quality evidences is one of the main reasons why concept-based explanations are receiving ever-growing consideration. Explanations are given in terms of human-understandable symbols (the \textit{concepts}) rather than raw features such as pixels or characters \cite{kim2018tcav,ghorbani2019towards,koh2020concept}. As a consequence, they seem more suitable to serve many strategic human purposes such as decision making tasks. For instance, a concept-based explanation may describe a high-level category through its attributes as in ``a \textit{human} has \textit{hands} and a \textit{head}''.
% However, many concept-based explanations still look ambiguous, it is not obvious how to \textit{quantitatively} assess their generality, and may not be suitable for effective decision making at all.
% How much effort requires analyzing a pairwise dependence plot \cite{friedman2008predictive} or a ranking of SHAP values \cite{NIPS2017_7062} or a decision tree with depth 10 \cite{breiman1984classification} for domain experts? How much for laypeople?
% If you are looking for a quick and comprehensible answer these methodologies will not suit your needs.
While collecting high-quality evidences for an explanation is a common feature of concept-based techniques, there are very few approaches formulating hypothesis and even less providing synthetic descriptions whose validity can be quantitatively assessed \cite{das2020opportunities}.
A possible solution is to rely on a formal language that is
% synthetic but also
very expressive, closely related to reasoning, and somewhat related to natural language expressions, such as First-Order Logic (FOL). A FOL explanation can be considered a special kind of a concept-based explanation, where the description is given in terms of logical predicates, connectives and quantifiers, such as ``$\forall x:\ \textit{is\_human}(x) \rightarrow \textit{has\_hands}(x) \wedge \textit{has\_head}(x)$'', that reads ``being human implies having hands and head''. However, FOL formulas generally express much more complex relationships among the concepts %that are
involved in a certain explanation. Compared to other concept-based techniques, logic-based explanations provide many key advantages, that we briefly described in what follows.
% \begin{itemize}
% CLARITY
An explanation reported in FOL is a rigorous and unambiguous statement (\textsc{clarity}). This formal clarity may serve cognitive-behavioral purposes such as engendering trust, aiding bias identification, or taking actions/decisions. For instance, dropping quantifiers and variables for simplicity, the formula ``\textit{snow} $\wedge$ \textit{tree} $\leftrightarrow$ \textit{wolf}'' may easily outline the presence of a bias in the collection of training data.
% MODULARITY
Different logic-based explanations can be combined to describe groups of observations or global phenomena (\textsc{modularity}). %Different observations of the same phenomenon may have completely different %logic-based
%explanations according to their characteristics.
For instance, for an image showing only the face of a person, an explanation could be ``(\textit{nose} $\wedge$ \textit{lips}) $\rightarrow$ \textit{human}'', while for another image showing a person from behind a valid explanation could be ``(\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})  $\rightarrow$ \textit{human}''. The two local explanations can be combined into ``(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears}) $\rightarrow$ \textit{human}''.
% MEASURABILITY
The quality of logic-based explanations can be quantitatively measured
    % on independent data sets
to check their correctness and completeness (\textsc{measurability}). For instance, once the explanation ``(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})'' is extracted for the class \textit{human}, this logic formula can be applied on a test set to check its generality in terms of quantitative metrics like accuracy, fidelity and consistency.
% SIMPLIFIABILITY
Finally, FOL-based explanations can be rewritten in
    different equivalent forms such as in \emph{Disjunctive Normal Form} (DNF) and \emph{Conjunctive Normal Form} (CNF)  (\textsc{simplifiability}). Further, techniques such as the Quine–McCluskey algorithm can be used to compact and simplify logic explanations \cite{mccoll1878calculus,quine1952problem,mccluskey1956minimization}. As toy example, consider the explanation ``(\textit{person} $\wedge$ \textit{nose}) $\vee$ ($\neg$\textit{person} $\wedge$ \textit{nose})'', that can be easily simplified in ``\textit{nose}''.
% \end{itemize}


This paper presents a unified framework for XAI where a neural network, the \emph{Logic Explained Network} (LEN), is trained to \textit{solve-and-explain} a categorical learning problem integrating elements from deep learning and logic.
Differently from vanilla neural architectures, LENs can be directly interpreted by means of a set of FOL formulas. In order to implement such a property, LENs require their inputs to represent the activation scores of human-understandable concepts. Then, specifically designed learning objectives allow LENs to make predictions in a way that is well suited for providing FOL-based explanations that involve the input concepts. In order to reach this goal, LENs exploit parsimony criteria aimed at keeping their structure simple.
% learn a set of explanations of its classification results, or for the class-assignments of another classifier.
%(eventually another neural network).
There are several different computational pipelines in which a LEN can be configured, depending on the properties  of the considered problem and on other potential experimental constraints. For example, LENs can be used to directly classify data in an explainable manner, or to explain another black-box neural classifier. Moreover, according to the user expectations, different kinds of logic rules may be provided.
Due to this intrinsic versatility of LENs, what we propose can also be taught as a generic framework that encompasses a large variety of use cases.

%This versatility makes the proposed framework
%and in particular LENs
%applicable to a wide range of learning tasks and in different use cases. % by providing logic-based explanations in different use cases. % and according to different user preferences.
Fig.~\ref{fig:framework} depicts a generic view on LENs, in which the main components are reported. A LEN (blue box -- function $f$) provides FOL explanations (purple box) of a set of output concepts (rightmost yellow-box) in function of the LEN inputs. Inputs might be other concepts (mid yellow box) computed by a neural network classifier (gray box -- function $g$) and/or concepts provided within the available data (leftmost yellow box). %The output concepts are the ones that are the main subject of the explanations (e.g., they could be the classes of a classification problem). Explanations involve the inputs of the LEN.
This generic structure can be instantiated in multiple ways, depending on the final goal of the user and on the properties of the considered problem. In order to provide the reader with an initial example/use-case (different configurations are explored in the paper), we consider an image classification problem with concepts organized into a two level hierarchy. In Fig.~\ref{fig:len} we report an instance of Fig.~\ref{fig:framework} in which a CNN-based neural classifier gets an input image, predicting the activations of a number of low-level concepts (organized in a vertical manner). The LEN $f$ processes such concepts, and it predicts the activation of higher-level output concepts. The LEN can provide a FOL description of each (high-level) output concept with respect to the (low-level) input ones. Another possible instance of the proposed framework consists in using the LEN to directly classify and explain some input data (that is basically the case in which the input concepts are immediately available in the data themselves, and not the output of another neural model), thus the LEN itself becomes an interpretable machine. Moreover, LENs can be paired with a black-box classifier operating on the same input data, and forced to mimic as much as possible the behaviour of the black-box, basically implementing an additional  explanation-oriented module. At a first glance, since the internal structure of LENs is subject to a number of constraints, LENs might not be as powerful as a black-box classifier. However, the versatility of LENs allows the user to customize his approach to the considered classification problem in order to find a satisfactory compromise between interpretability and accuracy.

We investigate three different use-cases that are inspired by the aforementioned instances, comparing different ways of implementing the LEN models. 
While most of the emphasis of this paper is on supervised classification, we also show how LEN can be exploited in fully unsupervised settings.
Additional human priors could be eventually incorporated into the learning process \cite{ciravegna2020constraint}, in the architecture \cite{koh2020concept}, and, following \cite{ciravegna2020constraint,ciravegna2020human}, what we propose can be trivially extended to semi-supervised learning (out of the scope of this paper).


%Furthermore, LENs can also be integrated with existing black-box classifiers to extract low-level concepts or to explain their classification results.




%The overall problem configuration of how a Logically Explained Network can be integrated with an existing classifier is shown in Fig. \ref{fig:framework} and further described in Sec. \ref{sec:use_cases}. A configuration example is reported in Fig. \ref{fig:len}.




%Out-of-the-box neural networks based on this framework span a wide range of flavors, from fully interpretable models to black-boxes providing different interpretability-VS-accuracy trade-off.
%high-quality explanations and state-of-the-art classification performance.

%Further, human priors expressed by FOL formulas can be naturally incorporated with LENs both in the learning process \cite{ciravegna2020constraint} and in the architecture \cite{koh2020concept}.

Our work contributes to the XAI research field in the following ways.
\begin{itemize}
    \item It provides a unifying framework for solving and explaining categorical learning problems with neural networks. We designed the LEN framework inspired by our previous experiences \cite{ciravegna2020human,ciravegna2020constraint}.
    \item It allows users to decide how to interconnect LENs in the classification task under investigation, and to express a set of preferences to get one or more customized explanations. We provide and experimentally evaluate three out-of-the-box preset models.
    % \item Supporting a wide range of logic-based explanations from \textit{local explanations} and \textit{node-level explanations}, explaining the prediction for an individual sample or a hidden neuron, to \textit{cluster explanations} up to \textit{class-level explanations} and \textit{global explanations}.
    \item It offers a wide range of logic-based explanations, also showing that they can be restricted in their scope, working at different levels of granularity (explaining a single sample, a subset of the available data, etc.).
    \item It reports experimental results confirming how LENs generalize better in terms of model accuracy than established white-box models such as decision trees on complex boolean tasks (as observed in \cite{tavares2020understanding}).
    \item It advertises our public implementation of LENs through a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on out-of-the-box LENs, implementing different trade-offs between intepretability/explainability and accuracy.
\end{itemize}

% \paragraph{Reading path}
The paper is organized as follows. Related works are described in Section \ref{sec:related}. Section \ref{sec:basics} gives a formal definition of a LEN and it describes its underlying assumptions, key paradigms and design principles. The methods used to extract logic formulas and to effectively train LENs are described in Section \ref{sec:methods}. Three out-of-the-box LENs, presented in Section \ref{sec:outofthebox}, are compared on a wide range of benchmarks in terms of classification performance and quality of the explanations, in Section \ref{sec:experiments}.
% A coding example showing how to use LENs with the associated python library is shown in Section \ref{sec:tool}.
Finally, Section \ref{sec:conclusion} outlines the social and economical impact of this work as well as future research directions.


\section{Related work}
\label{sec:related}


In the last few years, the demand for human-comprehensible models has significantly increased in safety-critical and data-sensible contexts. This popularity is justified by the emerging need for unveiling the decision process of pitch-black models like deep neural networks. To this aim, the scientific community has developed an important variety of XAI techniques, with different properties and goals. Several taxonomies have been proposed to categorize the XAI models, with partial overlapping and some ambiguities on the referred terminology. Without pretending to be exhaustive, in the following we only focus on some key-properties that are relevant to compare LENs with other existing approaches. In particular, we will describe related works considering the type of \textsc{result} they provide (feature-scoring vs. rule-based),
their specific \textsc{role} (interpretable models vs. explanation methods),
and the \textsc{scope} of the provided explanations (local vs. global). A brief summary of a few XAI works in terms of these features is reported in Tab.~\ref{tab:related_work} -- for more details on existing taxonomies we refer, e.g., to the following surveys \cite{adadi2018peeking,carvalho2019machine,marcinkevivcs2020interpretability,molnar2020interpretable}.

%\textsc{Results of Explanation Methods. }
XAI models can be differentiated according to the \textsc{result} of the produced explanation.
Most of the methods in literature usually focus on scoring or providing summary statistics of features. However, \textit{feature-scoring} methods
%
can be of scarce utility in decision support cases, whereas a comprehensible language may bring light on the black-box behaviour by identifying concept-based correlations.
% do not consider how concepts are interconnected, therefore, these explanations may not live up to the expectations.
On the other hand, \emph{rule-based} explanations are generally more comprehensible, since they usually rely on a formal language, such as FOL. Further, the learned rules can be directly applied to perform the learning task in place of the explained model.
%\textsc{Explanation Usage. }
Existing approaches has different \textsc{roles} in the XAI landscape, acting as intrinsically \emph{interpretable models} or as \emph{explanation methods}. 
As a matter of fact, the interpretability of a model can be achieved either by constraining the model to be interpretable per se (\emph{interpretable models}) or by applying some methods to get an explanation of an existing model (\emph{explanation methods}). Interpretable models are by definition {model specific}, while explanation methods can rely on a single model or be, as more commonly happens, {model agnostic}. In principle, interpretable models are the best suited to be employed as decision support systems. However, their decision function often is not smooth which makes them quite sensible to data distribution shifts and impairs their generalization ability on unseen observations \cite{tavares2020understanding,molnar2020interpretable}.
On the other hand, explanation methods can be applied to get approximated interpretation of state-of-the-art models. These methods are generally {``post hoc''}, since the explanations are produced when the training procedure is concluded.
%\textsc{Scope of Interpretability. }
A fundamental feature to distinguish among explainable methods is the \textsc{scope} of the provided explanations. \textit{Local} explanations are valid for a single given sample, while \textit{global} explanations {hold} on the whole input space. However, several models consider local explanations together with aggregating heuristics to get a global explanation.
Some of the most famous XAI techniques share the characteristics of being feature-scoring, local, post hoc methods.

% {\bf Methodology. }
% The algorithms employed by most XAI models can be roughly categorized into two main categories. \textit{Backpropagation}-based techniques analyze the gradients of the activation up to the input features, in order to identify the most relevant ones for the classification task. \textit{Perturbation}-based techniques, instead, observe how the machine output changes when altering a given input data. The aim of these methods is to understand which %are the most discriminative
% features (when altered) may drive the model to take different decisions.
% Nonetheless, not all algorithms belong to these two categories. In particular, \textit{Model-intrinsic} explanation methods significantly differ according to the training algorithms.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
                                    & \multicolumn{2}{c|}{\textbf{Result Type}} & \multicolumn{2}{c|}{\textbf{Scope}} & \multicolumn{2}{c}{\textbf{Role}} \\
                        & feature-scoring & rule-based & local & global & interpretable model & explanation method \\
\hline
LIME &\faCheckCircle & & \faCheckCircle            & & & \faCheckCircle  \\
SHAP &\faCheckCircle & & \faCheckCircle & & & \faCheckCircle  \\
% DeConv \cite{zeiler2014visualizing}                     &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           & \faCheckCircle         &               &                  \\
Activation Maximization & \faCheckCircle & & \faCheckCircle  &  &  & \faCheckCircle  \\
Saliency Maps &\faCheckCircle&& \faCheckCircle &      &              & \faCheckCircle \\
% Grad-CAM \cite{selvaraju2017grad}                       &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
SP-LIME &\faCheckCircle&& & \faCheckCircle &              & \faCheckCircle  \\
Class Model Visualization &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle                 \\
% TCAV \cite{kim2018tcav}                                 &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
LORE &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle \\
Anchors &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle  \\
DeepRED   &&\faCheckCircle& \faCheckCircle & \faCheckCircle &  & \faCheckCircle \\
GAM  &\faCheckCircle&&              & \faCheckCircle          & \faCheckCircle            &   \\
Decision Trees       &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
BRL                   &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
\hline
\textbf{LENs}                                           &&\faCheckCircle& \textbf{\faCheckCircle}    & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle} \\
\end{tabular}
}
\vspace{0.3cm}
\caption{Summary of related work. The first column lists a number of approaches in the context of XAI. The other columns are about different properties. See the paper text for more details and for a description of all the approaches. }
\label{tab:related_work}
\end{table}



Sometimes indeed, the easiest way to solve the explanation problem is simply to treat the model as a black-box and, sample-by-sample, determine which are the most important features for a prediction.
Prominent examples of algorithms falling in this area %are Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should}, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} and DeConvolution Neural Network (DeConv) \cite{zeiler2014visualizing}, which
accomplish this task by perturbing the input data.
Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should} trains a white-box model (e.g., a logistic regression) to mimic the predictions of a given model in the neighbourhood of the sample to explain. By analyzing the weights of the white-box model it identifies the most important group of pixels (superpixel).
Differently, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} computes the Shapley value of each feature by removing each of them in an iterative manner. %provides for local explanations by computing each input feature contributions in a certain prediction. In the Kernel SHAP version, the Shapley values of each feature are calculated by iteratively removing features in a similar way to what is done in LIME.
% Deconvolutional Network were initially introduce in \cite{zeiler2011adaptive} for unsupervised learning.
% Firstly introduced in \cite{zeiler2011adaptive}, DeConvolution Neural Network (DeConv) are used in \cite{zeiler2014visualizing} to %visualize the activation of a convolutional layer. In particular, they
%visually determine pixel importance for a certain prediction by analyzing how the classification output changes when part of the input image is masked.
Other important techniques %such as Activation Maximization \cite{erhan2010understanding}, Saliency Maps \cite{simonyan2013deep} and Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad}
provide the same type of explanations through gradient analysis. %Differently from the previous one, however, they determine feature importance  %in the context of Convolutional Neural Network (CNN).
Authors of Activation Maximization \cite{erhan2010understanding} firstly introduced this idea as an optimization problem. They explain the behaviour of a hidden/output unit by slightly modifying a given input data such that it maximizes its activation. An easier way to identify features causing a certain output has been found with Saliency Maps \cite{simonyan2013deep}, which project the classification loss until the input image.
% A further improvement has been introduced with Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} which allows to identify both class-specific image area and counterfactual explanations.
%They achieved this by modifying global average pooling with class activation mapping which allows to identify important image area with a single forward pass.
%
Other post hoc methods have been devised to extract global feature-scoring explanations, often starting from local explanations. %like LIME for Global Explanations \cite{ribeiro2016should} based on perturbation and Class Model Visualization \cite{simonyan2013deep} or Testing with Concept Activation Vectors \cite{kim2018interpretability} based on Backpropagation.
A submodular-pick algorithm extends the LIME module (SP-LIME) in %LIME for Global Explanations
\cite{ribeiro2016should} to provide global explanations. SP-LIME first finds superpixels of all input samples with the standard LIME module. Successively, it finds the minimum number of common superpixels that covers most of the images.
Starting from the idea of Activation Maximization, Class Model Visualization \cite{simonyan2013deep} finds the input sample that maximizes a certain class probability score in the whole input space. %Differently from Activation Maximization, here the input sample is not searched in the neighbourhood of a given sample, but in the whole input space.
Differently, LENs take another perspective with respect to these methods, still inheriting several of their properties (see Tab.~\ref{tab:related_work}). A LEN aims at providing human comprehensible decision support in terms of a set of FOL rules.


Explanation methods, indeed, can also supply FOL explanations.
LOcal Rule-based Explanations of black-box decision systems (LORE) \cite{guidotti2018local} extracts FOL explanations via tree induction. The authors of \cite{guidotti2018local} focus on local rules extracted through input perturbation. For each sample to explain, a simple decision tree is trained to mimic the behaviour of the black-box model in the neighbourhood of the sample. Both standard and counterfactual explanations can then be extracted  following the branches of the tree.
Again based on LIME, Anchors \cite{ribeiro2018anchors}  also provides local rules of black-box model prediction via input perturbation. In this case, rules are not extracted from a decision tree but are generated by solving a Multi-Armed-Bandit beam search problem.
Extending the CRED algorithm \cite{sato2001rule}, DeepRED  \cite{zilke2016deepred} employs a decomposition strategy to globally explain neural networks. Starting from the output nodes, each node in a layer is explained in terms of the activations of the previous ones through a decision tree. In the end, all rules for each class are merged in a single global rule in terms of input nodes only. For a single example a single local rule can be extracted following the firing path.
The approach proposed in this paper is in some sense similar to the DeepRED algorithm. Indeed, as it will become clear in the following sections, LENs can explain the behaviour of a neural network both end-to-end and layer by layer. However, LENs can be used to explain any black-box model as far as its input and output are interpretable (Section~\ref{sec:basics}). Furthermore, LENs support different forms of FOL rules, with different scopes and goals.

Interpretable models are generally capable of providing both local and global explanations. These explanations may be based again on feature-scoring as in Generalized Additive Models (GAM) \cite{hastie1987generalized} or on FOL rules as in Decision Tree \cite{breiman1984classification} and Bayesian Rule Lists (BRL) \cite{letham2015interpretable}. Meant to overcome the non-linearity assumptions of Linear regression, GAM learns to predict the given class for each feature via decision tree. In \cite{caruana2015intelligible}, authors proposed GA$^2$M where attribute interaction is allowed at a pair level. Recently a further extension employing neural network as non-linear function has been proposed in \cite{agarwal2020neural}, which, however, lose interpretability at feature-level.
Decision trees are a greedy learning algorithm which iteratively divides input data into smaller subsets until they only contain elements belonging to the same class. Different pruning algorithms have been also proposed to simplify the resulting structure and therefore the explanations \cite{quinlan1987simplifying}. Each path of a decision tree may be seen as a decision rule, i.e., an \textit{IF-THEN} statement.
Many algorithms also focus on exactly generating set of decision rules in different ways, either with sequential covering as in \cite{cohen1995fast} or by selecting the best rules from a pre-mined set via Bayesian statistics as in BRL.
%
Interestingly, LENs can be directly used to solve a learning task, being almost interpretable per se.
Employing an interpretable by-design neural network as classifier has the advantage that the extracted explanations will perfectly match the classifier predictions.
In addition, relying on a neural network, LEN generalization performance can be much better than standard interpretable-by-design methods, that generally have a very limited representation capacity.

Summing up, the proposed approach can be used both as interpretable model and explanation method. Indeed, the flexibility of LENs allows the user to find an appropriate trade-off between interpretability/explainability and accuracy that is well suited for the task at hand.
The explanation type of LENs is in terms of FOL rules and different explanation styles, corresponding to different types of logic formulas. The inner mechanism to extract such explanations is general enough to cover rules with different scopes, from local rules valid on a single sample to global rules that hold for an entire class.





\section{Logic Explained Networks}
\label{sec:basics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%O
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTATION REMINDER
%\fg{mettere in tabella es alla fine del 2.1?}
% {\color{red}
% \textbf{Notation}
% X = input space (non-interpretable)\\
% Y = symbolic output space (interpretable)\\
% C = symbolic "concept" space (interpretable)\\
% E = symbolic "rule" space (interpretable)\\

% n = \# samples\\
% d = \# features of X\\
% q = \# categories of Y\\
% k = \# categories of C\\
% r = \# categories of E\\
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DISCORSINO intro su cosa è il nostro modello, cosa fa, a cosa si appoggia.. caratteristiche generali


% Differently from several existing XAI models,
We consider a general framework in which a special kind of neural network, referred to as Logic Explained Network (LEN), is used to make predictions and provide explanations about them, or it is used to  explain the behaviour of another classifier, being it another neural network or another generic black-box model. Moreover, a LEN might also be used to explain relationships among some given data.
%LENs can be defined according to different criteria and exploited in different use cases.
In this section we will formally introduce LENs and the notation used throughout the paper. Then, instead of immediately diving into the internals of LENs (Section~\ref{sec:methods}) or describing the details of the specific neural architectures we considered (Section~\ref{sec:outofthebox}), we will first focus on
the different ways in which LENs can be set up. In particular, we consider how LENs can be instantiated in the framework of Fig.~\ref{fig:framework}, discussing a variety of computational pipelines (Section~\ref{sec:use_cases}), and on the type of explanations that we can ask the LEN to generate in function of our precise objectives (Section~\ref{sec:explanation_styles}). %Fig.~\ref{fig:scheme1} provides an overview of the main topics covered in this section.
In Fig.~\ref{fig:visual} (leftmost part) we provide an overview of the contents of this section. In the same figure, we also show how the following sections will cover the specific methods (Section~\ref{sec:methods}) and the considered neural architectures (Section~\ref{sec:outofthebox}).

\begin{figure}[h]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme1.png}
    \includegraphics[width=0.98\textwidth]{figs/LEN.pdf}
    % \input{tikz/framework}
    \caption{Visual overview of the organization of the paper for those sections that are about describing the whole LEN framework and the specific use-cases we selected. Starting from the nodes on the left, each path that ends to one of the nodes on the right creates a specific instance of the LEN framework. The proposed framework is generic enough to create several other instances than the ones we studied in this paper.} 
    \label{fig:visual}
\end{figure}

\iffalse
\begin{figure}[h]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme1.png}
    \includegraphics[width=0.6\textwidth]{figs/lens_1.pdf}
    % \input{tikz/framework}
    \caption{Basics of LENs (Section~\ref{sec:basics}). In order to setup a LEN-based model, first, the way the LENs communicate with a black-box classifier or directly with the data must be defined (what we refer to as computational \textsc{pipeline} Section~\ref{sec:use_cases}). The type of expected explanations has a direct consequence in the objective that drives the learning of the LENs parameters (\textsc{learning and explanations}, Section \ref{sec:explanation_styles}). {\color{red}[Remove the word 'explainer' from the 3 points in Pipeline.
    Remove the word 'explanations' from the white box on the right.]} 
    }
    \label{fig:scheme1}
\end{figure}
\fi

%There are different ways of letting LENs communicate with a black-box classifier

%and for which
%the main aspects on what LENs can be used for and which kind of explanation we may get with
%learning problems it applies (see Fig. \ref{fig:scheme1}).

%Let us consider a standard classification problem where a classifier f defines the membership values of

A LEN is a function $f$, implemented with a neural network, that maps data falling within a $k$-dimensional boolean hypercube onto data that fall within another $r$-dimensional boolean hypercube. Each dimension is about the activation strength of what we refer to as \textit{concept}, with the strict requirement of having a human-understandable description of each \textit{input} dimension/concept.
Formally, a LEN is a mapping $f: C \rightarrow E$, where $C = [0,1]^{k}$ is the \textit{input concept space}, and $E = [0,1]^{r}$ is the so called 
\textit{output concept space}. %\draft{(or also \textit{explanation space})}. 
% Explanations are given in terms of the input concepts, while the $r$ output concept activations are about the truth degrees of $r$ FOL rules. Whenever a LEN has been trained, the $i$-th output concept can be directly translated into a FOL rule $\rho_i$ such as the one shown in Fig.~\ref{fig:len}. Rules can be then aggregated to different extents, altering their granularity level from a local to a more global coverage of the available data.
\sm{Explanations produced by a LEN are about the relationships between the output and the input concepts, and they belong to the generic rule space $P$.
%are about the output concepts, and they are given in terms of the input ones. they belong to the generic rule space $P$.
%There are several ways of explaining output concepts, operating at different granularity levels, from a local to a more global coverage of the available data.
%In any case, LEN explanations are given in terms of the input concepts, i.e. they explain the relationships between the input and the output of the LEN.
%, while the $r$ output 
% concept activations
%\draft{predictions are about the validity of $r$ explanations that correspond to the}
%truth degrees of $r$ logic rules. 
In particular, whenever a LEN has been trained, the $i$-th output 
$f_i$
% concept
can be directly translated into a logic rule $\varphi_i$ and
explained by a FOL formula $\rho_i \in P$ that involves the input concepts, such as the one shown in Fig.~\ref{fig:len}. The FOL extraction process is general enough to offer the possibility of eventually devising logic rules that are aggregated to different extents, altering their granularity level from a local to a more global coverage of the available data.}


In order to provide a concrete meaning to the LEN model, we have to define the source of the input concept activations and how to learn the criteria that allow LENs to predict the output concepts and explanations. Amongst a variety of possible configurations that are instance of Fig.~\ref{fig:framework}, we will focus on a limited set of computational pipelines in which the input and output concept spaces are defined with respect to real-world use-cases. In some of them, LENs communicate with a black-box classifier, with the goal of providing explanations of its predictions, or with the goal of exploiting its predictions to model the LEN input concept activations.
In all the cases, for each input sample, LENs provide $r$ FOL explanations that might be directly associated to $r$ categories of a classification problem or they could be interpreted as $r$ generic different explanations of the input data. In the former case, LENs are trained in a supervised manner, while in the latter case they are trained in an unsupervised setting.

Before going into further details, we introduce the entities and the notation that will be used throughout the paper, \sm{paired with a short description to help the reader in following the paper and to have a quick reference to the main symbols.}
\begin{itemize}
\item We consider a scenario in which we have the use of a finite collection $\mathcal{X}$ of data samples to train LENs, that belong to $X\subseteq\mathbb{R}^d$ . \sm{There exists a mapping from $X$ to the space $C$ of input concept activations. The notation $\mathcal{C}$ indicates the finite set of concept activations obtained by mapping each sample of $\mathcal{X}$ onto $C$.}
%\item The notation $\mathcal{C}$ indicates a finite set of samples belonging to the space $C$ of the input concepts. The data in $\mathcal{C}$ are  associated to the data in $\mathcal{X}$, i.e., there is a mapping from each element in $\mathcal{X}$ onto a corresponding element in $\mathcal{C}$.
    \item We use the notation $q$ to indicate the total number of classes in a classification problem. Each data sample can be associated with one or more classes. No strict conditions are posed on the potential mutual exclusivity of the different classes, thus we consider the most generic setting that spans from multi-label to single-label classification. Moreover, classes could also be organized in a structured manner, such as in hierarchy. 
    \item \sm{Whenever we consider classification problems, classes are assumed to be} encoded with binary targets in $\{0,1\}^{q}$. The function $\bar{y}(\cdot)$ returns the target vector associated to the data sample passed as its argument, while $\bar{y}_i(\cdot)$ returns the \sm{$i$-th component of $\bar{y}(\cdot)$}, that is about the $i$-th class. \sm{What we propose holds also in the case in which targets are encoded with scores in the unit interval, so that we will frequently refer to generic data encoded in $Y=[0,1]^{q}$.} %The classification problem might also be structured in a hierarchical manner. In this case, at each level $\ell$ of the hierarchy we have $q^{(\ell)}$ classes, $\ell \in [1,h]$.
%In the case of hierarchically organized classes, the higher-level classes are predicted in function of the ones activated at the lower levels, $g^{(\ell)}: Y^{(\ell-1)} \rightarrow Y^{(\ell)}$, $\ell \in [1,h]$, where $Y^{(0)} = X$.
 \item \sm{We will use the notation $Y^{(a:b)}$ to indicate a projection of $Y$ limited to the dimensions going from index $a \geq 1$ to index $b \leq q$, included.}
\item The function $g$ is about a generic black-box neural classifier \sm{that computes the membership scores of the given input to a set of categories. Such categories could be exactly the ones of the considered classification problem (encoded in $Y$) or a subset of them (encoded in $Y^{(a:b)}$).}
%\footnote{With "black box classifier" we mean that there are no assumptions on the classifier structure. The classifier architecture could be totally unknown to the logically explained network, that only requires a $[0,1]$-valued I/O.}
 In detail, $g: X \rightarrow Y$ (resp. $g: X \rightarrow Y^{(a:b)}$), and $g(x)$  defines the membership scores of $x$ to the considered categories.
 %, i.e.,  $g(x)=(g_1(x),\ldots,g_q(x))\in Y$ (resp. $\in Y^{(a:b)}$). 
 Of course,  $g_i(x)=1$ when $x$ strongly belongs to class $i$ (resp. $a+i-1$). No special conditions are enforced in the definition of $g$. 
 \item The notation $\bar{f}$ is used to indicate a boolean instance of \sm{the main LEN} function $f$, in which each output of $f$ is projected to either $0$ or $1$.\footnote{When not directly specified, we will assume $0.5$ to be used as threshold value to compute the projection.} In order to refer to a single output of the vector function $f$ (or $\bar{f}$), the subscript will be used, e.g., $f_i$ (or $\bar{f}_i$). \item Similarly, for a vector $c \in \mathcal{C}$ with activation scores of $k$ concepts, $c_j$ is the $j$-th score, while $\bar{c}_j$ is the boolean instance of it.
 \item Any dimension of the space of input concepts $C$ includes a human-readable label. Logic rules generated by LENs will exploit such labels to give understandable name to predicates. In order to simplify the notation, whenever we \sm{make a mention to} the rule associated to a sample $c \in C$, we will use the already introduced symbol $\bar{c}_j$ also to refer to the human-understandable name of the $j$-th dimension \sm{of $C$}.
 \item \sm{Any dimension of the space of output concepts $E$ might or might not include a human-readable label, whether we consider supervised or unsupervised learning, respectively. In the former case, the already introduced notation $\bar{y}_i$ will also refer to the human-understandable name of the $i$-th output class, following the same simplification we described in the case of $\bar{c}_j$.}
 %\item \draft{Similarly, in any FOL rule, $\bar{y}_i$ will refer to the human-understandable name of the logic predicate corresponding to the $i$-th output class.}
 \item \sm{Any output $f_i$ is associated with a logic rule $\varphi_i$ \sm{given in terms of (the names of) the input concepts}.}
 \item \sm{We indicate with $\rho_i \in P$ the FOL formula that explains the $i$-th output concept by means of $\varphi_i$. The precise way in which $\varphi_i$ is exploited to build $\rho_i$ depends on whether we are considering supervised or unsupervised output concepts.}
 %\draft{Any output $f_i$ is associated with a human-understandable logic formula denoted by $\varphi_i$. For any $i=1,\ldots,r$,  a FOL formula related to $\varphi_i$, and eventually to a class $\bar{y}_i$, is denoted by $\rho_i$.}
\end{itemize}
The listed elements will play a precise role in different portions of the LEN framework.




\iffalse
such that:
\begin{itemize}
    \item Any input $c\in C$ consists in a $[0,1]$-valued feature or concept vector, i.e. $C \subseteq [0,1]^k$. $C$ is also said the \emph{concept space}. Concepts need to be semantically meaningful since they will be exploited to provide explanations. Many times $X=C$ if $X$ is already semantically meaningful; otherwise a mapping is required.
    \item $f$ can be any neural model, but it is required that $E\subseteq[0,1]^r$ where, for any $c\in C$, $i=1,\ldots,r$, $f_i(c)=1$   means that the $i$-th explanation holds for $c$, viceversa if $f_i(c)=0$. $f_i$ is sometimes called the $i$-th output of the LEN $f$. We refer to $E$ as the \emph{explanation space}. In standard supervised problems $E=Y$, however, LENs can also be employed in other contexts.
    % \item there is no pair $c^i,c^j\in C$, such that $\bar{f}(c^i) \neq \bar{f}(c^j)$ and $\bar{c}^i=\bar{c}^j$, where the overline notation denotes the boolean discretization (thresholded at $0.5$) of values from $[0,1]$ to $\{0,1\}$ values.
\end{itemize}



In a broad sense, a LEN for the classifier $g$ can be simply thought of as any neural model $f$ aiming at explaining the decision processes taken by $g$.

The explanations will generally hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrences or global principles among different classes.




% One of the main advantage of the proposed framework is its versatility, indeed a LEN can be defined according to different user-preferences by serving different purposes.
%In particular, the layout of a XAI pipeline based on LENs follows the definition of a few aspects concerning the classification problem under investigation and the properties of the required explanations. Setting these points allows the correct definition of a LEN in a learning problem. For clear, this is also schematized in Fig. \ref{fig:scheme1}.
LENs can be integrated in different learning problems with different classifier architectures. How the integration will take place depends on the nature of the input data and the presence of one or more concept bottlenecks among the classes under investigation. LENs can provide different kind of explanations both in supervised and unsupervised learning settings, according to user needs.
%In particular, we may be interested in individual explanation, i.e. the explanation of the decision taken by the classifier on a specific sample. However, we may also look for more general explanations, such as explaining the decisions taken for a whole class predictions, or even looking for more abstract relations among the classes.
Indeed, by now, we referred to LENs as neural networks aiming to accomplish a classification task.
%(either to explain the behaviour of a black box or to solve the classification problem itself).
However, LENs can also be used in unsupervised learning task.
In the latter case, the output of the LEN denotes the cluster-assignment.
\fi


\begin{figure}[t]
    \centering
    %\includegraphics[width=0.55\textwidth]{figs/E2E.pdf}
    $\vcenter{\hbox{\includegraphics[width=.40\textwidth]{figs/E2E.pdf}}}$ \quad %\\ \bigskip
    $\vcenter{\hbox{\includegraphics[width=.56\textwidth]{figs/e2e_explaining.pdf}}}$
    \caption{End-to-end (E2E) LENs directly work on input data that are interpretable per se and treated as concepts ($C=X$), while the output concepts are the activation scores of the classes of the dataset ($r = q = 2$). This is a real-world example from the MIMIC II dataset (see the experimental section), where patient features are used to classify if the patient will survive 28 days after hospital recovery. Left: the LEN solves the classification problem and provides explanation, also referred to as \textit{interpretable classification}. Right: the LEN \textit{provides explanations} of a black-box classifier. {\color{red}[Replace $X=C$ with $X$ (twice). Replace $C$ with $C=X$ (twice). Add $E$ in place of $f(C)$ (twice). Replace $g(C)$ with $Y^{(q)}$. Replace $Y$ (twice) with $Y^{(q)}$.]}}
    \label{fig:E2EExplainer}
\end{figure}

\subsection{Computational pipelines}
\label{sec:use_cases}
% In general, we can state that the above assumptions about the input data and the classifier are not always valid. However, in the following we will see how we can apply the LEN framework in different use cases where these conditions hold.
%Roughly speaking, a logically explained network $f$ is simply a function mapping $[0,1]$-values to $[0,1]$-values.
%, with the aim of providing itself the final classifications or to provide explanations for a classifier $g$.
%This very general definition allows the application of LENs to different contexts that can be made consistent with real-unit I/O.
%The most straightforward way of designing a computational pipeline involving LENs is to let the black-box classifier $g$ predict the activation scores of the $q$ classes and provide them to the LEN. In this way, we have $C = Y$, i.e., the LEN outpt concept space collides with $Y$. This is indeed feasible since $Y$ is bounded by a Boolean hypercube. %However, if the available data are already encoded in a symbolic manner in which the $d$ input features are actually  scores in $[0,1]$ (or in $\{0,1\}$ in the most extreme case) that can be considered the activation scores of $d$ concepts, then we can set $C = X$, and directly provide the data to the LEN.
%The output space of the LEN can be designed in multiple ways, depending on what is the final goal of the whole system. For example, it could collide with $Y$, i.e., the output space of the black-box $g$, $E=Y$, or it could be a totally new concept space.}

Amongst a large set of feasible input/output configurations of the LEN block, here we consider three different computational pipelines that are about three concrete scenarios/use-cases where LENs may be applied, that consist in what we refer to as \textsc{end-to-end}, \textsc{concept bottleneck}, and \textsc{cascading} pipelines.

%directly working on structured data; in a concept bottleneck-scenario where low-level concepts are first extracted from unstructured data (e.g. images); as a cascade of LENs providing explanations at different level of granularity.

%{\color{magenta}******* TBC ******}

% \paragraph{End-to-end explainer}
\textsc{End-to-end (E2E). } The most immediate instance of the LEN framework is the one in which the LEN block aims at directly explaining, and eventually solving, a supervised categorical learning problem. In this case, we have $C = X$, and $r = q$, as shown in Fig.~\ref{fig:E2EExplainer}. In order to make the first equality valid with respect to the LEN requirements, the $d$ input features of the data in $X$ must score in $[0,1]$ (or in $\{0,1\}$ in the most extreme case), so that they can be considered as activations of $d$ human-interpretable concepts. 
%, i.e., $X=C \xrightarrow[]{f} E$.
%An E2E LEN assumes that the features of the input space are meaningful individually, i.e. they correspond to human-interpretable concepts.
%Structured datasets usually fall into this category.
Of course, in order to create these conditions in different types of datasets, generic continuous features can be either discretized into different bins or booleanized by comparing them to a reference ground truth (e.g., for gene expression data, the gene signature obtained from control groups can be used as a reference).
An E2E LEN can perform a fully \textit{interpretable classification} task, having the double role of main classifier and explanation provider (Fig.~\ref{fig:E2EExplainer}, left), or it can work in parallel with another neural black-box classifier $g$, thus {providing explanations} of the predictions of $g$ (Fig.~\ref{fig:E2EExplainer}, right) -- what we refer to as \textit{explaining a black-box}.
\sm{In both the cases we have} $E = Y^{(q)}$. 
%used to explain the predictions of any black box model $g:X\rightarrow Y$,
%as shown in Fig. \ref{fig:E2EExplainer}.
The first solution is preferred when it is of fundamental importance to have a white-box classifier, while we can accept some drawbacks in terms of classification performances, due to the constrained nature of the LENs.
The second solution is instead useful in those context where the classification performance plays a key role, and we may accept approximate explanations of the decision taken.

\begin{figure}[t]
\centering
    %\includegraphics[width=0.55\textwidth]{figs/E2E.pdf}
    $\vcenter{\hbox{\includegraphics[width=.48\textwidth]{figs/CBM.pdf}}}$ \quad %\\ \bigskip
    $\vcenter{\hbox{\includegraphics[width=.48\textwidth]{figs/concept_relations.pdf}}}$
    \caption{Concept-bottleneck (CB) LEN. Left: the LEN is placed on top of a black box model $g$ which maps the input data into a first set of interpretable concepts. An MNIST-based experiments is shown (see the experimental section). Handwritten digits are first classified by $g$. A LEN is then employed to classify and explain whether the digit is even or odd -- \textit{interpretable classification}. {\color{red}[Replace $g^{(1)}(X)$ on top of the blue column of concepts with $C$. Replace $C$ (over the yellow table) with $C=Y^{(1:z)}$. Replace $f(g^{(1)})(X)$ with $E$. Remove the superscript $(1)$ everywhere here. Replace the $Y$ on the right with $Y^{(z+1:q)}$.]} Right: MNIST digits are classified as belonging to one of the 10 classes and whether they are even of odd by a black-box $g$ (see the experimental section).  %in a Concept-bottleneck pipeline
     A LEN groups these predictions in an unsupervised manner, and analyzes the relations within each cluster -- \textit{interpretable clustering}. Supervision labels are not provided for the LEN output. {\color{red}[Replace $g(X)$ on top of the blue column of concepts with $C$. Replace $C$ (over the yellow table) with $C=Y^{(q)}$. Replace  $f(g(X))$ with $E$. Fix (?) FOL Explanation of Cluster 2 (not 1).]}}
    \label{fig:CMBExplainer}
\end{figure}

% \paragraph{Concept-bottleneck explainer}
\textsc{Concept-bottleneck (CB). }
A Concept-Bottleneck LEN is a computational pipeline in which the LEN $f$ aims at explaining, and eventually solving, a categorical learning problem in which the data in $X$ are not readily exploitable as LEN inputs, and a black-box model $g$ computes the activations of an initial set of $z$ concepts out of the available data. The LEN solves the problem of predicting $r$ new concepts from the activations of the $z$ ones, as shown in Fig.~\ref{fig:CMBExplainer} (left/right). Differently from the E2E case, there is always a neural network $g$ processing the data, and the outcome of such processing is the input of the LEN. Formally, we have $g: X \rightarrow Y^{(z)}$, while $f: (C=Y^{(z)}) \rightarrow E$.
This two-level scenario can be implemented in a way that is coherent with the already discussed example of Fig.~\ref{fig:len}, that is what we also show in Fig.~\ref{fig:CMBExplainer} (left). In this case, each example is labeled with $q$ binary targets divided into two disjoint sets, where the black-box network predicts the first $z < q$ ones, and the LEN predicts the remaining $r = q-z$.
The LEN will be both responsible of predicting the higher level concepts and of explaining them in function of the lower level concepts yielded by the black-box model, thus still falling withing the context of \textit{interpretable classification}.
 We also consider the case in which the outcome of the LEN is not associated to any known classes, thus the LEN is trained in an unsupervised manner, as shown in  Fig.~\ref{fig:CMBExplainer} (right), thus implementing a form of \textit{interpretable clustering}. In both the cases, the black-box classifier $g$ is trained in a supervised manner.\footnote{The extraction process can be either implicit, through the analysis of the latent spaces learnt by the black-box \cite{kazhdan2020now}, or explicit by training a black-box to classify specific concepts \cite{koh2020concept}.}

%in which the features of the data in $X$ are not interpretable as activations of human-understandable concepts or they are too low-level to be directly involved into compact explanations (e.g., all the pixels of an image \cite{koh2020concept}). In this case, we assume to have information to process the data in order to extract an initial set of concepts that will be provided to the LEN.
%Then, given


%In this latter setting, a model $g$ can be used to extract high-level concepts $C$ from raw features in $X$, and then producing the final classification $Y$. In this case, we may assume $g=g^{(2)}\circ g^{(1)}$ with $X\xrightarrow[]{g^{(1)}}C\xrightarrow[]{g^{(2)}}Y$.
%Given the concepts extracted from $g$, a LEN $f$ may be exploited to produce a set of explanations $X \xrightarrow[]{g^{(1)}} C\xrightarrow[]{f}E$,
% and eventually solve the classification task (if $E=Y$)
%classify and explain the categorical learning problem at a higher level of abstraction, i.e. $X \xrightarrow[]{g} C\xrightarrow[]{f}E$ %$C \xrightarrow[]{f} E$
%as shown in Fig. \ref{fig:CMBExplainer} where $E=Y$.
% or even producing itself a solution by assuming $E=Y$.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.58\textwidth]{figs/cascade.png}

      \caption{Cascading LENs, an example taken from the V-Dem classification dataset (see the experimental section). The final classification on the status of the democracy is divided into two steps.
    %   $X=C^{(1)} \xrightarrow[]{f^{(1)}} C^{(2)}\xrightarrow[]{f^{(2)}} E$.
    First, the input data/concepts $C_1$ are mapped into high-level concepts $C_2$. %$= f_1(X)$.
    High-level concepts are then used to compute the final classification. %$= f_2(f_1(X))$.
    Cascading LENs can provide explanations at different levels of granularity, implementing multiple \textit{interpretable classifications}. {\color{red}[Replace $X=C_1$ with $X$. Add $C_1$ on top of the first column of blue concepts. Replace $f_1(X)$ with $E_1 = C_2$. Replace $f_2(f_1(X))$ with $E_2$. Replace $C_2$ on top with $Y^{(1:z)}$. Replace $Y$ on the right with $Y^{(z+1:q)}$.]}}
    \label{fig:CascadeExplainer}
\end{figure}

% \paragraph{Cascading explainers}
\textsc{Cascading. }
Cascading LENs can be used to provide explanations by means of a hierarchy of concept layers. In particular, multiple LENs are used to map concepts into a higher-abstraction level (without the need of any black-box $g$), %Each model is trained on a concept space to predict concepts at a higher level of abstraction which will feed the next LENs $C^{(i)} \xrightarrow[]{f^{(i)}} C^{(i+1)}$.
%The final model solves and explains the more abstract classification task $C^{(m)} \xrightarrow[]{f^{(m)}} E$
as shown in Fig.~\ref{fig:CascadeExplainer}. Each LEN provides explanations of its outputs with respect to its inputs, thus cascading LENs handle multiple levels of granularity. This structure provides a hierarchy of explanations and upholds human interventions at different levels of abstraction, providing a far deeper support for human-machine interactions. We indicate with $(C_1, E_1), (C_2, E_2), \ldots, (C_m, E_m)$ the input/output concept spaces of the $m$ cascading LENs, with $C_{j} = E_{j-1}$, $j > 1$. We will consider the case in which LENs are trained in a supervised manner, thus implementing multiple \textit{interpretable classifications}.



\subsection{\sm{Objectives}}
\label{sec:explanation_styles}
%Different pipelines may be employed to solve different learning problems while (eventually) producing different explanations.
%In addition,
%The user might be interested in finding explanations that hold whenever specific categories of the considered problem are predicted, 
% that hold on a certain portion of data
%or in letting the LEN autonomously discover a set of regularities among the input concepts.
In Section~\ref{sec:use_cases}, when describing the selected computational pipelines, we made a precise distinction among \textit{interpretable classification}, \textit{explaining a black-box}, and \textit{interpretable clustering}, that represent three different \sm{objectives} that the user might have in the problem at hand. These \sm{objectives} impose precise constraints in the selection of the learning criteria and on the form of the FOL formulas that can be obtained by the LENs, \sm{that will be described in detail in Section~\ref{sec:logic_rule_extr} (generic process of logic rule extraction), and in Section~\ref{sec:learncrit} (criteria and FOL rules)}.
%In addition to this choice, the user can select the granularity level of the logic rules, moving from \textit{example} to \textit{set}-level rules. The former are about single examples, while the latter covers more aggregated samples. 
%While all the formal details on the learning criteria and the rule types will be provided in  Section~\ref{sec:learncrit}, here we contextualize their role with respect to the properties of the previously described computational pipelines.
\sm{The most basic difference among the aforementioned objectives is about the criterion that drives the learning dynamics of $f$, since each LEN module can be trained in a supervised or an unsupervised fashion.}


\sm{Whenever LENs are exploited to both solve the classification problem and provide explanations, i.e., in \textit{interpretable classification},  
learning is driven by supervised criteria. Such criteria  exploit the available supervised data in order to develop $f$ not only to mach such supervisions as in classic supervised learning, but also to constraint $f$ to behave in a way that is coherent with the target type of FOL rules that the user is looking for, following an approach that is similar to what we studied in \cite{ciravegna2020human}. Each output concept of the LEN is associated to a target category named $\bar{y}_i$ of the considered learning problem, and LENs can provide a FOL explanation $\rho_i \in P$ of such category, so that the class-predicate $\bar{y}_i(\cdot)$ will be specifically involved into the extracted FOL formulas. For example, if \textit{person} is one of the output categories, LENs can explain the reasons behind the prediction of class $\bar{y}_i =$ \textit{person} with respect to the discovered relationship $\varphi_i$ involving the  activations/not-activations of some ($m_i$) of the $k$ input concepts ($m_i < k$). If such input concepts are  are  $\bar{c}_j=$ \textit{head},  $\bar{c}_z=$ \textit{hands}, $\bar{c}_h=$ \textit{body}, the system could learn that $\rho_i = \forall c \in C\colon \bar{y}_i(c) \leftrightarrow \varphi_i(c)$, where $\varphi_i(c) = \bar{c}_j(c) \land \bar{c}_z(c) \land \bar{c}_h(c)$, i.e., discarding the quantifier, \textit{person} $\leftrightarrow$ \textit{head} $\land$ \textit{hands} $\land$ \textit{body}. Interestingly, in the case of interpretable classification, LENs basically become 
 white-box classifiers, as is showcased by the concrete examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CMBExplainer} (left), Fig.~\ref{fig:CascadeExplainer}.}

In the case in which the user aim at \textit{explaining a black-box}, a LEN acts in parallel to a black-box classifier with the only goal of providing explanations, and it is forced to yield outputs that are as close as possible to the ones of the black-box, i.e., $f$ is forced to be close to $g$ when evaluated on the available data samples. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right) and it does not require any supervision, since learning can be driven by a coherence criterion between the outputs of $g$ and those of $f$ when processing the same data. \sm{\color{magenta}The type of FOL rules that LENs can extract are the same of the case of interpretable classification, thus the principles are followed to devise them.}
%
%
%For instance, in the selected computational pipelines of Section~\ref{sec:use_cases}, while most of the focus is on supervised learning, the Concept-bottleneck case is also about unsupervised learning of LENs (Fig.~\ref{fig:CMBExplainer} right).
%
%
%
%In the former case, each output concept of the LEN is associated to a target category of the considered learning problem, and LENs are developed by learning criteria that exploit the available supervisions (ection~\ref{sec:learncrit}). The rationale behind this approach it that LENs implicitly learn to predict each target class with respect to the input concepts, that are lower-level attributes. Then, LENs can provide a FOL explanation of such prediction, e.g., explanation of the target class \textit{person} with respect to the input concepts/attributes \textit{head, hands, body}. %We refer to this context as \textsc{targeted explanations}, and the learning process is driven by supervised criteria (Section~\ref{sec:learncrit}).
%Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations, i.e., in \textit{interpretable classification}, then it becomes a white-box classifier. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CascadeExplainer} (left), Fig.~\ref{fig:CMBExplainer} are all about this case.
%
%In the E2E case when $g$ is present or, more generally, whenever LENs act in parallel to a black-box classifier with the only goal of providing explanations, then LENs are forced to yield outputs that are as close as possible to the black-box, so $f$ is forced to be close to $g$. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right).
%

\sm{Differently, whenever the user is not aiming at explaining the target classes of a classification problem,} but he is interested in discovering \sm{generic} relations among different input concepts, \sm{LENs can be trained using unsupervised criteria, thus following the objective that we referred to as \textit{interpretable clustering}}.
The user might be interested in discovering  co-occurrences \sm{$\varphi_i$} of certain input concept activations in not-defined-before subsets $O_i$ of the concept space. \sm{This leads to FOL rules such as $\rho_i = \forall c \in O_i \colon \varphi_i(c)$, where, for example, $\varphi(c) = \bar{c}_e \lor \bar{c}_t$ and $\bar{c}_e = soccer\_ball$, $\bar{c}_t = foot$ for some samples (that can be thought as a cluster) in a collection of miscellaneous images}.
\sm{Of course, each output concept of the LEN is not associated to any known classes (as in the previous objective), but to a generic symbol} that is not defined in advance, as in Fig.~\ref{fig:CMBExplainer} (right). The activation score of the output concept can be tough as a cluster membership score, \sm{used to define whether the provided input belongs or not to subset $O_i$.}
%LENs yield an explanation for each of these symbols, that is about discovering relations among the input concepts. In this context, no supervisions are exploited, and the learning criterion is designed in order to cluster the input concepts into $r$ groups.

 %For instance, by analyzing the output of a multi-label classifier $C=g_1(X)$ in a CB pipeline, %with eventually several output classes,
%it could be interesting to get an explanation of the holding relationships among different classification outputs.
%For example, the user might be interested in discovering  co-occurrences of certain input concept activations, like $soccer\_ball \wedge foot$ for a set of football images.

\sm{The FOL rule generation in the case of the three objectives involves a process in which logic explanations are extracted from the LENs in a generic manner, before being instantiated into FOL formulas that well cope with the learning criterion associated with the specific objective. Due to such generality of the extraction mechanisms, and}
independently on \sm{the considered objective}, the user might also decide to automatically discover \sm{more focused} regularities that are about single examples, groups of data points, or, more generally, the whole dataset, moving from local to more global explanations.  %On the other hand, the user may also look for unbiased global explanations, like $zero\oplus one\oplus\ldots\oplus nine$, in a digit classification task.
%In both the cases, learning is driven by unsupervised criteria.
%Each output concept activation of the LEN module can be tough as a cluster membership score. Thus, another view of \textsc{untargeted explanations} can be directly related to the notion of \textit{interpretable clustering}, where LEN can provide explanation of each cluster, as shown in Fig.~\ref{fig:concept_relations} for the case of MNIST digits.
%As another example, consider the case of gene expression analysis, where neural networks are usually employed to group similar patients according to their genes activations. LENs can be used not only to perform such grouping (E2E), but also understand why such groups have been formed and in particular which are the most relevant gene activations in each group. 


%In the following we provide further insights for \textsc{targeted} and \textsc{untargeted explanations}.

%For this reason, we distinguish between the case in which LENs are trained in a supervised manner or with unsupervised criteria.

%A supervised task consists in learning and explaining a target \textit{class} with respect to a set of lower-level attributes, e.g. explanation of the class \textit{person} with respect to the attributes \textit{head, hands, body}. In this scenario LENs generate \textit{Supervised Explanations}.
%Alternatively, an unsupervised task consists in explaining hidden relations among \textit{concepts}, e.g. the classification outputs of another classifier or categorical attributes. In this scenario LENs yield \textit{Unsupervised Explanations}.
% Further, the explanation could have a global, local or even example-level validity. For instance, we may be interested in explaining a certain decision for a specific input, but also in universally valid regularities or simply most frequent co-occurrences among classes.
%In the following, we briefly discuss these two logical explanation styles %that are currently supported by the LENs framework
%which we respectively referred as \textit{Supervised Explanations} and \textit{Unsupervised Explanations}.
%In order to train a LEN to produce these %one or more of the following explanation styles, we can make use of ad hoc learning criteria, as successively discussed in Sec.\ref{sec:learncrit}


% \paragraph{Class-driven explanations}
%\textsc{Targeted explanations. }
% (local or global); \fg{richiederebbe spiegare, che mentre la LEN è vera esattamente dove la classe che spiega, la formula logica è soddisfatta dovunque.}
%Targeted explanations aim at providing a valid explanation for all the samples of a specific class.
%This may be achieved by training a LEN to provide \textit{interpretable classification} or to \textit{explain a black-box model}.
%represent different kinds of causalities for a selected class with respect to the other ones, or a set of lower-level concepts.
%Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations (E2E when no black-box is considered, CB, Cascading), then it becomes a white-box classifier.
%Learning of the LEN module is simply driven by a supervised objective function, in which $f$ is forced to be as close as possible to the corresponding $\bar{Y}$ on the available data. Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations (E2E when no black-box is considered, CB, Cascading), then it becomes a white-box classifier. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CascadeExplainer}, Fig.~\ref{fig:CMBExplainer} are all about targeted explanations. In the E2E case when $g$ is present or, more generally, whenever LENs act in parallel to a black-box classifier with the only goal of providing explanations, then LENs are forced to yield outputs that are as close as possible to the black-box, so $f$ is forced to be close to $g$. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right)., and that we refer to as \textit{explaining a black-box}

%One possibility is to use a LEN to directly accomplish a classification task. Indeed, it can provide an interpretable classification by training a LEN $f$ to satisfy $f_i\simeq Y_i$ for some $i\in\{1,\ldots,q\}$, i.e. to have $f_i(c)$ as close as possible to $Y_i(c)$ for any $c\in C$, where $Y_i(c)$ denotes the label of the $i$-th class on the input $c$, that the LEN is meant to both learn and explain. This solution is preferred when it is of fundamental importance to have a white-box classifier, while we can accept some drawbacks in terms of classification performances.
%However, we may also train a LEN $f$ to explain a black-box model $g$. Therefore, to satisfy $f_i\simeq g_i$ for some $i\in\{1,\ldots,d\}$, i.e. to have $f_i(c)$ as close as possible to $g_i(c)$ for any $c\in C$. This other solution is instead useful in those context where the classification performances play a key role and we may accept approximate explanations of the decision taken.
%It is worth noticing that when explaining a black-box model $g$, a LEN may also take into account the classifier predictions on unlabeled data, e.g. in a semi-supervised learning setting. This allows the LEN to produce explanations covering a larger set of data, but also possibly inaccurate.
%On the other hand, in the interpretable classification case the LEN learns explanations directly from (limited to) the labeled data.
% \begin{itemize}
%     \item
%     \textit{IF-Rules. } This kind of explanation provides a superset of a specific class assignment. For instance, an upper bound containing the class $flies$ can be defined according to the explanation "$flies\rightarrow bird\vee airplane$".
%     \item
%     \textit{Only IF-Rules. } In this case an explanation is required to provide a subset of a specific class assignment. A lower bound contained in the class $flies$ may be obtained with the explanation "$has\_wings \ \wedge \ has\_engine\rightarrow flies$".
%     \item
%     \textit{IFF-Rules. } An explanation  can completely characterize a certain class. For instance, the class $airplane$ can be defined according to the explanation "$airplane \leftrightarrow has\_wings\wedge has\_engine$".
% \end{itemize}
% We note that only with IFF-Rules explanations a LEN can be used for interpretable classification. Indeed, not any bird or plane can fly, so as a seagull can fly without having an engine. Hence, IF and Only IF-Rules are not suitable to correctly predict a specific class behaviour.
\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figs/E2E.pdf} \quad %\\ \bigskip
    \includegraphics[width=.48\textwidth]{figs/e2e_explaining.pdf}
        % Classification style: Explaining an existing classifier. Differently from the previous examples, here a LEN is used to explain the predictions made by an existing classifier $g(x)$ on the MIMIC classification task.}
    \caption{LENs Supervised Explanations: interpretable classification, where the LEN directly provides the final classification (left), or explaining a black-box model $g$ (right).}
    \label{fig:explainablevsexplanation}
\end{figure}
\fi

% \paragraph{Relations among concepts}
%\textsc{Untargeted explanations. }
%  (local or global): MI, Conversion to CNF
%A user may be interested in discovering relations among different input concepts without posing any preferences on any specific class. %For instance, by analyzing the output of a multi-label classifier $C=g_1(X)$ in a CB pipeline, %with eventually several output classes,
%it could be interesting to get an explanation of the holding relationships among different classification outputs.
%For example, the user might be interested in discovering  co-occurrences of certain input concept activations, like $soccer\_ball \wedge foot$ for a set of football images.
%Differently from the case of \textsc{targeted explanations}, the user might decide to automatically discover regularities that are not about the whole dataset, but that may hold only for a portion of the available data. On the other hand, the user may also look for unbiased global explanations, like $zero\oplus one\oplus\ldots\oplus nine$, in a digit classification task. In both the cases, learning is driven by unsupervised criteria.
%Each output concept activation of the LEN module can be tough as a cluster membership score. Thus, another view of \textsc{untargeted explanations} can be directly related to the notion of \textit{interpretable clustering}, where LEN can provide explanation of each cluster, as shown in Fig.~\ref{fig:concept_relations} for the case of MNIST digits.
%As another example, consider the case of gene expression analysis, where neural networks are usually employed to group similar patients according to their genes activations. LENs can be used not only to perform such grouping (E2E), but also understand why such groups have been formed and in particular which are the most relevant gene activations in each group. 

\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=0.58\textwidth]{figs/concept_relations.pdf}
    \caption{Automatic explanations. MNIST digits are classified as belonging to one of the 10 classes and whether they are even of odd by a black-box $g$.  %in a Concept-bottleneck pipeline
     A LEN groups these predictions in an unsupervised manner, and analyzes the relations within each cluster. Supervision labels are not provided for the LEN output. {\color{red}[Remove $g(X)$ and $f(g(X))$. FOL Explanation of Cluster 2 (not 1).]}}
    \label{fig:concept_relations}
\end{figure}
\fi

% \paragraph{Explanation Ranges}
% \textsc{Explanation Ranges. }
% As already mentioned, the explanations may hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrencies or global principles among different classes.
%\fg{aggiungere qualche esempio?}



\section{Methods}
% \section{Formulas, Criteria and Pruning}
\label{sec:methods}
This section presents the fundamental methods that are used to implement the ideas of LENs \sm{that were introduced in Section~\ref{sec:basics}}. 
% We start with the formal definition of the learning objectives (Section~\ref{sec:learncrit}), followed by the procedure that is used to extract FOL rules out of LENs for an individual observation  or in an aggregated manner (Section~\ref{sec:logic_rule_extr}). Finally, we discuss how to constraint LENs to avoid developing complex logic formulas by means of precise parsimony criteria (Section~\ref{sec:parsimony}). In Fig.~\ref{fig:visual} (middle) we provide an overview of the contents of this section.
\draft{We start by describing the procedure that is used to extract logic rules out of LENs for an individual observation  or in an aggregated manner (Section~\ref{sec:logic_rule_extr}). This procedure is common to any LEN \sm{objective}/use-case. Then, we provide the formal definition of the learning objectives that may ensure LENs output to provide required types of \sm{FOL} logic explanations  (Section~\ref{sec:learncrit}).}
Finally, we discuss how to constrain LENs to avoid developing complex logic formulas by means of precise parsimony criteria (Section~\ref{sec:parsimony}), \sm{that is crucial in order to bound the complexity of the explanations}. In Fig.~\ref{fig:visual} (middle) we provide an overview of the contents of this section.



\iffalse
\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme2.png}
    \includegraphics[width=0.85\textwidth]{figs/lens_2.pdf}
    % \input{tikz/methods}
    \caption{Inside the LEN block (Section~\ref{sec:methods}). We distinguish among three categories of methods that implement the principles behind LENs: learning criteria (Section~\ref{sec:learncrit}), FOL rule extraction (Section~\ref{sec:logic_rule_extr}), and parsimony criteria (Section~\ref{sec:parsimony}). {\color{red}[Swap cluster-level and class-level explanations. Rename example-level explanations with 'Example-level (local)'. Rename 'Class-level explanations' with 'Class-level (global). Do the same for 'cluster-level expl.']}}
    \label{fig:scheme2}
\end{figure}
\fi







% \subsection{FOL Rule Extraction}
\subsection{\draft{Extraction of logic explanations}}
\label{sec:logic_rule_extr}



Once a LEN has been trained, it can be associated one logic formula to each output concept $f_i$. As it will become clear shortly, extracting logic formulas out of a trained LEN can be done by inspecting its inputs/outputs accordingly to a boolean interpretation of them. 
\sm{We already introduced the notation $\varphi_i$ to very generically indicate the logic explanation of the output concept $i$, that will be properly formalized in the following.}
We \sm{overload such symbol to explicitly indicate, when needed, the information on the data on which the considered logic explanation holds true, using the notation} $\varphi_{i,\cdot}$, %the logic explanation of the output concept $i$, 
where the second subscript can refer either to a single data sample $c$, $\varphi_{i,c}$, or a \draft{set} $S$ of data samples, $\varphi_{i,S}$. 
% Whenever this is independently done for each single input sample, we get back \textsc{example-level explanations}, that we also refer to as \textit{local explanations}. Differently, whenever the explanations covers an entire category of examples, we talk about \textit{global explanations}, distinguishing between \textsc{class-level explanations} and \textsc{cluster-level explanations}. {\color{red}[I still don't understand what kind of explanations we can provide]}
\draft{In practice, $S$ denotes the sub-portion of the concept space that is covered by the $i$-th explanation, i.e. the set of concept tuples for which the corresponding formula $\varphi_{i,S}$ is true. By aggregating over multiple samples we may vary the scope of the logic formula from strictly local \textsc{example-level explanations} ($S=\{c\}$) to \textsc{set-level explanations} ($S\subseteq \mathcal{C}$), where eventually $S=\mathcal{C}$ in case of global logic formulas holding on the whole sampled concept space $\mathcal{C}$.}
%%%Old pieces
% Whenever this is independently done for each single input sample, we get back \textsc{example-level explanations}, that can be aggregated into \draft{\textsc{set-level explanations}}. 
% We refer to such explanations as \textit{local}, since their corresponding formulas only hold on a sub-portion of the concept space. However, local explanations can be combined and reformulated as \textit{global} explanations according to Eq. \ref{eq:dnf2cnf}.
%%%

 %As already mentioned, the explanations may hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrences or global principles among different classes.

% The logic formula becomes human understandable whenever concepts appearing in such a formula are replaced with human-interpretable strings that represent their name (similar consideration holds for $\hat{f}^i$, in what follows)

In detail, any LEN $f=(f_1,\ldots,f_r)$ requires both its inputs and outputs to belong to the real-unit interval. 
This apparent limitation allows any $f_i$, for $i=1,\ldots,r$, to be easily \draft{associated with a logic formula according to the following procedure.
First, \sm{the data in $\mathcal{C}$ is processed by $f$. Both such data and the outputs of $f$ are thresholded}, e.g., with respect to $0.5$, to obtain a set of boolean values. Then, \sm{for each output $i$}, we build an \textit{empirical truth-table} $\mathcal{T}^i$ by concatenating the $k$-columns of booleanized input concept tuples $\{ \bar{c},\ \forall c\in\mathcal{C}\}$, with the column of the corresponding outcomes $\bar{f}_i(c)$ (left-side of Fig. \ref{fig:tt2form_freq}). 
The truth-table $\mathcal{T}^i$ can be converted into a logic formula $\varphi_i$ in Disjunctive Normal Form (DNF) as usually done in \sm{related} literature \cite{mendelson2009introduction}.
However, \sm{the rationale behind LENs is to extract formulas that are compact, emphasizing the most relevant relationships among the input concepts, according to a specific parsimony index (that will be the subject of Section \ref{sec:parsimony}). Thus,} any $f_i$ will depend only on a proper subset of $m_i < k$ concepts, and the formula $\varphi_i$ will be built according to the restriction of $\mathcal{T}^i$ to \sm{$m_i < k$} columns, see e.g. Fig.~\ref{fig:tt2form}. Notice that, for convenience in the notation, we assumed the first $m_i$ columns to be one that play a role in the explanation, even if they could by any set of $m_i$ columns of $T^i$.}
In order to better point out the described procedure, 
we \sm{formally} define the set $O_i = \{c\in \mathcal{C}:\ \bar{f}_i(c)=1\}$ as the set of all the sampled concept tuples that make true the $i$-th output explanation, i.e., the \emph{support} of $\bar{f}_i$. %For instance, if we are interested in targeted explanations only, any $O_i$ will generally consist in the set of inputs that are classified as belonging to the $i$-th class by the LEN.
% \paragraph{Local Explanation}
% \paragraph{Example-Level Explanation}

%Each output concept $i$ is associated to one of more explanations $\varphi_i,\cdot$, depending on its granularity level. In what follows, we described the case 

\textsc{Example-level explanations. }
Given $c\in O_i \subseteq \mathcal{C}$, the booleanization $\sm{\bar{c}}$ of its continuous features may provide a natural way to get a logical explanation at example-level $\varphi_{i,c}$ as a logic formula. To make logic formulas more human understandable, the overline notation over concepts denotes here human-interpretable strings (or their negation) that represent their name,
\begin{equation}
    \varphi_{i,c} = \tilde{c}_1\wedge\ldots\wedge\tilde{c}_{m_i} \qquad\mbox{where } \tilde{c}_j:=
    \begin{cases}
        \bar{c}_j, & \mbox{if }c_j \geq 0.5\\
        \neg \bar{c}_j, &\mbox{if } c_j < 0.5\\
    \end{cases}\ ,
    \mbox{ for $j=1,\ldots,m_i$.}
    \label{eq:locexp}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/truth-table-counter.png}
    \caption{Aggregation of concept tuples with the same booleanization yields a common example-level explanation, and do not complicate the class-level explanation. For any example-level explanation, we may count how many samples it explains. Infrequent explanations may then be pruned to avoid explanation overfitting. {\color{red}READ THE PAPER TEXT AND FIX THE PICTURE, MAKE IT APPROPRIATE}}
    \label{fig:tt2form_freq}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=0.8\textwidth]{figs/truth-table.png}
    \caption{Extracting a logic formula from the truth-table of a binary boolean function $\bar{f}$. \fg{change figure: remove <->, ->, $\bar{f}$ and equality symbols, from the explanations. {\color{red}READ THE PAPER TEXT AND FIX THE PICTURE, MAKE IT APPROPRIATE}}}
    \label{fig:tt2form}
\end{figure}



% \paragraph{Aggregated Explanation}
\textsc{Set-level explanations. }
By considering Eq. \ref{eq:locexp} for any $c\in S$, with $S\subseteq O_i$, and aggregating all the example-level explanations, we may easily provide an explanation for a set of samples.
\begin{equation}
    \varphi_{i,S} = \displaystyle\bigvee_{c \in S}\varphi_{i,c} = \displaystyle\bigvee_{c \in S}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_{m_i}
\label{eq:agg_exp}
\end{equation}
\draft{\sm{Of course, some $\varphi_{i,c}$'s might be equivalent for different $c$'s, and repeated instance can be easily discarded keeping only one of them.} In case $S=O_i$, we simply write $\varphi_i$ in place of $\varphi_{i,S}$ and we refer to such set-level explanation as the \textsc{class-level explanation} of the $i$-th output concept $f_i$. \sm{In the rest of this section we will explore further details of what has been described so far.}}
% \textsc{Class-level explanation. }
% By considering Eq. \ref{eq:agg_exp} with $S=O_i$, i.e., aggregating all the example-level explanations of class $i$, we get an overall explanation $\varphi_i$ for the LEN output $f_i$.
% \begin{equation}
%     \varphi_i = \displaystyle\bigvee_{c \in O_i}\varphi_{i,c} = \displaystyle\bigvee_{c \in O_i}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_{m_i}.
% \label{eq:glo_exp}
% \end{equation}


%%%%tolto pezzo regole messo in sec learning criteria
%%%%

\begin{example}
\label{ex:xor}
Let's consider the boolean $XOR$ function, defined by $xor(0,0)=xor(1,1)=0$, $xor(1,0)=xor(0,1)=1$.
Let $f = [f_1]$ be a LEN that has been trained to approximate the $XOR$ function in the input space $C=[0,1]^2$. Then, if we consider e.g. the inputs $c^1=(0.2,0.7)$, $c^2=(0.6, 0.3)$, we get $\bar{c}^1=(0,1)$, $\bar{c}^2=(1,0)$, and therefore $\bar{f}_1(c^1)=\bar{f}_1(c^2)=1$. These examples yield respectively the example-level explanations $\varphi_{1,c^1}=\neg \bar{c}_1\wedge \bar{c}_2$ and $\varphi_{1,c^2}=\bar{c}_1\wedge\neg \bar{c}_2$, and the class-level explanation for $f_1$ is given by $\varphi_1=(\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)$. %In the same way, we may get the class-level explanation for the output $f_0$. 
% In the end, the following formulas represent the supervised explanations of the false and true classes, respectively:
% \[
% \forall c:\ \bar{f}_0(c)\leftrightarrow (\neg \bar{c}_1\wedge\neg \bar{c}_2)\vee(\bar{c}_1\wedge \bar{c}_2)\qquad\mbox{and}\qquad
% \forall c:\ \bar{f}_1(c)\leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)
% \]
The class-level explanation correctly match the truth-table of the boolean $XOR$ function.





% If we then consider that $f$ is composed of two hidden and one output neurons, we may want to explain the behaviour of each node. In particular, we may get that the first hidden neuron is represented by $ \tilde{h}_1^1  \leftrightarrow \neg \textit{c}_1\wedge \textit{c}_2$
% while the second $ \tilde{h}_2^1  \leftrightarrow \textit{c}_1\wedge \neg \textit{c}_2$. The output neurons $h^2 = f$ can be also represented in terms of the hidden neurons $f \leftrightarrow h_1^1 \vee h_2^1$ which in turns can be described again in terms of input concepts $f \leftrightarrow (\neg \textit{c}_1\wedge \textit{c}_2) \vee ( \textit{c}_1\wedge \neg\textit{c}_2)$.

\end{example}





Finally we mention that both example and set-level explanations can be recursively applied in case a cascading LEN or a single LEN with multiple $[0,1]$-valued layers are considered. For instance, given a cascading LEN as the one of Fig.~\ref{fig:CascadeExplainer}, we may get both example and class-level explanations of the concepts in $E_1 = C_2$ with respect to the ones in $C_1$, so as the concepts in $E_2$ with respect to the ones in $C_2$ and, in turn, in $C_1$. The modularity of logic formulas allows the composition of concepts at different levels that may express arbitrary complex relationships among them.



\draft{Logic explanations $\varphi_{i,S}$ generally hold only on a sub-portion $S$ of the sampled concept space $\mathcal{C}$.
% In the case in which the maximum MI criterion (Eq. \ref{eq:MI}) is used to drive the learning problem, each $\varphi_i$ will generally hold on a sub-portion of the concept space $O_i\subseteq C$. {\color{red}[This is also true for the supervised case, what is the difference?]}
However, we may get a logic formula providing an explanation holding everywhere by means of the disjunction
$\varphi = \varphi_1\vee\ldots\vee\varphi_r$, if we assume $O_1\cup\ldots\cup O_r=\mathcal{C}$.} Since $\varphi$ can turn out to be of little significance, if we are interested in simpler (and clearer) global explanations we may  convert $\varphi$ into an equivalent $\varphi'$ in \emph{Conjunctive Normal Form} (CNF). In particular, will there exist $r'$ and some clauses $\varphi'_1,\ldots,\varphi'_{r'}$ such that:
\begin{equation}
    \varphi=\bigvee_{i=1}^r\varphi_i \equiv \bigwedge_{i=1}^{r'}\varphi'_i=\varphi'.
\label{eq:dnf2cnf}
\end{equation}
As a result, we get a set of $r'$ explanations holding on the whole $\mathcal{C}$, indeed  $\varphi'_i(c)=1$ for every $c\in \mathcal{C}$, $i=1,\ldots,r'$.
Unfortunately, converting a boolean formula from DNF into CNF can lead to an exponential explosion of the formula.
% \fg{in che senso?}; in the following, we will see how to address this problem.
However, after having converted each $\varphi_i$ in CNF, the conversion can be computed in polynomial time with respect to the number of minterms in each $\varphi_i$ \cite{russell2016artificial}.



% \paragraph{Remarks}
The methodologies described so far illustrate how logic-based explanations can be aggregated to produce a range of explanations, from the characterization of individual observations to formulas explaining the model predictions for all the samples producing the same output concept.
The formula for a whole class can be obtained by aggregating all the minterms corresponding to example-level explanations of all the observations having the same concept output.
In theory, this procedure may lead to overly long formulas as each minterm may increase the complexity of the explanation. In practice, we observe that many observations share the same logic explanation, hence their aggregation does not change the complexity of the class-level formula (right-side Fig. \ref{fig:tt2form_freq}). In general, class-level explanations can be provided by aggregating just the most common explanations extracted from samples with the same output concept, avoiding a sort of ``explanation overfitting'' with the inclusion of noisy minterms which may correspond to outliers. Summing up, a possible limitation of this approach can be the readability of the logical rules, for instance in case (i) the number of input \draft{concepts} (the length of any minterm) $k \gg 1$, (ii) the size of the support $|O_i|$ is very large (possibly getting too many different minterms for any $f_i$). For these reasons, possible approaches to maintain an easy-to-understand set of very concise logical rules are fundamental to provide an useful explanation, e.g. as decision support. More details on how to select the most meaningful explanation terms are provided in Section \ref{sec:parsimony}.



\subsection{Learning criteria}
\label{sec:learncrit}

\draft{We just saw how a logic rule $\varphi_i$ can be associated to an output concept $f_i$. However to improve the expressiveness of logic explanations, \sm{in this section we will promote $\varphi_i$ to a FOL formula, to intersect logic and the usual approach to machine learning, in which a function trained on a finite collection of data is then generalized and applied to any out-of-sample inputs, following \cite{ciravegna2020constraint,ciravegna2020human,gnecco2015foundations} and related studies}. As a result, any $\bar{c}_j$ \sm{that composes $\varphi_i$} is thought of as a logic predicate defined on the concept space $C$, and such that $\bar{c}_j(c)=1$ if and only if $c_j>0.5$, for any $c\in C$. In addition, if for instance $\varphi_i=\bar{c}_2\wedge\neg \bar{c}_5$, we will write $\varphi_i(c)$ for $\bar{c}_2(c)\wedge\neg \bar{c}_5(c)$.}
Following the distinction among the user \sm{objectives} introduced in Section~\ref{sec:explanation_styles}, we focus on the loss functions that are optimized to train a LEN to develop the capability of providing explanations accordingly to such \sm{objectives}, that are similar to the outcomes of our previous experiences in \cite{ciravegna2020constraint,ciravegna2020human}.
For simplicity, here we will not distinguish among the different computational pipelines, thus referring to a single generic LEN block with $r$ output units in all the \sm{objectives} of \textsc{interpretable classification}, \textsc{explaining a black-box} and \textsc{interpretable clustering}.







\textsc{Interpretable classification. }
%In the case of \emph{Supervised Explanations}, we aim at providing explanations of certain classes. In this sense, we want our model $f$ to be active whenever the class we aim to explain is also active.
% (i.e. $f_i(c) = Y_i(c) = 1$)
% We do not distinguish here whether the LEN is performing an \textit{interpretable classification} ($f_i\simeq Y_i$) or it is \textit{explaining an existing classifier} ($f_i \simeq g_i$), since for what concerns the optimization function it does not make any difference.
%Let us assume the interpretable classification case. The case of explaining a black-box model $g$ can be obtained by replacing $Y_i(c)$ with $g_i(c)$ in the loss unctions. The only difference in the two cases is that while $Y_i(c) \in \{0, 1\}$ is a discrete membership function, $g_i(c) \in [0,1]$ provides the probability of class assignment.
%Further, for sake of simplicity, in what follows we will assume $f: C=X\rightarrow E=Y$.
\draft{Training a LEN by supervised learning is what is needed in order to create the conditions to extract explanations for specific categories, i.e. to bind a logic explanation provided by $\varphi_i$ to a specific output class of a classification problem. By denoting with $\bar{y}_i$ the binary predicate associated to the name of the output class $i$, we will consider three kind of FOL explanations $\rho_i$ expressed as the universal closure of an IF, Only IF or IFF rule, between $\varphi_i$ and $\bar{y}_i$.
%
These rules can be enforced in case of interpretable classification according to the following learning criteria.
% $\varphi_i$ can be related to the class $i$, by training the corresponding output $f_i$ of a LEN with supervised learning. 
}

IF rules mean that, in the extreme case, for each example of class $i$ we want the $i$-th output of the LEN to score one (and not necessarily vice-versa). In other words, \draft{the set of concept tuples $c$ belonging to the $i$-th class, i.e. such that $\bar{y}_i(c)=1$ has to be included in the support of $\bar{f}_i$, \sm{while no conditions are imposed when $\bar{y}_i(c)=0$ (recall that $f_i(c) \in [0,1]$)}.}
This behavior can be achieved by minimizing a hinge loss,
\begin{equation}
L_{\rightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \max\{0, \bar{y}_i(c) - f_i(c)\}\qquad  i \in [1,  r].\label{eq:IF}
\end{equation}
 Following a symmetric approach, in Only IF rules it may be the case of a class to be explained in terms of some lower-level concepts. This principle is easily enforced by switching the two terms of the loss function in Eq. \ref{eq:IF},
\begin{equation}
L_{\leftarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \max\{0, f_i(c) - \bar{y}_i(c)\}\qquad  i \in [1,  r].\label{eq:IF2}
\end{equation}
Both in IF and Only IF rule, in order to make the learning problem well posed, further conditions on $f$ must be included, to define its behaviour in the space areas not covered by the data and to avoid trivial solutions with constant $f$. \sm{For example, $f$ could have a fixed bias equal to $1$ no biases at all.}

At last, LEN can learn double implication rules (IFF) in which an explanation can completely characterize a certain class, \sm{and that is the type of explanation on which we focus}. %These rules require the support of the LEN and the support of the class to be strictly equal.
%For this reason,
Any function penalizing points for which $f_i(c)\neq \bar{y}_i(c)$ may be employed in this scenario, such as the the classic Cross-Entropy loss,
\begin{equation}
L_{\leftrightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \bar{y}_i(c)\log(f_i(c)) + \left( 1-\bar{y}_i(c) \right) \log \left( 1-(f_i(c)) \right).
% L_{\leftrightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} |f_i(c) - \bar{y}_i(c)|^2 \qquad  i \in [1,  r], 
\label{eq:IFF}
\end{equation}
%IFF loss function is preferred when a LEN performs E2E \textit{interpretable classification}, since we want the output of $f$ to be as close as possible to $\bar{Y}$ in order to maximize the classification accuracy.
% In this latter case if we want the same LEN to explain different, mutually exclusive classes, a Softmax activation function can be also employed.
\draft{
In any of these cases (Eq.~\ref{eq:IF}-\ref{eq:IFF}), we provide a logic explanation in First-Order Logic by means of the following equations, by introducing the FOL formulas $\rho_i$, for $i=1,\ldots,r$, ranging on the whole concept space $C$, \sm{thus generalizing the relationships discovered on the data samples}, 
\begin{align}
\text{IF-rule}: \qquad &  \rho_i = \forall c\in C:\ \bar{y}_i(c)\rightarrow\varphi_i(c). \label{eq:FOLexplIF}\\ 
     \text{Only IF-rule}: \qquad  & \rho_i = \forall c\in C:\ \varphi_i(c) \rightarrow  \bar{y}_i(c) \label{eq:FOLexplFI}\\
     \text{IFF-rule}: \qquad & \rho_i = \forall c\in C:\  \bar{y}_i(c) \leftrightarrow \varphi_i(c)\label{eq:FOLexplIFF}
\end{align}
In the same way, in case of a concept-bottleneck pipeline, we may still derive a FOL explanation according to a certain function $g:X\to C$ extracting LEN input concepts from raw features. For instance for the IFF-rule, we will get
\begin{equation}
\rho_i=\forall x \in  X:\ \bar{y}_i(g(x))\leftrightarrow\varphi_i(g(x))
\label{eq:FOLexplCB}
\end{equation}
\sm{We remark that} the logic predicate $\bar{y}_i$ appearing in the Eq.~\ref{eq:FOLexplIF}-\ref{eq:FOLexplCB}
is simply a \textit{virtual} predicate denoting the membership of a certain concept tuple $c\in C$ to the $i$-th output class. %. It coincides with the available class label of concept in $\mathcal{C}$, then 
%and the previous FOL formulas are correctly verified for any $c\in C$.
%
% In particular, any $f_i$ will be related to class labels $\bar{y}_i$ or class predictions $g_i$ for the interpretable classication and explaining a black-box cases, respectively. 
Despite the correspondence between $f_i$ and $\bar{y}_i$ can be enforced only on the sampled concept  space $\mathcal{C}$, we assume that any $\rho_i$ can generalize to unseen concept tuples in the whole concept space $C$, following \cite{ciravegna2020human,ciravegna2020human,gnecco2015foundations}.
}

















%%%%%%%%%%%%%%CUT

\textsc{Explaining a black-box. } In this case, the output of the LEN is forced to mimic the one of a black-box \draft{$g:C\rightarrow Y$, instead of the original problem output labels. This behaviour can be enforced by considering loss functions analogous to the ones in Eq.~\ref{eq:IF}-\ref{eq:IFF}, with $g_i$ in place of $\bar{y}_i$. For instance, for the IFF rule}
the coherence loss \sm{of Eq.~\ref{eq:IFF}} can be exploited \sm{to allow the LEN to mimic the behaviour of the black-box},
\begin{equation}
L_{\leftrightarrow}(g_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} g_i(c)\log(f_i(c)) + \left( 1-g_i(c) \right) \log \left( 1-(f_i(c)) \right)
 \label{eq:coher}
\end{equation}
\draft{As in the case of interpretable classification, IF, Only IF and IFF rules can be expressed according to Eq.~\ref{eq:FOLexplIF}-\ref{eq:FOLexplCB}. However, now the FOL explanations will be guaranteed to hold assuming that $\bar{y}_i(c)$ \sm{is not a virtual predicate, but it is explicitly associated to the (booleanized) black box predictions $g_i(c)$, that is what we enforce by learning on the discrete data sample $\mathcal{C}$}.
}
%
% In particular, any $f_i$ will be related to class labels $\bar{y}_i$ or class predictions $g_i$ for the interpretable classication and explaining a black-box cases, respectively. 

%the explanations provided by LENs are first-order logic formulas, and this newly devised pieces of knowledge can be reused and enforced on the output of the classifier $g$. This is commonly considered in the generic \emph{learning from constraints} framework \cite{gnecco2015foundations}, and it may be of particular interest, especially for semi-supervised settings. A similar strategy has already been considered e.g. in \cite{ciravegna2020constraint}, where a set of FOL formulas have been, at first extracted from data, and then converted into continuous loss functions to be injected in the learning objective.
%At last, the extracted formulas can also be used to check the behaviour of the classifier on test data, e.g. to detect adversarial samples as done in \cite{melacci2020domain}.

\textsc{Interpretable clustering. }
% \paragraph{Mutual Information Criterion}
% \paragraph{Relations among Concepts.}
Generic explanations can be achieved by means of fully unsupervised  principles \sm{that we borrow} from Information Theory. As a matter of fact, the maximization of the Mutual Information (MI) index between the input concept space $C$ and the output concept space $E$ allows the LEN to
be trained in a fully unsupervised way \cite{ciravegna2020constraint}. More specifically, a max-MI criterion (see \cite{melacci2012unsupervised} for further details) leads to the development of a LEN that has the tendency of producing 1-hot activation scores, such that $\forall c \in \mathcal{C}$ only one $f_i(c) \simeq 1$, while the others are close to zero. In a sense, it enforces the LEN to cluster the data in a way that each input sample belongs to a single cluster.
In order to define the MI index, we have to model the probability distribution of each $f_i$ to be active (close to 1) on a given sample $c$, that we implemented using the softmax operator on the LEN output. %Following the classic notation of discrete MI,
%$E$ is a discrete random variable associated to the output of the LEN functions while $C$ is the variable related to the data in the concept space.
The learning criterion to minimize in order to train the LEN is minus the MI index,
\begin{equation}
    L_{MI}(f,\mathcal{C}) = - H_{E}(f,\mathcal{C}) + H_{E|C}(f,\mathcal{C}) \ ,
	\label{eq:MI}
\end{equation}
where $ H_{E}$ and $ H_{E|C} $ denote  the entropy and the conditional entropy functions associated to the aforementioned probability distribution, respectively, and measured over the whole $\mathcal{C}$, as in  \cite{ciravegna2020constraint}.
%An outcome of the maximization of the MI index is that the supports of the explaining functions will tend to partition the input space $X$, i.e., $X=\bigcup_{j=1}^mX_j$ and $X_j\cap X_k=\emptyset$, for $j\neq k$ (see \cite{melacci2012unsupervised,betti2019cognitive} for further details).
\draft{
In this case, the support $O_i$ of $\bar{f}_i$ is exactly the cluster of data points where the $i$-th output of the LEN is active. Leaving $\varphi_i$ free to relate concepts in a purely unsupervised manner, we naturally get the FOL explanation}
\begin{equation}
\rho_i=\forall c \in O_i:\ \varphi_i(c).
\label{eq:FOLexplMI}
\end{equation}

Of course, in all the computational pipelines in which a classifier $g$ is also employed,
%In the particular case of a LEN providing explanations for an existing classifier $g$,
the available supervision is enforced on $g$ as well, e.g., by means of the Cross-Entropy loss. As a side note, we remark that what we are describing in a fully supervised setting can be trivially extended to the semi-supervised one, as we already investigated in \cite{ciravegna2020constraint,ciravegna2020human}.






\subsection{Parsimony} \label{sec:parsimony}
When humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one \cite{aristotlePosterior,mackay2003information}. 
\sm{In the case of LENs, the notion of simplicity is implemented by reducing the dependency of each output unit by all of the $k$ input concepts, encouraging only a subset of them to have a major role in computing the LEN output. Such subset is of size $m_i < k$ for the $i$-th output unit.}

Over the years, researchers have proposed many approaches to integrate ``\textit{the law of parsimony}'' into learning machines. \sm{These approaches can be eventually considered as potential solutions to implement a parsimony criteria in LENs, in order to find a valid way to fulfill the end-user requirements on the quality of the explanations and on the classification performance.}
%Here we describe a few fundamental parsimony criteria which may help in developing and implementing a variety of LENs. 
% \subsubsection{Occam's razors}
% \paragraph{Occam's razors}
% \textsc{Occam's Razors. }
\sm{For instance,} Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous techniques to put in practice the Occam's razor principles in the fields of statistics and machine learning. 
Among such techniques, $L1$-regularization \cite{santosa1986linear} has been recently shown to be quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages weight sparsity 
% \begin{equation}
    %$\lambda ||W||_1$.
% \end{equation}
by shrinking the less important weights %'s values
to zero  \cite{tibshirani1996regression}. %, this regularization technique completely removes some weights %altogether in the limit,
 \sm{This allows the model to ignore some neuron inputs, that, in the case of the first layer of a LEN, turns out in discarding or giving negligible weight to some of the input concepts, opening to simplified FOL explanations.
If $W$ collects (a subset of) the weights of the LEN that are subject to this regularization, the learning criterion is then augmented by adding $\lambda \| W \|_1$. Notice that the precise weights involved in $W$ might vary in function of the selected neural architecture to implement the LEN, that is the subject of Section~\ref{sec:outofthebox}.}
%This allows the model to ignore the associated input features and, therefore, to provide simpler explanations. For this reason, 
All the out-of-the-box LENs presented in the next section are trained using this parsimony criterion, \sm{that acts in different portions of the network in the considered instances of LENs, and that is combined with a pruning strategy amongst the ones that are defined in the following.}


\subsubsection{Pruning strategies}
\label{sec:pruning}
The action of parsimony criteria, such as regularizers or human priors, influences the learning process %of learning machines
towards specific local minima. Once the model has finally converged to the desired region of the optimization space, the effort can be speed up and finalized by pruning the neural network \cite{lecun1989optimal,hassibi1993second}, \sm{removing connections that are not expect to carry important information, accordingly to the selected pruning strategy}. Such a strategy has a profound impact both on the quality of the explanations but also on the classification performance \cite{frankle2018lottery}. Here we present three effective pruning strategies specifically devised for LENs, \sm{where the main goal is to keep the FOL formulas compact for each LEN output.}

% \paragraph{Node-level pruning}
\textsc{Node-level pruning. }
The most local way of implementing a pruning strategy consists in independently considering each neuron of the network.
Once we define the maximum \textit{fan-in} (number of non-pruned connections) for each neuron of a feed-forward neural network, \sm{we can remove all the connections associated to the smallest weights entering the neuron, until the target fan-in is matched}. We refer to this strategy as \textit{node-level pruning}.
%A fan-in pruning strategy generates a feed-forward graph where each neuron has the same number of incoming non-pruned connections.
%In particular, at the end of the training process, the absolute value of the weights in the  matrix $W^{i}$ is computed for each layer $i=1,\dots,L$.
\sm{When applied to all the neurons of the network, this strategy it reduces the number of paths connecting the network input to each output neuron.}
\sm{In detail,} the node-level approach prunes one by one the weights with the smallest absolute value, such that each neuron in the network has a fixed number \sm{$\zeta$} of incoming non-pruned weights. The parameter \sm{$\zeta$} must be decided in advance, and it determines the computational capabilities of the pruned model as well as the complexity of the logic formulas which can be extracted, \sm{since it reduces the number of paths connecting the network input to each output neuron}. To get reasonably simple explanations out of a neuron, the parameter $\zeta$ may range between $2$ and $9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Recent work on explainer networks has shown how node-level pruning strategies may lead to fully explainable models  \cite{ciravegna2020constraint}. However, we will show in the experimental section that this pruning strategy strongly reduces the classification performances.

% \paragraph{Network-level pruning}
\textsc{Network-level pruning. }
In order to overcome the heavy reduction of the \sm{computational} capacity of the node-level pruned models, we introduce the so-called \textit{network-level pruning}.
Indeed, \sm{the most evident pruning operation that has a precise role in reducing the number of concepts involving in the FOL explanations is the one that is directly applied to limit the impact of the each input concept into the first layer of neurons of the network.} %the main aim of pruning is to only reduce the number of input terms involved in the final explanations. 
%By directly limiting the number of input features considered by the network, we can achieve this result with a lighter impact on the overall model.
At each iteration step, \sm{the $L$2 norm of the connections departing from each input concept is computed}, \sm{If $w = [w_1,\ldots,w_k]$ is the vector that collects the resulting $k$ norms}, then we re-scale it in the interval $[0,1]$,
\begin{equation}
    w' = \frac{w}{\max_j \{ w_j,\ j=1,\ldots,w_k \}}
\end{equation}
\sm{where the division is intended to be applied in an element-wise fashion.}
In this way, $w'$ gives a normalized score to rank input concepts by importance. The \textit{network-level strategy} consists in pruning all the input features for which $w_j' < \tau$, where $\tau$ is a custom threshold (usually, $\tau = 0.5$). Alternatively, %the $\mu$ approach may
we can also retain the \sm{$\zeta$} most important input concepts and discard the ones by pruning the connections that depart from them, similarly to the criterion used in the  \textit{node-level pruning} for each single neuron. %The parameter $q$ is user-defined and may range between $2$ and $9$ to get sensibly compact explanations \cite{miller1956magical,cowan2001magical,ma2014changing}.
This pruning strategy is far less stringent compared to the node-level pruning as it affects only the first layer of the network and it does not prescribe a fixed fan-in for each neuron.

% \paragraph{ReLU pruning}
% \paragraph{Example-level Pruning}
\textsc{Example-level pruning. }
Example-level pruning is a particular strategy exploiting the well-studied local linearity property of neural networks whose activation functions in all hidden layers are Rectified Linear Units (ReLU Networks) \cite{hahnloser2000digital}.
% \paragraph{Local Linearity}
\sm{If the LEN is implemented as a ReLU Network}, for any input $c \in C$, the Directed Acyclic Graph (DAG) ${\cal G}$ describing the structure of the connections in the LEN, can be reduced to ${\cal G}_{c}$,
which only keeps the units corresponding to active neurons (the ones for which the ReLU activation is non-zero) and the corresponding arcs \sm{(referred to as ``firing path'')}.
Since all neurons operate in ``linear regime'' (affine functions) \sm{in the reduced ${\cal G}_{c}$}, as stated in the following,
\sm{the input-to-output transformation computed by the multi-layer feed-forward ReLU network \sm{with structure ${\cal G}_{c}$} is a composition of affine functions over the network hidden layers that, in turn, can be simplified with a single affine function, leading to 
\begin{equation}
    f(c) = \sigma (\hat{W}^{(c)} c + \hat{b}^{(c)}), 
    \label{eq:single}
\end{equation}    
\sm{being $\sigma$ the activation of the output layer and $\hat{W}^{(c)}$, $\hat{b}^{(c)}$ a weight matrix and biases (respectively) computed as described in the following}.}
\begin{theorem}
	\sm{Let $\{\xi_1,\ldots,\xi_L \}$ be a collection of affine functions, where
% 	\[
		$\xi_{\kappa}: U_{\kappa} \mapsto V_{\kappa}: u \mapsto W_{\kappa} u + b_{\kappa}$
% 	\]
	and $\forall \kappa=1,\ldots, L-1: \ \ U_{\kappa+1} \subset V_{\kappa}$. If a multi-layer network computes the last layer activations as
% 	\[
		$\xi_{L} \circ \xi_{L-1} \circ \dots \circ \xi_{2} \circ \xi_{1} c$,
% 	\]
	then such transformation is affine and we can re-write it as $\hat{W} c + \hat{b}$, where
	\begin{equation}
	    \hat{W} = \prod_{\kappa=1}^{L} W_{\kappa}, \qquad
	    \hat{b} = \sum_{\kappa=0}^{L-1}  b_{L-\kappa} \prod_{h=0}^{\kappa} W_{L-h+1}
	\end{equation}
	and $W_{L+1}:=I$.}
	\label{theorem:affine}
\end{theorem}

%Therefore, for a given input $c$ an affine function $f(c)$ can be devised. 
\sm{The proof of Theorem \ref{theorem:affine} is straightforward. Such a theorem perfectly applies to the case of ReLU networks once $\mathcal{G}_c$ has been fixed, since they boil down to simple network with linear activations. The theorem does not introduce any conditions on how input is represented or on the activation functions in the output layer.} %On the contrary, output nodes may be equipped with a sigmoid activation for binary or multi-label classification or a softmax activation function in case of multiclass.
\sm{Given $c \in C$, once \sm{${\cal G}_{c}$} has been determined, the function computed by the (deep) LEN has the following form, $f(c) = \sigma( \xi_{L}^{(c)} \circ \xi_{L-1}^{(c)} \circ \dots \circ \xi_{2}^{(c)} \circ \xi_{1}^{(c)} c )$, that reduces to $f(c) = \sigma (\hat{W}^{(c)} c + \hat{b}^{(c)})$, where the superscript ${(c)}$ is added to the symbols of Theorem \ref{theorem:affine} to highlight the fact they are specifically instantiated in the case of the network with structure ${\cal G}_{c}$. The reduced form of $f$ is much easier than considering the one of the original deep network.
However, ${\cal G}_{c}$ might vary for each input $c$, thus we might get different transformations for different input samples.}
Indeed, \sm{for each sample we can compute the corresponding ${\cal G}_{c}$ and, in turn, $\hat{W}^{(c)}$ and $\hat{b}^{(c)}$, that we can prune as described in the case of network-level pruning, keeping only the connections associate to the most important concepts for the considered sample.}


\section{Out-of-the-box LENs}\label{sec:outofthebox}


Crafting state-of-the-art fully interpretable models is not an easy task; rather, there is a trade-off between interpretability and performances.
The framework \sm{introduced in Section~\ref{sec:basics}, with the methods described in Section~\ref{sec:methods}}, is designed to provide the building-blocks to create a wide range of models having different interpretability vs. accuracy
% interpretability-VS-explainability-VS-performance
trade-offs.
Here, we \sm{showcase three out-of-the-box neural networks that implement different LENs, whose key properties are about different ways of exploiting the parsimony strategies, as visually anticipated in Fig.~\ref{fig:visual} (right). In Fig. \ref{fig:out-of-the-box} we sketch the so-called $\psi$, $\mu$, and ReLU out-of-the-box LENs that will be described in the following. Briefly,} the $\psi$ network, originally proposed in \cite{ciravegna2020constraint}, is a fully interpretable model with limited learning capacity and that provides mediocre explanations; the $\mu$ network is a neural model that can provide high-quality explanations, good learning capabilities and modest interpretability; the ReLU network is a black-box model ensuring state-of-the-art learning capabilities and good explanations at the cost of very low interpretability. The characteristics of these three LENs are also summarized in Table~\ref{tab:LENs}.


\begin{table}[ht]
\centering
\caption{Out-of-the-box LENs and their main properties.}
\label{tab:LENs}
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{LEN}                            & \textbf{Pruning} & \textbf{Activation}  & \textbf{Learning}  & \textbf{Explanation}   & \textbf{Interpretability}\\
\midrule

$\psi$ Network (Fig. \ref{fig:psi_net}) & Node-level        & Sigmoid                       & Low                           & Low                               & Very high     \\
$\mu$ Network (Fig. \ref{fig:mu_net})   & Network-level     & Any                           & High                          & Very high                         & High          \\
ReLU Network (Fig. \ref{fig:ReLU_net})  & Example-level     & ReLU                          & Very high                     & High                              & Low           \\

\bottomrule
\end{tabular}
}
\end{table}


\begin{figure}[ht]
    \centering

     \begin{subfigure}{1\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth]{figs/psi_nn.png}
         \caption{$\psi$ network (Subsection \ref{subsec:psi}). {\color{red}remove ->, <-> and what follows on the right - NOT ALWAYS: put $\bar{h}_1=$ on the left and so on, also $e=$, but remove it in the class explanation!. Rename 'explanation' in 'rule' (twice). Rename 'class' in 'output'}}
         \label{fig:psi_net}
     \end{subfigure}\\

     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/mu_nn.png}
         \caption{$\mu$ network (Section \ref{subsec:mu}). {\color{red}remove ->, <-> and what follows on the right. Rename 'explanation' in 'rule' (twice). Rename 'class' in 'output'.}}
         \label{fig:mu_net}
     \end{subfigure}
     \qquad
     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/ReLU_nn.png}
         \caption{ReLU network (Section \ref{subsec:ReLU}).{\color{red}remove ->, <-> and what follows on the right. Rename 'explanation' in 'rule' (twice). REMOVE THE VERTICAL YELLOW THING $c^1$}}
         \label{fig:ReLU_net}
     \end{subfigure}

    \caption{Out-of-the-box LENs  \sm{showcased in the case of interpretable classification, with examples of logic rules extracted using the procedure of  Section~\ref{sec:logic_rule_extr}}. (a) $\psi$ networks
    %(Subsection \ref{subsec:psi})
    only admit $[0,1]$-valued neurons with low fan-in, hence we can associate a boolean formula to each neuron by analysing its I/O truth-Table~(b) $\mu$ networks
    %(Subsection \ref{subsec:mu})
    do not have interpretable hidden neurons but the input concepts are drastically pruned which allows to provide simple network-level explanations. (c) ReLU networks
    %(Subsection \ref{subsec:ReLU})
    supply explanations for each example by means of the equivalent affine transformation. However, nor the nodes, nor the network can be logically interpreted. {\color{red} ALL FIGS: replace $X=C$ with $X$. Replace $E$ with $Y$. Replace $c_0$ with $c_1$ and so on both in yellow boxes and in RULES! Do the same with $h$.}}
    \label{fig:out-of-the-box}
\end{figure}

\subsection{$\psi$ Network} \label{subsec:psi}
A $\psi$ network, originally proposed in \cite{ciravegna2020constraint,ciravegna2020human}, \sm{perfectly suits the framework of LENs}. A $\psi$ network is based on three design principles:
($i$) all activation functions for all neurons (including hidden units) should be sigmoids;
($ii$) a strong $L$1-regularization is used in all the layers to shrink the less important weight values towards zero;
($iii$) a node-level pruning strategy is considered, where each neuron of the network must have the same number of incoming non-pruned weights (suggested values are between 2 and 9). This number is directly proportional to the number of terms involved in the explanations.
\sm{In \cite{ciravegna2020constraint}, the rule generation mechanism involves the extraction of rules from each neurons of the network (also the hidden ones), and the node-level pruning favours simple rules on each neuron. Rules are then combined to get the final explanations, and the number of hidden layers in the network needed to be small to avoid issues in the rule-merging procedure.}
A black-box model $g$ (a convolutional neural network) is used to predict a set of categories from a data set $X$ (images), and the authors used a $\psi$ network to explain the behaviour of classifier $g$, \sm{in terms of the outputs of $g$}.
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.24]{figs/psi_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

\sm{We can cast the $\psi$ network in the generic framework of this paper.} The computational pipeline presented in the original work is basically a Concept-Bottleneck pipeline.
\sm{However, from the perspective of the rule-extraction mechanism, the $\psi$ network can be seen as a Cascading LEN where each layer corresponds to a new level of LEN, each of them generating rules. However, the network is trained as a whole, since only the first layer gets human-understandable concepts (whole the Cascading pipeline of Section~\ref{sec:use_cases} prescribes input concepts at each LEN level). The neuron-specific explanations are then aggregated in order generate final explanations only involving the input concepts.}
%\draft{Furthermore, it can provide both example and set-level explanations, and it is the only LEN providing compounded node-by-node explanations.} 
%As a matter of fact, thanks to the node-level pruning strategy, the $\psi$ network allows to interpret (and extract a corresponding logic formula) from each node.
By recalling Example \ref{ex:xor}, \draft{for instance} a $\psi$ network with \sm{a single hidden layer with} two hidden nodes may learn the logic formula:
\begin{equation}
\varphi_1= (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2),
\label{eq:xor}
\end{equation}
with the hidden nodes learning the formulas $\bar{h}_1= \neg \bar{c}_1\wedge \bar{c}_2$ and $\bar{h}_2 = \bar{c}_1\wedge \neg\bar{c}_2$ respectively, and the output node $f_1$ learning $\varphi_1 = \bar{h}_1 \vee \bar{h}_2$.

% PROS AND CONS
We remark that the $\psi$ network is specifically designed to be a fully interpretable neural network, therefore, here we also show its performances as a classifier in different contexts.
As shown in Fig. \ref{fig:psi_net}, this network provides a high level of interpretability since each neuron can be explained.
On the contrary, the strong regularization and the restrictive pruning strategy lead to poor classification accuracy making $\psi$ networks hard to train and not suitable for solving complex categorical learning problems. Besides, the provided explanations can be very expressive but they can not be outstanding as expected, due to the \sm{limited learning capabilities of the model}.

\subsection{$\mu$ Network}  \label{subsec:mu}
A $\mu$ network is a LEN based on a multi-layer perceptron \sm{without the strong constraints on the neuron fan-in of the $\psi$ net. In particular,} a $\mu$ network is based on two design principles:
    ($i$) a strong L1-regularization is used only \sm{in the weights connecting the input to the first layer of the network};
    ($ii$) a network-level pruning strategy, which only prunes the input neurons.
After the pruning step, the $\mu$ network can be fine-tuned to \sm{better adapt it} to the new configuration. No assumptions need to be made nor on the hidden layers nor on the activation functions. However, by applying a network-level pruning strategy, the same set of retained \sm{input concepts} is used for the whole network. On the one side, this allows to logically-interpret the network \sm{in a compact manner} and, therefore, to provide explanations. On the other side, this may represent a severe limitations for multi-class classification since each class may rely on \sm{its own input concepts}, but these may be very different among the classes. \sm{However, $\mu$ networks can be efficiently adapted to multi-class experiments (as the ones of Section \ref{sec:experiments}) by splitting the multi-class problem into a set of binary classification problems (one per class), i.e. using a set of light binary $\mu$ networks.}

%This LEN can provide a wide range of logic-based explanations (i.e. local, cluster, and class-level).
%For each $\mu$ network, an explanation is provided in terms of the input concepts.
Still considering Example \ref{ex:xor}, $\mu$ networks with different number of hidden layers may easily learn the same logic formulas.
The network-level pruning strategy in this specific example should not prune any input features since both $c_1$ and $c_2$ are important for the final classification. However, if we suppose also some other redundant features to be present, they would be likely discarded in favor of $c_1$ and $c_2$, as shown in Fig. \ref{fig:mu_net}.
%As described in Sec. \ref{sec:logic_rule_extr}
\sm{Assuming the network to have correctly learn the provided examples, the support set $O_1$ will be composed by the second and third examples of the yellow-box in Fig. \ref{fig:mu_net}, that will yield the following example-level explanations (respectively)}
\draft{\[
\neg c_1 \wedge c_2 \quad \text{and} \quad c_1 \wedge \neg c_2.
\]}
The two explanations can be then considered altogether \sm{(Eq.~\ref{eq:agg_exp})} to totally explain the whole class $1$ (class-level explanation) by
\[
\varphi_1 = \bigvee_{c \in O_1}\varphi_{i,c} =
 (\neg \bar{c}_1\wedge \bar{c}_2) \vee ( \bar{c}_1\wedge \neg\bar{c}_2).
\]
Thanks to the permissive pruning strategy, the learning \sm{capabilities} of the network \sm{are almost the same of a non-constrained network}. As a consequence, $\mu$ networks are suitable for solving and explaining more complex categorical learning problems. \sm{As we will show in Section~\ref{sec:experiments},} the quality of the explanations provided by the $\mu$ networks are among the highest between the proposed models. At last, a mild-level of interpretability is also guaranteed since $\mu$ nets can be logically interpreted as \sm{whole, but not over the single neurons as in $\psi$ networks}.

\subsection{ReLU network}  \label{subsec:ReLU}
Another example of LEN which provides a different accuracy vs. interpretability trade-off is the ReLU network. %is a special case of a $\mu$ network sharing most of its characteristics but with a few different properties.
It is based on three design principles:
    ($i$) all activation functions for all \emph{hidden} neurons are rectified linear units;
    ($ii$) a mild L1-regularization is applied \sm{to all the weights associated to each layer of the network};
    ($iii$) an example-level pruning strategy is used, i.e. a specialized pruning strategy for each sample.
\sm{Principle $iii$ can be applied due to the presence of} rectified linear units activation functions. %, i.e. a pruning strategy which is applied for each sample.
This is not a limitations since it is one of the most widely used and efficient activation functions employed in deep learning \cite{glorot2011deep,ramachandran2017searching}.
\sm{What makes this instance of LEN significantly different from both $\psi$ and $\mu$ nets, is that the pruning strategy does not alter at all the network structure. This is due to the fact that pruning is applied to the weights  that belong to the single-affine instance of $f(c)$ of Eq.~\ref{eq:single}, whose values are collected in $\hat{W}^{(c)}$ and are only computed for rule-extraction purposes.} This means that the original capacity of the model is fully preserved, eventually leading to state-of-the-art classification performances. However, this type of pruning does not provide any insights of the model behaviour, \sm{since it is only about the considered example $c$}, and they may not always lead to optimum explanations.

Recalling again Example \ref{ex:xor}, a ReLU network with  hidden layers \sm{can learn the correct logic formula by aggregating different example-level explanations, as we did in the case of the $\mu$ network. For example, in Fig.~\ref{fig:ReLU_net} we show the case of the processing second sample from the yellow table, that provides a portion of the explanation of the XOR function.} \sm{However, when we restrict the connections to the arcs of $\mathcal{G}_{c}$ for a certain sample $c$, we actually discard several weights of the original ReLU network, i.e., the ones of all the connections that are not needed for correctly classify the considered $c$. This implies that the single-affine instance of $f(c)$ of Eq.~\ref{eq:single}, being it function of $\mathcal{G}_c$, has a very localized dependence on the space region to which $c$ belongs. Since Eq.~\ref{eq:single} is the form of the LEN from which we extract the example-level explanation, there is the serious risk of getting back an explanation that does not carry much information from the original structure $\mathcal{G}$ and that does not globally applies to the whole class. As a matter of fact, there might be strong differences on the example level explanations of samples, even when belonging to the same class. }

%the local explanations of a certain point $c$ may not be as correct as the ones provided by the $\mu$ networks. Indeed, it can be demonstrated that the affine function $f^*$, actually corresponds to the nearest decision boundary to the points.
% On the other hand, an example-based pruning strategy may be provide more unstable explanations as the pruning may be negatively affected by the presence of outliers.
%\draft{Hence the corresponding weights may miss some important features to explain $c$, and then a ReLU network may explain the XOR problems with an uncorrected formula, like}
%\begin{equation}
%\varphi_1 = \bigvee_{c \in O_1}\varphi_{i,c} =
% (\neg \bar{c}_1) \vee (\neg\bar{c}_2).
%\end{equation}
Summing up, this LEN does provide the best performances in terms of classification accuracy thanks to the example-level pruning strategy \sm{that do not alter the original net}. However, this comes at the cost of poor model interpretability and mild explanation capacity.

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figs/ReLU_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


\section{Benchmarking out-of-the-box LENs} \label{sec:experiments}
In this section, we quantitatively assess the quality of the explanations and the performance of LENs, compared to state-of-the-art white-box models. \sm{We considered several tasks, covering multiple combinations  of computational pipelines (Section~\ref{sec:use_cases}) and objectives (Section~\ref{sec:explanation_styles})}. The summary of each task is reported in Table \ref{tab:datasets}.
A brief description of each task, the corresponding dataset and all the related experimental details are exposed in Section \ref{sec:exp_details}. In Section \ref{sec:exp_metrics} six quantitative metrics are defined and used to compare LENs with the considered state-of-the-art methods.

\begin{table}[ht]
\centering
\caption{Experiments.}
\label{tab:datasets}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Dataset} & \textbf{Description} & \textbf{Pipeline (Sec.~\ref{sec:use_cases})}  & \textbf{Objective (Sec.~\ref{sec:explanation_styles})}\\
\midrule

MIMIC-II  (Fig. \ref{fig:E2EExplainer})                      & \small{Predict patient survival from clinical data}       &E2E & Interpretable classification   \\
MNIST E/O (Fig. \ref{fig:CMBExplainer})                         & \small{Predict parity from digit images}                  & CB & Interpretable classification  \\
CUB (Fig. \ref{fig:len})                                    & \small{Predict bird species from bird images}             & CB & Interpretable classification \\
V-Dem (Fig. \ref{fig:CascadeExplainer})                     & \small{Predict electoral democracy from social indexes}   & Cascading & Interpretable classification  \\
MIMIC-II (EBB)     & \small{Predict patient survival from clinical data}       & E2E & Explaining black box       \\
MNIST E/O (ICLU)                     & \small{Cluster digit properties from digit images}        & CB & Interpretable clustering      \\
\bottomrule
\end{tabular}
}
\end{table}


% \subsection{Software tool and usability}
% \label{sec:tool}
In order to make the LENs framework accessible to the whole community, we released of a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on methods and out-of-the-box LENs. The Python code and the scripts used for the experiments, including parameter values and documentation, is freely available under Apache 2.0 Public License from a GitHub repository\footnote{\url{https://github.com/pietrobarbiero/deep-logic}}. \sm{The code is based on our} Deep Logic library, \sm{that} is designed to make out-of-the-box LENs accessible to researchers and neophytes by means of intuitive APIs requiring only a few lines of code to train and get explanations from a LEN, as we sketch in the code example of Listing \ref{code:example}.
\begin{center}
\begin{minipage}{0.65\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny, language=Python, label=code:example, caption=Example on how to use the Deep Logic library.]
import deep_logic as dl

# import train, validation and test data loaders
[...]

# instantiate a mu network
model = dl.models.MuNN(n_classes=n_classes, n_features=n_features,
                       hidden_neurons=[200], loss=torch.nn.CrossEntropyLoss(),
                       l1_weight=0.001, fan_in=10)

# fit the model
model.fit(train_data, val_data, epochs=100, l_r=0.0001)

# get predictions on test samples
outputs, labels = model.predict(test_data)

# get first-order logic explanations for a specific target class
target_class = 1
formula = model.get_global_explanation(x_val, y_val, target_class)

# compute explanation accuracy
accuracy = dl.logic.test_explanation(formula, target_class, x_test, y_test)
\end{lstlisting}
\end{minipage}
\end{center}

% \textbf{Unless required by applicable law or agreed to in writing, software is distributed on an "as is" basis, without warranties or conditions of any kind, either express or implied.}

\subsection{Dataset and classification task details}
\label{sec:exp_details}
We considered five categorical learning problems ranging from computer vision to medicine and democracy. Some datasets (e.g. CUB) were already annotated with high-level concepts (e.g. bird attributes) which can be exploited to train a concept bottleneck pipeline. For datasets without annotations for high-level concepts, we transformed the input space into a predicate space (i.e. $\mathbb{R}^9 \rightarrow [0,1]^d$) to make it suitable for training LENs. According to the considered data type, we will evaluate and discuss the usage of  different LEN pipelines and objectives, as already anticipated in Table~\ref{tab:datasets}).
For the sake of consistency, \sm{in all the experiments based on supervised learning criteria (Section~\ref{sec:learncrit})} LENs were trained by optimizing Eq.~\ref{eq:IFF}, therefore extracting IFF rules, \sm{that better cope with the ground truth of the datasets}. However, as already discussed in Section~\ref{sec:learncrit}, also Eq.~\ref{eq:IF} and Eq.~\ref{eq:IF2} \sm{could be considered, yielding different target rule types. In the following we describe the details of each task.}


\textsc{MIMIC-II - {\scriptsize E2E, Interpretable classification}.}
The Multiparameter Intelligent Monitoring in Intensive Care II (MIMIC-II, \cite{saeed2011multiparameter,goldberger2000physiobank}) is a public-access intensive care unit (ICU) database consisting of 32,536 subjects (with 40,426 ICU admissions) admitted to
%medical, surgical, cardiovascular and neonatal ICUs, surgical recovery units, and coronary care units
ICUs at a single tertiary care hospital. The dataset contains detailed description of a variety of clinical data classes: general,
%(e.g. patient demographics, hospital admission and discharge dates, hospital death dates, etc),
physiological, % (e.g.	nurse-verified vital signs, blood pressure, heart rate, etc),
results of clinical laboratory tests, % (e.g. hematology, blood chemistries, urinalysis, microbiology, etc),
records of medications, fluid balance, %(e.g. solutions, urine, estimated blood loss, etc),
and free text notes and reports of imaging studies (e.g. x-ray, CT, MRI, etc). In our experiments, we removed the text-based input features and
%discretize some of the continuous features into a set of categories in order to get a one-hot encoded representation. For instance,
we discretized blood pressure (BP) into five different categories (one-hot encoded): very low BP, low BP, normal BP, high BP, and very high BP. After such preprocessing step, we obtained an input space $X$ composed of $90$ key features.
The task consists in training a classifier function to identify recovering or dying patients, after 28 days from ICU admission ($Y = [0,1]^{2}$). In particular, we considered the case of
% {\bf Interpretable classification. }
\textit{interpretable classification} where an End-to-End LEN $C \rightarrow E$ is employed to \sm{directly} carry out the classification task, i.e., with $C=X$ and $E=Y$.

\textsc{MIMIC-II (EBB) - {\scriptsize E2E, Explaining a black-box model}.} On the same dataset, a second task is set up. A black-box model $g$ is employed to solve the \sm{previously described} classification task. The end-to-end LEN $f$ instead is trained to mimic the behaviour of the black box $g$, \sm{using the learning criterion of Eq.~\ref{eq:coher}.}

% \subsubsection{Concept bottleneck explainers}
% \label{sec:exp_cbm}

% \paragraph{MNIST Even/Odd}
\textsc{MNIST E/O - {\scriptsize CB, Interpretable classification}.}
The Modified National Institute of Standards and Technology database (MNIST, \cite{lecun1998mnist}) contains a large collection of images representing handwritten digits. The input space $X \subset \mathbb{R}^{28\times 28}$ is composed of 28x28 pixel images of digits \sm{from $0$ to $9$. However, the task we aim to solve is slightly different from the common digit-classification. We are interested in determining if a digit is either odd or even, and explain the assignment to one of these classes in terms of the specific digit categories from $0$ to $9$. In the notation of this paper, we can consider that each image comes with $12$ attributes, where the first $10$ ones are binary attributes about the specific digit type, i.e., from $0$ to $9$, while the last $2$ ones are binary labels that encode whether the digit is even or odd \sm{($Y=[0,1]^{12}$)}.}
\sm{We consider a concept-bottleneck pipeline that consists of a concept space $C$ that is about the attributes of the specific digit type.
We focus on the objective of 
% {\bf Interpretable classification}
\textit{interpretable classification} of the odd/even classes, so that} the mapping $X \rightarrow C$, with $C=Y^{§(1:10)}$ is learned by a ResNet10 classifier $g$ \cite{he2016deep}  trained from scratch, while a LEN $f$ is used to learn both the mapping and the explanation as a function $C \rightarrow E$, with $E=Y^{(11:12)}$.

% The $\mu$ network is equipped with a single hidden layer with 10 neurons and the $L_1$ loss weight $\lambda = 10^{-2}$.
% The $ReLU$ network is equipped with two hidden layers composed of 30, 10 hidden neurons respectively and $\lambda = 10^{-3}$.
% The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^-3$ and fan-in = 5.
% All networks have been trained for 200 epochs with learning rate = $10^ {-3}$.

\textsc{MNIST E/O (ICLU) - {\scriptsize CB, Interpretable clustering}.}
 The same dataset has been used with the objective of 
% {\bf Interpretable Clustering}
\textit{interpretable clustering}.  \sm{In this case, we considered a concept space $C = Y = [0,1]^{12}$} which comprise both the digits and the even/odd labels. The mapping $X \rightarrow C$ is learned again by a Resnet10 model $g$ trained as a multi-label classifier, while the LEN $f$ performs clustering from $C \rightarrow E$, where $E = [0,1]^{2}$ space, in order two extract two clusters \sm{that are expected to group data due to two properties of the concept space that are not-defined in advance.}
% In this case,
% the $\mu$ network is equipped with two hidden layer with 20, 10 neurons respectively and the $L_1$ loss weight $\lambda = 10^{-3}$.
% The $ReLU$ network is equipped with two hidden layers composed of 50, 30 hidden neurons and $\lambda = 10^{-4}$.
% The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^{-2}$ and fan-in = 2.
% The $\mu$ and the $ReLU$ networks have been trained for 100 epochs with learning rate = $10^{-3}$ while for the $\psi$ network is equal to $10^{-2}$.

%Quantitative results are reported in Table \ref{tab:exp_metrics_mnist_cbm} while Table \ref{tab:exp_formula_mnist_cbm} shows for each fold the explanation extracted from trained explainers.
\textsc{CUB - {\scriptsize CB, Interpretable Classification}.}
The Caltech-UCSD Birds-200-2011 dataset (CUB, \cite{wah2011caltech}) is a fine-grained classification dataset. It includes 11,788 images representing $200$ different bird species. \sm{Moreover,} 312 \sm{lower-level} binary attributes have been also attached to each image representing visual characteristics (color, pattern, shape) of particular parts (beak, wings, tail, etc.). Attributes annotations, however, is quite noisy. Similarly to \cite{koh2020concept}, we denoised attributes by considering class-level annotations, i.e. a certain attribute is set as present only if it is also present in at least 50\% of the images of the same class. Furthermore we only considered attributes present in at least 10 classes (species) after this refinement. \sm{In the end, a total of $108$ \sm{lower-level} attributes have been retained and paired with the higher-level attributes about the $200$ species, so that each image is represented with binary targets in $Y = [0,1]^{200+108=308}$ (where the first $108$ targets are for the lower-level attributes). In a concept-bottleneck pipeline with the LEN objective of \textit{interpretable classification}, 
the mapping $X \rightarrow C$ from images to lower-level concepts ($C=Y^{(1:108}$) is performed again with a ResNet10 model $g$ trained from scratch while a LEN $f$ learns the final function that classifies the  bird specie, $C \rightarrow E$, with $E=Y^{(109:308)}$.}


\textsc{V-Dem - {\scriptsize Cascading, Interpretable classification.}}
Varieties of Democracy (V-Dem, \cite{pemstein2018v,coppedge2021v}) is a dataset containing a collection of indicators of latent regime characteristics over 202 countries from 1789 to 2020. The database include $483$ low-level indicators (e.g. media bias, party ban, high-court independence, initiatives permitted, etc), $82$ mid-level indices (e.g. freedom of expression, freedom of association, equality before the law, etc), and 5 high-level indices of democracy principles (i.e. electoral, liberal, participatory, deliberative, and egalitarian). \sm{In the experiments, we considered each example to be paired with low/mid level indices and the information on electoral/non-electoral democracies taken from high level indices. Keeping the same order of the previous description, each sample is then paired with binary targets in $Y=[0,1]^{483+82+2=567}$. We considered the \textit{interpretable classification} objective in the problem of classifying electoral/non-electoral democracies in a cascading LEN with two LEN components, where $C_1=Y^{(1:483)}$, $E_1=C_2=Y^{(484:566)}$, and $E_2=Y^{(566:567)}$. In detail, cascading LENs are trained to learn the map $C_1 \rightarrow E_1$ with $E_1=C_2$ and $C_2 \rightarrow E_2$, with $E_2=Y^{(566:567)}$.}
{\color{red}I don't understand: if interpretable classification is applied to each element of the cascade stack, then we get rules out of each of the element of the stack. Are we showing them in the experiments?}

\subsection{Metrics}
\label{sec:exp_metrics}
Seven metrics are used to compare the performance of LENs with respect to state-of-the-art approaches.
While measuring classification metrics is necessary for models to be viable in practice to perform interpretable classification tasks, assessing the quality of the explanations is required to justify their use for explainability. In contrast with other kind of explanations, logic-based formulas can be evaluated quantitatively. Given a classification problem, first we extract a set of rules from a trained model and then we test/\sm{evaluate} each explanation on an unseen set of samples.
The results for each metric are reported in terms of the mean and the standard error of the mean, computed over a 10-fold cross validation \cite{krzywinski2013error}. Only in the CUB experiments a 5-fold cross validation is performed due to timing issues related to BRL (each training of BRL on CUB lasts about 3 hours)---\sm{competitors were described in Section~\ref{sec:related}.}
In particular, for each experiment we consider the following metrics.
% (1) the test accuracy of the classifier, (2) the test accuracy of the explanation, (3) the complexity of the explanation, (4) the fidelity of the explanation with respect to the classifier, (5) the elapsed time required to extract the explanations, (6) the consistency of the explanation over different runs, and (7) the normalized mutual information (for unsupervised tasks only).
% \cite{andrews1995survey}.

\begin{itemize}
\item \textsc{Model accuracy}: it measures how well \sm{the  LEN or the competitor classifier correctly identifies the target classes (Table~\ref{tab:model-accuracy}), in the case of interpretable classification.} When the LEN explains the predictions of a black box classifier, this metric represents the accuracy of the black box classifier. {\color{red}Major issue: MIMIC-II EEB is only in one of the tables below, wtf?}
\item \textsc{Explanation accuracy}: it measures how well the extracted logic formula correctly identify the target  classes (Table~\ref{tab:explanation-accuracy}).
\item \textsc{Complexity of an explanation}: it measures how hard would it be for a human being to understand the logic formula (Table~\ref{tab:complexity}). \sm{This is simulated} by standardizing the explanations in disjunctive normal form and then by counting the number of terms of the standardized formula.
\item \textsc{Fidelity of an explanation}: it measures how well the predictions obtained by applying the extracted explanations match the predictions obtained when simply  using the classifier (Table~\ref{tab:fidelity}). When the LEN is the classifier itself (i.e. interpretable classification), this metric represents the match between the extracted explanation and the LEN prediction. Instead, when the LEN is explaining the predictions of a black box classifier, this metric represents the \sm{agreement between the extracted explanation and the prediction of black box classifier.}
\item \textsc{Rule extraction \sm{time}}: it measures the time required to obtain an explanation from scratch (Fig.~\ref{fig:time}). It is computed as the sum of the time required to train the model and the time required to extract the formula from a trained model. This is justified by the fact that for some models, like BRL, training and rule extraction consist of just one simultaneous process.
\item \textsc{Consistency of an explanation}: it measures the similarity of the extracted explanations over different runs (Table~\ref{tab:consistency}). It is computed by counting how many times the same concepts appear in the logic formulas over different folds of a cross-validation or over different initialization seeds. {\color{red}How many seeds? how many runs?}
% \item The \textsc{normalized mutual information} measures the quality of the clusters obtained in the interpretable clustering experiments. It is calculated as the mutual information of Eq. \ref{eq:MI}, divided by the Entropy $H_E$ so that it reports a number always comprehended between $[0,1]$.
\end{itemize}

\begin{table}
\centering
\caption{Model accuracy (\%). The two best results are in bold.}
\label{tab:model-accuracy}
\resizebox{0.79\textwidth}{!}{\begin{tabular}{lll|lll}
\toprule
{} &              Tree &               BRL &        $\psi$ net &          ReLU net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $77.53 \pm 1.45$ &  $76.40 \pm 1.22$ &  $77.19 \pm 1.09$ &  $\bf{80.11} \pm 1.87$ &  $\bf 80.00 \pm 0.95$ \\
\textbf{vDem    } &  $85.61 \pm 0.57$ &  $\bf 91.23 \pm 0.75$ &  $89.78 \pm 1.64$ &  $\bf{92.08} \pm 0.37$ &  $90.40 \pm 0.51$ \\
\textbf{MNIST E/O} &  $99.75 \pm 0.01$ &  $99.80 \pm 0.02$ &  $99.80 \pm 0.03$ &  $\bf{99.88} \pm 0.02$ &  $\bf 99.83 \pm 0.01$ \\
\textbf{CUB     } &  $81.62 \pm 1.17$ &  $90.79 \pm 0.34$ &  $91.92 \pm 0.27$ &  $\bf{92.29} \pm 0.40$ &  $\bf 92.21 \pm 0.33$ \\
\bottomrule
\end{tabular}}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Model's accuracy (\%)}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lllllll}
% \toprule
% {} &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL & Black box \\
% \midrule
% \textbf{MIMIC-II     }  &  ${\bf 86.60 \pm 0.30}$ &  $85.36 \pm 0.78$ &  $84.01 \pm 0.09$ &  $79.56 \pm 0.80$ &  $86.15 \pm 0.51$ & N/A \\
% \textbf{MIMIC-II (EBB)}  &  N/A &  N/A &  N/A &  N/A &  N/A  & $85.13 \pm 0.70$\\
% \textbf{V-Dem         } &  $91.96 \pm 0.42$ &  $91.88 \pm 0.37$ &  $79.23 \pm 2.20$ &  $92.11 \pm 0.38$ &  ${\bf 92.23 \pm 0.38}$ & N/A \\
% \textbf{MNIST}          &  $99.75 \pm 0.02$ &  $99.81 \pm 0.01$ &  $99.80 \pm 0.01$ &  ${\bf 99.96 \pm 0.01}$ &  $99.80 \pm 0.01$ & N/A \\
% \textbf{CUB          }  &  ${\bf 92.26 \pm 0.28}$ &  $92.19 \pm 0.27$ &  $91.72 \pm 0.56$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ & N/A \\

% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}
\centering
\caption{Explanation accuracy (\%). The two best results are in bold (in case of ties in the average values, we highlighted all the involved models).}
\label{tab:explanation-accuracy}
\resizebox{0.83\textwidth}{!}{\begin{tabular}{lll|lll}
\toprule
{} &              Tree &               BRL &        $\psi$ net &          ReLU net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $69.15 \pm 2.24$ &  $\bf 70.59 \pm 2.17$ &  $49.51 \pm 3.92$ &  $70.28 \pm 1.67$ &  ${\bf 71.84 \pm 1.82}$ \\
\textbf{vDem    } &  $85.45 \pm 0.58$ &  ${\bf 91.21 \pm 0.75}$ &  $67.08 \pm 9.68$ &  $\bf 90.21 \pm 0.55$ &  $88.18 \pm 1.07$ \\
\textbf{MNIST E/O} &  $\bf 99.74 \pm 0.01$ &  ${\bf 99.79 \pm 0.02}$ &  $65.64 \pm 5.05$ &  $\bf 99.74 \pm 0.02$ &  $\bf 99.74 \pm 0.02$ \\
\textbf{CUB     } &  $89.36 \pm 0.92$ &  ${\bf 96.02 \pm 0.17}$ &  $76.10 \pm 0.56$ &  $87.96 \pm 2.81$ &  $\bf 93.69 \pm 0.27$ \\
\textbf{MIMIC-II (EBB)} &  ${\bf85.75 \pm 0.51}$ &  $81.07 \pm 3.33$ &  $83.90 \pm 1.25$ &  $85.53 \pm 0.61$ &  $\bf 85.70 \pm 0.48$ \\
\bottomrule
\end{tabular}}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Explanation's accuracy (\%)}
% \label{tab:explanation-accuracy}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $85.08 \pm 0.48$ &  $82.09 \pm 1.38$ &  $82.83 \pm 0.66$ &  $79.56 \pm 0.80$ &   ${\bf86.15 \pm 0.51}$ \\
% \textbf{MIMIC-II (EBB)} &  ${\bf85.75 \pm 0.51}$ &  $81.07 \pm 3.33$ &  $83.90 \pm 1.25$ &  $85.53 \pm 0.61$ &  $85.70 \pm 0.48$ \\
% \textbf{V-Dem         } &  $90.81 \pm 1.24$ & ${\bf94.65 \pm 0.32}$ &  $80.29 \pm 2.99$ &  $92.11 \pm 0.38$ &  $92.23 \pm 0.38$ \\
% \textbf{MNIST}         &  $99.67 \pm 0.01$ &  $98.04 \pm 1.60$ &  $75.47 \pm 0.46$ &  ${\bf99.96 \pm 0.01}$  &  $99.80 \pm 0.01$ \\
% \textbf{CUB*         } &  ${\bf96.15 \pm 0.16}$ &  $93.98 \pm 1.97$ &  $80.41 \pm 2.31$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ \\

% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}
\centering
\caption{Complexity of explanations. The two best results are in bold.}
\label{tab:complexity}
\resizebox{0.86\textwidth}{!}{\begin{tabular}{lll|lll}
\toprule
{} &              Tree &                   BRL &         $\psi$ net &           ReLU net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $66.60 \pm 1.45$ &     $57.70 \pm 35.58$ &   $\bf 20.60 \pm 5.36$ &  $39.50 \pm 11.62$ &  ${\bf 15.80 \pm 1.37}$ \\
\textbf{vDem    } &  $30.20 \pm 1.20$ &    $145.70 \pm 57.93$ &    ${\bf 5.40 \pm 2.70}$ &   $18.40 \pm 2.17$ &   $\bf 9.10 \pm 0.94$ \\
\textbf{MNIST E/O} &  ${\bf 47.50 \pm 0.72}$ &  $1352.30 \pm 292.62$ &  $96.90 \pm 10.01$ &   $\bf 73.30 \pm 5.77$ &  $80.50 \pm 4.85$ \\
\textbf{CUB     } &  $45.92 \pm 1.16$ &       ${\bf 8.87 \pm 0.11}$ &   $15.96 \pm 0.96$ &   $60.57 \pm 6.95$ &  $\bf 14.65 \pm 0.16$ \\
\bottomrule
\end{tabular}}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Complexity}
% \label{tab:complexity}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {}                     &        $\mu$ net &         ReLU net &       $\psi$ net &                 Tree &               BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $5.10 \pm 0.35$ &  $23.40 \pm 11.20$ &  ${\bf2.60 \pm 0.16}$ &  $1342.60 \pm 16.94$ &  $20.70 \pm 4.08$ \\
% \textbf{MIMIC-II (EBB)} &  $7.00 \pm 0.70$ &    $6.40 \pm 0.95$ &  ${\bf1.30 \pm 0.15}$ &   $432.10 \pm 16.46$ &  $22.90 \pm 4.13$ \\
% \textbf{V-Dem         } &  $9.60 \pm 1.17$ &    $4.90 \pm 0.10$ &  ${\bf2.00 \pm 0.49}$ &    $294.10 \pm 7.88$ &   $8.70 \pm 0.97$ \\
% \textbf{MNIST}         &  ${\bf22.00 \pm 4.67}$ &  $48.10 \pm 1.43$ &  $24.85 \pm 2.89$ &  $632.35 \pm 5.01$ &  $1291.05 \pm 234.40$ \\
% \textbf{CUB          } &  $10.53 \pm 0.08$ &  $29.25 \pm 3.26$ &  $28.36 \pm 2.75$ &  $138.83 \pm 5.31$ &  ${\bf4.10 \pm 0.09}$ \\


% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}
\centering
\caption{Fidelity of explanations (\%). Tree and BRL trivially get 100\%. We highlighted in bold the best LEN model.}
\label{tab:fidelity}
\resizebox{0.82\textwidth}{!}{\begin{tabular}{lll|lll}
\toprule
{} &               Tree &                BRL &         $\psi$ net &          ReLU net &         $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &   $51.63 \pm 6.68$ &  $75.62 \pm 2.07$ &  $\bf 88.37 \pm 2.73$ \\
\textbf{vDem    } &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &  $69.67 \pm 10.43$ &  $\bf 96.36 \pm 0.64$ &  $94.73 \pm 2.16$ \\
\textbf{MNIST E/O} &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &   $65.68 \pm 5.05$ &  $\bf 99.85 \pm 0.02$ &  $99.83 \pm 0.02$ \\
\textbf{CUB     } &  $100.00 \pm 0.00$ &  $100.00 \pm 0.00$ &   $77.34 \pm 0.52$ &  $89.28 \pm 2.90$ &  $\bf 95.21 \pm 0.25$ \\
\bottomrule
\end{tabular}}
\end{table}


% \begin{table}[!h]
% \centering
% \caption{Fidelity (\%)}
% \label{tab:fidelity}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $96.23 \pm 0.81$ &  $87.84 \pm 2.12$ &  $84.63 \pm 0.67$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
% \textbf{MIMIC-II (EBB)} &  $92.28 \pm 0.90$ &  $86.58 \pm 4.00$ &  $90.32 \pm 1.27$ &   $93.07 \pm 0.53$ &   ${\bf94.82 \pm 0.50}$ \\
% \textbf{V-Dem         } &  $91.52 \pm 1.13$ &  $94.62 \pm 0.37$ &  $82.45 \pm 1.80$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
% \textbf{MNIST}         &  $99.90 \pm 0.03$ &  $98.14 \pm 1.60$ &  $75.53 \pm 0.46$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
% \textbf{CUB*         } &  $97.82 \pm 0.15$ &  $95.37 \pm 2.06$ &  $81.89 \pm 2.35$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\

% \bottomrule
% \end{tabular}
% }
% \end{table}

\iffalse
\begin{table}
\centering
\caption{Rule extraction time (seconds). The two best results are in bold.}
\label{tab:extraction}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{lll|lll}
\toprule
{} &             Tree &                       BRL &             $\psi$ net &            ReLU net &             $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $\bf 0.06 \pm 0.00$ &         $440.24 \pm 9.75$ &       $\bf 36.69 \pm 6.11$ &    $87.51 \pm 8.44$ &      $44.22 \pm 3.38$ \\
\textbf{vDem    } &  $\bf 0.49 \pm 0.07$ &     $22843.21 \pm 194.49$ &       $49.27 \pm 1.13$ &    $\bf 47.41 \pm 5.94$ &     $100.96 \pm 4.42$ \\
\textbf{MNIST E/O} &  $\bf 2.72 \pm 0.02$ &      $2594.79 \pm 177.34$ &     $\bf 385.58 \pm 17.82$ &  $907.18 \pm 67.75$ &     $414.21 \pm 7.48$ \\
\textbf{CUB     } &  $\bf 8.11 \pm 0.65$ &  $264678.29 \pm 56521.40$ &  $3707.29 \pm 1006.54$ &  $\bf 305.19 \pm 30.42$ &  $1173.87 \pm 146.42$ \\
\bottomrule
\end{tabular}}
\end{table}
\fi

% \begin{table}[!h]
% \centering
% \caption{Rule extraction time (s)}
% \label{tab:extraction}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {} &        $\mu$ net &         ReLU net &       $\psi$ net &             Tree &              BRL \\
% \midrule
% \textbf{MIMIC-II     } &  $13.32 \pm 0.30$ &  $266.22 \pm 166.90$ &   $8.81 \pm 0.15$ &  ${\bf0.02 \pm 0.00}$ &  $495.59 \pm 7.13$ \\
% \textbf{MIMIC-II (EBB)} &  $15.30 \pm 0.19$ &     $18.46 \pm 1.00$ &  $10.14 \pm 0.03$ &  ${\bf0.01 \pm 0.00}$ &  $543.43 \pm 3.39$ \\
% \textbf{V-Dem         } &  $34.40 \pm 0.78$ &     $34.24 \pm 0.32$ &  $20.83 \pm 0.04$ &  ${\bf0.06 \pm 0.00}$ &   $53.69 \pm 0.41$ \\
% \textbf{MNIST}         &  $173.24 \pm 6.77$ &  $221.07 \pm 4.06$ &  $236.71 \pm 3.36$ &  ${\bf2.04 \pm 0.04}$ &  $836.14 \pm 3.15$ \\
% \textbf{CUB          } &  $726.19 \pm 2.43$ &  $660.30 \pm 121.16$ &  $2094.49 \pm 730.50$ &  ${\bf4.17 \pm 0.07}$ &  $9863.52 \pm 147.57$ \\

% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=.8\textwidth,trim=0 15 0 0,clip]{figs/elapsed_time_plot.pdf}
    \caption{Rule extraction time (seconds). Time required to train models and to extract the explanations. Our models compare favorably with the competitors, with the exception of Decision Trees. BRL is by one to three order of magnitude slower than our approaches. Error bars show the 95\% confidence interval of the mean.}
    \label{fig:time}
\end{figure}


\begin{table}
\centering
\caption{Rule consistency (\%).}
\label{tab:consistency}
\resizebox{0.55\textwidth}{!}{\begin{tabular}{lll|lll}
\toprule
{} &     Tree &       BRL & $\psi$ net &  ReLU net & $\mu$ net \\
\midrule
\textbf{MIMIC-II} &  $40.49$ &   $30.48$ &    $27.62$ &   $53.75$ &   $71.43$ \\
\textbf{vDem    } &  $72.00$ &   $73.33$ &    $38.00$ &   $64.62$ &   $41.67$ \\
\textbf{MNIST E/O} &  $41.67$ &  $100.00$ &    $96.00$ &  $100.00$ &  $100.00$ \\
\textbf{CUB     } &  $21.47$ &   $42.86$ &    $41.43$ &   $44.17$ &   $76.92$ \\
\bottomrule
\end{tabular}}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Rule consistency (\%)}
% \label{tab:consistency}
% \begin{tabular}{llllll}
% \toprule
% {} & $\mu$ net & ReLU net & $\psi$ net &     Tree &      BRL \\
% \midrule
% \textbf{MIMIC-II     } &   $51.00$ &  $26.00$ &    $37.14$ &  ${\bf81.50}$ &  $28.33$ \\
% \textbf{MIMIC-II (EBB)} &   $41.18$ &  $35.56$ &    $43.33$ &  ${\bf60.36}$ &  $22.22$ \\
% \textbf{V-Dem         }&   $71.67$ &  ${\bf98.00}$ &    $15.83$ &  $36.86$ &  $76.25$ \\
% \textbf{MNIST}         &   $60.00$ &  ${\bf100.00}$ &    $50.00$ &  $50.95$ &  ${\bf100.00}$ \\
% \textbf{CUB          } &   ${\bf58.82}$ &  $58.40$ &    $43.08$ &  $21.79$ &  $30.00$ \\
% \bottomrule
% \end{tabular}
% \end{table}


\subsection{Results and discussion}
% \textsc{Interpretable classification. }
\sm{Our results are organized in order to compare the behaviour of the models in all the considered tasks jointly, with the exception of interpretable clustering, that will be discussed in a separate manner.}
Experiments of Table~\ref{tab:model-accuracy} show how \sm{all the considered out-of-the-box LENs} generalize better than decision trees on complex boolean functions (e.g. CUB and MIMIC-II) as expected \cite{tavares2020understanding}\sm{, and they also usually overcome BRL. LENs based on ReLU networks are definitely the ones with better classification accuracy, confirming the intuitions reported in Section~\ref{subsec:ReLU}, that, however, are not far from $\mu$ nets.}
These results must be paired with the ones of Table~\ref{tab:explanation-accuracy}, since having large classification performance and very low explanation quality would represent a major issue. 
For most experiments the formulas extracted from LENs are either better or almost as accurate as the formulas found by decision trees or mined by BRL, \sm{even if the top-performance are about BRL. What makes the LEN result preferable to the one of BRL is the significantly better (reduced) complexity of the considered explanations, as shown in Table~\ref{tab:complexity}. Notice that less complex rules implies more readable formulas, that is a crucial feature in the context of Explainable AI.} More specifically, the complexity of LEN explanations is usually lower than the complexity of the rules extracted both from a decision tree or mined by BRL. The complexity of decision tree formulas is never below 100 terms, making them useless for quick decision making. \sm{Comparing the results of the different out-of-the-box LENs, we observe that $\psi$ networks yield moderately complex explanations, sometimes with limited accuracy, while ReLUs, due to the variability of example-level rules, lead to more complex explanations. Overall, the case of $\mu$ networks is the most attractive one, confirming the quality of their parsimony/pruning criteria.}

\sm{Moving to more fine-grained details, Table~\ref{tab:fidelity} show how white-box models, like decision trees and BRL, outperform LENs in terms of fidelity. This is due to the fact that such models make predictions that are specifically based on the explanation they provide, therefore fidelity is (trivially)} always 100\%. However, we see how the fidelity of the formulas extracted by the $\mu$ and the ReLU network is often higher than $90\%$. This means that almost any prediction has been correctly explained, making these networks very close to white boxes. Fig.~\ref{fig:time} compares the rule extraction times. BRL is the slowest rule extractor over all the experiments, and LENs are faster by one to three orders of magnitude. Decision trees are the fastest overall. In terms of consistency, Table~\ref{tab:consistency}, there is not a dominant method, while we can see how this result is clearly impacted by the considered dataset/task. \sm{Our intuition is that those datasets that are more coherently represented by the data in the different folds are of course expected to lead to more consistent behaviours.}

Fig.~\ref{fig:multi-objective} shows \sm{a combined view of two of the main metrics considered so far, reporting} the Pareto frontiers \cite{marler2004survey} for each experiment in terms of the complexity of the explanation and its classification error ($100$ minus the model accuracy). 
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.32\textwidth]{figs/mimic.pdf}
    \includegraphics[width=0.32\textwidth]{figs/mimic_explain_classifier.pdf}
    \includegraphics[width=0.32\textwidth]{figs/mnist.pdf}\\
    \includegraphics[width=0.32\textwidth]{figs/cub.pdf}
    \includegraphics[width=0.32\textwidth]{figs/vDem.pdf}
    \\
    \includegraphics[width=0.7\textwidth]{figs/legend.pdf}
    \\
    \caption{Pareto frontiers (dotted black line) in terms of average test error and average complexity of the explanations. The vertical dotted red line marks the maximum explanation complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). {\color{red}Rename MNIST in MNIST E/O. Rename MIMIC-II (explain classifier) in MIMIC-II (EBB). Replace crosses with circles in MIMIC-II(explain classifier), and remove the x-label. The y-label of MNIST is partially cut off!}}
    \label{fig:multi-objective}
\end{figure}
{\color{red}The simplest and most accurate formulas are found by the LENs, whose complexity is frequently below the maximum complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Across all the experiments, there is at least one set of formulas extracted from out-of-the-box LEN dominating both BRL and decision trees. I CANNOT READ THESE COMMENTS WHEN LOOKING AT THE PICTURES. WTF?}

\sm{Our experimental analysis quantitatively demonstrates the quality of LENs and of the FOL rules they extract. In order to provide the reader also a qualitative view on the type of rules that get extracted by the compared models, 
 Table~\ref{tab:best-rules} reports a representative subset of the formula over the different tasks. Comparing the LEN models, we can appreciate the compactness of rules coming from the {\color{red}$\mu$} network. All the LEN-rules are way more compact than the ones from Tree, and usually also the ones from BRL.}


\sm{A separate investigation is dedicated to the interpretable clustering objective in MNIST E/O (ICLU). Of course, competitors are not involved into this experience, since they only operate in a supervised manner, while LENs can also handle the unsupervised discovery of FOL formulas.}
%As introduced in the MNIST E/O dataset explanation we performed clustering starting from a Concept space composed of the 10 digits and the even/odd labels. T
LENs are instructed two \sm{develop} two clusters considering the data represented in the concept space where the digit identity and the property of being even/odd are encoded. \sm{Of course, we want to evaluate whether LEN can discover that data can be grouped into two balanced clusters of even and odd digits, and to provide explanations of them (such as, \textit{odd and not  even} and \textit{odd and not even}). We remark that this task does not use any supervisions, and we recall that the LEN does not know that odd/even are mutually exclusive properties, but they are just two input concepts out of 12.} In Table \ref{tab:exp_metrics_mnist_mi}, \sm{all the previously introduced metrics are reported for this task, with the exception of the model accuracy (since no supervision is available), that is replace by the Mutual Information index that is at the basis of the learning criterion (Section~\ref{sec:learncrit})}. 
\begin{table}[!h]
\centering
\caption{MNIST E/O (ICLU). All the metrics are reported, with the model accuracy replace with the (normalized) Mutual Information (MI) rescaled in $[0,100]$.}
\label{tab:exp_metrics_mnist_mi}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
     Method & \sm{MI} & Exp. accuracy (\%) &       Complexity & Extraction time (sec) & Rule consistency (\%) \\
\midrule
 $\psi$  net &     $99.90 \pm 0.01$ &           $99.90 \pm 0.01$ &  $2.00 \pm 0.00$ &     $0.33 \pm 0.15$ &             $100.00$ \\
 $\mu$ net &     $94.91 \pm 4.99$ &           $95.41 \pm 4.50$ &  $2.30 \pm 0.64$ &     $2.36 \pm 0.75$ &              $35.00$ \\
   ReLU net &     $96.87 \pm 3.04$ &           $95.97 \pm 3.94$ &  $2.15 \pm 0.39$ &     $4.15 \pm 1.62$ &              $45.00$ \\
\bottomrule
\end{tabular}
}
\end{table}
We can see that all methods are capable of almost fully maximizing the (normalized) \sm{mutual information}. \sm{We inspected the rules, and we saw that while all the LENs correctly consider odd and even as predicates that participates to the FOL rules,  only the} $\psi$ network consistently explains the two clusters in terms of only such important labels (even and odd), as we can see from the complexity of the rules (that is higher than 2 for the $\mu$ network and ReLU net) and for the consistency of terms used in the explanation ($100\%$ for the $\psi$ network).
Other examples and application of interpretable clustering have been performed in \cite{ciravegna2020constraint, ciravegna2020human} employing the $\psi$ network only.

% \subsection{Other experiences}

% \textsc{Explanation as a defense}















% \subsection{Rules Extracted}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
{\renewcommand{\arraystretch}{1.5}
\begin{table}[!h]
\centering
\caption{A selection of some of the best rules extracted for each experiment. {\color{red}Non e' che $\mu$ e $\psi$ sono invertite?}}
\label{tab:best-rules}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
\multicolumn{1}{l}{\textbf{Dataset}}    & \textbf{Model}  & \textbf{Rule} \\ \hline
\multirow{5}{*}{MIMIC-II}      & $\mu$ net  & $Death \leftarrow \makecell[l]{stroke \wedge age\_HIGH  \wedge \neg atrial\_fibrillation} $  \\
                               & ReLU net   & $Death \leftarrow \makecell[l]{stroke \wedge age\_HIGH \wedge \neg atrial\_fibrillation \wedge \neg sapsi\_first\_LOW \wedge \neg sapsi\_first\_HIGH} $  \\
                               & $\psi$ net & $Death \leftarrow stroke \vee bun\_first\_NORMAL \vee sapsi\_first\_HIGH $  \\
                               & Tree       & $Death \leftarrow \quad ^*$formula is too long (1000+ terms) \\
                               & BRL        & $Death \leftarrow \makecell[l]{(stroke \wedge resp \wedge \neg age\_LOW \wedge \neg sapsi\_first\_LOW) \\
                               \vee (stroke  \wedge age\_HIGH \wedge \neg age\_LOW  \wedge  \neg sapsi\_first\_LOW) }$  \\ \hline
\multirow{5}{*}{MIMIC-II (EBB)} & $\mu$ net  & $Death \leftarrow atrial_fibrillation \wedge stroke \wedge \neg sapsi\_first\_HIGH \wedge \neg weight\_first\_NORMAL $  \\
                               & ReLU net   & $Death \leftarrow stroke \wedge \neg sapsi\_first\_LOW  \wedge  \neg sapsi\_first\_HIGH \wedge \neg sodium\_first\_LOW $  \\
                               & $\psi$ net & $Death \leftarrow stroke \wedge age\_HIGH $  \\
                               & Tree       & $Death \leftarrow  \quad ^*$formula is too long (100+ terms)  \\
                               & BRL        & $Death \leftarrow \makecell[l]{stroke \wedge age\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW) \\ \vee  (stroke \wedge platelet\_first\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW } $  \\  \hline
\multirow{5}{*}{MNIST}         & $\mu$ net  & $Even \leftarrow \neg One \wedge \neg Three \wedge \neg Five \wedge \neg Seven \wedge \neg Nine $  \\
                              & ReLU net   & $Even \leftarrow \makecell[l]{(Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Two \wedge \neg Zero \wedge \neg One \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Four \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Six \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Eight \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Nine) } $ \\
                              & $\psi$ net & $Even \leftarrow \makecell[l]{(Six \wedge Zero \wedge \neg One \wedge \neg Seven)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Three)  \\
                              \vee (Six \wedge Zero \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge \neg One \wedge \neg Seven \wedge \neg Three) \\
                              \vee (Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)}$  \\
                              & Tree       & $Even \leftarrow \quad ^*$formula is too long \\
                              & BRL        & $Even \leftarrow  \makecell[l]{(Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two)) \vee (Eight \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two))
                              \\ \vee (Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Seven \wedge \neg Two)) \\
                              \vee (Two \wedge \neg One \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \\ \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two)) \\
                              \vee (Four \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \\ \wedge  \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One)) \\
                              \vee (Zero \wedge \neg Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \\
                              \wedge \neg (Nine \wedge \neg Zero) \wedge \neg (One \wedge \neg Two) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One))
                              }$  \\ \hline
\multirow{5}{*}{CUB}          & $\mu$ net  & $ Black\ foot\ albatross \leftarrow \makecell[l]{  bill \ shape \ hooked \ seabird \ \wedge \  size \ medium \wedge \ wing \ pattern \ solid \\
                              \wedge \neg wing color \ black \wedge \neg  underparts\ color\ white \wedge \neg upper\ tail\ color\ grey \\
                              \wedge \neg breast\ color\ white \wedge \neg  throat\ color\ white \wedge \neg tail\ pattern\ solid \wedge \neg  crown\ color\ white} $  \\
                              & ReLU net   & $ Black\ foot\ albatross \leftarrow  \makecell[l]{ size\  medium  \wedge \neg  bill\  shape\  allpurpose  \\
                              \wedge \neg  upperparts\  color\  black  \wedge \neg  head\  pattern\  plain  \wedge \neg  under\  tail\  color\  yellow \\  \wedge \neg  under\  tail\  color\  black  \wedge \neg  nape\  color\  buff  \\
                              \wedge \neg  wing\  shape\  roundedwings  \wedge \neg  shape\  perchinglike  \\
                              \wedge \neg  leg\  color\  grey  \wedge \neg  leg\  color\  black  \wedge \neg  bill\  color\  grey  \\
                              \wedge \neg  bill\  color\  black  \wedge \neg  wing\  pattern\  multicolored }$\\
                              & $\psi$ net & $ Black\ foot\ albatross \leftarrow  \makecell[l]{(bill \ shape \ hooked\ seabird \wedge tail \ pattern \ solid \wedge \neg underparts \ color \ white \\
                              \wedge ( \neg  \ breast \ color \ white \vee \neg   \ wing \ color \ grey)) }$  \\
                              & Tree       & $ Black\ foot\ albatross \leftarrow  ^*$formula is too long (1000+ terms)  \\
                              & BRL        & $ Black\ foot\ albatross \leftarrow  \makecell[l]{( bill\  shape\  hooked\  seabird \wedge forehead\ color\ blue \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white) \\
                              \vee ( bill\  shape\  hooked\  seabird \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white \wedge  \neg  tail\  pattern\  solid)}$ \\
\hline
\multirow{5}{*}{V-Dem}         & $\mu$ net  & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & ReLU net   & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & $\psi$ net & $Elect\_ Dem \leftarrow v2x\_frassoc\_thick \wedge v2xeg\_eqaccess $  \\
                               & Tree       & $Elect\_ Dem \leftarrow \quad ^*$formula is too long (1000+ terms)  \\
                               & BRL        & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\ \hline
\end{tabular}%
}
\end{table}}



% These challenging or product-oriented contexts are the actual targets of XAI research. This great research effort have produced a variety of quite interesting and efficient approaches to unveil the decision process of black-box models. Some of the most common taxonomies are based on a few discriminative criteria (intrinsic interpretability VS post-hoc, model-specific VS model-agnostic, local VS global explanations), but the most important characteristic, i.e. the \textit{form} of the explanation, is often overlooked.

% include white-box models, model-agnostic approaches \cite{ribeiro2016model} and example-based explanations \cite{aamodt1994case,kim2016examples,barbiero2020uncovering}.


% decision trees \cite{breiman1984classification}, or decision rules: oneR \cite{holte1993very}, RIPPER \cite{cohen1995fast}, Bayesian Rule Lists \cite{letham2015interpretable}).

% \begin{itemize}
%     \item many interesting works around explainability, from fully interpretable models (LR, DT, DR), to surrogates (LIME, Anchors, SHAP, etc) to example-based
%     \item great effort on scoring/ranking features/concepts
%     \item that's NOT the whole point
%     \item what matters (even more?) is how concepts are related (PDP? mah...)
%     \item what is the effort for the end user for analyzing a pairwise dependence plot or a ranking or a decision tree with depth 5?
%     \item good explanations must be simple
%     \item simple <-> few concepts involved? well yes, but...
%     \item traditional methods tend to assume: simplicity -> simple relationships among concepts (linear, max PDP)
%     \item we argue: why??
% \end{itemize}

% % -idee generali su che tipo di bestie c'è per fare expl..
% % -s'è già detto che i sistemi a regole sono più utili per fare supporto a umani.. che robe c'è in giro, perchè il nostro è più fiho
% % - il survey congnitivo dice che regole buone devono essere semplici.. -> pruning! che tipi di pruning usa sta gente che fa expl?

% What Is an Explanation? An explanation is the answer to a why-question (Miller 2017).


% to mention: (Bayesian Rule Lists: \cite{letham2015interpretable} tipo decision trees)

% \begin{itemize}
%     \item taxonomy
%     \begin{itemize}
%         \item intrinsic or post-hoc? LENs support both!
%         \item result of the interpretation:
%         \begin{itemize}
%             \item Feature summary statistic (feature importance or pairwise feature interactions or rank visualization)
%             \item Model internals (weights in linear models or the learned tree structure)
%             \item Data point (counterfactual explanations or identification of prototypes of predicted classes)
%             \item Intrinsically interpretable model
%         \end{itemize}
%         \item Model-specific or model-agnostic?
%         \item Local or global?
%     \end{itemize}
%     \item Properties of Explanation Methods
%     \begin{itemize}
%         \item Expressive Power is the "language" or structure of the explanations (IF-THEN rules, decision trees, a weighted sum, natural language or something else)
%         \item Translucency describes how much the explanation method relies on looking into the machine learning model
%         \item Portability
%         \item Algorithmic Complexity
%     \end{itemize}
%     \item Properties of Individual Explanations
%     \begin{itemize}
%         \item Accuracy: How well does an explanation predict unseen data?
%         \item Fidelity: How well does the explanation approximate the prediction of the black box model?
%         \item Consistency: How much does an explanation differ between models that have been trained on the same task and that produce similar predictions?
%         \item Stability: How similar are the explanations for similar instances?
%         \item Comprehensibility: How well do humans understand the explanations?
%         \item Certainty: Does the explanation reflect the certainty of the machine learning model?
%         \item Degree of Importance: How well does the explanation reflect the importance of features or parts of the explanation?
%         \item Novelty: Does the explanation reflect whether a data instance to be explained comes from a "new" region far removed from the distribution of training data?
%         \item Representativeness: How many instances does an explanation cover?
%     \end{itemize}
%     \item good explanations
%     \begin{itemize}
%         \item Explanations are contrastive (Lipton 1990)
%         \item Explanations are selected (simple)
%         \item Explanations are social. They are part of a conversation
%         \item Explanations focus on the abnormal. People focus more on abnormal causes to explain events (Kahnemann and Tversky, 1981).
%         \item Explanations are truthful. Good explanations prove to be true in reality
%         \item Good explanations are consistent with prior beliefs of the explainee
%         \item Good explanations are general
%     \end{itemize}
%     \item interpretable models: logistic regression, decision trees, decision rules and the RuleFit algorithm
%     \item model agnostic:
%     \begin{itemize}
%         \item plots: Accumulated local effects, Partial Dependence Plot, Individual Conditional Expectation
%         \item surrogates: Global Surrogate, Local Surrogate (LIME), \textbf{Scoped Rules (Anchors)} (many scenarios require discretization, many calls to the ML model), \textbf{SHAP} (SHapley Additive exPlanations)
%     \end{itemize}
%     \item example based: Counterfactual explanations, Prototypes
%     \item neural networks: Feature Visualization, Concepts, Modell Distillation (How can we explain a neural network with a simpler model?)
% \end{itemize}

% \paragraph{Occam's razors}
% In his Posterior Analytics, Aristotle stated: "We may assume the superiority ceteris paribus [other things being equal] of the demonstration which derives from fewer postulates or hypotheses" \cite{aristotlePosterior}. The \textit{law of parsimony} presented by the Greek philosopher has deeply influenced researchers and scientists across the centuries. In other words, when humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one. Researchers have proposed many approaches to integrate this parsimony principle into learning machines over the years. Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous approaches. Among such techniques, $L1$-regularization \cite{santosa1986linear,tibshirani1996regression} has been recently shown quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages sparsity by shrinking the less important weight's values to zero thus removing some weights altogether in the limit. Following \cite{ciravegna2020human}, the models analyzed in this work are mainly based on $L1$-regularization. However, in future works it may also worth exploring the integration of LENs with concept-based parsimony criteria \cite{chen2020concept} or with fuzzy-logic regularizers which have recently been used to combine deductive reasoning and human priors with deep learning \cite{marra2019lyrics}.





\draft{
\subsection{LENs as Adversarial Defense}\label{sec:LEN4adv_att}
In nowadays machine learning literature, there is a serious concerns about the vulnerability of several machine learning models, such as neural networks, to the so called \textit{adversarial examples}, input samples that are maliciously altered with a slight perturbation that may lead to wrong predictions, even if they do not look to be visually altered for a human (in the case of images). This kind of issue has received a lot of attention, and several work has been done to develop some techniques, \textit{adversarial defenses}, to prevent an AI model from fraudulent \textit{adversarial attacks} \cite{miller2020adversarial,ozdag2018adversarial}.
Recently, it has been shown how explicit domain knowledge, expressed by a set of FOL formulas, can be used to discriminate if a certain sample has to be considered as adversarial \cite{melacci2020domain}, especially in case of multi-label classification. 
%
However this approach requires that the logic rules are already available for the considered task, so that a domain expert is expected to collect them.}
%

Interestingly, LENs can be applied to a set of clean data to automatically learn a set of FOL rules that may capture the important properties of the target domain. Then, these rules can be used to detect adversarial samples as in the framework introduced in \cite{melacci2020domain}, since they are exactly of the same type of the LEN ones.
% The explanations provided by LENs are first-order logic formulas, and this newly devised pieces of knowledge can be reused and enforced on the output of the classifier $g$. This is commonly considered in the generic \emph{learning from constraints} framework \cite{gnecco2015foundations}, and it may be of particular interest, especially for semi-supervised settings. A similar strategy has already been considered e.g. in \cite{ciravegna2020constraint}, where a set of FOL formulas have been, at first extracted from data, and then converted into continuous loss functions to be injected in the learning objective.
% Furthermore, the extracted formulas can also be used to check the behaviour of the classifier on test data, e.g. to detect adversarial samples as done in \cite{melacci2020domain}.
\sm{Without any attempts of being exhausting on this topic, we briefly explored whether what we stated in the previous sentence would work in practice. We considered the bird-identification dataset (CUB 200), facing the classification problem in its original multi-label fashion, where a convolutional neural network $g$ (ResNet18) is trained from scratch to classify both the 200 classes and the ones of the additional bird attributes. With the goal of making $g$ capable of rejecting adversarial examples, {\color{red}we plugged a LEN on top of it (concept-bottleneck) with the objective of interpretable clustering}, with {\color{red}$E=[0,1]^{?}$}, thus extracting {\color{red}$?$} FOL formulas with the discovered relationships among the CUB classes. These formulas are directly plugged in the rejection mechanism of \cite{melacci2020domain}, thus making $g$ equipped with a rejection function. Following \cite{melacci2020domain}, we fixed the adversarial perturbation {\color{red}upper-bound to $\epsilon=?$}, and {\color{red}we augmented the test data with ? adversarial examples} generated with {\color{red} the white-box not-domain-knowledge aware multi-label attack of \cite{melacci2020domain}}, measuring the adversarial-aware accuracy used in such a paper, that here we refer to as robust accuracy.}
The experimental results for the three out-of-the-box LENs introduced in Section \ref{sec:outofthebox} are shown in Fig.~\ref{fig:adv_def}.
\sm{Interestingly, the accuracy of the attacked $g$ classifier increases in a significant manner using the rules extracted by LENs, confirming the validity of the proposed approach. The ReLU net leads to more detailed rules that better defend $g$, even if they introduce a larger computational burden in the defense mechanism, since they are usually more complex that the ones of the $\mu$ net.}


%
\begin{figure}[!ht]
    \centering
    \includegraphics[width=.42\textwidth]{figs/cub_adv_plot.pdf}
    \caption{Quality of the explanations extracted by the LENs in terms of robust accuracy when used to defend a model \sm{from adversarial examples}. In pink, the accuracy of the model when facing a white box attack without any defense. Error bars show the 95\% confidence interval of the mean. }
    \label{fig:adv_def}
\end{figure}




\section{Conclusions and Future Work} 
\label{sec:conclusion}

\sm{In this paper we presented the framework of Logic Explained Networks (LENs), presenting an in-depth study on the idea of using a neural model either to provide explanations for an existing one or for directly facing a classification problem in an interpretable manner. Explanations are provided by First-Order Logic formulas, whose type is strongly interconnected with the learning criterion that drives the development of LENs. Our framework covers a large set of computational pipelines and different user objectives, and we investigated and experimented the case of three out-of-the-box LEN models, showing that they represent a balanced trade-off among a set of important properties, comparing favourably with state-of-the art white box classifiers.}

The extraction of a first-order logic explanation requires symbolic input and output spaces. This constraint is the main limitation of our framework, as narrows the range of applications down to symbolic I/O problems. In some contexts, such as computer vision, the use of LENs may require additional annotations and attribute labels to get a consistent symbolic layer of concepts. However, recent work may partially solve this issue leading to more cost-effective concept annotations \cite{ghorbani2019towards,kazhdan2020now}.
%
Another area to focus on might be the improvement of out-of-the-box LENs. The efficiency and the classification performances of fully interpretable LENs, i.e. $\psi$ network, is still quite limited due to the extreme pruning strategy. Even more flexible approaches, like $\mu$ networks, are not as efficient as standard neural models when tackling multi-class or multi-label classification problems, as they require a bigger architecture to provide a disentangled explanation for each class.
%
In our vision this framework would thrive and express its full potential by interacting with the external world and especially with humans in a dynamic way. In this case, logic formulas might be rewritten as sentences to allow for a more natural interaction with end users. Moreover, a dynamic interaction may call for an extended expressivity leading to higher-order or temporal logic explanations. Finally, in some contexts different neural architectures as graph neural networks might be worth exploring as they may be more suitable to solve the classification problem.


Current legislation in US and Europe binds AI to provide explanations especially when the economical, ethical, or financial impact is significant \cite{gdpr2017,law10code}. This work contributes to a lawful and safer adoption of some of the most powerful AI technologies allowing deep neural networks to have a greater impact on society. %Extracting first-order logic explanations from deep neural networks enables satisficing knowledge distillation while achieving performances comparable with the state of the art. 
The formal language of logic provides clear and synthetic explanations, suitable for laypeople, managers, and in general for decision makers outside the AI research field.
%
The experiments show how this framework can be used to aid bias identification and to make black boxes more robust to adversarial attacks. % by giving an explanation for the attack itself.
As out-of-the-box LENs are easy to use even for neophytes and can be effectively used to understand the behavior of an existing algorithm, our approach might be used to reverse engineer competitor products, to find vulnerabilities, or to improve system design. From a scientific perspective, formal knowledge distillation from state-of-the-art networks may enable scientific discoveries or confirmation of existing theories.


\section*{Acknowledgments}

{\color{red}This work was partially supported by the European Union’s Horizon 2020 research and innovation programme under grant agreement No 848077.}

This work was partially supported by the PRIN 2017 project RexLearn (Reliable and Explainable Adversarial Machine Learning), funded by the Italian Ministry of Education, University and Research (grant no. 2017TWNMH2)




\bibliographystyle{apalike}  % Sry Pietro, just had to
\bibliography{references}  %%% Remove comment to use the external .bib file (using bibtex).
%%% and comment out the ``thebibliography'' section.

\end{document}


==> main_old.tex <==

% \usepackage{icml2021}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[pagebackref=true,
    breaklinks=true,
    colorlinks,
    linkcolor=blue,
    citecolor=blue,
    filecolor=black,
    urlcolor=blue,
    bookmarks=false]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{caption}
\usepackage{subcaption}

\usepackage{physics}
\usepackage{amsmath}
\usepackage{tikz}
\usepackage{mathdots}
\usepackage{yhmath}
\usepackage{cancel}
\usepackage{color}
\usepackage{siunitx}
\usepackage{array}
\usepackage{multirow}
\usepackage{amssymb}
\usepackage{gensymb}
\usepackage{tabularx}
\usepackage{booktabs}
\usetikzlibrary{fadings}
\usetikzlibrary{patterns}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{shapes}


\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

\usepackage{pifont}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{float}
\usepackage{fontawesome}
\usepackage{makecell}

\def\UrlFont{\rmfamily}
\usepackage{fancyhdr}
\usepackage{mathrsfs} 
\usepackage{color}
\usepackage{hyperref}
\usepackage{longtable}
\hypersetup{colorlinks=true}
% \usepackage[linesnumbered, ruled]{algorithm2e}


\newtheorem{definition}{Definition}[]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{example}{Example}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\graphicspath{ {./images/} }


\def\[#1\]{$$#1$$}

\def\frac#1#2{{#1\over#2}}
\def\eps{\varepsilon}

\def\bbR{{\bf R}}
\def\X{{\bf X}}
\def\meno{\medskip\noindent}

\newcommand{\fg}[1]{\textcolor{red}{F: #1}}
\newcommand{\gc}[1]{\textcolor{red}{G: #1}}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.5}


\title{Logic Explainer Networks}

\author{}
% \author{
%  Ziyue Qi \\
%   School of Coumputing and Information\\
%   University of Pittsburgh\\
%   Pittsburgh, PA 15213 \\
%   \texttt{ziq2@pitt.edu} \\
%   %% examples of more authors
%   \And
%  Zixuan Lu \\
%   School of Coumputing and Information\\
%   University of Pittsburgh\\
%   Pittsburgh, PA 15213 \\
%   \texttt{ZIL50@pitt.edu} \\
%   \And
%  Yuchen Lu \\
%   School of Coumputing and Information\\
%   University of Pittsburgh\\
%   Pittsburgh, PA 15213 \\
%   \texttt{yul217@pitt.edu} \\
  %% \AND
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
% }

\begin{document}
\maketitle
\begin{abstract}
Despite the increasing popularity of deep learning application, in real wold domains the employment of deep neural networks is still limited and strongly criticized due to their lack of interpretability. In particular, providing a comprehensible explanation for a certain classification task can be crucial in decision support contexts. To this aim, rule-based explanations expressed in a high-level language are particularly relevant. In this paper we developed a general tool for XAI to show how a mindful design may lead to interpretable deep learning models called Logic Explainer Networks (LENs), which only require the input and the output of the model to be semantically meaningful predicates. LENs are capable to provide both local and global explanations of the predictions made by the LEN itself. Explanations are given as first-order-logic formulas expressed in terms of input concepts. As a special case, we describe and discuss three out-of-the-box LEN-based models. Experimental results on a number of different datasets and tasks confirm how on average LENs not only generalize better and but also provide more meaningful explanations than established white-box models such as decision trees and Bayesian rule lists.
% Deep learning is yet to fulfill the expectations around its dramatic impact on society. In many real-world contexts, the employment of deep neural networks is still limited and strongly criticized due to their lack of interpretability. The urgent need for interpretable models is proven by the growing hype around explainable-AI research. We believe that the research to date is taking for granted that deep neural networks should be thought as black boxes. We argue that the time has come for a paradigm shift, we need interpretability \textit{by design}. In this work we show how a mindful design may lead to interpretable deep learning models, regardless to the number of features, layers, and parameters. The proposed approach only requires that the input and output features to be predicates on semantically meaningful concepts. The resulting trained model is able to provide I) for each sample a local first-order logic formula explaining the prediction in terms of the input concepts (e.g. $\textrm{Bird}(x_i) \iff \textrm{Beak}(x_i) \land \neg \textrm{Arm}(x_i)$) and II) for each task a global explanation as a first-order logic formula (e.g. $\forall x, \textrm{Bird}(x) \iff (\textrm{Beak}(x) \land \textrm{Wing(x)}) \lor (\textrm{Plumage}(x) \land \neg \textrm{Skin}(x))$). We show the potential and generality of the approach in different experimental scenarios, outperforming state-of-the-art concept bottleneck models in computer vision and end-to-end approaches on structured datasets.
% By and large the spectacular results of deep learning are somewhat criticized because of the lack of remarkable human-like explanations of their decision mechanisms. In this paper, we show that the traditional black-box that we typically obtain at the end of deep learning can surprisingly be given paired with a truly symbolic description that arises from the specific piece-wise linear computation related to rectifiers neurons. We show that the computation carried out by deep nets with rectifiers can be given a symbolic description and that the we can enforce algebraic structures somewhat related to classic logic frameworks that are popular in AI. 
% Deep learning needs a shift from 
% The need for interpretable deep learning models has become of crucial importance in many sectors. Experts working in critical context, from healthcare to autonomous driving, can not simply rely on end-to-end black box models to take their decisions. Recently, many works aimed at explaining neural networks or creating interactable models. 
% In this project we propose one of the first attempt to build an interpretable neural network by design. The output nodes of the proposed network are completely explained through first-order logic rules. Explanations are given in terms of concepts, predicted by previous network layers. In the experiments, both supervised and unsupervised learning applications of the interpretable neural networks are shown.
% This paper introduces Logic Explainer Networks (LENs), a versatile neural model for logic-based explanations. This framework integrates elements from deep learning and logic with the aim of providing a set of explanations for a classification task. A major advantage of LENs is that they are very general and can be applied in principle to any neural architecture and to solve any classification problem.
\end{abstract}

% \section*{Index - Architecture of the paper}
% \begin{enumerate}
%     \item Introduction
%         \begin{enumerate}
%             \item Motivation
%             \item Why you may need logic-based explanations?
%             \item Proposal
%         \end{enumerate}
%     \item LENs: Logic Explainer Networks
%         \begin{enumerate}
%             \item Data \& Pipeline (Use cases) 
%             \item Classification style
%             \item Explanation style
%         \end{enumerate}
%     \item Methods
%         \begin{enumerate}
%             \item FOL rule extraction
%             \item Learning criteria
%             \item Parsimony criteria
%             \item Activation functions
%         \end{enumerate}
%     \item Out-of-the-box LENs
%     \item Benchmarking out-of-the-box LENs
%         \begin{enumerate}
%             \item Applications
%             \item Discussion
%             \item Explanation as defense
%         \end{enumerate}
%     \item Related Work
%     \item Conclusions
% \end{enumerate}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth, trim= 0 0 0 0, clip]{figs/abstract.pdf}
    \caption{The Logic Explainer Network (LEN) % is a framework which 
    employs neural networks to provide explanations of different learning tasks. In this case a LEN is placed on top of a convolutional neural network $g(x)$ in order to i) classify to which species the bird in the image belongs to and ii) provide an explanation on why it should belong to this class. The image comes from the CUB 200-2011 fine-grained classification dataset.}
    % \fg{Forse metterei proprio la regola che tira fuori che mi sembra più chiara.., tipo bill shape and.. ..not bill color -> bird}
    \label{fig:len}
\end{figure}




\section{Introduction}
The lack of transparency in the decision process of some machine learning models, such as neural networks, holds up their application in many safety-critical domains \cite{chander2018working}. Employing black-box models may be unacceptable in contexts such as industry, medicine or courts, where the potential economical or ethical repercussions are calling for lawmakers to discourage from a reckless application of non-interpretable models \cite{gdpr2017,law10code,goddard2017eu,gunning2017explainable}. As a consequence, research in Explainable Artificial Intelligence (XAI) has become strategic and has been massively encouraged, leading to the development of a variety of techniques that aim at explaining black-box models \cite{das2020opportunities,brundage2020toward} or at developing effective interpretable models \cite{carvalho2019machine,rudin2019stop}. 
% Some of the latter case, like decision rules, provide one of the best forms of explanations as they were originally developed for decision support systems \cite{sprague1980framework}.

The notions of \emph{interpretability} and \emph{explainability} were historically used as synonyms, however nowadays the distinction between interpretable models and models providing explanations has become more clear, as recently discussed by different authors \cite{gilpin2018explaining,lipton2018mythos,marcinkevivcs2020interpretability}. 
In some contexts, the use of a black-box model may be unnecessary or even not preferable \cite{rudin2019stop}. For instance, a proof of concept, a prototype, or the solution to a simple classification problem can be easily based on standard out-of-the-box AI solutions which are interpretable by design.
However, interpretable models may generally miss to capture complex relationships among data. Hence, in order to achieve state-of-the-art performance in more challenging problems, it may be necessary to exploit black-box models that, in turn, may require an additional explanatory model to gain the trust of the user. 

In the literature, there is a wide consensus on the necessity of having an explanation for machine learning models that are employed in safety-critical domains, while there is not even agreement on what an \emph{explanation} actually is, nor if it could be formally defined \cite{doshi2017towards,lipton2018mythos}.
An explanation should serve cognitive-behavioral purposes such as: engendering trust, aiding bias identification, or taking actions/decisions \cite{srinivasanexplanation}. An explanation may help humans understanding the black-box, may allow for joint decision making a deeper human-machine interaction \cite{koh2020concept}, and may engender trust on fully automated tasks. All of this is possible as long as the explanations are useful from a human perspective.
% and take into account how humans think and make decisions
In a nutshell, an explanation is an answer to a "why" question \cite{miller2019explanation}. But what is that characterize a good explanation? As a matter of fact, what makes an explanation good or bad depends on "the degree to which a human can understand the cause of a decision" \cite{miller2019explanation}. The goodness of an explanation is intimately connected to how humans collect evidences and eventually make decisions. 
In Herbert Simon's words we may say that a good explanation is \textit{satisficing} \cite{simon1956rational}, i.e. \textit{it either gives an optimal description of a simplified version of the black box (e.g. a surrogate model) or a satisfactory description for the black box itself}
% \footnote{"Decision makers can satisfice either by finding optimum solutions for a simplified world, or by finding satisfactory solutions for a more realistic world".}
\cite{simon1979rational}. However, the notion itself of explanation generally depends on both the domain of the application and who it is aimed at \cite{carvalho2019machine}.
% This is the reason why, different criteria and taxonomies 
% such as the \textit{scope}, the \textit{usage} and the \textit{methodology} have been identified as key-properties to define a XAI technique \cite{das2020opportunities}. 


%%%%%%%%%%%OLD
% Despite many important contributions, some major XAI shortcomings are still to be settled:
% \begin{itemize}
%     \item \textit{\textbf{Versatility}}: Many interpretable models are special purpose, requiring specific neural architectures, input data and task labels \cite{ciravegna2020constraint}, or providing a limited variety of explanations \cite{koh2020concept}.
%     \item \textit{\textbf{Quantitative metrics}}: In XAI literature there are no neural models showing a generalization ability significantly better than established white-box models like decision trees \cite{ciravegna2020constraint} \fg{citazione giusta?}. Besides, for many forms of explanations (e.g. stance-based) is quite hard to provide quantitative measures of completeness and correctness \cite{das2020opportunities}.
%     \item \textit{\textbf{Qualitative properties}}: 
%     The form of the explanations are not suitable for many strategic human purposes. For instance, humans struggle with the use of stance-based explanations (e.g. saliency maps) for decision making \cite{das2020opportunities,srinivasanexplanation}. Further, there is not agreement on what a satisfying explanation should be, since it mostly depends on the context where it is required.
% \end{itemize}
% If special purpose solutions may still be acceptable for some applications, XAI approaches cannot overlook the imperative role of serving human purposes. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The need for high-quality evidences is one of the main reasons why concept-based explanations are receiving ever-growing consideration. Such techniques allow for explanations given in terms of human-understandable symbols (the \textit{concepts}) rather than raw features such as pixels or characters \cite{kim2018tcav,ghorbani2019towards,koh2020concept}. As a consequence, they seem more suitable to serve many strategic human purposes such as decision making tasks. For instance, a concept-based explanation may describe a high-level category through its attributes as in: "a \textit{human} has \textit{hands} and a \textit{head}".
% However, many concept-based explanations still look ambiguous, it is not obvious how to \textit{quantitatively} assess their generality, and may not be suitable for effective decision making at all.
% How much effort requires analyzing a pairwise dependence plot \cite{friedman2008predictive} or a ranking of SHAP values \cite{NIPS2017_7062} or a decision tree with depth 10 \cite{breiman1984classification} for domain experts? How much for laypeople?
% If you are looking for a quick and comprehensible answer these methodologies will not suit your needs.
While collecting high-quality evidences for an explanation is a common feature of concept-based techniques, there are very few approaches formulating hypothesis and even less providing synthetic descriptions whose validity can be quantitatively assessed \cite{das2020opportunities}.
A possible solution is to rely on a formal language that is
% synthetic but also 
very expressive and closely related to natural language and reasoning, such as First-Order Logic (FOL). A FOL explanation can be considered a special kind of concept-based explanation, where the description is given in terms of logical predicates, connectives and quantifiers, such as "$\forall x:\ \textit{is\_human}(x) \rightarrow \textit{has\_hands}(x) \wedge \textit{has\_head}(x)$". However, FOL formulas may generally express much more complex relationships among the concepts that are involved in a certain explanation. Compared to other concept-based techniques, logic-based explanations may provide many key advantages.
% \begin{itemize}

    \textsc{Clarity. } An explanation reported in FOL is a rigorous and unambiguous statement. This formal clarity may serve cognitive-behavioral purposes such as: engendering trust, aiding bias identification, or taking actions/decisions. For instance, the formula "\textit{snow} $\wedge$ \textit{tree} $\leftrightarrow$ \textit{wolf}" may easily outline the presence of a bias in the collection of training data.
    
    \textsc{Modularity. } Different logic-based explanations can be combined to describe groups of observations or global phenomena. Different observations of the same phenomenon may have completely different logic-based explanations according to their characteristics. For instance, for an image showing only the face of a person the explanation could be "(\textit{nose} $\wedge$ \textit{lips}) $\rightarrow$ \textit{human}", while for another image showing a person from behind a valid explanation could be "(\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})  $\rightarrow$ \textit{human}". The two local explanations can be combined as in "(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears}) $\rightarrow$ \textit{human}".
    
    \textsc{Measurability. } The quality of logic-based explanations can be quantitatively measured
    % on independent data sets 
    to check their correctness and completeness. For instance, once the explanation "(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})" is extracted for the class \textit{human}, this logical formula can be applied on a test set to check its generality in terms of quantitative metrics like confidence, support, and accuracy.
    
    \textsc{Simplifiability. } FOL-based explanations can be rewritten in 
    different equivalent forms according to user preferences, such as in \emph{Disjunctive Normal Form} (DNF) and \emph{Conjunctive Normal Form} (CNF). Further, existing techniques such as Quine–McCluskey algorithm can be used to get compact and simplified equivalent expression of a certain explanation \cite{mccoll1878calculus,quine1952problem,mccluskey1956minimization}. For instance, the explanation "(\textit{person} $\wedge$ \textit{nose}) $\vee$ ($\neg$\textit{person} $\wedge$ \textit{nose})" can be easily simplified in "\textit{nose}".
% \end{itemize}



This paper presents a unified framework for XAI where a neural network, the \emph{Logic Explainer Network} (LEN, see Figure \ref{fig:framework}), is trained to learn a set of explanations for the class-assignments of a certain classifier (eventually another neural network), or to produce itself the classification results. LENs can be thought of as sub-symbolic explanations, that can be easily interpreted in a set of first-order logic formulas. In addition, different preferences on the kind of explanation and the LEN style can be expressed and will turn out in different kind of logic rules. This versatility makes the proposed framework and in particular LENs applicable to a wide range of classification tasks, by providing logic-based explanations in different use cases and according to different user preferences. 
The overall problem configuration of how a logic explainer network can be integrated with an existing classifier is shown in Fig. \ref{fig:len}, and further described in Sec. \ref{sec:use_cases}.  
Hence, the presented framework integrates elements from deep learning and logic with the aim of providing a set of explanations for a classification task. A major advantage of LENs is that they can be implemented by several neural architectures and can be applied in principle to explain any
classifier decision process. Out-of-the-box neural networks based on this framework span a wide range of flavors, from fully interpretable models to black-boxes providing both high-quality explanations and state-of-the-art classification performance.
Further, human priors expressed by FOL formulas can be naturally incorporated with LENs both in the learning process \cite{ciravegna2020constraint} and in the architecture \cite{koh2020concept}. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/lens_framework.pdf}
    \caption{LENs framework. \gc{Mi sa che ci sono i box all'interno Logic Explainer Network che sono "dietro" al box stesso (cambia il colore)}}
    \label{fig:framework}
\end{figure}

Our work contributes to the XAI research field with the following advances:
\begin{itemize}
    \item Providing a unifying framework for solving and explaining classification problems with neural networks.
    \item Providing to any user the possibility to express a set of preferences to get one or more customized explanations about the classification task under investigation. We also provide and experimentally evaluate three out-of-the-box preset models.
    % \item Supporting a wide range of logic-based explanations from \textit{local explanations} and \textit{node-level explanations}, explaining the prediction for an individual sample or a hidden neuron, to \textit{cluster explanations} up to \textit{class-level explanations} and \textit{global explanations}.
    \item Supporting a wide range of logic-based explanations at different level of granularity such as, \textit{example}, \textit{local} and \textit{global}-based explanations, aiming at explain a single sample, a subset of the available data or the whole dataset, respectively.
    \item Sustaining the implementation of LENs through the release of a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on out-of-the-box LENs with different interpretability-VS-explainability-VS-accuracy trade-offs.
    \item Presenting experimental results confirming how LENs generalize better than established white-box models such as decision trees on complex Boolean tasks (as observed in \cite{tavares2020understanding}).
\end{itemize}

% \paragraph{Reading path} 
The paper is organized as follows. Related works are covered in Section \ref{sec:related}. Section \ref{sec:basics} gives a formal definition of a \emph{Logic Explainer Network} and describes its underlying assumptions, key paradigms and design principles. The methods used to extract logic formulas and to effectively train LENs are described in Section \ref{sec:methods}. Three out-of-the-box LENs presented in Section \ref{sec:outofthebox} are compared on a wide range of benchmarks in terms of classification performance and quality of the explanations (Section \ref{sec:experiments}). A coding example showing how to use LENs with the associated python library is shown in Section \ref{sec:tool}. Finally, Section \ref{sec:conclusion} outlines the social and economical impact of this work as well as future research directions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%FORSE LO METTEREI PRIMA DEI PUNTI PRECEDENTI, CHE DIVENTEREBBERO MOTIVATION PER LE REGOLE IN FORMA LOGICA, O POTREMMO COMPATTARE TUTTO INSIEME 
% \fg{work in progress:
% 1) spiegazioni e/o modelli interpretabili esistenti sono spesso definiti per funzionare in casi molto specifici, e quindi non sono molto applicabili/versatili
% -> il nostro framework può essere applicato a qualsiasi architettura e per un qualunque problema di classificazione;
% -> tra l'altro, eventuale conoscenza aggiuntiva sul problema (gerarchie, constraints, ecc) potrebbero essere agganciate molto naturalmente.
% 2) mancano in letteratura modelli spiegabili con performance decenti;
% -> il nostro può fornire trade/offs performance vs complessità delle regole
% 3) è importante prevedere diversi tipi di spiegazione perchè non c'è una definizione univoca di cosa sia una spiegazione;
% -> user preferences su tipi di spiegazioni} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \paragraph{Why you may need logic-based explanations?}
% % \section{Background/Related Work?}
% \label{sec:motivation}

% Among existing approaches, concept-based explanations are receiving ever-growing consideration because they allow for explanations given in terms of human-understandable symbols (the \textit{concepts}) rather than raw features such as pixels or characters \cite{kim2018tcav,ghorbani2019towards,koh2020concept}. For instance, a concept-based explanation may describe a high-level category through its attributes as in: "a \textit{human} has \textit{hands} and a \textit{head}".
% In this regard, Mental models are a specific class of concept-based explanations consisting of rules which are triggered when a certain set of conditions becomes active \cite{holland1989induction,srinivasanexplanation}. For example, a mental model of \textit{human} can be represented by the association rule: "If (\textit{hands}, \textit{head}) then (\textit{human})" \cite{mayes2005theories}.
% The general class of mental models also includes as a special case logic-based explanations, such as "\textit{head} $\wedge$ \textit{hands} $\leftrightarrow$ \textit{human}". Compared to other kind of XAI techniques, logic-based explanations provide many advantages.

% \begin{itemize}
% \item Finally, the quality of logic-based explanations can be quantitatively measured on independent data sets to check their correctness and completeness.
%     \item \textit{\textbf{Human-centered}}: A logic-based explanation serves cognitive-behavioral purposes such as: engendering trust, aiding bias identification, or taking actions/decisions. \fg{Non direi natively designed, cosa volevi dire?} For instance, the formula "\textit{snow} $\wedge$ \textit{tree} $\leftrightarrow$ \textit{wolf}" may easily outline the presence of a bias in the collection of training data.
%     \item \textit{\textbf{Rational}} The explanation has a rational and rigorous form. For instance, the sentence "\textit{hands}, \textit{wings}, and \textit{head} are important concepts to describe a \textit{human}" may be lead to misunderstandings, while the formula "\textit{head} $\wedge$ (\textit{hands} $\vee$  $\neg$\textit{wings}) $\leftrightarrow$ \textit{human}" immediately clarifies non-linear relationships between the concepts and the equivocal role of the item \textit{wings}.
%     \item \textit{\textbf{Meaningful}} The elements (i.e. concepts) of a logic-based explanation are meaningful \textit{individually}. For instance, the concept \textit{head} has a meaning per se, while \textit{pixel n. 42} has not.
%     \item \textit{\textbf{Coherent}}
%     %. In general, an argument is coherent if the concepts and their interconnections make sense to the reader.
%     A logic-based explanation is an intrinsically coherent \fg{??} way of combining individual elements concepts, as it illustrates an argument with a deductive structure. From a set of clauses (e.g. "\textit{head} $\wedge$ (\textit{hands} $\vee$  $\neg$\textit{wings}) %"(\textit{hands} $\wedge$ \textit{head}) $\vee$ (\textit{head} $\wedge \neg$\textit{wings})")
%     it follows a certain conclusion (e.g. "\textit{human}").
%     \item \textit{\textbf{Simple}} From Aristotle onwards, logicians have developed a variety of rigorous methodologies to efficiently simplify logical expressions. This allows for the simplification of overly complex formulas into compact descriptions of the phenomenon.
%     \item \textit{\textbf{Consistent}} \fg{Consistente e coerente sono sinonimi, deciderei cosa tenere} Logic-based explanations are consistent with both the model's prediction and the observed phenomenon. For instance, if the model detects a \textit{human} in an certain image, then the logic-based explanation will give a formula explaining why the human has been detected, such as: "\textit{head} $\wedge$ (\textit{hands} $\vee$  $\neg$\textit{wings}) $\leftrightarrow$ \textit{human}" 
%     %"(\textit{hands} $\wedge$ \textit{head}) $\vee$ (\textit{head} $\wedge \neg$\textit{wings}) $\leftrightarrow$ \textit{human}".
%     \item \textit{\textbf{Local}} Different observations of the same phenomenon may have completely different logic-based explanations according to their characteristics. For instance, for an image showing only the face of person the explanation could be "(\textit{nose} $\wedge$ \textit{lips}) $\leftrightarrow$ \textit{human}", while for another image showing a person from behind a valid explanation could be "(\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})  $\leftrightarrow$ \textit{human}".
%     %"(\textit{nose} $\wedge$ \textit{lips} $\wedge \neg$ \textit{mask}) $\leftrightarrow$ \textit{human}", while in COVID times it could be "($\neg$ \textit{nose} $\wedge \neg$ \textit{lips} $\wedge$ \textit{mask}) $\leftrightarrow$ \textit{human}" (if the face mask is covering the lips).}
%     \item \textit{\textbf{Modular}} Different logic-based explanations can be rigorously combined and aggregated to describe groups of observations or global phenomena. For instance, the two previous explanations can be combined as in "(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears}) $\leftrightarrow$ \textit{human}".
% \end{itemize}



\section{Related work}
\label{sec:related}
%%% taxonomy:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DALLA 4
% XAI literature can be roughly partitioned into two categories: works focusing on white-box interpretable models and those aiming at providing satisficing explanations of model behaviours which are treated as black boxes. In the first category we can find models like Bayesian Rule Lists, Decision Tree; in the latter, post-hoc explanation algorithm such as LIME, SHAP but also saliency-map fall. 
% Based on this distinction and differently from other papers in literature, we here define \textit{Interpretability} and \textit{Explainability} as two different properties of machine learning models. \fg{In che senso? Volevi dire che noi offriamo entrambe le cose come 2 estremi di un unico modello?}

% \begin{definition}[Interpretability] 
% Interpretability is the extent to which the behavior of a model can be easily comprehended by a human.
% \end{definition}

% \begin{definition}[Explainability]
% It is the capacity to provide comprehensible explanations of the decisions taken by a certain model. 
% \end{definition}
% \fg{Da dove sono prese queste definizioni? Metterei citazione} 

% It is important to notice that both definitions point their attention on the model and not on the algorithm used to train it, which in this respect can be ignored.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the last few years, the demand for human-comprehensible models has significantly increased in safety-critical and data-sensible contexts. This popularity is justified by the emerging need for unveiling the decision process of pitch-black models like deep neural networks. To this aim, the scientific community has developed an important variety of XAI techniques, with different properties and goals. Several taxonomies have been proposed to categorize the XAI models, with partial overlapping and some ambiguity on the referred terminology. Without pretending to be exhaustive, in the following description we only focus on some key-properties that are relevant to compare LENs with other existing approaches. In particular, we will discriminate related work by relying on the \emph{result}, feature-scoring vs rule-based, on the \emph{usage}, interpretable models vs explanation methods, and on the \textit{scope}, local vs global, of the provided explanations. A brief summary of a few XAI works in terms of these features is reported in Tab. \ref{tab:related_work}. For more details on existing taxonomies we refer e.g. to the following surveys \cite{adadi2018peeking,carvalho2019machine,marcinkevivcs2020interpretability,molnar2020interpretable}.

\textsc{Results of Explanation Methods. }
XAI models can be differentiated according to the result of the produced explanation. 
Most of the methods in literature usually focus on scoring or providing summary statistics of features. However, \textit{feature-scoring} methods
%
can be of scarce utility in decision support cases, whereas a comprehensible language may bring light on the black-box behaviour by identifying concept-based correlations.
% do not consider how concepts are interconnected, therefore, these explanations may not live up to the expectations. 
On the other hand, \emph{rule-based} explanations are generally more comprehensible, since they usually rely on a formal language, such as first-order logic. Further, the learned rules can be directly applied to perform the learning task in place of the explained model.

\textsc{Explanation Usage. }
The interpretability of a model can be achieved either by constraining the model to be interpretable per se (\emph{interpretable models}) or by applying some methods to get an explanation of an existing model (\emph{explanation methods}). Interpretable models are by definition \emph{model specific}, while explanation methods can rely on a single model or be, as more commonly happens, \emph{model agnostic}. In principle, interpretable models are the best suited to be employed as decision support systems. However, their decision function often is not smooth which makes them quite sensible to data distribution shifts and impairs their generalization ability on unseen observations \cite{tavares2020understanding,molnar2020interpretable}. 
On the other hand, explanation methods can be applied to get approximated interpretation of state-of-the-art models. These methods are generally \textit{post hoc}, since the explanations are produced when the training procedure is concluded. 

\textsc{Scope of Interpretability. }
A fundamental feature to distinguish among explainable methods is whether they provide \textit{local} explanations, valid for a given sample, or \textit{global} explanations, valid on the whole input space. However, several models consider local explanations together with aggregating heuristics to get a global explanation.

% {\bf Methodology. }
% The algorithms employed by most XAI models can be roughly categorized into two main categories. \textit{Backpropagation}-based techniques analyze the gradients of the activation up to the input features, in order to identify the most relevant ones for the classification task. \textit{Perturbation}-based techniques, instead, observe how the machine output changes when altering a given input data. The aim of these methods is to understand which %are the most discriminative 
% features (when altered) may drive the model to take different decisions. 
% Nonetheless, not all algorithms belong to these two categories. In particular, \textit{Model-intrinsic} explanation methods significantly differ according to the training algorithms.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
                                    & \multicolumn{2}{c|}{Results of Explanation Methods} & \multicolumn{2}{c|}{Scope of Interpretability} & \multicolumn{2}{c}{Expanation Usage} \\
                        & feature-scoring & rule-based & local & global & interpretable model & explanation method \\ 
\hline
LIME &\faCheckCircle & & \faCheckCircle            & & & \faCheckCircle  \\
SHAP &\faCheckCircle & & \faCheckCircle & & & \faCheckCircle  \\
% DeConv \cite{zeiler2014visualizing}                     &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           & \faCheckCircle         &               &                  \\
Activation Maximization & \faCheckCircle & & \faCheckCircle  &  &  & \faCheckCircle  \\
Saliency Maps &\faCheckCircle&& \faCheckCircle &      &              & \faCheckCircle \\
% Grad-CAM \cite{selvaraju2017grad}                       &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
SP-LIME &\faCheckCircle&& & \faCheckCircle &              & \faCheckCircle  \\
Class Model Visualization &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle                 \\
% TCAV \cite{kim2018tcav}                                 &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
LORE &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle \\
Anchors &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle  \\
DeepRED   &&\faCheckCircle& \faCheckCircle & \faCheckCircle &  & \faCheckCircle \\
GAM  &\faCheckCircle&&              & \faCheckCircle          & \faCheckCircle            &   \\
Decision Trees       &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
BRL                   &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
\textbf{LENs}                                           &&\faCheckCircle& \textbf{\faCheckCircle}    & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle} \\
\end{tabular}
}
\vspace{0.1cm}
\caption{Summary of related work according to taxonomies.
}
\label{tab:related_work}
\end{table}

Some of the most famous XAI techniques share the characteristic of being feature-scoring, local, post hoc methods.
Sometimes indeed, the easiest way to solve the explanation problem is simply to treat the model as a black-box and sample by sample determine which are the most important features for a prediction. 
Prominent examples of algorithms falling in this area %are Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should}, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} and DeConvolution Neural Network (DeConv) \cite{zeiler2014visualizing}, which
accomplish this task by perturbing the input data. 
Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should} trains a white-box model (e.g. a logistic regression) to mimic the predictions of a given model in the neighbourhood of the sample to explain. By analyzing the weights of the white-box model it identifies the most important patch of pixels (superpixel).
Differently, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} computes the Shapley value of each feature by iteratively removing each one of them. %provides for local explanations by computing each input feature contributions in a certain prediction. In the Kernel SHAP version, the Shapley values of each feature are calculated by iteratively removing features in a similar way to what is done in LIME.
% Deconvolutional Network were initially introduce in \cite{zeiler2011adaptive} for unsupervised learning.
% Firstly introduced in \cite{zeiler2011adaptive}, DeConvolution Neural Network (DeConv) are used in \cite{zeiler2014visualizing} to %visualize the activation of a convolutional layer. In particular, they 
%visually determine pixel importance for a certain prediction by analyzing how the classification output changes when part of the input image is masked. 
Other important techniques %such as Activation Maximization \cite{erhan2010understanding}, Saliency Maps \cite{simonyan2013deep} and Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} 
provide the same type of explanations through gradient analysis. %Differently from the previous one, however, they determine feature importance  %in the context of Convolutional Neural Network (CNN). 
Authors of Activation Maximization \cite{erhan2010understanding} firstly introduced this idea as an optimization problem. They explain the behaviour of a hidden/output unit by slightly modifying a given input data such that it maximizes its activation. An easier way to identify features causing a certain output has been found with Saliency Maps \cite{simonyan2013deep}, which project the classification loss until the input image. 
% A further improvement has been introduced with Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} which allows to identify both class-specific image area and counterfactual explanations.
%They achieved this by modifying global average pooling with class activation mapping which allows to identify important image area with a single forward pass.
%
Other post-hoc methods have been devised to extract global feature-scoring explanations, often starting from local explanations. %like LIME for Global Explanations \cite{ribeiro2016should} based on perturbation and Class Model Visualization \cite{simonyan2013deep} or Testing with Class Activation Vectors \cite{kim2018interpretability} based on Backpropagation. 
A submodular-pick algorithm extends the LIME module (SP-LIME) in %LIME for Global Explanations 
\cite{ribeiro2016should} to provide global explanations. SP-LIME first finds superpixels of all input samples with the standard LIME module. Successively, it finds the minimum number of common superpixels that covers most of the images.
Starting from the idea of Activation Maximization,  Class Model Visualization \cite{simonyan2013deep} finds the input sample that maximizes a certain class probability score in the whole input space. %Differently from Activation Maximization, here the input sample is not searched in the neighbourhood of a given sample, but in the whole input space. 
Differently, LENs take a quite different perspective with respect to these methods: a LEN aims at providing human comprehensible decision support in terms of a set of FOL rules.


Explanation methods, indeed, can also supply FOL explanations. 
LOcal Rule-based Explanations of black-box decision systems (LORE) \cite{guidotti2018local} extracts FOL explanations via tree induction. They focus on local rules extracted through input perturbation. For each sample to explain, a simple decision tree is trained to mimic the behaviour of the black-box model in the neighbourhood of the sample. Both standard and counterfactual explanations can then be extracted  following the branches of the tree. 
Again based on LIME, Anchors \cite{ribeiro2018anchors}  also provides local rules of black-box model prediction via input perturbation. In this case, rules are not extracted from a decision tree but are generated by solving a Multi-Armed-Bandit beam search problem. 
Extending the CRED algorithm \cite{sato2001rule}, DeepRED  \cite{zilke2016deepred} employs a decompositional strategy to globally explain neural networks. Starting from the output nodes, each node in a layer is explained in terms of the activations of the previous ones through a decision tree. In the end, all rules for each class are merged in a single global rule in terms of input nodes only. For a single example a single local rule can be extracted following the firing path. 
The approach proposed in this paper is in some sense similar to the DeepRED algorithm. Indeed, LENs can explain the behaviour of a neural network both end-to-end and layer by layer. However, LENs can be used to explain any black-box model as far as its input and output are interpretable, as we will see in Sec. \ref{sec:basics}. Further, LENs support different forms of FOL rules, with different scopes and goals.

Interpretable models are generally capable to provide both local and global explanations. These explanations may be based again on feature-scoring as in Generalized Additive Models (GAM) or on FOL rules as in Decision Tree \cite{breiman1984classification} and Bayesian Rule Lists (BRL) \cite{letham2015interpretable}. Meant to overcome the non-linearity assumptions of Linear regression, GAM learns to predict the given class for each feature via decision tree. In \cite{caruana2015intelligible}, authors proposed GA$^2$M where attribute interaction is allowed at a pair level. Recently a further extension employing neural network as non-linear function has been proposed in \cite{agarwal2020neural}, which, however, lose interpretability at feature-level.
Decision trees are a greedy learning algorithm which iteratively divides input data into smaller subsets until they only contain elements belonging to the same class. Different pruning algorithms have been also proposed to simplify the resulting structure and therefore the explanations \cite{quinlan1987simplifying}. Each path of a decision tree may be seen as a decision rule i.e. an \textit{IF-THEN} statement. 
The set of rules may be generated in different ways, either with sequential covering as in \cite{cohen1995fast} or by selecting the best rules from a pre-mined set via Bayesian statistics as in BRL. 
%
Also Logic Explainer Networks can be used to solve a learning task itself, being almost interpretable per se. 
Employing an interpretable by-design neural network as classifier, however, has the advantage that the extracted explanations will perfectly match the classifier predictions. 
In addition, relying on a neural network, LEN generalization performance can be much better than standard interpretable-by-design methods, that generally have a very limited representation capacity.

To summing up, the proposed approach can be used both as interpretable model and explaination method, allowing LENs to be suitable to deal with the Interpretability-versus-Accuracy trade-off. 
The explanation type of LENs is in terms of FOL rules and different explanation styles, corresponding to different kind of logic formulas, can be expressed. Such explanations are extracted with different scopes, from local rules valid on a single sample to global rules valid for an entire class.
%\fg{dire da qualche parte che noi non siamo ne intrinsic, visto che dobbiamo fare approx booleana per le regole, nè post-hoc, visto che le LEN sono co-trainate e non interpretano a posteriori le uscite di un classificatore.. Anche se ci sono costruite sopra...}


% Many authors have tried to list the characteristics of a good explanation, but in the end what will make it good or bad depends on "the degree to which a human can understand the cause of a decision" \cite{miller2019explanation}. All quality metrics are based on human perceptions. This is why we think many standard white-box models are not suitable for providing good explanations (e.g. naive Bayes classifier \cite{harry2004optimality}, k-nearest neighbors \cite{fix1951discriminatory} or logistic regression \cite{berkson1953statistically}). They were not designed for this purpose, hence their explanations are far from being useful. How good is an explanation listing the weight values of a logistic regression? Other approaches, like example-based explanations \cite{aamodt1994case,kim2016examples}, yield more intuitive explanations but their main focus is on individual predictions rather than the entire model behavior. 

% Such limitations can partially be solved using some machine learning and data mining approaches like decision trees \cite{breiman1984classification} or decision rule mining (e.g. oneR \cite{holte1993very}, RIPPER \cite{cohen1995fast}, Bayesian Rule Lists \cite{letham2015interpretable}). Decision rules provide one of the best forms of explanations by design.  

% Sometimes the easiest way to solve a learning problem is simply a black-box. This is where model-agnostic approaches come into play \cite{ribeiro2016model}. They can provide explanations for any machine learning model. The fact that many trendy techniques fall in this area is not a coincidence (e.g. LIME \cite{ribeiro2016should}, Anchors \cite{ribeiro2018anchors}, or SHAP \cite{lundberg2017unified}, Grad-cam \cite{selvaraju2017grad}). Their popularity is justified by the pressing need for unveiling the decision process of pitch-black models like deep neural networks. However, the outlook of their explanations may not live up to the expectations. The main issue is that these methodologies usually focus on scoring/ranking the input features/concepts or on providing activation maps over the input. The way concepts are interconnected is usually not explored. If I know that the concepts "head", "arms" and "wings" are needed to determine the concept "human", what do I know about their mutual relationships? Even worse, when the problem becomes more challenging (e.g. genomics) the explanations may become incomprehensible. Which biologist can make use of a ranking of thousands or millions of features (e.g. genes)?




\section{LENs: Logic Explainer Networks}
\label{sec:basics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%OLD
% This section presents the core features of the proposed framework and some key paradigms for solving and explaining classification problems using LENs.

% Let us consider a binary classification problem where, for any input sample $c \in C$, a classifier $f: C \rightarrow E$ assigns the input to one of two possible categories either $E=0$ or $E=1$. From here on, we assume the following conditions on the input space and on the classifier.
% \begin{enumerate}
%     \item Any input $c\in C$ consists in a array of $[0,1]$-valued features, i.e. $C \subset [0,1]^k$.
%     \item The classifier $f$ is a deep feed-forward neural network. The prediction $\hat{e}$, is obtained by applying a sigmoid (or a softmax) activation function to compute the probability of class assignment.
%     % \item There is no pair of observations $c^i,c^j\in C$, such that $\bar{e}(c^i) \neq \bar{e}(c^j)$ and $\bar{c}^i=\bar{c}^j$, where the overline notation denotes the boolean discretization (thresholded at $0.5$) of values from $[0,1]$ to $\{0,1\}$ values.
%     % For instance, the boolean discretization of $c_i = 0.2$ and $c_j = 0.9$ corresponds to $\bar{c}_i = 0$ and $\bar{c}_j = 1$.
% \end{enumerate}

% \begin{definition}[Logic Explainer Network]
% A Logic Explainer Network (LEN) is a mapping $f: C \rightarrow E$, aiming at solving and providing logic formulas to explain a classification problem where the aforementioned conditions hold.
% \end{definition}

% The above conditions can be easily generalized to multi-task classification problems, where for any input sample $c \in C$, the model $f: C\rightarrow E$ assigns a set of membership degrees $f(c)=(f_1(c),\ldots,f_r(c))\in[0,1]^r$ to $r$ different classes.

% The layout of a XAI pipeline based on LENs requires a mindful analysis of three main aspects of the classification problem:
% \begin{enumerate}
%     \item \textit{\textbf{Data \& pipeline}}: Are you working with unstructured (e.g. images) or structured data (e.g. gene expression)? Do you have annotations for tasks or concepts? Do you need one or more concept bottlenecks? (Cfr. with Subsection \ref{sec:use_cases}).
%     \item \textit{\textbf{The classification style}}: Do you want to explain the behavior of an existing classifier (i.e. do you need an explainable surrogate model)? Or do you want to solve and explain the original classification problem with the explainer? (Cfr. with Subsection \ref{sec:classification_styles}).
%     \item \textit{\textbf{The explanation style}}: Do you want a local explanation for an individual observation? Do you want an explanation for a cluster of samples or for a whole class? Would you like to have an explanation for the behavior of the hidden neurons of the explainer? (Cfr. with Subsection \ref{sec:explanation_styles}).
% \end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTATION REMINDER
%\fg{mettere in tabella es alla fine del 2.1?}
% {\color{red}
% \textbf{Notation}
% X = input space (non-interpretable)\\
% Y = symbolic output space (interpretable)\\
% C = symbolic "concept" space (interpretable)\\
% E = symbolic "rule" space (interpretable)\\

% n = \# samples\\
% d = \# features of X\\
% q = \# categories of Y\\
% k = \# categories of C\\
% r = \# categories of E\\
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DISCORSINO intro su cosa è il nostro modello, cosa fa, a cosa si appoggia.. caratteristiche generali


% Differently from several existing XAI models, 
We consider a general framework in which a special kind of neural network, a LEN, is used to explain the behaviour of another classifier, be it another neural network or any black-box model, or to provide explainable predictions itself. Any LEN can be defined according to certain criteria and exploited in different use cases. This section describes the main aspects on what LENs can be used for and which kind of explanation we may get with LENs.

Let us consider a binary classification problem where, for any input sample $x \in X\subset\mathbb{R}^d$, a black box\footnote{With "black box classifier" we mean that there are no assumptions on the classifier structure. The classifier architecture could be totally unknown to the logic explainer network, that only requires a $[0,1]$-valued I/O.} classifier $g: X \rightarrow Y$ defines the membership values of the input to one or more categories, i.e. $g(x)=(g_1(x),\ldots,g_q(x))\in [0,1]^q = Y$, with $g_i(x)=1$ (resp. $g_i(x)=0$) meaning that $x$ belongs (does not belong) to class $i$.
In a broad sense, a \textit{Logic Explainer Network} for the classifier $g$ can be simply thought of as any neural model $f$ aiming at explaining the decision processes taken by $g$. 
More formally, a Logic Explainer Network (LEN) is a mapping $f: C \rightarrow E$ such that:
\begin{itemize}
    \item any input $c\in C$ consists in a $[0,1]$-valued feature or concept vector, i.e. $C \subseteq [0,1]^k$. $C$ is also said the \emph{concept space}.
    \item $f$ can be any neural model, but it is required that $E\subseteq[0,1]^r$ where, for any $c\in C$, $i=1,\ldots,r$, $f_i(c)=1$   means that the $i$-th explanation holds for $c$, viceversa if $f_i(c)=0$. $f_i$ is sometimes called the $i$-th explainer of the LEN $f$, we refer to $E$ as the \emph{explanation space}.
    % \item there is no pair $c^i,c^j\in C$, such that $\bar{f}(c^i) \neq \bar{f}(c^j)$ and $\bar{c}^i=\bar{c}^j$, where the overline notation denotes the boolean discretization (thresholded at $0.5$) of values from $[0,1]$ to $\{0,1\}$ values.
\end{itemize}

One of the main advantage of the proposed framework is its versatility, indeed a LEN can be defined according to different user-preferences by serving different purposes. In particular, the layout of a XAI pipeline based on LENs follows the definition of a few aspects concerning the classification problem under investigation and the properties of the required explanations. Setting these points allows the correct definition of a LEN in a learning problem. For clear, this is also schematized in Fig. \ref{fig:scheme1}.
% In particular, three  groups of questions needs to be answered in order to correctly define a LEN structure.   

\begin{figure}[h]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme1.png}
    \includegraphics[width=1\textwidth]{figs/lens_1.pdf}
    \caption{Setting up a Logic Explainer Network.}
    \label{fig:scheme1}
\end{figure}

\begin{enumerate}
    \item \textsc{Data \& pipeline. } 
    %  according to the problem at hand, different solutions can be adopted to extract meaningful explanations. 
    % Are you working with unstructured (e.g. images) or structured data (e.g. gene expression)? Do you have annotations for tasks or concepts? Do you need one or more concept bottlenecks?
    LENs can be integrated in different classification problems with different classifier architectures. How the integration will take place depends on the nature of the input data and the presence of one or more concept bottlenecks among the classes under investigation.
    
    \item \textsc{Classification style. }
    % in general, a LEN is employed in order to explain the behavior of an existing classifier (i.e. to create an explainable surrogate model). However, you can also solve and explain the original classification problem with a LEN. Do you need more powerful models or precise explanations?
    LENs can be used either to explain the behaviour of an existing classifier or to solve the classification problem itself. In the latter case, the output of the LEN denotes the final class-assignment.

    \item \textsc{Explanation style. }
    % LEN can provide different kind of explanations, according to user needs. Do you want a local explanation for an individual observation? Do you want an explanation for a cluster of samples or for a whole class? Do you also needs explanations of the behavior of the hidden neurons of the explainer?
    LENs can provide different kind of explanations, according to user needs. In particular, we may be interested in individual explanation, i.e. the explanation of the decision taken by the classifier on a specific sample. However, we may also look for more general explanations, such as explaining the decisions taken for a whole class predictions, or even looking for more abstract relations among the classes.
    
\end{enumerate}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figs/E2E.png}
    \caption{E2E LEN directly works on input data $X$ that is interpretable per se and treated as concepts, i.e. ($C=X$). Here an example on the MIMIC II dataset is reported where patient features and symptoms are used to classify if it will survive 28 days after hospital recovery.}
    \label{fig:E2EExplainer}
\end{figure}

\subsection{Data \& pipeline} 
\label{sec:use_cases}
% In general, we can state that the above assumptions about the input data and the classifier are not always valid. However, in the following we will see how we can apply the LEN framework in different use cases where these conditions hold.
Roughly speaking, a logic explainer network $f$ is simply a function mapping $[0,1]$-values to $[0,1]$-values, with the aim of providing explanations for a classifier $g$ or to provide $f$ itself the final classifications. This very general definition allows the application of LENs to different contexts that can be made consistent with real-unit I/O. We here consider three different scenarios where LENs may be applied: as an end-to-end explainer directly working on structured data; in a concept bottleneck-scenario where low-level concepts are first extracted from unstructured data (e.g. images); as a cascade of explainers providing explanations at different level of granularity.

% \paragraph{End-to-end explainer}
\textsc{End-to-end Explainer. } 
An end-to-end logic explainer network (E2E LEN) is a model aiming at explaining, and eventually solving, a classification problem from real-unit features, i.e. $X=C \xrightarrow[]{f} E$. An E2E LEN assumes that the features of the input space are meaningful individually, i.e. they correspond to human-interpretable concepts. Structured datasets usually fall into this category. Continuous features can be either discretized into different bins or booleanized by comparing them to a reference ground truth (e.g. for gene expression data, the gene signature obtained from control groups can be used as a reference).
% E2E explainers can perform a fully interpretable classification task by replacing the classification model $g$ completely, i.e. $C=X \xrightarrow[]{f} Y=E$ as shown in Fig. \ref{fig:E2EExplainer}, but may also be used to explain the predictions of a separated model $g$, i.e. $C=X \xrightarrow[]{f} g(X)=E$. This will be more extensively discussed in Sec.\ref{sec:classification_styles}.
An E2E LEN can be used to explain the predictions of any black box model $g:X\rightarrow Y$, as shown in Fig. \ref{fig:E2EExplainer}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figs/CBM.png}
    \caption{In the Concept-bottleneck scenario, the LEN is placed on top of a black box model $g$ which maps the unstructured input data $X$ into interpretable concepts $C$. Here the toy MNIST experiments is shown. Handwritten digits are first classified by $g(x)$. A LEN is employed on top to classify and explain whether the digit is even or odd.}
    \label{fig:CMBExplainer}
\end{figure}

% \paragraph{Concept-bottleneck explainer}
\textsc{Concept-bottleneck Explainer. } 
% A concept-bottleneck LEN is a model $f$ collaborating with a black-box $g$ to solve and explain a classification problem where the input features are not meaningful individually, e.g. pixels \cite{koh2020concept}. In this setting, the black-box model is used as an automatic preprocessing for extracting high-level concepts from raw features. The extraction can be either implicit, though the analysis of the latent spaces learnt by the black-box \cite{kazhdan2020cme}, or explicit by training the black-box to classify concepts explicitly \cite{koh2020concept}, i.e. $X \xrightarrow[]{g} C$ as shown in Fig. \ref{fig:CMBExplainer}. Given the concepts extracted from the black-box, the explainer solves and explains the classification problem at a higher level of abstraction, $C \xrightarrow[]{g} E$.
A concept-bottleneck logic explainer network is a model $f$ aiming at explaining, and eventually solving, a classification problem where the input features are either not meaningful individually, e.g. pixels of an image \cite{koh2020concept}, or out of the bounds of the real-unit interval.
In this setting, a black-box model $g$ can be used to automatically extract high-level concepts from raw features, i.e. $X \xrightarrow[]{g^{(1)}} C\xrightarrow[]{g^{(2)}}Y$, with $g=g^{(2)}\circ g^{(1)}$.
The extraction can be either implicit, through the analysis of the latent spaces learnt by the black-box \cite{kazhdan2020now}, or explicit by training the black-box to classify specific concepts \cite{koh2020concept}. Given the concepts extracted from $g$, a LEN $f$ may e.g. explain the classification problem at a higher level of abstraction, i.e. $C \xrightarrow[]{f} E$  as shown in Fig. \ref{fig:CMBExplainer}.
% or even producing itself a solution by assuming $E=Y$.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figs/cascade.png}
    % \caption{A possible structure of a Cascade LEN combined with a Concept Bottleneck model. The model $g$ provides interpretable low-level concepts $C_1$. The level of abstraction of these concepts, however, is not sufficient to correctly explain the classification task Y. Therefore, a further layer of concepts/explainer $C_2 \xrightarrow[]{f_2} Y$ is employed.}
      %\caption{A possible structure of a Cascade LEN combined with a multi Concept Bottleneck model. The model $g$ provides interpretable concepts $C^{(1)},C^{(2)},Y$. Therefore, we may consider a cascade of LENs $C^{(1)} \xrightarrow[]{f^{(1)}} C^{(2)}\xrightarrow[]{f^{(2)}} E$.}
      \caption{Structure of Cascade LEN on the V-Dem classification dataset. The final classification on the status of the democracy is divided into two steps.
    %   $X=C^{(1)} \xrightarrow[]{f^{(1)}} C^{(2)}\xrightarrow[]{f^{(2)}} E$. 
    First the input features $X$ are mapped to high-level concepts $C_2$. %$= f_1(X)$. 
    High-level concepts are then used to classify $Y$. %$= f_2(f_1(X))$. 
    LEN can provide explanations in terms of high level $C_2$ or low-level concepts $C_1$.}
    \label{fig:CascadeExplainer}
\end{figure}

% \paragraph{Cascading explainers}
\textsc{Cascading Explainers. }
Cascading explainers can be used to provide explanations by means of a hierarchy of concept layers. Each explainer is trained on a concept space to predict concepts at a higher level of abstraction which will feed the next explainer $C^{(1)} \xrightarrow[]{f^{(1)}} C^{(2)} \xrightarrow[]{f^{(2)}} C^{(3)}$. The final explainer solves and explains the more abstract classification task $C^{(m)} \xrightarrow[]{f^{(m)}} E$ as shown in Fig. \ref{fig:CascadeExplainer}. This structure provides a hierarchy of explanations and upholds human interventions at different levels of abstraction, providing a far deeper support for human-machine interactions.



\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figs/E2E.png} \quad %\\ \bigskip
    \includegraphics[width=.48\textwidth]{figs/e2e_explaining.png}
    \caption{LENs classification styles:  interpretable classification, where the LEN directly provides the final classification (left), explaining an existing classifier e.g. a black-box model $g$ (right).
    % Classification style: Explaining an existing classifier. Differently from the previous examples, here a LEN is used to explain the predictions made by an existing classifier $g(x)$ on the MIMIC classification task.} 
    \gc{Manca la scritta $g(x)$ sopra la rete grigia nella figura} }
    \label{fig:explainablevsexplanation}
\end{figure}

\subsection{Classification styles} \label{sec:classification_styles}

% Logic explainer networks can be used, as a special case, to provide class-driven explanations. However, the user may decide to use a LEN to explain an existing classifier, but also to perform the classification itself.
In all the previously described cases, LENs are always considered together with a black-box classifier $g$. This is meant because in general, we may want to keep the function $g$ to solve the classification task, while we will use the LEN to explain one or more components $g_i$s of $g$.
For the following description, we assume without loss of generality that $C=X \xrightarrow[]{g} Y$, since in case $X\subset\mathbb{R}^d$, $g$ should have one or more concept bottlenecks, such as $X \xrightarrow[]{g^{(1)}} C\xrightarrow[]{g^{(2)}}Y$. Then, we will may repeat the following arguments with $f_i\circ g^{(1)}$ in place of $f_i$, and $x$ in place of $c$.

\textsc{Explaining an existing classifier. } On one hand, we may train a LEN $f$ to satisfy $f_i\simeq g_i$ for some $i\in\{1,\ldots,d\}$, i.e. to have $f_i(c)$ as close as possible to $g_i(c)$ for any $c\in C$. %We refer to this scenario as \textit{Explaining an existing classifier}.
This solution may be useful in those context where the classification performances play a key role and we may accept approximate explanations of the decision taken. 

\textsc{Interpretable Classification. } However, the LEN can also be used to directly accomplish the classification task. Indeed it can provide an explainable classification by training a LEN $f$ to satisfy $f_i\simeq Y_i$ for some $i\in\{1,\ldots,q\}$, i.e. to have $f_i(c)$ as close as possible to $Y_i(c)$ for any $c\in C$, where $Y_i(c)$ denotes the label of the $i$-th class on the input $c$, that the LEN is meant to both learn and explain. This other solution is instead preferred when it is of fundamental importance to have a white-box classifier, while we can accept some drawbacks in terms of classification performances.
It is worth noticing that in explaining an existing classifier, a LEN may also take into account the classifier predictions on unlabeled data, e.g. in a semi-supervised learning setting.
%This allows the LEN to produce explanations covering a larger set of data, but also possibly inaccurate. On the other hand, in the interpretable classification case the LEN learns explanations directly from (limited to) the labeled data. 


\subsection{Explanation styles}
\label{sec:explanation_styles}
%%%OLD
% Here we illustrate how logic-based explanations can be formally aggregated generating a range of explanations from the characterization of individual observations to formulas explaining clusters of samples up to class-level rules describing model's predictions for all the samples of a target class.

% \paragraph{Local explanations}
% A local explanation provides a description of the model's prediction for an individual observation. A logic-based local explanation consists of a minterm, i.e. a logical formula, with a value of 1 (i.e. \textit{true}), where each literal appears at most once. Such explanations have a precise structure as they correspond to a conjunctive normal form where each clause corresponds to a literal (i.e. a concept). For instance, let us consider a model trained to learn the $XOR$ function, defined by $XOR(0,0)=XOR(1,1)=0$, $XOR(1,0)=XOR(0,1)=1$. Let us assume the model's prediction for the observation $c^i=(0.1,0.8)$ is $\hat{e}^i=0.8$. A local explanation for the prediction might be $\neg c_1 \wedge c_2 \rightarrow e=1$. On the contrary, for the sample $c^j=(0.7,0.2)$ where $\hat{e}^j=0.9$ the explanation may look like $c_1 \wedge \neg c_2 \rightarrow e=1$. When the input space is large, i.e. $k \gg 1$, Occam's razors and pruning strategies can be applied in order to avoid formulas incorporating redundant literals, thus controlling the complexity of local explanations.

% \paragraph{Cluster explanations}
% Logic-based local explanations for different observations can be aggregated through a formal procedure. As outlined in the previous paragraph, the formula obtained for each sample corresponds to a minterm identifying a specific row of a truth table $T$ defined on the input space, i.e. $T \subset [0,1]^k$. Using De Morgan's laws and the material implication, two or more minterms can be formally aggregated in a disjunctive normal form. For instance, the two minterms $\neg c_1 \wedge c_2 \rightarrow e=1$ and $c_1 \wedge \neg c_2 \rightarrow e=1$ can be aggregated into the formula $(\neg c_1 \wedge c_2) \vee (c_1 \wedge \neg c_2) \rightarrow e=1$.

% \paragraph{Class-level explanations}
% Class-level explanations are a special case of aggregated explanations aiming at providing a valid explanation for all the elements of a specific class. The formula can be obtained by aggregating all the minterms corresponding to local explanations of all the observations having the same class label. In theory this procedure may lead to overly long formulas as each minterm may increase the complexity of the explanation. In practice we observe that many observations share the same logic explanation, hence their aggregation will increase the complexity of the class-level formula by a constant factor. In general, class-level explanations can be provided by aggregating just the most common explanations extracted from samples with the same class label, avoiding a sort of "explanation overfitting" with the inclusion of noisy minterms which may correspond to outliers.

% \paragraph{Node-level explanations}
% A deeper level of explanations is given when each node of the network is analyzed and a corresponding logic formula is extracted in terms of input features $h_{11} = c_1 \wedge \neg c_2$. For the nodes in the following layers a compositional strategy is followed, i.e. $h_{21} = h_{11} \vee h_{12} = (c_1 \wedge \neg c_2) \vee (c_2 \wedge c_3)$. This procedure may be repeated until the output nodes which are eventually explained in terms of input features, similarly to Class-level explanations. This strategy leads to the higher level of interpretability, since the behaviour of each node in the network is explained. However, due to the composition of explanations, it prevents the employment of very deep neural network.





Different use cases may require different kinds of explanations with (eventually) different validity supports. For instance, a user may be interested in getting an explanation of a classifier in terms of relations among its classification outputs. However, we may also be interested in explaining a specific class, e.g. with respect to a set of lower-level attributes, like an explanation of the class \textit{person} with respect to the attributes \textit{head, hands, body}. 
Further, the explanation could have a global, local or even example-level validity. For instance, we may be interested in explaining a certain decision for a specific input, but also in universally valid regularities or simply most frequent co-occurrences among classes.
In the following, we briefly discuss the logical explanation styles that are currently supported by the LENs framework. These cases have been also previously discussed in \cite{ciravegna2020human} as different scenarios. In order to train a LEN to produce one %or more 
of the following explanation styles, we can make use of ad hoc learning criteria, as successively discussed in Sec.\ref{sec:learncrit}

% \paragraph{Class-driven explanations}
\textsc{Class-driven Explanations. }
% (local or global); \fg{richiederebbe spiegare, che mentre la LEN è vera esattamente dove la classe che spiega, la formula logica è soddisfatta dovunque.}
Class-driven explanations aim at providing a valid explanation for all the samples of a specific class. This may be achieved by training a LEN to represent different kinds of causalities for a selected class with respect to the other ones, or a set of lower-level concepts. In particular, we will consider the following kinds of implication rules.
\begin{itemize}
    \item 
    \textit{IF-Rules. } This kind of explanation provides a superset of a specific class assignment. For instance, an upper bound containing the class $flies$ can be defined according to the explanation "$flies\rightarrow bird\vee airplane$".
    \item 
    \textit{Only IF-Rules. } In this case an explanation is required to provide a subset of a specific class assignment. A lower bound contained in the class $flies$ may be obtained with the explanation "$has\_wings \ \wedge \ has\_engine\rightarrow flies$".
    \item 
    \textit{IFF-Rules. } An explanation  can completely characterize a certain class. For instance, the class $airplane$ can be defined according to the explanation "$airplane \leftrightarrow has\_wings\wedge has\_engine$".
\end{itemize}
We note that only with IFF-Rules explanations a LEN can be used for interpretable classification. Indeed, not any bird or plane can fly, so as a seagull can fly without having an engine. Hence, IF and Only IF-Rules are not suitable to correctly predict a specific class behaviour.

% \paragraph{Relations among concepts}
\textsc{Relations among Concepts. }
%  (local or global): MI, Conversion to CNF
% \gc{Potrebbe anche essere impiegato in uno scenario E2E dove i cluster sono le regole e le Y, per cui non partirei subito dicendo che si è in un multi-label classification problem (che prevede uno scenario Concept Bottleneck).}
A user may be interested in discovering relations among different concepts or classes without posing any preference on any specific class. For instance, in a multi-label classification problem, with eventually several output classes, it could be interesting to get an explanation of the holding relationships among different classification outputs. 
As an example, the co-occurrences of certain concept activations, like $soccer\_ball \wedge foot$ for a set of football images, may hold only for a (small) portion of the available data. However, we may also look for global explanations, like $zero\vee one\vee\ldots\vee nine$ in a digit classification task.

Not only, even when a completely unlabeled dataset is given, one may still use LENs to perform interpretable clustering. Let's take as an example the case of gene expression analysis where it is difficult to have large numbers of annotated data. Neural networks are usually employed to group similar patients according to their genes activations. LENs can be used to also understand why such groups have been formed and in particular which are the most relevant gene activations in common.

% \paragraph{Explanation Ranges}
\textsc{Explanation Ranges. }
As already mentioned, the explanations may hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrencies or global principles among different classes.
%\fg{aggiungere qualche esempio?}



\section{Methods}
% \section{Formulas, Criteria and Pruning}
\label{sec:methods}

This section presents the fundamental methods that are exploited to extract and ensure the style of a certain logic-based explanation for LENs (see Fig. \ref{fig:scheme2}).
First we illustrate how different loss functions can be optimized to achieve customizable classification and explanation styles. Then, we discuss how first-order logic rules can be extracted from LENs for an individual observation and how explanations can be aggregated to be representative of a cluster of samples. Finally, we provide an overview of some parsimony criteria which can be used to avoid overly complex logic formulas and, in turn, useless explanations.

\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme2.png}
    \includegraphics[width=1\textwidth]{figs/lens_2.pdf}
    \caption{Learning explanations with LENs can be performed according to the above reported methods: (i) learning criteria, (ii) FOL rule extraction, and (iii) parsimony criteria.}
    \label{fig:scheme2}
\end{figure}
%%%%%%%%%%%%%\fg{mettere qualche richiamo di logica al prim'ordine?}
% \textit{`In this paper, we use Classical Propositional Logic (PL) with  the  usual  set  of  logical  connectives $\{\neg,\vee,\wedge\}$.  A Boolean Formula (BF) is a string in the language of the PL. It can be recursively defined as: (i) a literal, which is a variable or a negated variable, (ii) a conjunction, which is a set of BFs separated by $\wedge$, or (iii) a disjunction, which is a set of formulas separated by $\vee$. A Boolean function is the function $f: \{0,1\}^k \rightarrow \{0,1\}$ defined by a Boolean formula. It takes as arguments an assignment for every variable in the formula and returns a value - zero or one - according to the semantics  of  the  connectives  in  the  formula.  An  evaluation  of  a BF is the result of calculating the Boolean function associated with it. A Conjunctive Normal Form (CNF) is a specific type of BF, where the formula is expressed as a conjunction of one or more clauses, which are disjunctions of literals.`}




\subsection{Learning criteria}
\label{sec:learncrit}
%Cross Entropy in genere; Che può essere binary se è single o multilabel, altrimenti Softamx Cross Entropy

As already described in Sec. \ref{sec:explanation_styles}, LENs may provide different kinds of explanation. In the following, we focus on the loss functions that are optimized to train a LEN to represent a certain explanation style. 

% \paragraph{Class-driven Criteria.} 
\textsc{Class-driven Criteria. } 
In the case of \emph{Class-driven Explanations}, we aim at providing explanations of certain classes. In this sense, we want our explainer $f$ to be active whenever the class we aim to explain is also active.
% (i.e. $f_i(c) = Y_i(c) = 1$)
We do not distinguish here whether the LEN is performing an \textit{interpretable classification} ($f_i\simeq Y_i$) or it is \textit{explaining an existing classifier} ($f_i \simeq g_i$), since for what concerns the optimization function it does not make any difference. \gc{Questa frase non è più vera credo, le ottimizzazioni IF and Only IF non possono essere utilizzate nel caso di interpertable classification} 
Let us assume the case of explaining an existing classifier\footnote{The interpretable classification case can be obtained by replacing $g_i$ with $Y_i$ in the loss functions.} $g$. Further, for sake of simplicity, in what follows we will assume $C=X\xrightarrow[]{g} Y$.


According to whether we want to extract IF, Only IF or IFF rules, different losses need to be optimized. In particular, IF rules like $\bar{g}_i \rightarrow \bar{f}_i$  require the support of the antecedent to be included in the support of the consequent (i.e. $\{c\in C: \bar{g}_i(c)=1\}\subseteq C_i$). This behavior can be achieved by minimizing a Hinge loss:
\begin{equation}
L_{\rightarrow}(g_i,f_i,C) = \sum_{c\in C} \max\{0, g_i(c)- f_i(c)\}\qquad  i \in [1,  r].\label{eq:IF}
\end{equation}
In the same way, we may be interested in Only IF rules like $\bar{f}_i\rightarrow\bar{g}_i$. This may the case in which a class is explained in terms of lower-level concepts. This is easily achieved by switching the two terms of the loss function in Eq. \ref{eq:IF}:
\begin{equation}
L_{\leftarrow}(g_i,f_i,C) = \sum_{c\in C} \max\{0, f_i(c) - g_i(c)\}\qquad  i \in [1,  r].\label{eq:IF2}
\end{equation}
At last, LEN can learn double implication rules (IFF), such as $\bar{f}_i \leftrightarrow \bar{g}_i$. These rules require the support of the explainer and the support of the class to be strictly equal. For this reason, any function penalizing points for which $f_i(c)\not=g_i(c)$ may be employed in this scenario, such as the Mean Square Error
\begin{equation}
L_{\leftrightarrow}(g_i,f_i,X) = \sum_{c\in C} |f_i(c) - g_i(c)| \qquad  i \in [1,  r], 
\end{equation}
or the classic Cross Entropy loss. In this latter case if we want the same LEN to explain different, mutually exclusive classes, a Softmax activation function can be also employed.  

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/concept_relations.pdf}
    \caption{Relations among concepts in a Concept-bottleneck pipeline again on the MNIST EVEN/ODD dataset. Concepts are first extracted by means of the $g(x)$ network. A LEN on top of it clusterize these concepts to analyze the relations among them.}
    \label{fig:concept_relations}
\end{figure}

\textsc{Relations among Concepts. }
% \paragraph{Mutual Information Criterion}
% \paragraph{Relations among Concepts.}
LENs can also learn rules which only take into consideration the relationships among concepts or final classes. This can be achieved by means of Information theory principles. As a matter of fact, the maximization of the Mutual Information (MI) index between the concept $C$ and the explanation $E$ spaces allows the outputs of the LEN $f$ to
be trained in a fully unsupervised way. More in details, it leads to mutually exclusive configuration such that $\forall c \in C$ only one $f_i(c) = 1$, while the others are close to zero \cite{melacci2012unsupervised}.

In order to define the MI index, we introduce the probability distribution $P_{E=i|C=c}(f)$, for all $i$, as the probability of $f_i$ to be active on $c$. Following the classic notation of discrete MI, 
$E$ is a discrete random variable associated to the set of explainer functions while $C$ is the variable related to the data in the concept space.\footnote{We implemented the probability distribution using the softmax operator, scaling the logits with a constant factor to ensure that when $f_i(x)=1$ all the other $f_{j\neq i}(x)=0$.}
 The penalty term to minimize is minus the MI index, that is
\begin{equation}
    L_{MI}(f,C) = - H_{E}(f,C) + H_{E|C}(f,C) \ ,
	\label{eq:MI}
\end{equation}
where $ H_{E}$ and $ H_{E|C} $ denote respectively the entropy and the conditional entropy functions associated to the aforementioned probability distribution and measured over the whole $C$. 
%An outcome of the maximization of the MI index is that the supports of the explaining functions will tend to partition the input space $X$, i.e., $X=\bigcup_{j=1}^mX_j$ and $X_j\cap X_k=\emptyset$, for $j\neq k$ (see \cite{melacci2012unsupervised,betti2019cognitive} for further details).

\textsc{Explaining an existing Classifier. }
\gc{questo titolo è leggermente fuorviante secondo me, uno si aspetterebbe di trovare la loss da ottimizzare quando spieghi un classificatore. Inoltre si fa il training della $g$ anche facendo interpretable classification in CBM} 
In the particular case of a LEN aiming at providing an explanation for an existing classifier $g$, the available supervision on $g$ will be enforced as well, e.g. by means of the cross-entropy loss, in the learning problem. Furthermore, the explanations provided by LENs are first-order logic formulas, and this newly devised pieces of knowledge can be reused and enforced on the output of the classifier $g$. This is commonly considered in the generic \emph{learning from constraints} framework \cite{gnecco2015foundations}, and it may be of particular interest, especially for semi-supervised settings. A similar strategy has already been considered e.g. in \cite{ciravegna2020constraint}, where a set of FOL formulas have been, at first extracted from data, and then converted into continuous loss functions to be injected in the learning objective.


\subsection{First-order logic rule extraction}
\label{sec:logic_rule_extr}
Any logic explainer network $f=(f_1,\ldots,f_r)$ requires both its inputs and outputs to belong to the real-unit interval. This apparent limitation allows any $f_i$, for $i=1,\ldots,r$, to be easily converted into a boolean function $\bar{f}_i$, e.g. by thresholding its I/O, e.g. with respect to $0.5$ value. Therefore, any boolean function $\bar{f}_i$ is converted into a FOL formula $\varphi_i$ in Disjunctive Normal Form (DNF) \cite{mendelson2009introduction} by means of its truth-table, see e.g. Fig. \ref{fig:tt2form}.
Given $C \xrightarrow[]{f} E$, we can define for any $i$ the set $C_i = \{c\in C:\ \bar{f}_i(c)=1\}$ as the set of all the $[0,1]$-valued concept tuples that make true the $i$-th explanation, i.e. the \emph{support} of $\bar{f}_i$. For instance, if we are interested in class-driven explanations only, i.e. $E=Y$, any $C_i$ will generally consist in the set of inputs that are classified as belonging to the $i$-th class by the LEN $f$.

% \paragraph{Local Explanation}
% \paragraph{Example-Level Explanation}
\textsc{Example-level explanation. }
Given $c=(c_1,\ldots,c_k)\in C_i$, the booleanization of its continuous values may provide a natural way to get a logical explanation at example-level $\varphi_{i,c}$ as a FOL formula. In particular, for any $c\in C_i$, we can consider the following as the \emph{Local Explanation} of the $i$-th explainer $f_i$ on example $c$. 
\begin{equation}
    \varphi_{i,c} = \tilde{c}_1\wedge\ldots\wedge\tilde{c}_k \qquad\mbox{where } \tilde{c}_j:= 
    \begin{cases}
        \bar{c}_j, & \mbox{if }c_j \geq 0.5\\
        \neg \bar{c}_j, &\mbox{if } c_j < 0.5\\
    \end{cases}\ ,    
    \mbox{ for $j=1,\ldots,k$.}
    \label{eq:locexp}
\end{equation}
\begin{figure}[t]
\centering
    \includegraphics[width=0.9\textwidth]{figs/truth-table.png}
    \caption{Extracting a logic formula from the truth-table of a binary boolean function $\bar{f}_1$.}
    \label{fig:tt2form}
\end{figure}
% \paragraph{Aggregated Explanation}

\textsc{Aggregated explanation. }
By considering Eq. \ref{eq:locexp} for any $c\in S$, and aggregating all the example-level explanations, we may easily provide a \emph{Cluster Explanation} $\varphi_{i,S}$ for a subset of samples $S \subseteq C_i$ as
\begin{equation}
    \varphi_{i,S} = \displaystyle\bigvee_{c \in S}\varphi_{i,c} = \displaystyle\bigvee_{c \in S}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_k
\label{eq:agg_exp}
\end{equation}
Any formula $\varphi_{i,S}$ can be thought of as a $\{0,1\}$-valued mapping defined on $C$, that is equal to 1 exactly on a cluster $S \subseteq C_i\subseteq C$. We may also get an explicit explanation relating $\varphi_{i,S}$ and the $i$-th explainer $f_i$ by the FOL formula:
\[
\forall c\in S:\ \varphi_{i,S}(c)\rightarrow \bar{f}_i(c)
\]

% \paragraph{Global Explanation}
% \paragraph{Class-Level Explanation}
\textsc{Class-level explanation. }
By considering Eq. \ref{eq:agg_exp} with $S=C_i$, i.e. aggregating all the example-level explanations, we get an overall explanation $\varphi_i$ for the explainer $f_i$.
\begin{equation}
    \varphi_i = \displaystyle\bigvee_{c \in C_i}\varphi_{i,c} = \displaystyle\bigvee_{c \in C_i}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_k
\label{eq:glo_exp}
\end{equation}
Also in this case, any formula $\varphi_i$ can be thought of as a $\{0,1\}$-valued mapping defined on $C$, that is equal to 1 exactly on $C_i\subseteq C$. We may get as \emph{Global Explanation} a FOL formula relating $\varphi_i$ and the $i$-th explainer $f_i$ by means of:
\[
\forall c\in C:\ \bar{f}_i(c)\leftrightarrow\varphi_i(c)
\]

% RECURSION\_STEP
% \paragraph{Compounding Explanations}
\textsc{Compounding explanations. }
Both example-level, aggregated and class-level explanations can be recursively applied in case a cascading explainer or a single explainer with multiple $[0,1]$-valued layers are considered. For instance, given a cascade LEN $C^{(1)}\xrightarrow[]{f^{(1)}} C^{(2)} \xrightarrow[]{f^{(2)}} E$, we may get both local and global explanation of the concepts in $C^{(2)}$ with respect to the ones in $C^{(1)}$, so as the concepts in $C^{(3)}$ with respect to the ones in $C^{(2)}$ and, in turn, in $C^{(1)}$. The modularity  of formulas allows the composition of concepts at different levels that may express arbitrary complex relationships among them.


% \paragraph{Aggregation of Cluster-Level Explanations}
\textsc{Aggregation of cluster-level explanations. }
We note that in case the mutual information criterion (Eq. \ref{eq:MI}) is adopted in the learning formulation, any $\varphi_i$ will generally hold on a sub-portion of the concept space $C_i\subseteq C$. However, we may get a FOL providing a global explanation by means of the disjunction
$\varphi = \varphi_1\vee\ldots\vee\varphi_r$, indeed $C_1\cup\ldots\cup C_r=C$. Since the formula $\varphi$ can be very complex, if we are interested in simpler global explanations we may  convert $\varphi$ into an equivalent $\varphi'$ in \emph{Conjunctive Normal Form} (CNF). In particular, there exist $r'$ and clauses $\varphi'_1,\ldots,\varphi'_{r'}$ such that: 
\[
\varphi=\bigvee_{i=1}^r\varphi_i \equiv \bigwedge_{i=1}^{r'}\varphi'_i=\varphi'.
\]
As a result, we get the following global explanations for $i=1,\ldots,r':
\forall c\in C:\ \varphi'_i(c)$.
Unfortunately, converting a boolean formula into CNF can lead to an exponential explosion of the formula; in the following, we will see how to address this problem. 
% However, after having converted each $\varphi_i$ in CNF, the conversion can be computed in polynomial time with respect to the number of minterms in each $\varphi_i$ \cite{russell2016artificial}.

\begin{example}
\label{ex:xor}
Let's consider the boolean $xor$ function, defined by $xor(0,0)=xor(1,1)=0$, $xor(1,0)=xor(0,1)=1$. 
Let $f$ be a LEN that has been trained to approximate the $xor$ function in the input space $C=[0,1]^2$. Then, if we consider e.g. the inputs $c^1=(0.2,0.7)$, $c^2=(0.6, 0.3)$, we get $\bar{c}^1=(0,1)$, $\bar{c}^2=(1,0)$, and therefore $\bar{f}_1(c^1)=\bar{f}_1(c^2)=1$. These examples yield respectively the local explanations $\varphi_{1,c^1}=\neg \bar{c}_1\wedge \bar{c}_2$ and $\varphi_{1,c^2}=\bar{c}_1\wedge\neg \bar{c}_2$, and the class-level explanation for $f_1$ is given by $\varphi_i=(\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)$. In the same way, we may get the class-level explanation for the explainer $f_0$. In the end, the following formulas represent the class-driven explanations of the false and true classes, respectively:
\[
\forall c:\ \bar{f}_0(c)\leftrightarrow (\neg \bar{c}_1\wedge\neg \bar{c}_2)\vee(\bar{c}_1\wedge \bar{c}_2)\qquad\mbox{and}\qquad
\forall c:\ \bar{f}_1(c)\leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)
\]
The two global explanations correctly match the truth table of the boolean $xor$ function.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figs/truth-table-counter.png}
    \caption{Aggregation of concept tuples with the same booleanization yields a common example-level explanation, and do not complicate the class-level explanation. For any example-level explanation, we may count how many samples it explains. Infrequent explanations may then be pruned to avoid explanation overfitting.}
    \label{fig:tt2form_freq}
\end{figure}

% If we then consider that $f$ is composed of two hidden and one output neurons, we may want to explain the behaviour of each node. In particular, we may get that the first hidden neuron is represented by $ \tilde{h}_1^1  \leftrightarrow \neg \textit{c}_1\wedge \textit{c}_2$ 
% while the second $ \tilde{h}_2^1  \leftrightarrow \textit{c}_1\wedge \neg \textit{c}_2$. The output neurons $h^2 = f$ can be also represented in terms of the hidden neurons $f \leftrightarrow h_1^1 \vee h_2^1$ which in turns can be described again in terms of input concepts $f \leftrightarrow (\neg \textit{c}_1\wedge \textit{c}_2) \vee ( \textit{c}_1\wedge \neg\textit{c}_2)$.

\end{example}

% \paragraph{Remarks}
The method described so far illustrates how logic-based explanations can be formally aggregated to produce a range of explanations, from the characterization of individual observations to formulas explaining the model predictions for all the samples of a target class.
The formula for a whole class can be obtained by aggregating all the minterms corresponding to local explanations of all the observations having the same class label.
In theory, this procedure may lead to overly long formulas as each minterm may increase the complexity of the explanation. In practice, we observe that many observations share the same logic explanation, hence their aggregation does not change the complexity of the class-level formula (Figure \ref{fig:tt2form_freq}). In general, class-level explanations can be provided by aggregating just the most common explanations extracted from samples with the same class label, avoiding a sort of "explanation overfitting" with the inclusion of noisy minterms which may correspond to outliers. To summing up, a possible limitation of this naive approach can be the readability of the logical rules, for instance in case (i) the number of input features (the length of any minterm) $d \gg 1$, (ii) the size of the support $|C_i|$ is very large (possibly getting too many different minterms for any $f_i$). For these reasons, possible approaches to maintain an easy-to-understand set of very concise logical rules are fundamental to provide an useful explanation, e.g. as decision support. More details on how to select the most meaningful explanation terms are provided in Sec. \ref{sec:parsimony}.



\subsection{Parsimony criteria} \label{sec:parsimony}
When humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one \cite{aristotlePosterior,mackay2003information}. Over the years, researchers have proposed many approaches to integrate "\textit{the law of parsimony}" into learning machines.
Here we describe a few fundamental parsimony criteria which may help in developing and implementing a variety of Logic Explainer Networks. A specific combination of the following methodologies may be adopted or ignored depending on end-user requirements on the explanations and on the classification performance.

% \subsubsection{Occam's razors}
% \paragraph{Occam's razors}
\textsc{Occam's Razors. }
Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous techniques to put in practice the Occam's razors principle in the fields of statistics and machine learning.
Among such techniques, $L1$-regularization \cite{santosa1986linear} has been recently shown quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages weight sparsity \cite{tibshirani1996regression}:
% \begin{equation}
    $\lambda ||W||_1$.
% \end{equation}
By shrinking the less important weights %'s values 
to zero, this regularization technique completely removes some weights %altogether in the limit, 
leading to sparse configurations. This allows to ignore the associated input features and, therefore, to provide simpler explanations. For this reason, all out-of-the-box LENs presented in the next section are trained using this parsimony criterion.

\subsubsection{Pruning strategies}
The action of parsimony criteria, such as regularizers or human priors, influences the learning process %of learning machines 
towards specific local minima. Once the model has finally converged to the desired region of the optimization space, the effort can be speed up and finalized by pruning the neural network \cite{lecun1989optimal,hassibi1993second}. The pruning strategy has a profound impact both on the quality of the explanations but also on the learning capacity model and, as a result, on the classification performance as well \cite{frankle2018lottery}. Here we present two effective pruning strategies specifically devised for LENs.

% \paragraph{Node-level pruning}
\textsc{Node-level pruning. }
A straightforward approach to pruning consists in defining the maximum \textit{fan-in} (number of non-pruned connections) for each neuron of a feed-forward neural network. We refer to this strategy as \textit{Node-level pruning}.
%A fan-in pruning strategy generates a feed-forward graph where each neuron has the same number of incoming non-pruned connections. 
At the end of the training process, the absolute value of the weight matrix $W_i$ is computed for each layer $i=1,\dots,L$. 
The node-level approach prunes one by one the weights with the smallest absolute value, such that each neuron in the network has a fixed number of incoming non-pruned weights $q \geq 2$. The parameter $q$ must be decided a priori and determines the learning capacity of the pruned model as well as the complexity of the logic formulas which can be extracted. To get reasonably simple explanations, the parameter $q$ may range between $2$ and $9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Recent work on explainer networks has shown how node-level pruning strategies may lead to fully explainable models  \cite{ciravegna2020constraint}. However, we will show in the experimental section that this pruning strategy strongly reduce the classification performances.

% \paragraph{Network-level pruning}
\textsc{Network-level pruning. }
In order to overcome the heavy reduction of the learning capacity of the node-level pruned models, we introduce here the \textit{Network-level pruning}. 
Indeed, the main aim of pruning is to only reduce the number of input terms involved in the final explanations. By directly limiting the number of input features considered by the network, we can achieve this result with a lighter impact on the overall model. 
Once the network has converged, the Frobenius norm of the first-layer weight matrix $W_1$ is computed: $w_1 = ||W_1||_2$. The vector $w_1$ is then re-scaled in the interval $[0,1]$:
\begin{equation}
    w_1' = \frac{w_1}{\max w_1}
\end{equation}
In this way, $w_1'$ gives a normalized score to rank input feature by importance. The \textit{Network-level strategy} consists in pruning all the input features where $w_1' < w_t$, where $w_t$ is a threshold set a priori (usually $w_t = 0.5$). Alternatively, %the $\mu$ approach may 
we can also retain the $q$ most important input features and prune the others for the entire first layer, as done in the \textit{Node-level pruning} for each single node. %The parameter $q$ is user-defined and may range between $2$ and $9$ to get sensibly compact explanations \cite{miller1956magical,cowan2001magical,ma2014changing}. 
This pruning strategy is far less stringent compared to the node-level pruning as it affects only the first layer and it does not prescribe a fixed fan-in for each neuron.

% \paragraph{ReLU pruning}
% \paragraph{Example-level Pruning}
\textsc{Example-level pruning. }
Example-level pruning is a particular strategy exploiting the well-studied local linearity property of neural networks whose activation functions in all hidden layers are Rectified Linear Units (ReLu Networks) \cite{hahnloser2000digital}. 
% \paragraph{Local Linearity}
For any input $x \in \mathbb{R}^d$, the initial Directed Acyclic Graph (DAG) ${\cal G}$ describing the structure of a ReLu Network, is reduced to ${\cal G}_{x}$,
which only keeps the units corresponding to active neurons and the corresponding arcs (firing path). 
Since all neurons operate in ``linear regime'' (affine functions), as stated in the following, 
the transformation $z: X \rightarrow Y$, which  is the composition of affine functions, corresponds to a single affine function $f^*(x) = W x + b$. 
\begin{theorem}
	Let $\{h_1,\ldots,h_L \}$ a collection of affine functions, where
% 	\[
		$h_{i}: X_{i} \mapsto Y_{i}: x \mapsto W_{i} x + b_{i}$
% 	\]
	and $\forall i=1,\ldots, L-1: \ \ X_{i+1} \subset Y_{i}$, then, 
% 	\[
		$z(x) = h_{L} \circ h_{L-1} \circ \dots \circ h_{2} \circ h_{1} x.$
% 	\]
	is affine and we have $f^*(x) = W x + b$, where
	\begin{equation}
	    W(L) = \prod_{\kappa=1}^{L} W_{\kappa}, \qquad 
		b(L) = \sum_{\kappa=0}^{L-1}  b_{L-\kappa} \prod_{h=0}^{\kappa} W_{L-h+1}  
	\end{equation}
	and $W_{L+1}:=I$.
	\label{theorem:affine}
\end{theorem}

Therefore, for a given input $x$ an affine function $f^*(x)$ can be devised. Notice that Theorem \ref{theorem:affine} only requires hidden layers node to be equipped with a ReLU activation function: nor the input nor the output nodes needs to employ it. %On the contrary, output nodes may be equipped with a sigmoid activation for binary or multi-label classification or a softmax activation function in case of multiclass.
Since the function $f^*(x)$ is affine, its interpretation is already much easier than considering the initial deep network $f(x) = h_{L} \circ h_{L-1} \circ \dots \circ h_{2} \circ h_{1} x$. Indeed, for each sample we can calculate the Frobenius norm of the corresponding weight matrix $w_L = ||W(L)||_2$. At last, similarly to what is done in the network-level pruning, we can retain the most important input features which satisfy $w'_L > w_t$, where again $w'_L = \frac{w_L}{\max w_L}$ and $w_t$ is set to 0.5. 

% \subsection{Discussion}
% {\color{red} DA RIEMPIRE CON ESEMPI}


% \begin{itemize}
%     \item $\psi$ networks
%         \begin{itemize}
%             \item Assumptions: wild pruning sigmoid activations
%             \item Properties of explanations: local or global explanations, modular formulas
%             \item Limitations: poor accuracy, formula explosion
%         \end{itemize}
%     \item ReLU networks
%         \begin{itemize}
%             \item Assumptions:ReLU activations, high|w|+ pruning
%             \item Properties of explanations: closest decision boundary, local or global explanations as before
%             \item Limitations: high|w|, explanations worse than pruning
%         \end{itemize}
%     \item General NN
%         \begin{itemize}
%             \item Assumptions: feature importance (e.g.  LIME or L1-norm) + pruning, no assumption on the network structure
%             \item Properties of explanations: local explanations and global explanations
%             \item Limitations: logical explanation given in terms of I/O only
%         \end{itemize}
% \end{itemize}

% \section{Related work} \label{sec:related}



\section{Out-of-the-box LENs}\label{sec:outofthebox}


Crafting state-of-the-art fully interpretable models is not an easy task; rather, there is a trade-off between interpretability and performances.
The proposed framework is designed to provide the building-blocks to create a wide range of models having different interpretability-VS-accuracy
% interpretability-VS-explainability-VS-performance
trade-offs.
Here, we show how to combine the methods presented in the previous section to design three different out-of-the-box LENs (Figure \ref{fig:out-of-the-box}): a) the $\psi$ network, as proposed in \cite{ciravegna2020constraint} which is a fully interpretable model with limited learning capacity and providing mediocre explanations; b) the $\mu$ network, a neural model providing high-quality explanations, great learning performances and modest interpretability;  c) the ReLU network, a black box model ensuring state-of-the-art learning performance and good explanations at the cost of very low interpretability. The characteristics of these three LENs are also resumed in Tab. \ref{tab:LENs}.


\begin{table}[ht]
\centering
\caption{Out-of-the-box LENs summary.}
\label{tab:LENs}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{LEN}                            & \textbf{Pruning strategy} & \textbf{Activation}  & \textbf{Learning}  & \textbf{Explanation}   & \textbf{Interpretability}\\
\midrule

$\psi$ Network (Fig. \ref{fig:psi_net}) & Node-level        & Sigmoid                       & Low                           & Low                               & Very high     \\
$\mu$ Network (Fig. \ref{fig:mu_net})   & Network-level     & Any                           & High                          & Very high                         & High          \\
ReLU Network (Fig. \ref{fig:relu_net})  & Example-level     & ReLU                          & Very high                     & High                              & Low           \\

\bottomrule
\end{tabular}
}
\end{table}


\begin{figure}[ht]
    \centering
     
     \begin{subfigure}{1\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth]{figs/psi_nn.png}
         \caption{$\psi$ network.}
         \label{fig:psi_net}
     \end{subfigure}\\
     
     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/mu_nn.png}
         \caption{$\mu$ network.}
         \label{fig:mu_net}
     \end{subfigure}
     \qquad
     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/relu_nn.png}
         \caption{ReLU network.}
         \label{fig:relu_net}
     \end{subfigure}
     
    \caption{Out-of-the-box LENs. (a) $\psi$ networks only admit $[0,1]$-valued neurons with low fan-in, hence we can associate a boolean formula to each neuron by analysing its I/O truth-table. (b) $\mu$ networks do not have interpretable hidden neurons but the input concepts are drastically pruned which allows to provide simple network-level explanations. (c) ReLU networks supply explanations for each sample by means of the equivalent affine transformation. However, nor the nodes, nor the network can be logically interpreted.
    \fg{mancano i segnati sulle $c_i$?}}
    \label{fig:out-of-the-box}
\end{figure}

\subsection{The $\psi$ network} 
A $\psi$ network is a Logic Explainer Network already proposed by \cite{ciravegna2020constraint,ciravegna2020human}. A $\psi$ network is based on three design principles: 
(i) all activation functions for all neurons (including hidden units) should be Sigmoid;
(ii) a strong L1-regularization is used in all layers to shrink the less important weight's values towards zero;
(iii) a Node-level pruning strategy, where each neuron of the network must have the same number of incoming non-pruned weights (suggested values are between 2 and 9). This number is directly proportional to the number of terms involved in the explanations. 
Also the number of hidden layers in the network needs to be set carefully, since the number of terms exponentially grows with the number of layers. 
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.24]{figs/psi_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
The typical use case presented in the original work is a concept-bottleneck scenario. A black-box model $g$ (e.g. a convolutional neural network) is used to predict a set of categories $C$ from an unstructured data set $X$ (e.g. images). The authors used a $\psi$ network to explain the behaviour of the classifier $g$, i.e. $C \xrightarrow[]{f} g(X)$. The $\psi$ network is specifically designed to be a fully interpretable neural network, therefore, here we also show its performances as a classifier in different contexts. It can provide the whole set of logic-based explanations: example-level, aggregated, class-level, and it is the only LEN providing also compounding node by node explanations. As a matter of fact, thanks to the node-level pruning strategy, the $\psi$ network allows to interpret (and extract a corresponding logic formulas) from each node. 

Recalling Example \ref{ex:xor}, a $\psi$ network with two hidden nodes may learn the logic formula 
\begin{equation}
\forall c:\ \bar{f}_1(c)\leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2),
\label{eq:xor}
\end{equation}
with hidden nodes learning $h_1(c) \leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)$, $h_2(c) \leftrightarrow ( \bar{c}_1\wedge \neg\bar{c}_2)$ and output node $f_1 \leftrightarrow h_1 \vee h_2$.
A $\psi$ network can be seen as a Cascade Explainer where each layer corresponds to a new level of explainer. However, the network is always trained as a whole since no symbolic concept is provided at each level. Furthermore, also the explanations are always given in terms of input features for this reason. 
As reported in Fig. \ref{fig:psi_net}, this network provides the highest level of interpretability since the $\psi$ network provides for an explanation of the behaviour of each neuron. 
On the contrary, the strong regularization and the restrictive pruning strategy lead to poor classification accuracy making $\psi$ networks hard to train and not suitable for solving complex classification problems. Besides, the provided explanations can be very expressive but they can be not outstanding as expected, due to the limited learning performance. 

\subsection{The $\mu$ network} 
A $\mu$ network is a LEN based on a standard multi-layer perceptron. A $\mu$ network is based on two design principles:
    (i) a strong L1-regularization is used only in the first layer of the network;
    (ii) a Network-level pruning strategy, which only prune the  neurons (features).
After the pruning step, the $\mu$ network can be fine-tuned to adjust to the new configuration. No assumption need to be made nor on the hidden layers nor on the activation functions. However, by applying a Network-level strategy, the same set of retained features is used for the whole network. On the one side, this allows to logically-interpret the network and, therefore, to provide explanations. On the other side, this may represent a severe limitations for multi-class classification since each class may rely on few features, but these may be very different between each class. Therefore, in the multi-class experiments of Sec. \ref{sec:experiments}, we train a set of light binary $\mu$ networks, one for each class. 

%This LEN can provide a wide range of logic-based explanations (i.e. local, cluster, and class-level).
%For each $\mu$ network, an explanation is provided in terms of the input concepts. 
Recalling Ex. \ref{ex:xor}, a $\mu$ network with variable number of hidden layers, may learn the logic formula in \ref{eq:xor}.
The Network-level strategy in this case should not prune any input features since both $c_1$ and $c_2$ are important for the final classification. In case instead also some redundant features are present, they are discard in favor of $c_1$ and $c_2$ as shown in Fig. \ref{fig:mu_net}. 
%As described in Sec. \ref{sec:logic_rule_extr} 
For some points the network will learn the aggregated explanations:
\begin{equation}
\forall c \in S_1: \neg c_1 \wedge c_2 \rightarrow f_1(c) \quad \text{and} \quad \forall c \in S_2: c_1 \wedge \neg c_2 \rightarrow f_1(c). 
\end{equation}
The two explanations can be then considered altogether to explain the class $C_1$: 
\begin{equation}
\forall c\in C:\ \bar{f}_1(c)\leftrightarrow\varphi_1(c) = \bigvee_{c \in C_i}\varphi_{i,c} =
 (\neg \bar{c}_1\wedge \bar{c}_2) \vee ( \bar{c}_1\wedge \neg\bar{c}_2).
 \label{eq:mu}
\end{equation}

Thanks to the permissive pruning strategy, the learning capacity of the network remains intact for the most part. As a consequence, $\mu$ networks are suitable for solving and explaining more complex classification problems. The quality of the explanations provided by the $mu$ networks are among the higher between the proposed models. At last, a mild-level of interpretability is also guaranteed since it can be logically interpreted at a network-level. 

\subsection{The ReLU network} Another example of LEN which provides a different accuracy-vs-interpretability trade-off is the ReLU network. %is a special case of a $\mu$ network sharing most of its characteristics but with a few different properties. 
It is based on three design principles:
    (i) all activation functions for all \emph{hidden} neurons are rectified linear units;
    (ii) a mild L1-regularization in all layers of the network;
    (iii) an Example-level pruning strategy, i.e. a specialized pruning strategy for each sample.
The pruning employed in this LEN is an example-level pruning, which is available since it employs rectified linear units activation functions. %, i.e. a pruning strategy which is applied for each sample. 
This is not a limitations since it is one of the most widely used and efficient activation functions employed in deep learning \cite{glorot2011deep,ramachandran2017searching}.
On the contrary, this pruning strategy, does not cut the connections of the explainer $f$ as it is applied on the affine function $f^*$ directly to get a custom explanation for each observation. This means that the original capacity of the explainer is fully preserved, eventually leading to state-of-the-art classification performances. However, this type of pruning does not provide any insights of the model behaviour and may not always lead to optimum explanations.

Recalling again Example \ref{ex:xor}, a ReLu network with variable number of hidden layers, may learn the correct logic formula by aggregating local examples as it is done in \ref{eq:mu}. However, the local explanations of a certain point $c$ may not be as correct as the ones provided by the $\mu$ networks. Indeed, it can be demonstrated that the corresponding affine function $f*$, actually corresponds to the nearest decision boundary to the points. 
% On the other hand, an example-based pruning strategy may be provide more unstable explanations as the pruning may be negatively affected by the presence of outliers.
Therefore, the corresponding weights may miss some important features to explain $c$. A Relu network sometimes may explain the XOR problems with the wrong formula:
\begin{equation}
\forall c\in C:\ \bar{f}_1(c)\leftrightarrow\varphi_1(c) = \bigvee_{c \in C_i}\varphi_{i,c} =
 (\neg \bar{c}_1) \vee (\neg\bar{c}_2).
\end{equation}
Summing up, this LEN does provide the best performances in terms of classification accuracy thanks to the example-level pruning strategy. However, this comes at the cost of null model interpretability and mild explanation capacity. 
% 

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figs/relu_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


\section{Benchmarking out-of-the-box LENs} \label{sec:experiments}
In this section, we quantitatively assess the quality of the explanations and the performance of Logic Explainer Networks compared to state-of-the-art white-box models. Each task is uniquely defined by the tuple "pipeline / classification style / explanation style". The summary of each task is reported in Table \ref{tab:datasets}.
A brief description of each task, the corresponding dataset and all the related experimental details are exposed in Subsection \ref{sec:exp_details}. In Subsection \ref{sec:exp_metrics} six quantitative metrics are defined and used to compare LENs with state-of-the-art methods.

\begin{table}[ht]
\centering
\caption{Experiments.}
\label{tab:datasets}
\resizebox{\textwidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Data \& Pipeline} & \textbf{Classification style} & \textbf{Explanation style} & \textbf{Dataset} \\
\midrule

End-to-end explainer  & Interpretable classification & Class-driven & MIMIC-II (Fig. \ref{fig:E2EExplainer}) \\
Concept-bottleneck explainer  & Interpretable classification & Class-driven & MNIST (Fig. \ref{fig:CMBExplainer})\\
Concept-bottleneck explainer  & Interpretable classification & Class-driven & CUB (Fig. \ref{fig:len}) \\
Cascading explainers  & Interpretable classification & Class-driven & V-Dem (Fig. \ref{fig:CascadeExplainer}) \\
End-to-end explainer  & Explaining black box & Class-driven & MIMIC-II (EC) (Fig. \ref{fig:explainablevsexplanation}) \\
Concept-bottleneck explainer  & - & Concept relations & MNIST (Fig. \ref{fig:concept_relations}\\

\bottomrule
\end{tabular}
}
\end{table}


% \subsection{Software tool and usability}
% \label{sec:tool}
In order to make the LENs framework accessible to the whole community, we released of a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on methods and out-of-the-box LENs. The Python code and the scripts used for the experiments, including parameter values and documentation, is freely available under Apache 2.0 Public License from a GitHub repository\footnote{\url{https://github.com/pietrobarbiero/deep-logic}}.

The Deep Logic library is designed to make out-of-the-box LENs accessible to researchers and neophytes by means of intuitive APIs requiring only a few lines of code to train and get explanations from an explainer (as shown in the code example \ref{code:example}).

\begin{lstlisting}[language=Python, label=code:example, caption=Example on how to use the Deep Logic library.]
import deep_logic as dl

# import train, validation and test data loaders
[...]

# instantiate a mu network
model = dl.models.MuNN(n_classes=n_classes, n_features=n_features,
                       hidden_neurons=[200], loss=torch.nn.CrossEntropyLoss(), 
                       l1_weight=0.001, fan_in=10)

# fit the model
model.fit(train_data, val_data, epochs=100, l_r=0.0001)

# get predictions on test samples
outputs, labels = model.predict(test_data)

# get first-order logic explanations for a specific target class
target_class = 1
formula = model.get_global_explanation(x_val, y_val, target_class)
# compute explanation accuracy
accuracy = dl.logic.test_explanation(formula, target_class, x_test, y_test)
\end{lstlisting}

% \textbf{Unless required by applicable law or agreed to in writing, software is distributed on an "as is" basis, without warranties or conditions of any kind, either express or implied.}

\subsection{Dataset and classification task details}
\label{sec:exp_details}
For the experimental analysis, we consider five classification problems ranging from computer vision to medicine and democracy. Some datasets (e.g. CUB) were already annotated with high-level concepts (e.g. bird attributes) which can be exploited to train a concept bottleneck pipeline. For datasets without annotations for high-level concepts, we transform the input space into a predicate space (i.e. $\mathbb{R}^d \rightarrow [0,1]^d$) to make it suitable for training logic explainers. According to the considered data type, we evaluate and discuss the usage of  different LEN pipeline, classification and explanation style (see Tab. \ref{tab:datasets}).

% \subsubsection{End-to-end explainers} \label{sec:exp_e2e}
%\paragraph{dSprites} 
%The Disentanglement testing Sprites dataset (dSprites, \cite{matthey2017dsprites}) consists of $n=737,280$ black-and-white images artificially generated from 6 ground truth independent latent factors. These factors are \textit{color}, \textit{shape}, \textit{scale}, \textit{rotation}, \textit{x} and \textit{y} positions of a sprite. The input space $X \subset \mathbb{R}^{64 \times 64}$ is composed of 64x64 pixel images. From each latent factor we extract a set of categorical concepts (one-hot-encoded). For instance, from the \textit{shape} factor we extract the categories: \textit{square}, \textit{ellipse}, and \textit{heart}. For continuous features, such as \textit{rotation}, we first discretize the latent factor into a set of bins, before the extraction of a one-hot encoded representation, as proposed by \cite{kazhdan2020now}. Through this procedure, we obtain a concept space $C \subset [0,1]^{50}$. Following \cite{kazhdan2020now}, we set up a high-level classification task $Y \subset [0,1]$ where the explainer is trained to identify images corresponding to a specific combination of shape and scale, i.e. \textit{square} and \textit{small} (an image containing a sprite whose shape is a square and whose size is small). A ResNet10 is used to learn the function $X \xrightarrow[]{g} C$, while the mapping $C \xrightarrow[]{f} Y$ is learned by the explainer. Quantitative results are reported in Table \ref{tab:exp_metrics_dsprites} while Table \ref{tab:exp_formula_dsprites} shows for each fold the explanation extracted from trained explainers.
% \paragraph{Cell differentiation}
% In this experiment, we analyze single-cell gene expression data from hematopoietic stem and differentiated cells in zebrafish obtained using Smart-Seq \cite{athanasiadis2017single} \footnote{The zebrafish dataset used for this paper is made publicly available by Athanasiadis et al.1 on ArrayExpress under the accession numbers E-MTAB-3947, E-MTAB-4617 and E-MTAB-5530 and also at https://www.sanger.ac.uk/science/tools/basicz.}. The dataset consists of $d=1845$ gene expression measurements identified by \cite{athanasiadis2017single} from $n=1422$ zebrafish single cells. The original transcriptomics data were log-normalized. However, in order to feed logic explainers, we perform an additional min-max normalization such that the expression values for each gene is scaled in $[0,1]$, as proposed by \cite{bica2020unsupervised}. This way the input space $X=C \subset [0,1]^{1845}$ corresponds to a multivariate Bernoulli distribution. The classification task $Y \subset [0,1]$ is for the explainer to identify stem cells that will differentiate into Monocytes (in contrast with HSPCs, Neutrophils, Erythrocytes, and Thrombocytes). An end-to-end explainer is used to learn the function $X=C \xrightarrow[]{f} Y$. Quantitative results are reported in Table \ref{tab:exp_metrics_celldiff} while Table \ref{tab:exp_formula_celldiff} shows for each fold the explanation extracted from trained explainers.

\textsc{MIMIC-II. }
The Multiparameter Intelligent Monitoring in Intensive Care II (MIMIC-II, \cite{saeed2011multiparameter,goldberger2000physiobank}) is a public-access intensive care unit (ICU) database consisting of 32,536 subjects (with 40,426 ICU admissions) admitted to medical, surgical, cardiovascular and neonatal ICUs, surgical recovery units, and coronary care units at a single tertiary care hospital. The dataset contains detailed description of a variety of clinical data classes: general (e.g. patient demographics, hospital admission and discharge dates, hospital death dates, etc), physiological (e.g.	nurse-verified vital signs, blood pressure, heart rate, etc), results of clinical laboratory tests (e.g. hematology, blood chemistries, urinalysis, microbiology, etc), records of medications, fluid balance (e.g. solutions, urine, estimated blood loss, etc), and free text notes and reports of imaging studies (e.g. x-ray, CT, MRI, etc). In our experiments, we remove some of the input features (e.g. text-based features) and discretize some of the continuous features into a set of categories in order to get a one-hot encoded representation. For instance, we discretize blood pressure (BP) into five different categories (one-hot encoded): very low BP, low BP, normal BP, high BP, and very high BP. After such preprocessing step, we obtain an input space $X=C \subset [0,1]^d$ composed of $d=90$ key features. 
The task consists in training a classifier function to identify recovering ($Y=1$) or dying ($Y=0$) patients, after 28 days from ICU admission. In particular, we consider the case of
% {\bf Interpretable classification. }
\textit{Interpretable classification} where an end-to-end explainer $X=C \xrightarrow[]{f} Y$ is employed to carry out the classification task.
But we also considered the case of 

\textsc{MIMIC-II (EC). }
\textit{Explaining an existing classifier} where a black-box model $X=C \xrightarrow[]{g} Y$ is employed to solve the classification task, with predictions $g(X) \approx Y$. The end-to-end explainer $X=C \xrightarrow[]{f} g(X)$ instead is trained to mimic the behaviour of the black box $g$.

%OLD
% \paragraph{Interpretable classification}
% End-to-end explainers, $X=C \xrightarrow[]{f} Y$, are trained to identify recovering ($Y=1$) or death \fg{dead? o intendi il nome della classe? in caso metterei in corsivo} patients ($Y=0$) after 28 days from ICU admission.

% \paragraph{Explaining an existing classifier} 
% A black box model $X=C \xrightarrow[]{g} Y$ is trained to identify recovering ($Y=1$) or death patients ($Y=0$) after 28 days from ICU admission. 
% Once trained, this black box model is used to obtain a set of predictions $g(X) \approx Y$. End-to-end explainers (i.e. "student models"), $X=C \xrightarrow[]{f} g(X)$, are trained to mimic the behaviour of the black box $g$ (i.e. "the teacher").
%\fg{beh in realtà possono essere cotrainati, non deve essere fatto a posteriori}


% \subsubsection{Concept bottleneck explainers}
% \label{sec:exp_cbm}

% \paragraph{MNIST Even/Odd}
\textsc{MNIST Even/Odd. }
The Modified National Institute of Standards and Technology database (MNIST, \cite{lecun1998mnist}) contains a large collection of images representing handwritten digits. The input space $X \subset \mathbb{R}^{28\times 28}$ is composed of 28x28 pixel images while the concept space $C \subset [0,1]^{10}$ is represented by digits from $0$ to $9$. 
However, the task we aim to solve is slightly different from the common digit-classification. In the case of 
% {\bf Interpretable classification}
\textit{interpretable classification}, indeed, assuming $Y \subset [0,1]^2$, we are interested in determining if a digit is either odd or even, and explain the assignment to one of these classes in terms of the high-level concepts $C$ (digits). The mapping $X \xrightarrow[]{g} C$ is learned by a ResNet10 classifier \cite{he2016deep}  trained from scratch, while a LEN can used to learn both the mapping and the explanation as a function $C \xrightarrow[]{f} Y$. 
The $\mu$ network is equipped with a single hidden layer with 10 neurons and the $L_1$ loss weight $\lambda = 10^{-2}$. 
The $ReLU$ network is equipped with two hidden layers composed of 30, 10 hidden neurons respectively and $\lambda = 10^{-3}$. 
The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^-3$ and fan-in = 5. 
All networks have been trained for 200 epochs with learning rate = $10^ {-3}$.
In the case of 
% {\bf Interpretable Clustering}
\textit{Interpretable clustering}, we consider a concept space $C \subset [0,1]^{12}$ which comprise both the digits and the even/odd labels. The mapping $X \xrightarrow[]{g} C$ is learned again by a Resnet10 trained as a multi-label classifier, while the LENs perform clustering from $C \xrightarrow[]{f} Y$, where $Y \subset [0,1]^{2}$ space, in order two extract two clusters. In this case, 
the $\mu$ network is equipped with two hidden layer with 20, 10 neurons respectively and the $L_1$ loss weight $\lambda = 10^{-3}$. 
The $ReLU$ network is equipped with two hidden layers composed of 50, 30 hidden neurons and $\lambda = 10^{-4}$. 
The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^{-2}$ and fan-in = 2. 
The $\mu$ and the $ReLU$ networks have been trained for 100 epochs with learning rate = $10^{-3}$ while for the $\psi$ network is equal to $10^{-2}$.

%Quantitative results are reported in Table \ref{tab:exp_metrics_mnist_cbm} while Table \ref{tab:exp_formula_mnist_cbm} shows for each fold the explanation extracted from trained explainers.
\textsc{CUB Dataset. }
The Caltech-UCSD Birds-200-2011 dataset (CUB, \cite{wah2011caltech}) is a fine-grained classification dataset. It includes 11,788 images representing $r = 200$ ($Y \subset [0,1]^{200}$) different bird species. 312 binary attributes have been also collected for each image representing visual characteristics (color, pattern, shape) of particular parts (beak, wings, tail, etc.). Attributes annotations, however, is quite noisy. Similarly to \cite{koh2020concept}, we denoised attributes by considering class-level annotations, i.e. a certain attribute is set as present only if it is also present in at least 50\% of the images of the same class. Furthermore we only considered attributes present in at least 10 classes after this refinement. In the end, a total of $d = 108$ attributes ($C \subset [0,1]^{108}$) have been retained. The mapping $X \xrightarrow[]{g} C$ from images to attribute concepts is performed again with a ResNet10 \cite{he2016deep} trained from scratch while an explainer learns the final function $C \xrightarrow[]{f} Y$.


\subsubsection{Cascading explainers}
\textsc{V-Dem. }
Varieties of Democracy (V-Dem, \cite{pemstein2018v,coppedge2021v}) is a dataset containing a collection of indicators of latent regime characteristics over 202 countries from 1789 to 2020. The database include $d_1 = 483$ low-level indicators $C_1 \subset [0,1]^{d_1}$ (e.g. media bias, party ban, high-court independence, initiatives permitted, etc), $d_2 = 82$ mid-level indices $C_1 \subset [0,1]^{d_2}$ (e.g. freedom of expression, freedom of association, equality before the law, etc), and 5 high-level indices of democracy principles (i.e. electoral, liberal, participatory, deliberative, and egalitarian). In the experiments a binary classification problem is considered to identify electoral democracies ($Y=1$) from non-electoral democracies ($Y=0$). Cascading explainers $f_1$ and $f_2$ are trained to learn the map $C_1 \xrightarrow[]{f_1} C_2 \xrightarrow[]{f_2} Y$.



\subsection{Quantitative metrics for explainers and explanations}
\label{sec:exp_metrics}
Seven metrics are used to compare the performance of LENs with respect to state-of-the-art approaches.
While measuring classification metrics is necessary for explainers to be viable in practice to perform interpretable classification tasks, assessing the quality of the explanations is required to justify their use for explainability. In contrast with other kind of explanations, logic-based formulas can be evaluated quantitatively. Given a classification problem, first we extract a set of rules from a trained explainer and then we test each explanation on an unseen set of samples.

The results for each metric are reported in terms of the mean and the standard error of the mean, computed over a 10-fold cross validation \cite{krzywinski2013error}. Only in the CUB experiments a 5-fold cross validation is performed due to timing issues related to BRL (each training of BRL on CUB lasts about 3 hours).
For each experiment we measure: 
% (1) the test accuracy of the classifier, (2) the test accuracy of the explanation, (3) the complexity of the explanation, (4) the fidelity of the explanation with respect to the classifier, (5) the elapsed time required to extract the explanations, (6) the consistency of the explanation over different runs, and (7) the normalized mutual information (for unsupervised tasks only). 
% \cite{andrews1995survey}.

\begin{itemize}
\item The \textsc{model accuracy} measures how well the classifier correctly identifies the target class (see Table. \ref{tab:model-accuracy}). When the explainer is the classifier itself (i.e. interpretable classification), this metric represents the accuracy of the explainer. Instead, when the LEN is explaining the predictions of a black box classifier (e.g. explaining an existing classifier), this metric represents the accuracy of the black box classifier.
\item The \textsc{explanation accuracy} measures how well the extracted logic formula correctly identifies the target  class (see Table. \ref{tab:explanation-accuracy}).
\item The \textsc{complexity of an explanation} measures how hard would it be for a human being to understand the logic formula (see Table. \ref{tab:complexity}). This metric is computed by standardizing the explanations in disjunctive normal form and then by counting the number of terms of the standardized formula.
\item The \textsc{fidelity of an explanation} measures how well the predictions obtained using the extracted explanation match the predictions obtained using the classifier (see Table. \ref{tab:fidelity}). When the explainer is the classifier itself (i.e. interpretable classification), this metric represents the match between the extracted explanation and the explainer. Instead, when the LEN is explaining the predictions of a black box classifier (e.g. explaining an existing classifier), this metric represents the match between the extracted explanation and the black box classifier.
\item The \textsc{rule extraction} measures the time required to obtain an explanation from scratch. It is computed as the sum of the time required to train the (see Table. \ref{tab:extraction}) explainer and the time required to extract the formula from a trained explainer. This is justified by the fact that for some explainers, like BRL, training and rule extraction consist of just one simultaneous process.
\item The \textsc{consistency of an explanation} measures the similarity of the extracted explanations over different runs (see Table. \ref{tab:consistency}). It is computed by counting how many times the same concepts appear in the logic formulas over different folds of a cross-validation or over different initialization seeds.
% \item The \textsc{normalized mutual information} measures the quality of the clusters obtained in the interpretable clustering experiments. It is calculated as the mutual information of Eq. \ref{eq:MI}, divided by the Entropy $H_E$ so that it reports a number always comprehended between $[0,1]$.
\end{itemize}


\subsection{Results and Discussion}
\textsc{Interpretable classification. } 
Experiments show how LENs generalize better than decision trees on complex Boolean functions (e.g. CUB and MIMIC-II) as already observed in \cite{tavares2020understanding} (Table. \ref{tab:model-accuracy}). For most experiments the formulas extracted from LENs are either better or almost as accurate as the formulas found by decision trees or mined by BRL (Table. \ref{tab:explanation-accuracy}). The complexity of LEN explanations is usually lower than the complexity of the rules extracted from a decision tree or mined by BRL. The complexity of decision tree formulas is never below 100 terms, making them useless for quick decision making (Table. \ref{tab:complexity}). White-box models like decision trees and BRL outperform out-of-the-box LENs in terms of fidelity. However, the fidelity of the formulas extracted by the $\mu$ and the ReLU network is often higher than $90\%$. This means that almost any prediction has been correctly explained, making these networks very close to white boxes (Table. \ref{tab:fidelity}). BRL is the slowest rule extractor over all the experiments by one order of magnitude, while the decision tree is the fastest overall (Table. \ref{tab:extraction}). In terms of consistency there is not a dominant method (Table. \ref{tab:consistency}).

Fig. \ref{fig:multi-objective} shows the Pareto frontiers \cite{marler2004survey} for each experiment in terms of the complexity of the explanation and its classification error ($100 -$ classification accuracy). The simplest and most accurate formulas are found by explainer networks, whose complexity is almost always below the maximum complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Across all the experiments, there is at least one set of formulas extracted from out-of-the-box LEN dominating both BRL and decision trees.

For each dataset and for each method Table \ref{tab:best-rules} reports some compact FOL formula extracted.

\textsc{Interpretable Clustering. } 
As introduced in the MNIST Even/Odd dataset explanation we performed clustering starting from a Concept space composed of the 10 digits and the even/odd labels. The LEN are instructed two extract 2 clusters possibly respecting the even/odd division of digits. In Table \ref{tab:exp_metrics_mnist_mi} the metrics regarding this task are reported. We can see that all methods are capable to maximize the normalized mutual information. However only the $\psi$ network is capable to consistently explain the two clusters in terms of the important labels (even and odd), as we can see from the complexity of the rules (higher than 2 for the $\mu$ and ReLu net) and for the consistency of terms used in the explanation (100\% for the $\psi$ network). 
Other examples and application of Interpretable Clustering has been performed in \cite{ciravegna2020constraint, ciravegna2020human} employing the $\psi$ network only.


\textsc{Explanation as a defense}



% \begin{table}[ht]
% \centering
% \caption{XOR}
% \label{tab:exp_metrics_xor}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llll}
% \hline
% \textbf{Method} & \textbf{Model's accuracy (\%)} & \textbf{Explanation's accuracy (\%)} & \textbf{Explanation's extraction (s)} \\ \hline
% \textbf{Pruning} & $100.00 \pm 0.00$ & $100.00 \pm 0.00$ & $0.01 \pm 0.00$ \\
% \textbf{LIME}    & $100.00 \pm 0.00$ & $100.00 \pm 0.00$ & $0.61 \pm 0.01$ \\
% \textbf{ReLU} & $100.00 \pm 0.00$ & $100.00 \pm 0.00$ & $0.01 \pm 0.00$ \\
% \textbf{$\psi$ net}     & $78.89 \pm 6.51$  & $90.00 \pm 5.84$  & $0.03 \pm 0.00$ \\
% \textbf{Decision tree}    & $100.00 \pm 0.00$ & $100.00 \pm 0.00$ & $0.00 \pm 0.00$ \\ \hline
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[ht]
% \centering
% \caption{MNIST (CBM)}
% \label{tab:exp_metrics_mnist_cbm}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llll}
% \hline
% \textbf{Method} & \textbf{Model's accuracy (\%)} & \textbf{Explanation's accuracy (\%)} & \textbf{Explanation's extraction (s)} \\ \hline
% \textbf{Pruning}       & $100.00 \pm 0.00$ & $100.00 \pm 0.00$ & $82.79 \pm 9.30$ \\
% \textbf{ReLU} & $100.00 \pm 0.00$ & $89.97 \pm 6.33$  & $73.61 \pm 0.20$ \\
% \textbf{$\psi$ net}    & $83.16 \pm 2.28$  & $51.63 \pm 7.45$  & $0.06 \pm 0.01$  \\
% \textbf{Decision tree} & $100.00 \pm 0.00$ & $100.00 \pm 0.00$ & $0.00 \pm 0.00$  \\ \hline
% \end{tabular}%
% }
% \end{table}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/mimic2.pdf}
    \includegraphics[width=0.49\textwidth]{figs/mimic_explain_classifier.pdf}\\
    \includegraphics[width=0.49\textwidth]{figs/mnist.pdf}
    \includegraphics[width=0.49\textwidth]{figs/cub.pdf}\\
    \includegraphics[width=0.49\textwidth]{figs/vdem_low2mid.pdf}
    \\
    \includegraphics[width=0.7\textwidth]{figs/legend.pdf}
    \caption{Pareto frontiers (dotted black line) in terms of average test error and average complexity of the explanations. Formulas out-of-the-box extracted from out-of-the-box LENs are reported as circles while BRL and decision trees as crosses. The vertical dotted red line marks the maximum explanation complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}).}
    \label{fig:multi-objective}
\end{figure}



% \begin{table}[ht]
% \centering
% \caption{Model's accuracy (\%)}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% {} &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
% \midrule
% \textbf{MIMIC-II     }  &  ${\bf 86.60 \pm 0.30}$ &  $85.36 \pm 0.78$ &  $84.01 \pm 0.09$ &  $79.56 \pm 0.80$ &  $86.15 \pm 0.51$ \\
% \textbf{MIMIC-II (EC)}  &  $85.13 \pm 0.70$ \gc{?} &  $85.13 \pm 0.70$ \gc{?}&  $85.13 \pm 0.70$ \gc{?}&  $85.13 \pm 0.70$ \gc{?}&  $85.13 \pm 0.70$ \gc{?}\\
% \textbf{V-Dem         } &  $91.96 \pm 0.42$ &  $91.88 \pm 0.37$ &  $79.23 \pm 2.20$ &  $92.11 \pm 0.38$ &  ${\bf 92.23 \pm 0.38}$ \\
% \textbf{MNIST}          &  $99.75 \pm 0.02$ &  $99.81 \pm 0.01$ &  $99.80 \pm 0.01$ &  ${\bf 99.96 \pm 0.01}$ &  $99.80 \pm 0.01$ \\
% \textbf{CUB          }  &  ${\bf 92.26 \pm 0.28}$ &  $92.19 \pm 0.27$ &  $91.72 \pm 0.56$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ \\

% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[h]
\centering
\caption{Model's accuracy (\%)}
\label{tab:model-accuracy}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllll}
\toprule
{} &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL & Black box \\
\midrule
\textbf{MIMIC-II     }  &  ${\bf 86.60 \pm 0.30}$ &  $85.36 \pm 0.78$ &  $84.01 \pm 0.09$ &  $79.56 \pm 0.80$ &  $86.15 \pm 0.51$ & N/A \\
\textbf{MIMIC-II (EC)}  &  N/A &  N/A &  N/A &  N/A &  N/A  & $85.13 \pm 0.70$\\
\textbf{V-Dem         } &  $91.96 \pm 0.42$ &  $91.88 \pm 0.37$ &  $79.23 \pm 2.20$ &  $92.11 \pm 0.38$ &  ${\bf 92.23 \pm 0.38}$ & N/A \\
\textbf{MNIST}          &  $99.75 \pm 0.02$ &  $99.81 \pm 0.01$ &  $99.80 \pm 0.01$ &  ${\bf 99.96 \pm 0.01}$ &  $99.80 \pm 0.01$ & N/A \\
\textbf{CUB          }  &  ${\bf 92.26 \pm 0.28}$ &  $92.19 \pm 0.27$ &  $91.72 \pm 0.56$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ & N/A \\

\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Explanation's accuracy (\%)}
\label{tab:explanation-accuracy}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
\midrule
\textbf{MIMIC-II     } &  $85.08 \pm 0.48$ &  $82.09 \pm 1.38$ &  $82.83 \pm 0.66$ &  $79.56 \pm 0.80$ &   ${\bf86.15 \pm 0.51}$ \\
\textbf{MIMIC-II (EC)} &  ${\bf85.75 \pm 0.51}$ &  $81.07 \pm 3.33$ &  $83.90 \pm 1.25$ &  $85.53 \pm 0.61$ &  $85.70 \pm 0.48$ \\
\textbf{V-Dem         } &  $90.81 \pm 1.24$ & ${\bf94.65 \pm 0.32}$ &  $80.29 \pm 2.99$ &  $92.11 \pm 0.38$ &  $92.23 \pm 0.38$ \\
\textbf{MNIST}         &  $99.67 \pm 0.01$ &  $98.04 \pm 1.60$ &  $75.47 \pm 0.46$ &  ${\bf99.96 \pm 0.01}$  &  $99.80 \pm 0.01$ \\
\textbf{CUB*         } &  ${\bf96.15 \pm 0.16}$ &  $93.98 \pm 1.97$ &  $80.41 \pm 2.31$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ \\


\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Complexity}
\label{tab:complexity}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{}                     &        $\mu$ net &         ReLU net &       $\psi$ net &                 Tree &               BRL \\
\midrule
\textbf{MIMIC-II     } &  $5.10 \pm 0.35$ &  $23.40 \pm 11.20$ &  ${\bf2.60 \pm 0.16}$ &  $1342.60 \pm 16.94$ &  $20.70 \pm 4.08$ \\
\textbf{MIMIC-II (EC)} &  $7.00 \pm 0.70$ &    $6.40 \pm 0.95$ &  ${\bf1.30 \pm 0.15}$ &   $432.10 \pm 16.46$ &  $22.90 \pm 4.13$ \\
\textbf{V-Dem         } &  $9.60 \pm 1.17$ &    $4.90 \pm 0.10$ &  ${\bf2.00 \pm 0.49}$ &    $294.10 \pm 7.88$ &   $8.70 \pm 0.97$ \\
\textbf{MNIST}         &  ${\bf22.00 \pm 4.67}$ &  $48.10 \pm 1.43$ &  $24.85 \pm 2.89$ &  $632.35 \pm 5.01$ &  $1291.05 \pm 234.40$ \\
\textbf{CUB          } &  $10.53 \pm 0.08$ &  $29.25 \pm 3.26$ &  $28.36 \pm 2.75$ &  $138.83 \pm 5.31$ &  ${\bf4.10 \pm 0.09}$ \\


\bottomrule
\end{tabular}
}
\end{table}

\begin{table}
\centering
\caption{Fidelity (\%)}
\label{tab:fidelity}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
\midrule
\textbf{MIMIC-II     } &  $96.23 \pm 0.81$ &  $87.84 \pm 2.12$ &  $84.63 \pm 0.67$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
\textbf{MIMIC-II (EC)} &  $92.28 \pm 0.90$ &  $86.58 \pm 4.00$ &  $90.32 \pm 1.27$ &   $93.07 \pm 0.53$ &   ${\bf94.82 \pm 0.50}$ \\
\textbf{V-Dem         } &  $91.52 \pm 1.13$ &  $94.62 \pm 0.37$ &  $82.45 \pm 1.80$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
\textbf{MNIST}         &  $99.90 \pm 0.03$ &  $98.14 \pm 1.60$ &  $75.53 \pm 0.46$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
\textbf{CUB*         } &  $97.82 \pm 0.15$ &  $95.37 \pm 2.06$ &  $81.89 \pm 2.35$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\


\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Rule extraction (s)}
\label{tab:extraction}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{} &        $\mu$ net &         ReLU net &       $\psi$ net &             Tree &              BRL \\
\midrule
\textbf{MIMIC-II     } &  $13.32 \pm 0.30$ &  $266.22 \pm 166.90$ &   $8.81 \pm 0.15$ &  ${\bf0.02 \pm 0.00}$ &  $495.59 \pm 7.13$ \\
\textbf{MIMIC-II (EC)} &  $15.30 \pm 0.19$ &     $18.46 \pm 1.00$ &  $10.14 \pm 0.03$ &  ${\bf0.01 \pm 0.00}$ &  $543.43 \pm 3.39$ \\
\textbf{V-Dem         } &  $34.40 \pm 0.78$ &     $34.24 \pm 0.32$ &  $20.83 \pm 0.04$ &  ${\bf0.06 \pm 0.00}$ &   $53.69 \pm 0.41$ \\
\textbf{MNIST}         &  $173.24 \pm 6.77$ &  $221.07 \pm 4.06$ &  $236.71 \pm 3.36$ &  ${\bf2.04 \pm 0.04}$ &  $836.14 \pm 3.15$ \\
\textbf{CUB          } &  $726.19 \pm 2.43$ &  $660.30 \pm 121.16$ &  $2094.49 \pm 730.50$ &  ${\bf4.17 \pm 0.07}$ &  $9863.52 \pm 147.57$ \\

\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Rule consistency (\%)}
\label{tab:consistency}
\begin{tabular}{llllll}
\toprule
{} & $\mu$ net & ReLU net & $\psi$ net &     Tree &      BRL \\
\midrule
\textbf{MIMIC-II     } &   $51.00$ &  $26.00$ &    $37.14$ &  ${\bf81.50}$ &  $28.33$ \\
\textbf{MIMIC-II (EC)} &   $41.18$ &  $35.56$ &    $43.33$ &  ${\bf60.36}$ &  $22.22$ \\
\textbf{V-Dem         }&   $71.67$ &  ${\bf98.00}$ &    $15.83$ &  $36.86$ &  $76.25$ \\
\textbf{MNIST}         &   $60.00$ &  ${\bf100.00}$ &    $50.00$ &  $50.95$ &  ${\bf100.00}$ \\
\textbf{CUB          } &   ${\bf58.82}$ &  $58.40$ &    $43.08$ &  $21.79$ &  $30.00$ \\

\bottomrule
\end{tabular}
\end{table}



% \begin{table}[ht]
% \centering
% \caption{MNIST (CBM)}
% \label{tab:exp_metrics_mnist_cbm}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
%          {\bf Method} & {\bf Mod. accuracy (\%)} & {\bf Exp. accuracy (\%)} & {\bf Complexity} & {\bf Time (s)} & {\bf Consistency (\%)}  \\
% \midrule
%                  LR &     $99.84 \pm 0.01$ &            N/A             &    N/A             &     N/A             &                  N/A \\
%                 BRL &     $99.73 \pm 0.01$ &           $99.73 \pm 0.01$ &   $22.95 \pm 2.98$ &     $0.23 \pm 0.09$ &              $82.00$ \\
%               Tree &    $100.00 \pm 0.00$ &          $100.00 \pm 0.00$ &  $639.95 \pm 6.17$ &     $0.00 \pm 0.00$ &              $49.30$ \\
%           $\mu$ net &     $99.80 \pm 0.01$ &           $99.66 \pm 0.01$ &   $18.50 \pm 3.50$ &    $11.16 \pm 0.18$ &              $55.00$ \\
%          $\psi$ net &     $99.81 \pm 0.01$ &           $76.03 \pm 0.62$ &   $19.60 \pm 0.79$ &     $0.13 \pm 0.01$ &              $50.00$ \\
%           ReLU net &      $100.00 \pm 0.00$ &           $95.17 \pm 2.35$ &   $44.05 \pm 2.97$ &    $21.51 \pm 1.16$ &             $100.00$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{table}[!ht]
% \centering
% \caption{CUB}
% \label{tab:exp_metrics_cub}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllll}
% \toprule
%     %   {\bf Method} & {\bf Mod. accuracy (\%)} & {\bf Exp. accuracy (\%)} & {\bf Complexity} & {\bf Time (s)} & {\bf Consistency (\%)}  \\
%         {\bf Method} & {\bf Mod. accuracy (\%)} & {\bf Exp. accuracy (\%)} & {\bf Complexity}      {\bf Fidelity (\%)} &   {\bf Rule extraction (s)} & {\bf Rule consistency (\%) }\\

% \midrule
%         %         LR  &     $92.38 \pm 0.24$ &            N/A             &    N/A             &     N/A             &                  N/A \\
%         %         BRL &     $82.37 \pm 0.53$ &           $82.37 \pm 0.53$ &    $4.24 \pm 0.10$ &     $0.03 \pm 0.00$ &              $30.00$ \\
%         %       Tree &     $89.30 \pm 0.42$ &           $89.30 \pm 0.42$ &  $138.83 \pm 5.31$ &     $0.01 \pm 0.00$ &              $21.79$ \\
%         %   $\mu$ net &     $91.51 \pm 0.37$ &           $99.13 \pm 0.20$ &    $7.93 \pm 0.15$ &     $2.27 \pm 0.13$ &              $62.86$ \\
%         %  $\psi$ net &     $91.68 \pm 0.55$ &           $98.94 \pm 0.34$ &   $28.78 \pm 1.73$ &     $5.38 \pm 1.43$ &              $42.86$ \\
%         %   ReLU net &     $91.89 \pm 0.23$ &           $99.59 \pm 0.08$ &   $20.02 \pm 2.20$ &     $2.40 \pm 0.39$ &              $54.29$ \\
%         %         LR  &     $92.38 \pm 0.24$ &            N/A             &    N/A             &     N/A             &                  N/A \\
%         %  LR &     $92.38 \pm 0.24$ &            N/A             &    N/A             &     N/A            &       $0.78 \pm 0.77$ \\
%          LR &     $92.38 \pm 0.24$ &            N/A             &    N/A             &     N/A            &       $0.78 \pm 0.77$ &                 N/A  \\
%       Tree &     $89.30 \pm 0.42$ &           $89.30 \pm 0.42$ &  $138.83 \pm 5.31$ &  $100.00 \pm 0.00$ &       $4.17 \pm 0.07$ &              $21.79$ \\
%         BRL &     $82.18 \pm 0.43$ &           $82.18 \pm 0.43$ &    $4.10 \pm 0.09$ &  $100.00 \pm 0.00$ &  $9863.52 \pm 147.57$ &              $30.00$ \\
%  $\psi$ net &     $91.72 \pm 0.56$ &           $98.87 \pm 0.32$ &   $28.36 \pm 2.75$ &   $98.91 \pm 0.32$ &  $2094.49 \pm 730.50$ &              $43.08$ \\
%   $\mu$ net &     $92.26 \pm 0.28$ &           $99.93 \pm 0.00$ &   $10.53 \pm 0.08$ &   $99.95 \pm 0.00$ &     $726.19 \pm 2.43$ &              $58.82$ \\
%   ReLU net &     $92.19 \pm 0.27$ &           $99.78 \pm 0.14$ &   $29.25 \pm 3.26$ &   $99.81 \pm 0.14$ &   $660.30 \pm 121.16$ &              $58.40$ \\


% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[h]
\centering
\caption{MNIST Mutual Information}
\label{tab:exp_metrics_mnist_mi}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
     Method & Model's accuracy (\%) & Explanation's accuracy (\%) &       Complexity & Rule extraction (s) & Rule consistency (\%) \\
\midrule
  $\mu$ net &     $99.90 \pm 0.01$ &           $99.90 \pm 0.01$ &  $2.00 \pm 0.00$ &     $0.33 \pm 0.15$ &             $100.00$ \\
 $\psi$ net &     $94.91 \pm 4.99$ &           $95.41 \pm 4.50$ &  $2.30 \pm 0.64$ &     $2.36 \pm 0.75$ &              $35.00$ \\
   ReLU net &     $96.87 \pm 3.04$ &           $95.97 \pm 3.94$ &  $2.15 \pm 0.39$ &     $4.15 \pm 1.62$ &              $45.00$ \\
\bottomrule
\end{tabular}
% \begin{tabular}{lllll}
% \toprule
%      Method & Normalized MI &       Complexity & Rule extraction (s) & Rule consistency (\%) \\
% \midrule
%   $\mu$ net &     ${\bf91.89 \pm 0.02}$ &  $2.30 \pm 0.64$ &     $199.69 \pm 5.29$ &              $35.00$ \\
%  $\psi$ net &     ${\bf91.89 \pm 0.00}$ &  $\bf{2.00 \pm 0.00}$ &     $\bf{102.31 \pm 0.41}$ &             ${\bf100.00}$ \\
%   ReLU net &     $91.87 \pm 0.03$ &  $2.15 \pm 0.39$ &     $196.51 \pm 4.48$ &              $45.00$ \\
% \bottomrule
% \end{tabular}
}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% \begin{table}[ht]
% \centering
% \caption{MNIST (CME)}
% \label{tab:exp_metrics_mnist_cme}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llll}
% \hline
% \textbf{Method} & \textbf{Model's accuracy (\%)} & \textbf{Explanation's accuracy (\%)} & \textbf{Explanation's extraction (s)} \\ \hline
% \textbf{Pruning}       & $99.28 \pm 0.00$ & $99.28 \pm 0.00$ & $58.75 \pm 1.26$  \\
% \textbf{ReLU} & $99.28 \pm 0.00$ & $74.57 \pm 9.94$ & $114.94 \pm 1.55$ \\
% \textbf{$\psi$ net}    & $79.15 \pm 3.28$ & $52.05 \pm 5.46$ & $0.11 \pm 0.02$   \\
% \textbf{Decision tree} & $99.28 \pm 0.00$ & $99.28 \pm 0.00$ & $0.00 \pm 0.00$   \\ \hline
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[!ht]
% \centering
% \caption{Cell differentiation}
% \label{tab:exp_metrics_celldiff}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llll}
% \hline
% \textbf{Method} & \textbf{Model's accuracy (\%)} & \textbf{Explanation's accuracy (\%)} & \textbf{Explanation's extraction (s)} \\ \hline
% \textbf{Pruning}       & $94.59 \pm 0.56$  & $85.93 \pm 1.16$  & $21.18 \pm 5.19$ \\
% \textbf{ReLU} & $95.99 \pm 0.48$  & $85.10 \pm 1.45$  & $2.56 \pm 0.16$ \\
% \textbf{$\psi$ net}    & $83.05 \pm 0.32$  & $54.98 \pm 11.36$ & $0.02 \pm 0.00$ \\
% \textbf{Decision tree} & $91.92 \pm 0.53$ & $91.92 \pm 0.53$ & $0.00 \pm 0.00$ \\ \hline
% \end{tabular}%
% }
% \end{table}


% \begin{table}[!ht]
% \centering
% \caption{MIMIC-II (interpretable classification).}
% \label{tab:exp_metrics_mimic_exp_class}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llll}
% \toprule
% \textbf{Method} & \textbf{Model's accuracy (\%)} & \textbf{Explanation's accuracy (\%)} & \textbf{Complexity}\\
% \midrule
%  $\mu$ net &     $85.42 \pm 0.44$ &           $85.42 \pm 0.44$ &     $2.20 \pm 0.29$ \\
%   ReLU net &     $85.64 \pm 0.56$ &           $32.73 \pm 6.68$ &     $5.20 \pm 0.90$ \\
% $\psi$ net &     $84.01 \pm 0.09$ &           $82.83 \pm 0.66$ &     $2.60 \pm 0.16$ \\
%       Tree &     $79.56 \pm 0.80$ &           $79.56 \pm 0.80$ & $1342.60 \pm 16.94$ \\
%       BRL &     $86.60 \pm 0.43$ &           $85.64 \pm 0.63$ &    $11.50 \pm 2.13$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{table}[!ht]
% \centering
% \caption{MIMIC-II (explain classifier).}
% \label{tab:exp_metrics_mimic_classifier}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllll}
% \toprule
% \textbf{Method} & \textbf{Model's accuracy (\%)} & \textbf{Explanation's accuracy (\%)} & \textbf{Complexity} & \textbf{Fidelity (\%)} \\
% \midrule
%  $\mu$ net &     $90.04 \pm 0.70$ &           $76.65 \pm 8.53$ &    $1.80 \pm 0.36$ & $81.05 \pm 9.03$ \\
%   ReLU net &     $95.66 \pm 0.38$ &           $72.74 \pm 6.33$ &    $8.20 \pm 1.55$ & $74.77 \pm 7.95$ \\
% $\psi$ net &     $88.40 \pm 0.95$ &           $77.42 \pm 5.00$ &    $1.30 \pm 0.15$ & $81.25 \pm 5.56$ \\
%       Tree &     $83.33 \pm 0.61$ &           $83.33 \pm 0.61$ & $701.50 \pm 11.92$ & $91.10 \pm 0.91$ \\
%       BRL &     $91.89 \pm 0.52$ &           $85.36 \pm 0.59$ &   $11.60 \pm 2.39$ & $90.54 \pm 0.78$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{table}[!ht]
% \centering
% \caption{V-Dem (cascading explainers).}
% \label{tab:exp_metrics_vdem}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llll}
% \toprule
% \textbf{Method} & \textbf{Model's accuracy (\%)} & \textbf{Explanation's accuracy (\%)} & \textbf{Complexity}\\
% \midrule
%  $\mu$ net &     $91.08 \pm 0.93$ &           $85.11 \pm 1.42$ &   $9.30 \pm 0.75$ \\
%   ReLU net &     $92.67 \pm 0.44$ &           $54.47 \pm 2.72$ &   $4.20 \pm 0.55$ \\
% $\psi$ net &     $79.23 \pm 2.20$ &           $79.85 \pm 2.87$ &   $2.00 \pm 0.49$ \\
%       Tree &     $92.11 \pm 0.38$ &           $92.11 \pm 0.38$ & $294.10 \pm 7.88$ \\
%       BRL &     $91.93 \pm 0.25$ &           $93.44 \pm 1.37$ &   $7.70 \pm 0.68$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}



% \begin{table}[!ht]
% \centering
% \caption{CUB}
% \label{tab:exp_metrics_cub}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllll}
% \toprule
% {\bf Method} & {\bf Mod. accuracy (\%)} & {\bf Exp. accuracy (\%)} & {\bf Complexity} & {\bf Time (s)} & {\bf Consistency (\%)}  \\
% \midrule
% \textbf{Pruning} &            $91.63 \pm 0.17$ &           $95.99 \pm 2.58$ &              $0.51 \pm 0.04$ \\
% \textbf{ReLU} &              $91.84 \pm 0.22$ &           $95.71 \pm 1.16$ &              $0.16 \pm 0.02$ \\
% \textbf{$\psi$ net} &        $65.54 \pm 1.32$ &           $63.87 \pm 0.43$ &              $0.04 \pm 0.00$ \\
% \textbf{Decision tree} &      $89.08 \pm 0.28$ &           $89.08 \pm 0.28$ &              $0.01 \pm 0.00$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}



% \begin{table}[!ht]
% \centering
% \caption{MIMIC-II (interpretable classification).}
% \label{tab:exp_metrics2_mimic_exp_class}
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{lll}
% \toprule
% \textbf{Method} & \textbf{Rule extraction (s)} & \textbf{Rule consistency (\%)} \\
% \midrule
%  $\mu$ net &     $0.06 \pm 0.01$ &              $44.00$ \\
%   ReLU net &     $0.21 \pm 0.02$ &              $31.43$ \\
% $\psi$ net &     $0.03 \pm 0.00$ &              $37.14$ \\
%       Tree &     $0.00 \pm 0.00$ &              $81.50$ \\
%       BRL &     $0.01 \pm 0.00$ &              $24.55$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{table}[!ht]
% \centering
% \caption{MIMIC-II (explain classifier).}
% \label{tab:exp_metrics2_mimic_classifier}
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{lll}
% \toprule
% \textbf{Method} & \textbf{Rule extraction (s)} & \textbf{Rule consistency (\%)} \\
% \midrule
%  $\mu$ net &     $0.04 \pm 0.01$ &              $31.67$ \\
%   ReLU net &     $3.96 \pm 2.98$ &              $32.50$ \\
% $\psi$ net &     $0.00 \pm 0.00$ &              $32.50$ \\
%       Tree &     $0.00 \pm 0.00$ &              $74.53$ \\
%       BRL &     $0.01 \pm 0.00$ &              $23.12$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{table}[!ht]
% \centering
% \caption{V-Dem (cascading explainers).}
% \label{tab:exp_metrics2_vdem}
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{lll}
% \toprule
% \textbf{Method} & \textbf{Rule extraction (s)} & \textbf{Rule consistency (\%)} \\
% \midrule
%  $\mu$ net &     $2.91 \pm 0.16$ &              $62.50$ \\
%   ReLU net &     $3.10 \pm 0.12$ &              $39.00$ \\
% $\psi$ net &     $0.03 \pm 0.00$ &              $15.83$ \\
%       Tree &     $0.00 \pm 0.00$ &              $36.86$ \\
%       BRL &     $0.03 \pm 0.01$ &              $82.86$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}





% \subsection{Rules Extracted}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
{\renewcommand{\arraystretch}{2.5}
\begin{table}[]
\centering
\caption{A selection of some of the best rules extracted for each experiment.}
\label{tab:best-rules}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
\multicolumn{1}{l}{\textbf{Dataset}}    & \textbf{Explainer}  & \textbf{Rule} \\ \hline
\multirow{5}{*}{MIMIC-II}      & $\mu$ net  & $Death \leftarrow stroke \wedge age\_HIGH  \wedge \neg atrial\_fibrillation $  \\
                               & ReLU net   & $Death \leftarrow stroke \wedge age\_HIGH \wedge \neg atrial_fibrillation \wedge \neg sapsi\_first\_LOW \wedge \neg sapsi\_first\_HIGH $  \\
                               & $\psi$ net & $Death \leftarrow stroke \vee bun\_first\_NORMAL \vee sapsi\_first\_HIGH $  \\
                               & Tree       & $Death \leftarrow \quad ^*$formula is too long (1000+ terms) \\ 
                               & BRL        & $Death \leftarrow \makecell[l]{(stroke \wedge resp \wedge \neg age\_LOW \wedge \neg sapsi\_first\_LOW) \\
                               \vee (stroke  \wedge age\_HIGH \wedge \neg age\_LOW  \wedge  \neg sapsi\_first\_LOW) }$  \\ \hline
\multirow{5}{*}{MIMIC-II (EC)} & $\mu$ net  & $Death \leftarrow atrial_fibrillation \wedge stroke \wedge \neg sapsi\_first\_HIGH \wedge \neg weight\_first\_NORMAL $  \\
                               & ReLU net   & $Death \leftarrow stroke \wedge \neg sapsi\_first\_LOW  \wedge  \neg sapsi\_first\_HIGH \wedge \neg sodium\_first\_LOW $  \\
                               & $\psi$ net & $Death \leftarrow stroke \wedge age\_HIGH $  \\
                               & Tree       & $Death \leftarrow  \quad ^*$formula is too long (100+ terms)  \\ 
                               & BRL        & $Death \leftarrow \makecell[l]{stroke \wedge age\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW) \\ \vee  (stroke \wedge platelet\_first\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW } $  \\  \hline
\multirow{5}{*}{MNIST}         & $\mu$ net  & $Even \leftarrow \neg One \wedge \neg Three \wedge \neg Five \wedge \neg Seven \wedge \neg Nine $  \\
                              & ReLU net   & $Even \leftarrow \makecell[l]{(Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\ 
                              \vee (Two \wedge \neg Zero \wedge \neg One \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\ 
                              \vee (Four \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\ 
                              \vee (Six \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Eight \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Nine) } $ \\
                              & $\psi$ net & $Even \leftarrow \makecell[l]{(Six \wedge Zero \wedge \neg One \wedge \neg Seven)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Three)  \\
                              \vee (Six \wedge Zero \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge \neg One \wedge \neg Seven \wedge \neg Three) \\
                              \vee (Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)}$  \\
                              & Tree       & $Even \leftarrow \quad ^*$formula is too long \\
                              & BRL        & $Even \leftarrow  \makecell[l]{(Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two)) \vee (Eight \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two)) 
                              \\ \vee (Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Seven \wedge \neg Two)) \\ 
                              \vee (Two \wedge \neg One \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \\ \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two)) \\
                              \vee (Four \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \\ \wedge  \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One)) \\
                              \vee (Zero \wedge \neg Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \\
                              \wedge \neg (Nine \wedge \neg Zero) \wedge \neg (One \wedge \neg Two) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One))
                              }$  \\ \hline
\multirow{5}{*}{CUB}          & $\mu$ net  & $ Black\ foot\ albatross \leftarrow \makecell[l]{  bill \ shape \ hooked \ seabird \ \wedge \  size \ medium \wedge \ wing \ pattern \ solid \\
                              \wedge \neg wing color \ black \wedge \neg  underparts\ color\ white \wedge \neg upper\ tail\ color\ grey \\
                              \wedge \neg breast\ color\ white \wedge \neg  throat\ color\ white \wedge \neg tail\ pattern\ solid \wedge \neg  crown\ color\ white} $  \\
                              & ReLU net   & $ Black\ foot\ albatross \leftarrow  \makecell[l]{ size\  medium  \wedge \neg  bill\  shape\  allpurpose  \\ 
                              \wedge \neg  upperparts\  color\  black  \wedge \neg  head\  pattern\  plain  \wedge \neg  under\  tail\  color\  yellow \\  \wedge \neg  under\  tail\  color\  black  \wedge \neg  nape\  color\  buff  \\
                              \wedge \neg  wing\  shape\  roundedwings  \wedge \neg  shape\  perchinglike  \\
                              \wedge \neg  leg\  color\  grey  \wedge \neg  leg\  color\  black  \wedge \neg  bill\  color\  grey  \\
                              \wedge \neg  bill\  color\  black  \wedge \neg  wing\  pattern\  multicolored }$\\
                              & $\psi$ net & $ Black\ foot\ albatross \leftarrow  \makecell[l]{(bill \ shape \ hooked\ seabird \wedge tail \ pattern \ solid \wedge \neg underparts \ color \ white \\
                              \wedge ( \neg  \ breast \ color \ white \vee \neg   \ wing \ color \ grey)) }$  \\
                              & Tree       & $ Black\ foot\ albatross \leftarrow  ^*$formula is too long (1000+ terms)  \\
                              & BRL        & $ Black\ foot\ albatross \leftarrow  \makecell[l]{( bill\  shape\  hooked\  seabird \wedge forehead\ color\ blue \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white) \\
                              \vee ( bill\  shape\  hooked\  seabird \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white \wedge  \neg  tail\  pattern\  solid)}$ \\ 
\hline
\multirow{5}{*}{V-Dem}         & $\mu$ net  & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & ReLU net   & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & $\psi$ net & $Elect\_ Dem \leftarrow v2x\_frassoc\_thick \wedge v2xeg\_eqaccess $  \\
                               & Tree       & $Elect\_ Dem \leftarrow \quad ^*$formula is too long (1000+ terms)  \\
                               & BRL        & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\ \hline
\end{tabular}%
}
\end{table}}



% These challenging or product-oriented contexts are the actual targets of XAI research. This great research effort have produced a variety of quite interesting and efficient approaches to unveil the decision process of black-box models. Some of the most common taxonomies are based on a few discriminative criteria (intrinsic interpretability VS post-hoc, model-specific VS model-agnostic, local VS global explanations), but the most important characteristic, i.e. the \textit{form} of the explanation, is often overlooked.

% include white-box models, model-agnostic approaches \cite{ribeiro2016model} and example-based explanations \cite{aamodt1994case,kim2016examples,barbiero2020uncovering}. 


% decision trees \cite{breiman1984classification}, or decision rules: oneR \cite{holte1993very}, RIPPER \cite{cohen1995fast}, Bayesian Rule Lists \cite{letham2015interpretable}).

% \begin{itemize}
%     \item many interesting works around explainability, from fully interpretable models (LR, DT, DR), to surrogates (LIME, Anchors, SHAP, etc) to example-based
%     \item great effort on scoring/ranking features/concepts
%     \item that's NOT the whole point
%     \item what matters (even more?) is how concepts are related (PDP? mah...)
%     \item what is the effort for the end user for analyzing a pairwise dependence plot or a ranking or a decision tree with depth 5?
%     \item good explanations must be simple
%     \item simple <-> few concepts involved? well yes, but...
%     \item traditional methods tend to assume: simplicity -> simple relationships among concepts (linear, max PDP)
%     \item we argue: why??
% \end{itemize}

% % -idee generali su che tipo di bestie c'è per fare expl.. 
% % -s'è già detto che i sistemi a regole sono più utili per fare supporto a umani.. che robe c'è in giro, perchè il nostro è più fiho
% % - il survey congnitivo dice che regole buone devono essere semplici.. -> pruning! che tipi di pruning usa sta gente che fa expl?

% What Is an Explanation? An explanation is the answer to a why-question (Miller 2017).


% to mention: (Bayesian Rule Lists: \cite{letham2015interpretable} tipo decision trees)

% \begin{itemize}
%     \item taxonomy
%     \begin{itemize}
%         \item intrinsic or post-hoc? LENs support both!
%         \item result of the interpretation:
%         \begin{itemize}
%             \item Feature summary statistic (feature importance or pairwise feature interactions or rank visualization)
%             \item Model internals (weights in linear models or the learned tree structure)
%             \item Data point (counterfactual explanations or identification of prototypes of predicted classes)
%             \item Intrinsically interpretable model
%         \end{itemize}
%         \item Model-specific or model-agnostic?
%         \item Local or global?
%     \end{itemize}
%     \item Properties of Explanation Methods
%     \begin{itemize}
%         \item Expressive Power is the "language" or structure of the explanations (IF-THEN rules, decision trees, a weighted sum, natural language or something else)
%         \item Translucency describes how much the explanation method relies on looking into the machine learning model
%         \item Portability 
%         \item Algorithmic Complexity
%     \end{itemize}
%     \item Properties of Individual Explanations
%     \begin{itemize}
%         \item Accuracy: How well does an explanation predict unseen data?
%         \item Fidelity: How well does the explanation approximate the prediction of the black box model?
%         \item Consistency: How much does an explanation differ between models that have been trained on the same task and that produce similar predictions?
%         \item Stability: How similar are the explanations for similar instances?
%         \item Comprehensibility: How well do humans understand the explanations?
%         \item Certainty: Does the explanation reflect the certainty of the machine learning model?
%         \item Degree of Importance: How well does the explanation reflect the importance of features or parts of the explanation?
%         \item Novelty: Does the explanation reflect whether a data instance to be explained comes from a "new" region far removed from the distribution of training data?
%         \item Representativeness: How many instances does an explanation cover?
%     \end{itemize}
%     \item good explanations
%     \begin{itemize}
%         \item Explanations are contrastive (Lipton 1990)
%         \item Explanations are selected (simple)
%         \item Explanations are social. They are part of a conversation
%         \item Explanations focus on the abnormal. People focus more on abnormal causes to explain events (Kahnemann and Tversky, 1981).
%         \item Explanations are truthful. Good explanations prove to be true in reality
%         \item Good explanations are consistent with prior beliefs of the explainee
%         \item Good explanations are general
%     \end{itemize}
%     \item interpretable models: logistic regression, decision trees, decision rules and the RuleFit algorithm
%     \item model agnostic: 
%     \begin{itemize}
%         \item plots: Accumulated local effects, Partial Dependence Plot, Individual Conditional Expectation
%         \item surrogates: Global Surrogate, Local Surrogate (LIME), \textbf{Scoped Rules (Anchors)} (many scenarios require discretization, many calls to the ML model), \textbf{SHAP} (SHapley Additive exPlanations)
%     \end{itemize}
%     \item example based: Counterfactual explanations, Prototypes
%     \item neural networks: Feature Visualization, Concepts, Modell Distillation (How can we explain a neural network with a simpler model?)
% \end{itemize}

% \paragraph{Occam's razors}
% In his Posterior Analytics, Aristotle stated: "We may assume the superiority ceteris paribus [other things being equal] of the demonstration which derives from fewer postulates or hypotheses" \cite{aristotlePosterior}. The \textit{law of parsimony} presented by the Greek philosopher has deeply influenced researchers and scientists across the centuries. In other words, when humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one. Researchers have proposed many approaches to integrate this parsimony principle into learning machines over the years. Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous approaches. Among such techniques, $L1$-regularization \cite{santosa1986linear,tibshirani1996regression} has been recently shown quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages sparsity by shrinking the less important weight's values to zero thus removing some weights altogether in the limit. Following \cite{ciravegna2020human}, the models analyzed in this work are mainly based on $L1$-regularization. However, in future works it may also worth exploring the integration of LENs with concept-based parsimony criteria \cite{chen2020concept} or with fuzzy-logic regularizers which have recently been used to combine deductive reasoning and human priors with deep learning \cite{marra2019lyrics}.




\section{Conclusion} \label{sec:conclusion}

\subsection{Limitations and future research directions}
The extraction of a first-order-logic explanation requires symbolic input and output spaces. This constraint is the main limitation of our framework, as narrows the range of applications down to symbolic I/O problems. In some contexts, such as computer vision, the use of LENs may require additional annotations and attribute labels to get a consistent symbolic layer of concepts. However, recent work on automatic concept extraction may partially solve this issue leading to more cost-effective concept annotations \cite{ghorbani2019towards,kazhdan2020now}.

Another area to focus on might be the improvement of out-of-the-box LENs. The efficiency and the classification performances of fully interpretable LENs, i.e. $\psi$ network, is still quite limited due to the extreme pruning strategy. Even more flexible approaches, like $\mu$ networks, are not as efficient as standard neural models when tackling multi-class or multi-label classification problems, as they require a bigger architecture to provide a disentangled explanation for each class.

In our vision this framework would thrive and express its full potential by interacting with the external world and especially with humans in a dynamic way. In this case, logic formulas might be rewritten as sentences to allow for a more natural interaction with end users. Moreover, a dynamic interaction may call for an extended expressivity leading to higher-order or temporal logic explanations. Finally, in some contexts different explainer architectures as graph neural networks might be worth exploring as they may be more suitable to solve the classification problem.


\subsection{Broader impact}
Current legislation in US and Europe binds AI to provide explanations especially when the economical, ethical, or financial impact is significant \cite{gdpr2017,law10code}. This work contributes to a lawful and safer adoption of some of the most powerful AI technologies allowing deep neural networks to have a greater impact on society. Extracting first-order-logic explanations from deep neural networks enables satisficing knowledge distillation while achieving performances comparable with the state of the art. The formal language of logic provides clear and synthetic explanations, suitable for laypeople, managers, and in general for decision makers outside the AI research field. 

The experiments show how this framework can be used to aid bias identification and to make black boxes more robust to adversarial attacks by giving an explanation for the attack itself. As out-of-the-box LENs are easy to use even for neophytes and can be effectively used to understand the behavior of an existing algorithm, our approach might be used to reverse engineer competitor products, to find vulnerabilities, or to improve system design. From a scientific perspective, formal knowledge distillation from state-of-the-art networks may enable scientific discoveries or confirmation of existing theories.


\section*{Acknowledgments and Disclosure of Funding}
We thank ... for useful feedback and suggestions.

This work was partially supported by the European Union’s Horizon 2020 research and innovation programme under grant agreement No 848077.





% \begin{itemize}
%     \item reliable concept bottlenecks may require concept annotation (but...)
%     \item only for classification / clustering (not suitable for regression) -> can we extend the framework?
%     \item multi-class classification requires for $\mu$ nets to have very big architectures (or one network for each task) -> not efficient!
%     \item get more efficient and deeper fully interpretable models like $\psi$ nets
%     \item integration with reasoning in a single pipeline?
%     \item interaction with the external world (like reinforcement learning)?
%     \item reformulate a logic rule as a less formal description (like a sentence) for laypeople?
%     \item higher-order logic? temporal logic? ethical logic?
%     \item other neural architectures for the explainer are not covered but might be worth exploring, especially GNNs
% \end{itemize}

% \begin{itemize}
%     \item legislation bounds AI to give explanations especially when the economical, ethical or financial impact is big -> hence this work broadly contributes to let black-boxes like NN have an impact on society!
%     \item the coolest thing is: it is very flexible (it can be used for ANY classification problem), the PYPI and OOTB LENs are easy to to use for neophytes! -> all developers can use it!
%     \item the explanations can be arbitrarily simple and their structure (FOL) is fantastic for decision making -> they can be effectively used to provide explanations to non-developers and laypeople!
%     \item it can be efficiently used to aid bias identification and in making black-boxes more robust against adversarial attacks -> detection of attack and understanding of the impact
%     \item as a result: it may enable safer industrial applications, product developments (self-driving cars)
%     \item applications in management for joint decision making! like decision trees but better!
%     \item finally it may enable scientific discovery by distilling knowledge from trained NNs
%     \item concerns about privacy issues as it may be used to understand the behaviour of any algorithm and infer how the product is made
%     \item but the same feature may be used for improving system design!
%     \item elements for discussion
%     \begin{itemize}
%         \item Is there any direct or indirect malicious use of this research result?
%         \item Will it cause security or privacy issues?
%         \item Who will use your research?  Is it a foundational research, or could it be directly applied or productized?
%         \item Does  your  research  contribute  to  progress  on  safety,  security,  beneficial uses, or defense against malicious use?
%         \item How could your research be involved in an accident with harmful consequences?
%         \item Safeguarding Against Biases
%         \item Making AI Trustworthy
%         \item Complying with Right to Explanation Legislation: In the regulation of algorithms, AI is legally bound to give an explanation of its decisions to the users, especially when it significantly affects them legally or financially. Some examples of right to explanation regulations are the General Data Protection Regulation in the EU, the US Code of Federal Regulations and the Digital Republic Act of France. XAI, therefore, enables AI to comply with the legal requirement to provide an explanation.
%         \item Improving System Design
%         \item Making AI Robust Against Adversarial Attacks
%         \item Making Scientific Discoveries
%     \end{itemize}
% \end{itemize}

% toc
% \section{Logic Explainer Networks}



% \subsection{Classification styles}
% \begin{itemize}
%     \item Interpretable classification (or explainability by design)
%     \item Explanation of an existing classifiers
% \end{itemize}

% \subsection{Explanation styles}
% \begin{itemize}
%     \item Class driven (IFF, IF)
%     \item Relations among classes (MI, CNF)
% \end{itemize}


% \paragraph{Firing paths in relu nets}
% For any input $\textbf{x} \in \mathbb{R}^{d}$, the initial DAG ${\cal G}$ of a deep network equipped with ReLU activations is reduced to ${\cal G}_{\textbf{x}}$
% which only keeps the units corresponding to active neurons and the corresponding arcs (firing path). 
% Since all neurons operate in ``linear regime'' (affine functions), as stated in the following, 
% the transoformation $f(\textbf{x}) = \hat{y}$, which is the composition of affine functions, corresponds to a single affine function.

% \begin{itemize}
%     \item define what is an affine function
%     \item theorem: composition of affine functions correspond to a single affine function
%     \item define what is a firing path in a NN (for a single input)
%     \item show that (in a relu net) a firing path is a composition of affine functions, so: a firing path corresponds to a single affine function (shallow neural network) $f^*$
%     \item show that, by analyzing the parameters of $f^*$, it is possible to identify the most relevant features which explain the prediction for a single input
%     \item define local explanation for a single input: conjunction of relevant features (possibly negated)
%     \item define global explanation for a class: disjunction of local explanations for inputs sharing the same class prediction
% \end{itemize}







\bibliographystyle{apalike}  % Sry Pietro, just had to
\bibliography{references}  %%% Remove comment to use the external .bib file (using bibtex).
%%% and comment out the ``thebibliography'' section.

\end{document}


==> main_sm.tex <==

% \usepackage{icml2021}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[pagebackref=true,
    breaklinks=true,
    colorlinks,
    linkcolor=blue,
    citecolor=blue,
    filecolor=black,
    urlcolor=blue,
    bookmarks=false]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{caption}
\usepackage{subcaption}

\setcounter{secnumdepth}{6}


\usepackage{tikz}
% \usetikzlibrary{decorations}
\usetikzlibrary{decorations.text}
\usetikzlibrary{arrows.meta,bending,decorations.markings}


\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

\usepackage{pifont}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{float}
\usepackage{fontawesome}
\usepackage{makecell}

\def\UrlFont{\rmfamily}
\usepackage{fancyhdr}
\usepackage{mathrsfs} 
\usepackage{color}
\usepackage{hyperref}
\usepackage{longtable}
\hypersetup{colorlinks=true}
% \usepackage[linesnumbered, ruled]{algorithm2e}


\newtheorem{definition}{Definition}[]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{example}{Example}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\graphicspath{ {./images/} }


\def\[#1\]{$$#1$$}

\def\frac#1#2{{#1\over#2}}
\def\eps{\varepsilon}

\def\bbR{{\bf R}}
\def\X{{\bf X}}
\def\meno{\medskip\noindent}

\newcommand{\fg}[1]{\textcolor{red}{F: #1}}
\newcommand{\gc}[1]{\textcolor{red}{G: #1}}
\newcommand{\sm}[1]{\textcolor{blue}{#1}}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.5}


\title{\sm{Logic} Explained Networks}

\author{Gabriele Ciravegna\thanks{Equal contribution}\hspace{1.2mm}$^{1,2}$\hspace{1.2mm}\href{https://orcid.org/0000-0002-6799-1043}{\includegraphics[scale=0.06]{orcid.png}}, 
Pietro Barbiero$^{*3}$\hspace{1mm}\href{https://orcid.org/0000-0003-3155-2564}{\includegraphics[scale=0.06]{orcid.png}}, 
Francesco Giannini$^{*2}$, \\
\textbf{
Marco Gori$^{2,4}$\hspace{1mm}\href{https://orcid.org/0000-0001-6337-5430}{\includegraphics[scale=0.06]{orcid.png}}, 
Pietro Li\'o$^{3}$, 
Marco Maggini$^{2}$, 
Stefano Melacci$^{2}$\hspace{1mm}\href{https://orcid.org/0000-0002-0415-0888}{\includegraphics[scale=0.06]{orcid.png}}
}\\
$^{1}$Universita' di Firenze (Italy), $^{2}$Universita' di Siena (Italy), \\ $^{3}$University of Cambridge (UK), \sm{$^{4}$Universitè Côte d’Azur (France)}\\
\texttt{gabriele.ciravegna@unifi.it, pb737@cam.ac.uk, fgiannini@diism.unisi.it}\\
\texttt{\sm{marco.gori@unisi.it, pl219@cam.ac.uk, marco.maggini@unisi.it, mela@diism.unisi.it}}
}

\begin{document}
\maketitle
\begin{abstract}
\sm{The large and still increasing popularity of deep learning clashes with a major limit of neural network architectures, that consists in their lack of capability in providing human-understandable motivations of their decisions.}
%Despite the increasing popularity of deep \sm{networks in real-world application}, in real wold domains the employment of deep neural networks is still limited and strongly criticized due to their lack of interpretability. 
\sm{In situations in which the machine is expected to support the decision of human experts, providing a comprehensible explanation is feature of crucial importance.}
%providing a comprehensible explanation for a certain classification task can be crucial in decision support contexts. 
\sm{The language used to communicate the explanations must be formal enough to be implementable in a machine and friendly enough to be understandable by a wide audience.}
%To this aim, rule-based explanations expressed in a high-level language are particularly relevant. 
In this paper, we \sm{propose} a general approach to Explainable Artificial Intelligence \sm{in the case of neural architectures}, showing how a mindful design of the networks leads to interpretable deep learning models called \sm{Logic} Explained Networks (LENs). 
\sm{LENs} only require \sm{their inputs} to be semantically meaningful and human understandable predicates, \sm{and they provide explanations in terms of simple First-Order Logic formulas involving such predicates.} LENs are general enough to cover a large number of scenarios. Amongst them, we consider the case in which \sm{LENs are directly used as special classifiers} with the capability of being explainable, or when they act as additional networks with the role of creating the conditions for \sm{making a black-box classifier explainable by FOL.} 
Explanations can be either \sm{local (single-example level) or global (problem level)}, and,
despite supervised learning problems are mostly emphasized, 
%and are given as first-order logic formulas expressed in terms of input concepts. 
we also show that LENs can learn to provide explanations in unsupervised learning settings.
%to provide explanations of the predictions made either by a black-box model or by the LEN itself. 
We describe and \sm{evaluate three different use-cases of the LEN framework}, based on multiple out-of-the-box LEN models. Experimental results on several datasets and tasks \sm{show} that LENs not only \sm{yield better classifications than established white-box models}, such as decision trees and Bayesian rule lists, but \sm{they} also provide \sm{more compact} and meaningful explanations.
\end{abstract}


\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/vis_abs.png}
\caption{\sm{Logic Explained Networks (LENs) are neural networks capable of making predictions and providing First-Order Logic explanations. In detail, A LEN (blue box -- function $f$) provides FOL explanations (purple box -- function $\varphi$) of a set of output concepts (rightmost yellow-box -- output concepts belong to set $E$) in function of the LEN inputs, that might be other concepts (mid yellow box -- input concepts belong to $C$) computed by a neural network (gray box -- function $g$) and/or concepts provided within the available data (leftmost yellow box -- data belong to $X$), following the dotted connection). } %Colors are used in all figures to identify different parts of the framework: yellow boxes contain input data and concepts, output predictions and labels; grey boxes represent the black box classifier $g$ that can either provide final classification or extract low-level concepts; the blue box represents the LEN $f$; t
\sm{There are several different ways of instantiating this generic model into real-world problems, that are described in Section~\ref{sec:basics}. 
Within the blue box, the key components of LENs are listed, that are the main subject of Section~\ref{sec:methods}: } Learning Criteria (Section~\ref{sec:learncrit}), FOL Rule Extractor (Section~\ref{sec:logic_rule_extr}), and the Parsimony Criteria (Section~\ref{sec:parsimony}).
}
    \label{fig:framework}
\end{figure}

\begin{figure}[h]
    \centering

     \includegraphics[width=0.9\textwidth]{figs/abstract.pdf}
         \caption{\sm{An example of a possible instance of the generic model of Fig.~\ref{fig:framework}, inspired by the CUB 200-2011 fine-grained classification dataset. Classes are divided into a two-level hierarchy.} {\color{red}[Add a citation to the dataset.]} A LEN is placed on top of a convolutional neural network $g(\cdot)$ in order to \textit{(i)} classify the species of the bird in input and \textit{(ii)} provide an explanation on why it belongs to this class. {\color{red}[Add at least another output concept (no need to show its explanation). Avoid being to strictly close to the CUB dataset, otherwise the example is not clear. In other words, make black-footed-albatross the name of the output concept (instead of 'bird') and also add another one. Rename the input concepts with the names that are in the purple box. If they are too long, you can shorten them by renaming them in a more simple manner (hooked-bill, solid-wing, medium-size, white-throat, black-bill). Moreover, user the lower-case $x$ instead of $X$.]}}
         \label{fig:len}

\end{figure}


\section{Introduction}
The lack of transparency in the decision process of some machine learning models, such as neural networks, \sm{limits} their application in many safety-critical domains \cite{chander2018working}. Employing black-box\footnote{\sm{In the context of this paper, a black-box classifier is any classifier that cannot provide human understandable explanations about its decisions}} models may be unacceptable in contexts such as industry, medicine or courts, where the potential economical or ethical repercussions are calling for lawmakers to discourage from a reckless application of non-interpretable models \cite{gdpr2017,law10code,goddard2017eu,gunning2017explainable}. As a consequence, research in Explainable Artificial Intelligence (XAI) has become strategic and has been massively encouraged, leading to the development of a variety of techniques that aim at explaining black-box models \cite{das2020opportunities,brundage2020toward} or at developing effective interpretable models \cite{carvalho2019machine,rudin2019stop}. 
% Some of the latter case, like decision rules, provide one of the best forms of explanations as they were originally developed for decision support systems \cite{sprague1980framework}.

The notions of \emph{interpretability} and \emph{explainability} were historically used as synonyms, however nowadays the distinction between interpretable models and models providing explanations has become more \sm{evident}, as recently discussed by different authors \cite{gilpin2018explaining,lipton2018mythos,marcinkevivcs2020interpretability}. 
{\color{red}[Say something on the definitions of interpretability and explainability, connected to what follows (we need to define what we mean with these terms).]}
In some contexts, the use of a black-box model may be unnecessary or even not preferable \cite{rudin2019stop}. For instance, a proof of concept, a prototype, or the solution to a simple classification problem can be easily based on standard out-of-the-box AI solutions which are interpretable by design.
However, interpretable models may generally miss to capture complex relationships among data. Hence, in order to achieve state-of-the-art performance in more challenging problems, it may be necessary to exploit black-box models that, in turn, may require an additional explanatory model to gain the trust of the user. 

In the literature, there is a wide consensus on the necessity of having an explanation for machine learning models that are employed in safety-critical domains, while there is not even agreement on what an \emph{explanation} actually is, nor if it could be formally defined \cite{doshi2017towards,lipton2018mythos}.
An explanation should serve cognitive-behavioral purposes such as engendering trust, aiding bias identification, or taking actions/decisions \cite{srinivasanexplanation}. An explanation may help humans \sm{understand} the black box, may allow for a deeper human-machine interaction \cite{koh2020concept}, and may engender trust on fully automated tasks. All of this is possible as long as the explanations are useful from a human perspective.
% and take into account how humans think and make decisions
In a nutshell, an explanation is an answer to a ``why'' question %\cite{miller2019explanation}. 
%But what is that characterize a good explanation? 
and what makes an explanation good or bad depends on ``the degree to which a human can understand the cause of a decision'' \cite{miller2019explanation}. The goodness of an explanation is intimately connected to how humans collect evidences and eventually make decisions. 
In Herbert Simon's words we may say that a good explanation is \textit{satisficing} \cite{simon1956rational}, i.e. \textit{it either gives an optimal description of a simplified version of the black box (e.g. a surrogate model) or a satisfactory description for the black box itself}
% \footnote{"Decision makers can satisfice either by finding optimum solutions for a simplified world, or by finding satisfactory solutions for a more realistic world".}
\cite{simon1979rational}. However, the notion itself of explanation generally depends on both the domain of the application and who it is aimed at \cite{carvalho2019machine}.
% This is the reason why, different criteria and taxonomies 
% such as the \textit{scope}, the \textit{usage} and the \textit{methodology} have been identified as key-properties to define a XAI technique \cite{das2020opportunities}. 


The need for high-quality evidences is one of the main reasons why concept-based explanations are receiving ever-growing consideration. \sm{Explanations are} given in terms of human-understandable symbols (the \textit{concepts}) rather than raw features such as pixels or characters \cite{kim2018tcav,ghorbani2019towards,koh2020concept}. As a consequence, they seem more suitable to serve many strategic human purposes such as decision making tasks. For instance, a concept-based explanation may describe a high-level category through its attributes as in ``a \textit{human} has \textit{hands} and a \textit{head}''.
% However, many concept-based explanations still look ambiguous, it is not obvious how to \textit{quantitatively} assess their generality, and may not be suitable for effective decision making at all.
% How much effort requires analyzing a pairwise dependence plot \cite{friedman2008predictive} or a ranking of SHAP values \cite{NIPS2017_7062} or a decision tree with depth 10 \cite{breiman1984classification} for domain experts? How much for laypeople?
% If you are looking for a quick and comprehensible answer these methodologies will not suit your needs.
While collecting high-quality evidences for an explanation is a common feature of concept-based techniques, there are very few approaches formulating hypothesis and even less providing synthetic descriptions whose validity can be quantitatively assessed \cite{das2020opportunities}.
A possible solution is to rely on a formal language that is
% synthetic but also 
very expressive and closely related to natural language and reasoning, such as First-Order Logic (FOL). A FOL explanation can be considered a special kind of \sm{a} concept-based explanation, where the description is given in terms of logical predicates, connectives and quantifiers, such as ``$\forall x:\ \textit{is\_human}(x) \rightarrow \textit{has\_hands}(x) \wedge \textit{has\_head}(x)$''. However, FOL formulas generally express much more complex relationships among the concepts %that are 
involved in a certain explanation. Compared to other concept-based techniques, logic-based explanations provide many key advantages, \sm{that we briefly described in what follows}.
% \begin{itemize}
% CLARITY
An explanation reported in FOL is a rigorous and unambiguous statement (\textsc{clarity}). This formal clarity may serve cognitive-behavioral purposes such as engendering trust, aiding bias identification, or taking actions/decisions. For instance, \sm{dropping quantifiers and variables for simplicity}, the formula ``\textit{snow} $\wedge$ \textit{tree} $\leftrightarrow$ \textit{wolf}'' may easily outline the presence of a bias in the collection of training data.
% MODULARITY
Different logic-based explanations can be combined to describe groups of observations or global phenomena (\textsc{modularity}). %Different observations of the same phenomenon may have completely different %logic-based 
%explanations according to their characteristics. 
For instance, for an image showing only the face of a person, \sm{an} explanation could be ``(\textit{nose} $\wedge$ \textit{lips}) $\rightarrow$ \textit{human}'', while for another image showing a person from behind a valid explanation could be ``(\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})  $\rightarrow$ \textit{human}''. The two local explanations can be combined \sm{into} ``(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears}) $\rightarrow$ \textit{human}''.
% MEASURABILITY
The quality of logic-based explanations can be quantitatively measured
    % on independent data sets 
to check their correctness and completeness (\textsc{measurability}). For instance, once the explanation ``(\textit{nose} $\wedge$ \textit{lips}) $\vee$ (\textit{feet} $\wedge$ \textit{hair} $\wedge$ \textit{ears})'' is extracted for the class \textit{human}, this logic formula can be applied on a test set to check its generality in terms of quantitative metrics like accuracy, fidelity and consistency.
% SIMPLIFIABILITY
\sm{Finally,} FOL-based explanations can be rewritten in 
    different equivalent forms such as in \emph{Disjunctive Normal Form} (DNF) and \emph{Conjunctive Normal Form} (CNF)  (\textsc{simplifiability}). Further, techniques such as the Quine–McCluskey algorithm can be used to compact and simplify logic explanations \cite{mccoll1878calculus,quine1952problem,mccluskey1956minimization}. For instance, the explanation ``(\textit{person} $\wedge$ \textit{nose}) $\vee$ ($\neg$\textit{person} $\wedge$ \textit{nose})'' can be easily simplified in ``\textit{nose}''.
% \end{itemize}


This paper presents a unified framework for XAI where a neural network, the \emph{\sm{Logic} Explained Network} (LEN), is trained to \textit{solve-and-explain} a categorical learning problem \sm{integrating elements from deep learning and logic}. 
\sm{Differently from vanilla neural architectures}, LENs can be \sm{directly} interpreted \sm{by means of} a set of \sm{FOL} formulas. \sm{In order to implement such property, LENs require their inputs to represent the activation scores of human-understandable concepts. Then, specifically designed learning objectives allow LENs to make predictions in a way that is well suited for providing FOL-based explanations that involve the input concepts. In order to reach this goal, LENs exploit parsimony criteria aimed at keeping their structure simple.}
% learn a set of explanations of its classification results, or for the class-assignments of another classifier. 
%(eventually another neural network). 
\sm{There are several different computational pipelines in which a LEN can be configured, depending on the properties  of the considered problem and on other potential experimental constraints. For example, LENs can be used to directly classify data in an explainable manner, or to explain another black-box neural classifier. Moreover, according to the user expectations}, different kinds of logic rules may be provided. 
\sm{Due to this intrinsic versatility of LENs, what we propose can also be taught as a generic framework that encompasses a large variety of use cases.}

%This versatility makes the proposed framework 
%and in particular LENs 
%applicable to a wide range of learning tasks \sm{and in different use cases.} % by providing logic-based explanations in different use cases. % and according to different user preferences. 
\sm{Fig.~\ref{fig:framework} depicts a generic view on LENs, in which the main components are reported. A LEN (blue box -- function $f$) provides FOL explanations (purple box) of a set of output concepts (rightmost yellow-box) in function of the LEN inputs. Inputs might be other concepts (mid yellow box) computed by a neural network classifier (gray box -- function $g$) and/or concepts provided within the available data (leftmost yellow box). %The output concepts are the ones that are the main subject of the explanations (e.g., they could be the classes of a classification problem). Explanations involve the inputs of the LEN. 
This generic structure can be instantiated in multiple ways, depending on the final goal of the user and on the properties of the considered problem. In order to provide the reader with an initial example/use-case (different configurations are explored in the paper), we consider an image classification problem with concepts organized into a two level hierarchy. In Fig.~\ref{fig:len} we report an instance of Fig.~\ref{fig:framework} in which a CNN-based neural classifier gets an input image $X$, predicting the activations of a number of low-level concepts (organized in a vertical manner). The LEN $f$ processes such concepts, and it predicts the activation of higher-level output concepts. The LEN can provide a FOL description of each (high-level) output concept with respect to the (low-level) input ones. Another possible instance of the proposed framework consists in using the LEN to directly classify and explain some input data (that is basically the case in which the input concepts are immediately available in the data themselves, and not the output of another neural model), thus the LEN itself becomes an explainable machine. Moreover, LENs can be paired with a black-box classifier operating on the same input data, and forced to mimic as much as possible the behaviour of the black-box, basically implementing an additional  explanation-oriented module. At a first glance, since the internal structure of LENs is subject to a number of constraints, LENs might not be as powerful as a black-box classifier. However, the versatility of LENs allows the user to customize his approach to the considered classification problem in order to find a satisfactory compromise between interpretability and accuracy.}

\sm{We investigate three different use-cases that are inspired by the aforementioned instances, comparing different ways of implementing the LEN models. While most of the emphasis of this paper is on supervised classification, we also show how LEN can be exploited in fully unsupervised settings.}
Additional human priors could be eventually incorporated into the learning process \cite{ciravegna2020constraint}, in the architecture \cite{koh2020concept}, \sm{and, following \cite{ciravegna2020constraint,ciravegna2020human}, what we propose can be trivially extended to semi-supervised learning (out of the scope of this paper).}


%Furthermore, LENs can also be integrated with existing black-box classifiers to extract low-level concepts or to explain their classification results.




%The overall problem configuration of how a Logically Explained Network can be integrated with an existing classifier is shown in Fig. \ref{fig:framework} and further described in Sec. \ref{sec:use_cases}. A configuration example is reported in Fig. \ref{fig:len}.




%Out-of-the-box neural networks based on this framework span a wide range of flavors, from fully interpretable models to black-boxes providing different interpretability-VS-accuracy trade-off.  
%high-quality explanations and state-of-the-art classification performance.

%Further, human priors expressed by FOL formulas can be naturally incorporated with LENs both in the learning process \cite{ciravegna2020constraint} and in the architecture \cite{koh2020concept}. 

Our work contributes to the XAI research field in the following ways.
\begin{itemize}
    \item \sm{It provides} a unifying framework for solving and explaining categorical learning problems with neural networks. We designed the LEN framework inspired by our previous experiences \cite{ciravegna2020human,ciravegna2020constraint}.
    \item \sm{It allows users to decide how to interconnect LENs in the classification task under investigation,} and to express a set of preferences to get one or more customized explanations. We provide and experimentally evaluate three out-of-the-box preset models.
    % \item Supporting a wide range of logic-based explanations from \textit{local explanations} and \textit{node-level explanations}, explaining the prediction for an individual sample or a hidden neuron, to \textit{cluster explanations} up to \textit{class-level explanations} and \textit{global explanations}.
    \item \sm{It offers} a wide range of logic-based explanations at different level of granularity, such as \textit{example}, \textit{local} and \textit{global} explanations, aiming at explaining a single sample, a subset of the available data or the whole dataset, respectively.
    \item \sm{It reports} experimental results confirming how LENs generalize better in terms of model accuracy than established white-box models such as decision trees on complex Boolean tasks (as observed in \cite{tavares2020understanding}).    
    \item \sm{It advertises our public} implementation of LENs through a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on out-of-the-box LENs, implementing different trade-offs between intepretability, explainability and accuracy. {\color{red}[This goes back to my previous comment on better defining these terms.]}
\end{itemize}

% \paragraph{Reading path} 
The paper is organized as follows. Related works are described in Section \ref{sec:related}. Section \ref{sec:basics} gives a formal definition of a LEN and it describes its underlying assumptions, key paradigms and design principles. The methods used to extract logic formulas and to effectively train LENs are described in Section \ref{sec:methods}. Three out-of-the-box LENs, presented in Section \ref{sec:outofthebox}, are compared on a wide range of benchmarks in terms of classification performance and quality of the explanations, in Section \ref{sec:experiments}. 
% A coding example showing how to use LENs with the associated python library is shown in Section \ref{sec:tool}. 
Finally, Section \ref{sec:conclusion} outlines the social and economical impact of this work as well as future research directions.


\section{Related work}
\label{sec:related}


In the last few years, the demand for human-comprehensible models has significantly increased in safety-critical and data-sensible contexts. This popularity is justified by the emerging need for unveiling the decision process of pitch-black models like deep neural networks. To this aim, the scientific community has developed an important variety of XAI techniques, with different properties and goals. Several taxonomies have been proposed to categorize the XAI models, with partial overlapping and some ambiguities on the referred terminology. Without pretending to be exhaustive, in the following we only focus on some key-properties that are relevant to compare LENs with other existing approaches. In particular, we will \sm{describe} related works \sm{considering the type of} \textsc{result} \sm{they provide} (feature-scoring vs. rule-based), 
\sm{their specific} \sm{\textsc{role}} (interpretable models vs. explanation methods), 
and the \textsc{scope} of the provided explanations (local vs. global). A brief summary of a few XAI works in terms of these features is reported in Tab.~\ref{tab:related_work} -- for more details on existing taxonomies we refer, e.g., to the following surveys \cite{adadi2018peeking,carvalho2019machine,marcinkevivcs2020interpretability,molnar2020interpretable}.

%\textsc{Results of Explanation Methods. }
XAI models can be differentiated according to the \textsc{result} of the produced explanation. 
Most of the methods in literature usually focus on scoring or providing summary statistics of features. However, \textit{feature-scoring} methods
%
can be of scarce utility in decision support cases, whereas a comprehensible language may bring light on the black-box behaviour by identifying concept-based correlations.
% do not consider how concepts are interconnected, therefore, these explanations may not live up to the expectations. 
On the other hand, \emph{rule-based} explanations are generally more comprehensible, since they usually rely on a formal language, such as \sm{FOL}. Further, the learned rules can be directly applied to perform the learning task in place of the explained model.
%\textsc{Explanation Usage. }
\sm{Existing approaches has different \textsc{roles} in the XAI landscape, acting as intrinsically \emph{interpretable models} or as \emph{explanation methods}. }
\sm{As a matter of fact,} the interpretability of a model can be achieved either by constraining the model to be interpretable per se (\emph{interpretable models}) or by applying some methods to get an explanation of an existing model (\emph{explanation methods}). Interpretable models are by definition {model specific}, while explanation methods can rely on a single model or be, as more commonly happens, {model agnostic}. In principle, interpretable models are the best suited to be employed as decision support systems. However, their decision function often is not smooth which makes them quite sensible to data distribution shifts and impairs their generalization ability on unseen observations \cite{tavares2020understanding,molnar2020interpretable}. 
On the other hand, explanation methods can be applied to get approximated interpretation of state-of-the-art models. These methods are generally {``post hoc''}, since the explanations are produced when the training procedure is concluded. 
%\textsc{Scope of Interpretability. }
A fundamental feature to distinguish among explainable methods \sm{is the \textsc{scope} of the provided explanations. \textit{Local} explanations are valid for a single given sample, while \textit{global} explanations {hold} on the whole input space}. However, several models consider local explanations together with aggregating heuristics to get a global explanation.

% {\bf Methodology. }
% The algorithms employed by most XAI models can be roughly categorized into two main categories. \textit{Backpropagation}-based techniques analyze the gradients of the activation up to the input features, in order to identify the most relevant ones for the classification task. \textit{Perturbation}-based techniques, instead, observe how the machine output changes when altering a given input data. The aim of these methods is to understand which %are the most discriminative 
% features (when altered) may drive the model to take different decisions. 
% Nonetheless, not all algorithms belong to these two categories. In particular, \textit{Model-intrinsic} explanation methods significantly differ according to the training algorithms.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
                                    & \multicolumn{2}{c|}{\sm{\textbf{Result Type}}} & \multicolumn{2}{c|}{\textbf{Scope}} & \multicolumn{2}{c}{\sm{\textbf{Role}}} \\
                        & feature-scoring & rule-based & local & global & interpretable model & explanation method \\ 
\hline
LIME &\faCheckCircle & & \faCheckCircle            & & & \faCheckCircle  \\
SHAP &\faCheckCircle & & \faCheckCircle & & & \faCheckCircle  \\
% DeConv \cite{zeiler2014visualizing}                     &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           & \faCheckCircle         &               &                  \\
Activation Maximization & \faCheckCircle & & \faCheckCircle  &  &  & \faCheckCircle  \\
Saliency Maps &\faCheckCircle&& \faCheckCircle &      &              & \faCheckCircle \\
% Grad-CAM \cite{selvaraju2017grad}                       &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
SP-LIME &\faCheckCircle&& & \faCheckCircle &              & \faCheckCircle  \\
Class Model Visualization &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle                 \\
% TCAV \cite{kim2018tcav}                                 &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
LORE &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle \\
Anchors &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle  \\
DeepRED   &&\faCheckCircle& \faCheckCircle & \faCheckCircle &  & \faCheckCircle \\
GAM  &\faCheckCircle&&              & \faCheckCircle          & \faCheckCircle            &   \\
Decision Trees       &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
BRL                   &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &               \\
\hline
\textbf{LENs}                                           &&\faCheckCircle& \textbf{\faCheckCircle}    & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle} \\
\end{tabular}
}
\vspace{0.3cm}
\caption{Summary of related work. \sm{The first column lists a number of approaches in the context of XAI. The other columns are about different properties. See the paper text for more details and for a description of all the approaches. }}
\label{tab:related_work}
\end{table}

Some of the most famous XAI techniques share the characteristic of being feature-scoring, local, post hoc methods.
Sometimes indeed, the easiest way to solve the explanation problem is simply to treat the model as a black-box and, sample-by-sample, determine which are the most important features for a prediction. 
Prominent examples of algorithms falling in this area %are Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should}, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} and DeConvolution Neural Network (DeConv) \cite{zeiler2014visualizing}, which
accomplish this task by perturbing the input data. 
Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should} trains a white-box model (e.g., a logistic regression) to mimic the predictions of a given model in the neighbourhood of the sample to explain. By analyzing the weights of the white-box model it identifies the most important \sm{group} of pixels (superpixel).
Differently, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} computes the Shapley value of each feature by removing each of them \sm{in an iterative manner}. %provides for local explanations by computing each input feature contributions in a certain prediction. In the Kernel SHAP version, the Shapley values of each feature are calculated by iteratively removing features in a similar way to what is done in LIME.
% Deconvolutional Network were initially introduce in \cite{zeiler2011adaptive} for unsupervised learning.
% Firstly introduced in \cite{zeiler2011adaptive}, DeConvolution Neural Network (DeConv) are used in \cite{zeiler2014visualizing} to %visualize the activation of a convolutional layer. In particular, they 
%visually determine pixel importance for a certain prediction by analyzing how the classification output changes when part of the input image is masked. 
Other important techniques %such as Activation Maximization \cite{erhan2010understanding}, Saliency Maps \cite{simonyan2013deep} and Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} 
provide the same type of explanations through gradient analysis. %Differently from the previous one, however, they determine feature importance  %in the context of Convolutional Neural Network (CNN). 
Authors of Activation Maximization \cite{erhan2010understanding} firstly introduced this idea as an optimization problem. They explain the behaviour of a hidden/output unit by slightly modifying a given input data such that it maximizes its activation. An easier way to identify features causing a certain output has been found with Saliency Maps \cite{simonyan2013deep}, which project the classification loss until the input image. 
% A further improvement has been introduced with Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} which allows to identify both class-specific image area and counterfactual explanations.
%They achieved this by modifying global average pooling with class activation mapping which allows to identify important image area with a single forward pass.
%
Other post hoc methods have been devised to extract global feature-scoring explanations, often starting from local explanations. %like LIME for Global Explanations \cite{ribeiro2016should} based on perturbation and Class Model Visualization \cite{simonyan2013deep} or Testing with Class Activation Vectors \cite{kim2018interpretability} based on Backpropagation. 
A submodular-pick algorithm extends the LIME module (SP-LIME) in %LIME for Global Explanations 
\cite{ribeiro2016should} to provide global explanations. SP-LIME first finds superpixels of all input samples with the standard LIME module. Successively, it finds the minimum number of common superpixels that covers most of the images.
Starting from the idea of Activation Maximization, Class Model Visualization \cite{simonyan2013deep} finds the input sample that maximizes a certain class probability score in the whole input space. %Differently from Activation Maximization, here the input sample is not searched in the neighbourhood of a given sample, but in the whole input space. 
Differently, LENs take a quite different perspective with respect to these methods, \sm{still inheriting several of their properties (see Tab.~\ref{tab:related_work})}. A LEN aims at providing human comprehensible decision support in terms of a set of FOL rules.


Explanation methods, indeed, can also supply FOL explanations. 
LOcal Rule-based Explanations of black-box decision systems (LORE) \cite{guidotti2018local} extracts FOL explanations via tree induction. \sm{The authors of \cite{guidotti2018local}} focus on local rules extracted through input perturbation. For each sample to explain, a simple decision tree is trained to mimic the behaviour of the black-box model in the neighbourhood of the sample. Both standard and counterfactual explanations can then be extracted  following the branches of the tree. 
Again based on LIME, Anchors \cite{ribeiro2018anchors}  also provides local rules of black-box model prediction via input perturbation. In this case, rules are not extracted from a decision tree but are generated by solving a Multi-Armed-Bandit beam search problem. 
Extending the CRED algorithm \cite{sato2001rule}, DeepRED  \cite{zilke2016deepred} employs a decomposition strategy to globally explain neural networks. Starting from the output nodes, each node in a layer is explained in terms of the activations of the previous ones through a decision tree. In the end, all rules for each class are merged in a single global rule in terms of input nodes only. For a single example a single local rule can be extracted following the firing path. 
The approach proposed in this paper is in some sense similar to the DeepRED algorithm. Indeed, \sm{as it will become clear in the following sections}, LENs can explain the behaviour of a neural network both end-to-end and layer by layer. However, LENs can be used to explain any black-box model as far as its input and output are interpretable (Section~\ref{sec:basics}). \sm{Furthermore}, LENs support different forms of FOL rules, with different scopes and goals.

Interpretable models are generally capable of providing both local and global explanations. These explanations may be based again on feature-scoring as in Generalized Additive Models (GAM) or on FOL rules as in Decision Tree \cite{breiman1984classification} and Bayesian Rule Lists (BRL) \cite{letham2015interpretable}. Meant to overcome the non-linearity assumptions of Linear regression, GAM learns to predict the given class for each feature via decision tree. In \cite{caruana2015intelligible}, authors proposed GA$^2$M where attribute interaction is allowed at a pair level. Recently a further extension employing neural network as non-linear function has been proposed in \cite{agarwal2020neural}, which, however, lose interpretability at feature-level.
Decision trees are a greedy learning algorithm which iteratively divides input data into smaller subsets until they only contain elements belonging to the same class. Different pruning algorithms have been also proposed to simplify the resulting structure and therefore the explanations \cite{quinlan1987simplifying}. Each path of a decision tree may be seen as a decision rule\sm{, i.e.,} an \textit{IF-THEN} statement. 
The set of rules may be generated in different ways, either with sequential covering as in \cite{cohen1995fast} or by selecting the best rules from a pre-mined set via Bayesian statistics as in BRL. 
%
\sm{Interestingly, LENs} can be \sm{directly} used to solve a learning task, being almost interpretable per se. 
Employing an interpretable by-design neural network as classifier has the advantage that the extracted explanations will perfectly match the classifier predictions. 
In addition, relying on a neural network, LEN generalization performance can be much better than standard interpretable-by-design methods, that generally have a very limited representation capacity.

Summing up, the proposed approach can be used both as interpretable model and explanation method. \sm{Indeed, the flexibility of LENs allows the user to find an appropriate trade-off between interpretability and accuracy that is well suited for the task at hand.} 
The explanation type of LENs is in terms of FOL rules and different explanation styles, corresponding to different \sm{types} of logic formulas. Such explanations are extracted with different scopes, from local rules valid on a single sample to global rules \sm{that hold} for an entire class.





\section{\sm{Logic} Explained Networks}
\label{sec:basics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%O
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTATION REMINDER
%\fg{mettere in tabella es alla fine del 2.1?}
% {\color{red}
% \textbf{Notation}
% X = input space (non-interpretable)\\
% Y = symbolic output space (interpretable)\\
% C = symbolic "concept" space (interpretable)\\
% E = symbolic "rule" space (interpretable)\\

% n = \# samples\\
% d = \# features of X\\
% q = \# categories of Y\\
% k = \# categories of C\\
% r = \# categories of E\\
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DISCORSINO intro su cosa è il nostro modello, cosa fa, a cosa si appoggia.. caratteristiche generali


% Differently from several existing XAI models, 
We consider a general framework in which a special kind of neural network, \sm{referred to as Logic Explained Network (LEN), is used to make predictions and provide explanations about them, or it is used to}  explain the behaviour of another classifier, \sm{being} it another neural network or \sm{another generic} black-box model. \sm{Moreover, a LEN might also be used to explain relationships among some given data.}
%LENs can be defined according to different criteria and exploited in different use cases. 
\sm{In this section we will formally introduce LENs and the notation used throughout the paper. Then, instead of immediately diving into the internals of LENs (Section~\ref{sec:methods}), we will focus on
the different ways in which LENs can be set up. In particular, we consider how LENs can be instantiated in the framework of Fig.~\ref{fig:len}, discussing a variety of computational pipelines (Section~\ref{sec:use_cases}), and on the type of explanations that we can ask the LEN to generate (Section~\ref{sec:explanation_styles}).} %Fig.~\ref{fig:scheme1} provides an overview of the main topics covered in this section.

\iffalse
\begin{figure}[h]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme1.png}
    \includegraphics[width=0.6\textwidth]{figs/lens_1.pdf}
    % \input{tikz/framework}
    \caption{\sm{Basics of LENs (Section~\ref{sec:basics}). In order to setup a LEN-based model, first, the way the LENs communicate with a black-box classifier or directly with the data must be defined (what we refer to as computational \textsc{pipeline} Section~\ref{sec:use_cases}). The type of expected explanations has a direct consequence in the objective that drives the learning of the LENs parameters (\textsc{learning and explanations}, Section \ref{sec:explanation_styles}). {\color{red}[Remove the word 'explainer' from the 3 points in Pipeline.
    Remove the word 'explanations' from the white box on the right.]} } 
    }
    \label{fig:scheme1}
\end{figure}
\fi

%There are different ways of letting LENs communicate with a black-box classifier

%and for which
%the main aspects on what LENs can be used for and which kind of explanation we may get with 
%learning problems it applies (see Fig. \ref{fig:scheme1}).

%Let us consider a standard classification problem where a classifier f defines the membership values of

\sm{A LEN is a function $f$, implemented with a neural network, that map data falling within a $k$-dimensional Boolean hypercube onto data that fall within another $r$-dimensional Boolean hypercube. Each dimension is about the activation strength of what we refer to as \textit{concept}, with the strict requirement of having a human-understandable description of each \textit{input} dimension/concept. 
Formally, LEN is a mapping $f: C \rightarrow E$, \sm{where $C = [0,1]^{k}$ is the \textit{input concept space}, and $E = [0,1]^{r}$} is the so called \textit{output concept space}. Explanations are given in terms of the input concepts, while the $r$ output concept activations are about the truth degrees of $r$ FOL rules. Whenever a LEN has been trained, the $i$-th output concept can be directly translated into a FOL rule $\varphi_i$ such as the one shown in Fig.~\ref{fig:len}. Rules can be then aggregated to different extents, altering their granularity level from a local to a more global coverage of the available data.
}

\sm{In order to provide a concrete meaning to the LEN model, we have to define the source of the input concept activations and how to learn the criteria that allow LENs to predict the output concepts/rules. Amongst a variety of possible configurations that are instance of Fig.~\ref{fig:framework}, we will focus on a finite set of computational pipelines in which the input and output concept spaces are defined with respect to real-world use-cases. In some of them, LENs communicate with a black-box classifier, with the goal of providing explanations of its predictions, or with the goal of exploiting its predictions to model the LEN input concept activations.
In all the cases, for each input sample, LENs provide $r$ FOL explanations that might be directly associated to $r$ categories of a classification problem or they could be interpreted as $r$ generic different explanations of the input data. In the former case, LENs are trained in a supervised manner, while in the latter case they are trained in an unsupervised setting.}

\sm{Before going into further details, we introduce the entities and the notation that will be used throughout the paper.
\begin{itemize}
\item We consider a scenario in which we have the use of a collection $\mathcal{X}$ of $n$ data samples belonging to $X\subseteq\mathbb{R}^d$ to train LENs. 
\item The notation $\mathcal{C}$ indicates a discrete set of $n$ elements belonging to the space $C$ of the input concepts. The data in $\mathcal{C}$ are directly associated to the data in $\mathcal{X}$, i.e., for each element in $\mathcal{X}$ there is a corresponding element in $\mathcal{C}$.
\item \sm{We use the notation $q$ to indicate the total number of classes in a classification problem. Each data sample can be associated with one or more classes. No strict conditions are posed on the potential mutual exclusivity of the different classes, thus we consider the most generic setting that spans from multi-label to single-label classification. Moreover, classes could also be organized in a structured manner, such as in hierarchy. Classes are encoded with binary targets belonging to $\bar{Y} = \{0,1\}^{q}$. We will use the notation $\bar{Y}_{(a:b)}$ to indicate a projection of $\bar{Y}$ limited to the dimensions going from index $a$ to index $b$ -- included. The function $\bar{y}(\cdot)$ returns the binary target vector associated to the data sample passed as its argument, while $\bar{y}_i(\cdot)$ returns the binary label restricted to the $i$-th class.} %The classification problem might also be structured in a hierarchical manner. In this case, at each level $\ell$ of the hierarchy we have $q^{(\ell)}$ classes, $\ell \in [1,h]$.
%\sm{In the case of hierarchically organized classes, the higher-level classes are predicted in function of the ones activated at the lower levels, $g^{(\ell)}: Y^{(\ell-1)} \rightarrow Y^{(\ell)}$, $\ell \in [1,h]$, where $Y^{(0)} = X$.}
\item The function $g$ is about a generic black-box neural classifier,
%\footnote{With "black box classifier" we mean that there are no assumptions on the classifier structure. The classifier architecture could be totally unknown to the logically explained network, that only requires a $[0,1]$-valued I/O.} 
 where $g: X \rightarrow Y^{(u)}$ defines the membership \sm{scores} of \sm{$x$} to $u$ categories, i.e.,  $g(x)=(g_1(x),\ldots,g_u(x))\in Y^{(u)}$, $Y^{(u)} = [0,1]^{u}$, $u\leq q$, with $g_i(x)=1$ (resp. $g_i(x)=0$) \sm{when} $x$ belongs (does not belong) to class $i$. \sm{The $u$ categories could be exactly the ones of the considered classification problem ($u = q$) or a subset of them ($u < q$). No special conditions are enforced in the definition of $g$.}
 \item The notation $\bar{f}$ is about a Boolean instance of function $f$, in which each output of $f$ is projected to either $0$ or $1$.\footnote{When not directly specified, we will assume $0.5$ to be used as threshold value to compute the projection.} In order to refer to a single output of the vector function $f$ (or $\bar{f}$), the subscript will be used, e.g., $f_i$ (or $\bar{f}_i$). Similarly, for a vector $c \in \mathcal{C}$ with activation scores of concepts, $c_i$ is the $i$-th score, while $\bar{c}_i$ is the Boolean instance of it.
 \item The $j$-th dimension of space $C$ includes a human-readable label. FOL rules generated by LENs will exploit such labels to give understandable name to predicates. In order to simplify the notation, whenever we provide the FOL rule associated to a sample $c \in \mathcal{C}$, we will use the already introduced symbol $\bar{c}_i$ also to refer to the label of the $i$-th dimension. Similarly, in FOL rules, $\bar{f}_i$ will refer to the understandable name of the $i$-th output concept (when available).
\end{itemize}}
The listed elements will play a precise role in different portions of the LEN framework.




\iffalse
such that:
\begin{itemize}
    \item Any input $c\in C$ consists in a $[0,1]$-valued feature or concept vector, i.e. $C \subseteq [0,1]^k$. $C$ is also said the \emph{concept space}. Concepts need to be semantically meaningful since they will be exploited to provide explanations. Many times $X=C$ if $X$ is already semantically meaningful; otherwise a mapping is required.
    \item $f$ can be any neural model, but it is required that $E\subseteq[0,1]^r$ where, for any $c\in C$, $i=1,\ldots,r$, $f_i(c)=1$   means that the $i$-th explanation holds for $c$, viceversa if $f_i(c)=0$. $f_i$ is sometimes called the $i$-th output of the LEN $f$. We refer to $E$ as the \emph{explanation space}. In standard supervised problems $E=Y$, however, LENs can also be employed in other contexts.
    % \item there is no pair $c^i,c^j\in C$, such that $\bar{f}(c^i) \neq \bar{f}(c^j)$ and $\bar{c}^i=\bar{c}^j$, where the overline notation denotes the boolean discretization (thresholded at $0.5$) of values from $[0,1]$ to $\{0,1\}$ values.
\end{itemize}



In a broad sense, a \sm{LEN} for the classifier $g$ can be simply thought of as any neural model $f$ aiming at explaining the decision processes taken by $g$. 

The explanations will generally hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrences or global principles among different classes.




% One of the main advantage of the proposed framework is its versatility, indeed a LEN can be defined according to different user-preferences by serving different purposes. 
%In particular, the layout of a XAI pipeline based on LENs follows the definition of a few aspects concerning the classification problem under investigation and the properties of the required explanations. Setting these points allows the correct definition of a LEN in a learning problem. For clear, this is also schematized in Fig. \ref{fig:scheme1}.
LENs can be integrated in different learning problems with different classifier architectures. How the integration will take place depends on the nature of the input data and the presence of one or more concept bottlenecks among the classes under investigation. LENs can provide different kind of explanations both in supervised and unsupervised learning settings, according to user needs. 
%In particular, we may be interested in individual explanation, i.e. the explanation of the decision taken by the classifier on a specific sample. However, we may also look for more general explanations, such as explaining the decisions taken for a whole class predictions, or even looking for more abstract relations among the classes. 
Indeed, by now, we referred to LENs as neural networks aiming to accomplish a classification task. 
%(either to explain the behaviour of a black box or to solve the classification problem itself). 
However, LENs can also be used in unsupervised learning task. 
In the latter case, the output of the LEN denotes the cluster-assignment.
\fi


\begin{figure}[t]
    \centering
    %\includegraphics[width=0.55\textwidth]{figs/E2E.pdf}
    $\vcenter{\hbox{\includegraphics[width=.40\textwidth]{figs/E2E.pdf}}}$ \quad %\\ \bigskip
    $\vcenter{\hbox{\includegraphics[width=.56\textwidth]{figs/e2e_explaining.pdf}}}$    
    \caption{\sm{End-to-end (E2E) LENs} directly work on input data that are interpretable per se and treated as concepts ($C=X$), \sm{while the output concepts are the activation scores of the classes of the dataset ($r = q$)}. \sm{This is a real-world example from the} MIMIC II dataset \sm{(see the experimental section)}, where patient features are used to classify if \sm{the patient} will survive 28 days after hospital recovery. Left: the LEN solves the classification problem and provides explanation, also referred to as \textit{interpretable classification}. Right: the LEN \textit{provides explanations} of a black-box classifier. {\color{red}[Replace $X=C$ with $X$ (twice). Replace $C$ with $C=X$ (twice). Add $E=[0,1]^{q}$ in place of $f(C)$ (left only). Add $E=Y^{(q)}$ in place of $f(C)$ (right only). Replace $g(C)$ with $Y^{(q)}$. Replace $Y$ (twice) with $\bar{Y}$.]}}
    \label{fig:E2EExplainer}
\end{figure}

\subsection{Computational Pipelines} 
\label{sec:use_cases}
% In general, we can state that the above assumptions about the input data and the classifier are not always valid. However, in the following we will see how we can apply the LEN framework in different use cases where these conditions hold.
%Roughly speaking, a logically explained network $f$ is simply a function mapping $[0,1]$-values to $[0,1]$-values.
%, with the aim of providing itself the final classifications or to provide explanations for a classifier $g$. 
%This very general definition allows the application of LENs to different contexts that can be made consistent with real-unit I/O. 
%The most straightforward way of designing a computational pipeline involving LENs is to let the black-box classifier $g$ predict the activation scores of the $q$ classes and provide them to the LEN. In this way, we have $C = Y$, i.e., the LEN outpt concept space collides with $Y$. This is indeed feasible since $Y$ is bounded by a Boolean hypercube. %However, if the available data are already encoded in a symbolic manner in which the $d$ input features are actually  scores in $[0,1]$ (or in $\{0,1\}$ in the most extreme case) that can be considered the activation scores of $d$ concepts, then we can set $C = X$, and directly provide the data to the LEN. 
%The output space of the LEN can be designed in multiple ways, depending on what is the final goal of the whole system. For example, it could collide with $Y$, i.e., the output space of the black-box $g$, $E=Y$, or it could be a totally new concept space.}

\sm{Among a large set of feasible input/output configurations of the LEN block, here we consider three different computational pipelines that are about three concrete scenarios/use-cases where LENs may be applied, that consist in what we refer to as \textsc{end-to-end}, \textsc{concept bottleneck}, and \textsc{cascading} pipelines.}

%directly working on structured data; in a concept bottleneck-scenario where low-level concepts are first extracted from unstructured data (e.g. images); as a cascade of LENs providing explanations at different level of granularity.

%{\color{magenta}******* TBC ******}

% \paragraph{End-to-end explainer}
\textsc{End-to-end. } The most immediate instance of the LEN framework is the one in which the \sm{LEN block} aims at \sm{directly} explain, \sm{and eventually solve,} a \sm{supervised} categorical learning problem. \sm{In this case, we have $C = X$, and $r = q$, as shown in Fig.~\ref{fig:E2EExplainer}. In order to make the first equality valid with respect to the LEN requirements, the $d$ input features of the data in $X$ must be scores in $[0,1]$ (or in $\{0,1\}$ in the most extreme case), so that they can be considered as activations of $d$ human-interpretable concepts. }
%, i.e., $X=C \xrightarrow[]{f} E$. 
%An E2E LEN assumes that the features of the input space are meaningful individually, i.e. they correspond to human-interpretable concepts. 
%Structured datasets usually fall into this category. 
\sm{Of course, in order to create these conditions in different types of datasets, generic} continuous features can be either discretized into different bins or booleanized by comparing them to a reference ground truth (e.g., for gene expression data, the gene signature obtained from control groups can be used as a reference).
An E2E LEN can perform a fully \textit{interpretable classification} task, having the double role of main classifier and explanation provider (Fig.~\ref{fig:E2EExplainer}, left), or they can work in parallel with another neural black-box classifier $g$, thus {providing explanations} of the predictions of $g$ (Fig.~\ref{fig:E2EExplainer}, right) \sm{with $E = Y^{(q)}$} -- what we refer to as \textit{explaining a black-box}.
%used to explain the predictions of any black box model $g:X\rightarrow Y$, 
%as shown in Fig. \ref{fig:E2EExplainer}.
This first solution is preferred when it is of fundamental importance to have a white-box classifier, while we can accept some drawbacks in terms of classification performances, due to the constrained nature of the LENs.
The second solution is instead useful in those context where the classification performance plays a key role, and we may accept approximate explanations of the decision taken. 

\begin{figure}[t]
\centering
    %\includegraphics[width=0.55\textwidth]{figs/E2E.pdf}
    $\vcenter{\hbox{\includegraphics[width=.48\textwidth]{figs/CBM.pdf}}}$ \quad %\\ \bigskip
    $\vcenter{\hbox{\includegraphics[width=.48\textwidth]{figs/concept_relations.pdf}}}$       
    \caption{\sm{Concept-bottleneck (CB) LEN}. Left: the LEN is placed on top of a black box model $g$ which maps the input data into a first set of interpretable concepts. An MNIST-based experiments is shown \sm{(see the experimental section)}. Handwritten digits are first classified by $g$. A LEN is \sm{then} employed to classify and explain whether the digit is even or odd -- \textit{interpretable classification}. {\color{red}[Replace $g^{(1)}(X)$ on top of the blue column of concepts with $C=Y^{(z)}$. Replace $f(g^{(1)})(X)$ with $E=[0,1]^{(q-z)}$. Remove the superscript $(1)$ everywhere here. Replace the $Y$ on the right with $\bar{Y}_{(z+1:q)}$. Replace $C$ on top with $\bar{Y}_{(1:z)}$.]} Right: \sm{MNIST digits are classified as belonging to one of the 10 classes and whether they are even of odd by a black-box $g$ \sm{(see the experimental section)}.  %in a Concept-bottleneck pipeline 
     A LEN groups these predictions in an unsupervised manner, and analyzes the relations within each cluster -- \textit{interpretable clustering}.} Supervision labels are not provided for the LEN output. {\color{red}[Replace $g(X)$ on top of the blue column of concepts with $C=Y^{(z)}$. Replace  $f(g(X))$ with $E=[0,1]^{r}$. Fix FOL Explanation of Cluster 2 (not 1).]}}
    \label{fig:CMBExplainer} 
\end{figure}

% \paragraph{Concept-bottleneck explainer}
\textsc{Concept-bottleneck. } 
A Concept-Bottleneck (CB) LEN is a computational pipeline in which the LEN $f$ aims at explaining, and eventually solving, a categorical learning problem \sm{in which the data in $X$ are not readily exploitable as LEN inputs, and a black-box model $g$ computes the activations of an initial set of $z$ concepts out of the available data. The LEN solves the problem of predicting $r$ new concepts from the activations of the $z$ ones, as shown in Fig.~\ref{fig:CMBExplainer} (left/right). Differently from the E2E case, there is always a neural network $g$ processing the data, and the outcome of such processing is the input of the LEN. Formally, we have $g: X \rightarrow Y^{(z)}$, while $f: (C=Y^{(z)}) \rightarrow E$.} 
This two-level scenario can be implemented in a way that is coherent with the already discussed example of Fig.~\ref{fig:len}, that is what we also show in Fig.~\ref{fig:CMBExplainer} (left). In this case, each example is labeled with $q$ binary targets divided into two disjoint sets, where the black-box network predicts the first $z < q$ ones, and the LEN predicts the remaining $r = q-z$.
The LEN will be both responsible of predicting the higher level concepts and of explaining them in function of the lower level concepts yielded by the black-box model, thus still falling withing the context of \textit{interpretable classification}.
 We also consider the case in which the outcome of the LEN is not associated to any known classes, thus the LEN is trained in an unsupervised manner, as shown in  Fig.~\ref{fig:CMBExplainer} (right), thus implementing a form of \textit{interpretable clustering}. In both the cases, the black-box classifier $g$ is trained in a supervised manner.\footnote{The extraction process can be either implicit, through the analysis of the latent spaces learnt by the black-box \cite{kazhdan2020now}, or explicit by training a black-box to classify specific concepts \cite{koh2020concept}.}

%\sm{in which the features of the data in $X$ are not interpretable as activations of human-understandable concepts or they are too low-level to be directly involved into compact explanations} (e.g., all the pixels of an image \cite{koh2020concept}). In this case, we assume to have information to process the data in order to extract an initial set of concepts that will be provided to the LEN. 
%Then, given


%In this latter setting, a model $g$ can be used to extract high-level concepts $C$ from raw features in $X$, and then producing the final classification $Y$. In this case, we may assume $g=g^{(2)}\circ g^{(1)}$ with $X\xrightarrow[]{g^{(1)}}C\xrightarrow[]{g^{(2)}}Y$.
%Given the concepts extracted from $g$, a LEN $f$ may be exploited to produce a set of explanations $X \xrightarrow[]{g^{(1)}} C\xrightarrow[]{f}E$, 
% and eventually solve the classification task (if $E=Y$)
%classify and explain the categorical learning problem at a higher level of abstraction, i.e. $X \xrightarrow[]{g} C\xrightarrow[]{f}E$ %$C \xrightarrow[]{f} E$  
%as shown in Fig. \ref{fig:CMBExplainer} where $E=Y$.
% or even producing itself a solution by assuming $E=Y$.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.58\textwidth]{figs/cascade.png}

      \caption{\sm{Cascading LENs}, \sm{an example taken from the V-Dem classification dataset (see the experimental section)}. The final classification on the status of the democracy is divided into two steps.
    %   $X=C^{(1)} \xrightarrow[]{f^{(1)}} C^{(2)}\xrightarrow[]{f^{(2)}} E$. 
    First, the input data/concepts $C_1$ are mapped into high-level concepts $C_2$. %$= f_1(X)$. 
    High-level concepts are then used to compute the final classification. %$= f_2(f_1(X))$. 
    Cascading LENs can provide explanations \sm{at different levels of granularity}, implementing multiple \textit{interpretable classifications}. {\color{red}[Replace $X=C_1$ with $X$. Add $C_1$ on top of the first column of blue concepts. Replace $f_1(X)$ with $E_1 = C_2$. Replace $f_2(f_1(X))$ with $E_2$. Replace $C_2$ on top with $\bar{Y}_{(1:z)}$. Replace $Y$ on the right with $\bar{Y}_{(z+1:q)}$.]}}
    \label{fig:CascadeExplainer} 
\end{figure}

% \paragraph{Cascading explainers}
\textsc{Cascading. }
Cascading LENs can be used to provide explanations by means of a hierarchy of concept layers. \sm{In particular, multiple LENs are used to map concepts into a higher-abstraction level (without the need of any black-box $g$), }%Each model is trained on a concept space to predict concepts at a higher level of abstraction which will feed the next LENs $C^{(i)} \xrightarrow[]{f^{(i)}} C^{(i+1)}$. 
%The final model solves and explains the more abstract classification task $C^{(m)} \xrightarrow[]{f^{(m)}} E$ 
as shown in Fig.~\ref{fig:CascadeExplainer}. \sm{Each LEN provides explanations of its outputs with respect to its inputs, thus cascading LENs handle multiple levels of granularity.} This structure provides a hierarchy of explanations and upholds human interventions at different levels of abstraction, providing a far deeper support for human-machine interactions. \sm{We indicate with $(C_1, E_1), (C_2, E_2), \ldots, (C_m, E_m)$ the input/output concept spaces of the $m$ cascading LENs, with $C_{j} = E_{j-1}$, $j > 1$. We will consider the case in which LENs are trained in a supervised manner, thus implementing multiple \textit{interpretable classifications}.}



\subsection{Learning \& Explanations}
\label{sec:explanation_styles}
%Different pipelines may be employed to solve different learning problems while (eventually) producing different explanations.
%In addition, 
\sm{Each LEN module can be trained in a supervised or an unsupervised fashion, according to the preference of the user with respect to the type of explanations generated by the LEN. %The user might be interested in finding explanations that hold whenever specific categories of the considered problem are predicted, }
% that hold on a certain portion of data 
%or \sm{in} letting the LEN \sm{autonomously discover a set of regularities among the input concepts.
In Section~\ref{sec:use_cases}, when describing the selected computational pipelines, we made a precise distinction among \textit{interpretable classification}, \textit{explaining a black-box}, and \textit{interpretable clustering}, that represent three different preferences that the user might have in the problem at hand. These preferences impose precise constraints in the selection of the learning criteria and on the form of the FOL rules that can be extracted by the LENs. In addition to this choice, the user can select the granularity level of the FOL rules, moving from \textit{local} to \textit{global} rules. The former are about single examples, while the latter covers the whole dataset. While all the formal details on the learning criteria and the rule types will be provided in  Section~\ref{sec:learncrit}, here we contextualize their role with respect to the properties of the previously described computational pipelines.} 

\sm{Whenever LENs are exploited to both solve the classification problem and provide explanations, i.e., in \textit{interpretable classification},  they become white-box classifiers. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CMBExplainer} (left), Fig.~\ref{fig:CascadeExplainer} are all about this case. Learning is driven by supervised criteria that exploit the available supervised data in order to create the conditions for extracting different types of FOL rules. Each output concept of the LEN is associated to a target category of the considered learning problem, and LENs can provide a FOL explanation of each prediction, e.g., explanation of the target class \textit{person} with respect to the input concepts/attributes \textit{head, hands, body}.}

\sm{In the case in which the user aim at \textit{explaining a black-box}, a LEN acts in parallel to a black-box classifier with the only goal of providing explanations, and it is forced to yield outputs that are as close as possible to the ones of the black-box, i.e., $f$ is forced to be close to $g$ on the available data samples. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right) and it does not require any supervisions, since learning is driven by a coherence criterion between the outputs of $g$ and those of $f$ when processing the same data.}

%
%For instance, in the selected computational pipelines of Section~\ref{sec:use_cases}, while most of the focus is on supervised learning, the Concept-bottleneck case is also about unsupervised learning of LENs (Fig.~\ref{fig:CMBExplainer} right).
%


%\sm{In the former case, each output concept of the LEN is associated to a target category of the considered learning problem, and LENs are developed by learning criteria that exploit the available supervisions (ection~\ref{sec:learncrit}). The rationale behind this approach it that LENs implicitly learn to predict each target class with respect to the input concepts, that are lower-level attributes. Then, LENs can provide a FOL explanation of such prediction, e.g., explanation of the target class \textit{person} with respect to the input concepts/attributes \textit{head, hands, body}. %We refer to this context as \textsc{targeted explanations}, and the learning process is driven by supervised criteria (Section~\ref{sec:learncrit}).
%\sm{Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations, i.e., in \textit{interpretable classification}, then it becomes a white-box classifier. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CascadeExplainer} (left), Fig.~\ref{fig:CMBExplainer} are all about this case. 
%
%\sm{In the E2E case when $g$ is present or, more generally, whenever LENs act in parallel to a black-box classifier with the only goal of providing explanations, then LENs are forced to yield outputs that are as close as possible to the black-box, so $f$ is forced to be close to $g$. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right).
%
\sm{A user may be interested in discovering relations among different \sm{input} concepts without posing any preferences on any pre-defined class.
For example, the user might be interested in discovering  co-occurrences of certain input concept activations in not-defined-before subsets of the dataset, such as $soccer\_ball \wedge foot$ for some samples in a collection of miscellaneous images.
In the case of \textit{interpretable clustering}, each output concept of the LEN is associated to a symbol that is not defined in advance, as in Fig.~\ref{fig:CMBExplainer} (right), and the activation score can be tough as a cluster membership score.
LENs yield an explanation for each of these symbols, that is about discovering relations among the input concepts. In this context, no supervisions are exploited, and the learning criterion is designed in order to cluster the input concepts into $r$ groups.}

 %For instance, by analyzing the output of a multi-label classifier $C=g_1(X)$ in a CB pipeline, %with eventually several output classes, 
%it could be interesting to get an explanation of the holding relationships among different classification outputs. 
%\sm{For example, the user might be interested in discovering}  co-occurrences of certain input concept activations, like $soccer\_ball \wedge foot$ for a set of football images.

\sm{Independently on what has been described so far, the user might decide to automatically discover regularities that are about single examples, groups of data points, an entire class, or, more generally, the whole dataset, moving from \textit{local} to \textit{global} explanations.} %On the other hand, the user may also look for unbiased global explanations, like $zero\oplus one\oplus\ldots\oplus nine$, in a digit classification task. 
%In both the cases, learning is driven by unsupervised criteria.
%Each output concept activation of the LEN module can be tough as a cluster membership score. Thus, another view of \textsc{untargeted explanations} can be directly related to the notion of \textit{interpretable clustering}, where LEN can provide explanation of each cluster, as shown in Fig.~\ref{fig:concept_relations} for the case of MNIST digits.
%As another example, consider the case of gene expression analysis, where neural networks are usually employed to group similar patients according to their genes activations. LENs can be used not only to perform such grouping (E2E), but also understand why such groups have been formed and in particular which are the most relevant gene activations in each group. }


%\sm{In the following we provide further insights for \textsc{targeted} and \textsc{untargeted explanations}.}

%For this reason, we distinguish between the case in which LENs are trained in a supervised manner or with unsupervised criteria.

%A supervised task consists in learning and explaining a target \textit{class} with respect to a set of lower-level attributes, e.g. explanation of the class \textit{person} with respect to the attributes \textit{head, hands, body}. In this scenario LENs generate \textit{Supervised Explanations}.
%Alternatively, an unsupervised task consists in explaining hidden relations among \textit{concepts}, e.g. the classification outputs of another classifier or categorical attributes. In this scenario LENs yield \textit{Unsupervised Explanations}.
% Further, the explanation could have a global, local or even example-level validity. For instance, we may be interested in explaining a certain decision for a specific input, but also in universally valid regularities or simply most frequent co-occurrences among classes.
%In the following, we briefly discuss these two logical explanation styles %that are currently supported by the LENs framework
%which we respectively referred as \textit{Supervised Explanations} and \textit{Unsupervised Explanations}.
%In order to train a LEN to produce these %one or more of the following explanation styles, we can make use of ad hoc learning criteria, as successively discussed in Sec.\ref{sec:learncrit}


% \paragraph{Class-driven explanations}
%\textsc{Targeted explanations. }
% (local or global); \fg{richiederebbe spiegare, che mentre la LEN è vera esattamente dove la classe che spiega, la formula logica è soddisfatta dovunque.}
%Targeted explanations aim at providing a valid explanation for all the samples of a specific class. 
%This may be achieved by training a LEN to provide \textit{interpretable classification} or to \textit{explain a black-box model}.
%represent different kinds of causalities for a selected class with respect to the other ones, or a set of lower-level concepts. 
%Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations (E2E when no black-box is considered, CB, Cascading), then it becomes a white-box classifier. 
%\sm{Learning of the LEN module is simply driven by a supervised objective function, in which $f$ is forced to be as close as possible to the corresponding $\bar{Y}$ on the available data. Whenever the LEN belongs to a computational pipeline in which it is expected to both solve the classification problem and provide explanations (E2E when no black-box is considered, CB, Cascading), then it becomes a white-box classifier. The examples of Fig.~\ref{fig:E2EExplainer} (left), Fig.~\ref{fig:CascadeExplainer}, Fig.~\ref{fig:CMBExplainer} are all about targeted explanations. In the E2E case when $g$ is present or, more generally, whenever LENs act in parallel to a black-box classifier with the only goal of providing explanations, then LENs are forced to yield outputs that are as close as possible to the black-box, so $f$ is forced to be close to $g$. This is what is shown in  Fig.~\ref{fig:E2EExplainer} (right)., and that we refer to as \textit{explaining a black-box}}

%One possibility is to use a LEN to directly accomplish a classification task. Indeed, it can provide an interpretable classification by training a LEN $f$ to satisfy $f_i\simeq Y_i$ for some $i\in\{1,\ldots,q\}$, i.e. to have $f_i(c)$ as close as possible to $Y_i(c)$ for any $c\in C$, where $Y_i(c)$ denotes the label of the $i$-th class on the input $c$, that the LEN is meant to both learn and explain. This solution is preferred when it is of fundamental importance to have a white-box classifier, while we can accept some drawbacks in terms of classification performances.
%However, we may also train a LEN $f$ to explain a black-box model $g$. Therefore, to satisfy $f_i\simeq g_i$ for some $i\in\{1,\ldots,d\}$, i.e. to have $f_i(c)$ as close as possible to $g_i(c)$ for any $c\in C$. This other solution is instead useful in those context where the classification performances play a key role and we may accept approximate explanations of the decision taken. 
%It is worth noticing that when explaining a black-box model $g$, a LEN may also take into account the classifier predictions on unlabeled data, e.g. in a semi-supervised learning setting. This allows the LEN to produce explanations covering a larger set of data, but also possibly inaccurate. 
%On the other hand, in the interpretable classification case the LEN learns explanations directly from (limited to) the labeled data. 
% \begin{itemize}
%     \item 
%     \textit{IF-Rules. } This kind of explanation provides a superset of a specific class assignment. For instance, an upper bound containing the class $flies$ can be defined according to the explanation "$flies\rightarrow bird\vee airplane$".
%     \item 
%     \textit{Only IF-Rules. } In this case an explanation is required to provide a subset of a specific class assignment. A lower bound contained in the class $flies$ may be obtained with the explanation "$has\_wings \ \wedge \ has\_engine\rightarrow flies$".
%     \item 
%     \textit{IFF-Rules. } An explanation  can completely characterize a certain class. For instance, the class $airplane$ can be defined according to the explanation "$airplane \leftrightarrow has\_wings\wedge has\_engine$".
% \end{itemize}
% We note that only with IFF-Rules explanations a LEN can be used for interpretable classification. Indeed, not any bird or plane can fly, so as a seagull can fly without having an engine. Hence, IF and Only IF-Rules are not suitable to correctly predict a specific class behaviour.
\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figs/E2E.pdf} \quad %\\ \bigskip
    \includegraphics[width=.48\textwidth]{figs/e2e_explaining.pdf}
    \caption{LENs Supervised Explanations: interpretable classification, where the LEN directly provides the final classification (left), or explaining a black-box model $g$ (right).
    % Classification style: Explaining an existing classifier. Differently from the previous examples, here a LEN is used to explain the predictions made by an existing classifier $g(x)$ on the MIMIC classification task.} 
    }
    \label{fig:explainablevsexplanation}
\end{figure}
\fi

% \paragraph{Relations among concepts}
%\textsc{\sm{Untargeted} explanations. }
%  (local or global): MI, Conversion to CNF
%A user may be interested in discovering relations among different \sm{input} concepts without posing any preferences on any specific class. %For instance, by analyzing the output of a multi-label classifier $C=g_1(X)$ in a CB pipeline, %with eventually several output classes, 
%it could be interesting to get an explanation of the holding relationships among different classification outputs. 
%\sm{For example, the user might be interested in discovering}  co-occurrences of certain input concept activations, like $soccer\_ball \wedge foot$ for a set of football images.
%\sm{Differently from the case of \textsc{targeted explanations}, the user might decide to automatically discover regularities that are not about the whole dataset, but that may hold only for a portion of the available data. On the other hand, the user may also look for unbiased global explanations, like $zero\oplus one\oplus\ldots\oplus nine$, in a digit classification task. In both the cases, learning is driven by unsupervised criteria.
%Each output concept activation of the LEN module can be tough as a cluster membership score. Thus, another view of \textsc{untargeted explanations} can be directly related to the notion of \textit{interpretable clustering}, where LEN can provide explanation of each cluster, as shown in Fig.~\ref{fig:concept_relations} for the case of MNIST digits.
%As another example, consider the case of gene expression analysis, where neural networks are usually employed to group similar patients according to their genes activations. LENs can be used not only to perform such grouping (E2E), but also understand why such groups have been formed and in particular which are the most relevant gene activations in each group. }

\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=0.58\textwidth]{figs/concept_relations.pdf}
    \caption{\sm{Automatic explanations. MNIST digits are classified as belonging to one of the 10 classes and whether they are even of odd by a black-box $g$.  %in a Concept-bottleneck pipeline 
     A LEN groups these predictions in an unsupervised manner, and analyzes the relations within each cluster.} Supervision labels are not provided for the LEN output. {\color{red}[Remove $g(X)$ and $f(g(X))$. FOL Explanation of Cluster 2 (not 1).]}}
    \label{fig:concept_relations}
\end{figure}
\fi

% \paragraph{Explanation Ranges}
% \textsc{Explanation Ranges. }
% As already mentioned, the explanations may hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrencies or global principles among different classes.
%\fg{aggiungere qualche esempio?}



\section{Methods}
% \section{Formulas, Criteria and Pruning}
\label{sec:methods}
\sm{This section presents the fundamental methods that are used to implement the ideas of LENs. We start with the formal definition of the learning objectives (Section~\ref{sec:learncrit}), followed by the procedure that is used to extract FOL rules out of LENs for an individual observation  or in an aggregated manner (Section~\ref{sec:logic_rule_extr}). Finally, we discuss how to constraint LENs to avoid developing complex logic formulas by means of precise parsimony criteria (Section~\ref{sec:parsimony}).}


%This section presents the fundamental methods that are exploited to extract and ensure the style of a certain logic-based explanation for LENs (see Fig. \ref{fig:scheme2}).
%First we illustrate how different loss functions can be optimized to achieve customizable classification and explanation styles. Then, we discuss how first-order logic rules can be extracted from LENs for an individual observation and how explanations can be aggregated to be representative of a cluster of samples. Finally, we provide an overview of some parsimony criteria which can be used to avoid overly complex logic formulas and, in turn, useless explanations.

\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.7\textwidth]{figs/scheme2.png}
    \includegraphics[width=0.85\textwidth]{figs/lens_2.pdf}
    % \input{tikz/methods}
    \caption{\sm{Inside the LEN block (Section~\ref{sec:methods}). We distinguish among three categories of methods that implement the principles behind LENs:} learning criteria (Section~\ref{sec:learncrit}), FOL rule extraction (Section~\ref{sec:logic_rule_extr}), and parsimony criteria (Section~\ref{sec:parsimony}). {\color{red}[Swap cluster-level and class-level explanations. Rename example-level explanations with 'Example-level (local)'. Rename 'Class-level explanations' with 'Class-level (global). Do the same for 'cluster-level expl.']}}
    \label{fig:scheme2}
\end{figure}




\subsection{Learning Criteria}
\label{sec:learncrit}
%Cross Entropy in genere; Che può essere binary se è single o multilabel, altrimenti Softamx Cross Entropy
\sm{Following the distinction among the user preferences introduced in }Section~\ref{sec:explanation_styles}, here we focus on the loss functions that are optimized to train a LEN to \sm{develop the capability of providing explanations accordingly to such preferences}, that are the outcome of our previous experiences in \cite{ciravegna2020human,ciravegna2020human}.
\sm{For simplicity, here we will not distinguish the different computational pipelines, thus referring to a single generic LEN block with $q$ output units in all the case of \textsc{interpretable classification}, \textsc{explaining a black-box}, and \textsc{interpretable clustering}. Given an input sample, for each of the $r$ output concepts LENs yield a FOL rule $\varphi_i$, $i=1,\ldots,r$. We will use the notion of \textit{support of $\bar{f}_i$}  to indicate the subset of data samples on which the $i$-th output concept holds true, and \textit{support or rule $\varphi_i$} to indicate the subset of data samples for which the FOL rule $\varphi_i$ holds true.} %We will use the notation $\bar{Y}(c) \in \bar{Y}$ to indicate the function that returns the binary label vector associated to a generic input $c \in C$. With an abuse of notation, we will use $C$ also to indicate the set of available training inputs in the concept space. Moreover, $f_i$ is the function that returns the $i$-th output of the LEN, $i=1,\ldots,r$, and $\bar{Y}_i(c)$ is the associated $i$-th binary label.

% \paragraph{Class-driven Criteria.} 
\textsc{Interpretable classification. } 
%In the case of \emph{Supervised Explanations}, we aim at providing explanations of certain classes. In this sense, we want our model $f$ to be active whenever the class we aim to explain is also active.
% (i.e. $f_i(c) = Y_i(c) = 1$)
% We do not distinguish here whether the LEN is performing an \textit{interpretable classification} ($f_i\simeq Y_i$) or it is \textit{explaining an existing classifier} ($f_i \simeq g_i$), since for what concerns the optimization function it does not make any difference.
%Let us assume the interpretable classification case. The case of explaining a black-box model $g$ can be obtained by replacing $Y_i(c)$ with $g_i(c)$ in the loss unctions. The only difference in the two cases is that while $Y_i(c) \in \{0, 1\}$ is a discrete membership function, $g_i(c) \in [0,1]$ provides the probability of class assignment.
%Further, for sake of simplicity, in what follows we will assume $f: C=X\rightarrow E=Y$.
\sm{Training a LEN by supervised learning is what is needed in order to create the conditions to extract explanations over precise classes. There are three different specificity levels of the explanations that can be enforced, focusing on IF, Only IF or IFF rules, }
\begin{eqnarray*}
\text{IF}: && \bar{f}_i \rightarrow \varphi_i \\
\text{Only IF}: && \varphi_i \rightarrow  \bar{f}_i \\
\text{IFF}: && \bar{f}_i \leftrightarrow \varphi_i
\end{eqnarray*}
where $i=1,\ldots,r$.
\sm{IF rules mean that, in the extreme case, for each example of class $i$ we want the $i$-th output of the LEN to score one (and not necessarily vice-versa). In other words, the support of $\bar{f}_i$ has to be included in the support of the rule.}
%and each of them provide a superset of a specific class assignment and therefore requires the support of the antecedent to be included in the support of the consequent (i.e. $\{c\in C: \bar{Y}_i(c)=1\}\subseteq C_i$).
\sm{This behavior} can be achieved by minimizing a hinge loss,
\begin{equation}
L_{\rightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \max\{0, \bar{y}_i(c) - f_i(c)\}\qquad  i \in [1,  r].\label{eq:IF}
\end{equation}
 Following a symmetric approach, in Only IF rules it may be the case of a class to be explained in terms of some lower-level concepts. \sm{This principle is easily enforced} by switching the two terms of the loss function in Eq. \ref{eq:IF},
\begin{equation}
L_{\leftarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} \max\{0, f_i(c) - \bar{y}_i(c)\}\qquad  i \in [1,  r].\label{eq:IF2}
\end{equation}
\sm{Both in IF and Only IF rule, in order to make the learning problem well posed, further conditions on $f$ must be included, to define its behaviour in the space areas not covered by the data and to avoid trivial solutions with constant $f$.}
At last, LEN can learn double implication rules (IFF) in which an explanation can completely characterize a certain class. %These rules require the support of the LEN and the support of the class to be strictly equal.
%For this reason,
\sm{Any} function penalizing points for which $f_i(c)\not=y_i(c)$ may be employed in this scenario, such as the Mean Square Error loss,
\begin{equation}
L_{\leftrightarrow}(\bar{y}_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} |f_i(c) - \bar{y}_i(c)|\sm{^2} \qquad  i \in [1,  r], \label{eq:IFF}
\end{equation}
or the classic Cross-Entropy loss.
%IFF loss function is preferred when a LEN performs E2E \textit{interpretable classification}, since we want the output of \sm{$f$} to be as close as possible to \sm{$\bar{Y}$} in order to maximize the classification accuracy. 
% In this latter case if we want the same LEN to explain different, mutually exclusive classes, a Softmax activation function can be also employed.  


\textsc{Explaining a black-box. } In this case, the output of the LEN is forced to mimic the one of the black-box $g$. A coherence loss can be exploited to reach this goal,
\begin{equation}
L_{g}(g_i,f_i,\mathcal{C}) = \sum_{c\in \mathcal{C}} |f_i(c) - g_i(c)|\sm{^2} \qquad  i \in [1,  r]. \label{eq:coher}
\end{equation}

%the explanations provided by LENs are first-order logic formulas, and this newly devised pieces of knowledge can be reused and enforced on the output of the classifier $g$. This is commonly considered in the generic \emph{learning from constraints} framework \cite{gnecco2015foundations}, and it may be of particular interest, especially for semi-supervised settings. A similar strategy has already been considered e.g. in \cite{ciravegna2020constraint}, where a set of FOL formulas have been, at first extracted from data, and then converted into continuous loss functions to be injected in the learning objective.
%At last, the extracted formulas can also be used to check the behaviour of the classifier on test data, e.g. to detect adversarial samples as done in \cite{melacci2020domain}.

\textsc{Interpretable clustering. }
% \paragraph{Mutual Information Criterion}
% \paragraph{Relations among Concepts.}
\sm{Generic explanations can be achieved by means of fully unsupervised  principles from Information Theory.} As a matter of fact, the maximization of the Mutual Information (MI) index between the input concept space $C$ and the \sm{output concept space} $E$ allows the LEN to
be trained in a fully unsupervised way \cite{ciravegna2020constraint}. More specifically, a max-MI criterion (see \cite{melacci2012unsupervised} for further details) \sm{leads to the development of a LEN that has the tendency of producing 1-hot activation scores,} such that $\forall c \in \mathcal{C}$ only one $f_i(c) = 1$, while the others are close to zero. \sm{In a sense, it enforces the LEN to cluster the data in a way that each input sample belongs to a single cluster.}
In order to define the MI index, \sm{we have to model the probability distribution $P_{i|c}(f)$, that is the probability of $f_i$ to be active (close to 1) on sample $c$ -- we implemented it using the softmax operator on the LEN output.} %Following the classic notation of discrete MI, 
%$E$ is a discrete random variable associated to the output of the LEN functions while $C$ is the variable related to the data in the concept space.
The penalty term to minimize \sm{to train the LEN} is minus the MI index,
\begin{equation}
    L_{MI}(f,\mathcal{C}) = - H_{E}(f,\mathcal{C}) + H_{E|C}(f,\mathcal{C}) \ ,
	\label{eq:MI}
\end{equation}
where $ H_{E}$ and $ H_{E|C} $ denote  the entropy and the conditional entropy functions associated to the aforementioned probability distribution, respectively, and measured over the whole $C$, as in  \cite{ciravegna2020constraint}. 
%An outcome of the maximization of the MI index is that the supports of the explaining functions will tend to partition the input space $X$, i.e., $X=\bigcup_{j=1}^mX_j$ and $X_j\cap X_k=\emptyset$, for $j\neq k$ (see \cite{melacci2012unsupervised,betti2019cognitive} for further details).

\sm{Of course, in all the computational pipelines} in which a classifier $g$ is also employed,
%In the particular case of a LEN providing explanations for an existing classifier $g$, 
the available supervision is enforced on $g$ as well, e.g., by means of the Cross-Entropy loss. As a side note, we remark that what we are describing in a fully supervised setting can be trivially extended to the semi-supervised one, as we already investigated in \cite{ciravegna2020constraint,ciravegna2020human}. 




\subsection{FOL Rule Extraction}
\label{sec:logic_rule_extr}
\sm{Once a LEN has been trained, it can associate one or more explanations for each output concept. We indicate with $\varphi_{i,\cdot}$ the explanation of concept $i$, where the second subscript can index either a single data sample $c$, $\varphi_{i,c}$, or a group $S$ of data samples, $\varphi_{i,S}$. As it will become clear shortly, extracting FOL rules out of a trained LEN can be done by inspecting its inputs/outputs accordingly to a Boolean interpretation of them. Whenever this is independently done for each single input sample, we get back \textsc{example-level explanations}, that we also refer to as \textit{local explanations}. Differently, whenever the explanations covers an entire category of examples, we talk about \textit{global explanations}, distinguishing between \textsc{class-level explanations} and \textsc{cluster-level explanations}. {\color{red}[I still don't understand what kind of explanations we can provide]}}

 %As already mentioned, the explanations may hold on different input sub-portions. In terms of FOL formulas, this means that the extracted rules will be satisfied on different subsets of the concept space. For instance, we may consider example-level explanations, i.e. explanations focusing on individual class assignments. Example-level explanations can be aggregated into clusters up to overall class-level explanations. However, we may also be interested in frequent co-occurrences or global principles among different classes.
 

\sm{In detail,} any LEN $f=(f_1,\ldots,f_r)$ requires both its inputs and outputs to belong to the real-unit interval. This apparent limitation allows any $f_i$, for $i=1,\ldots,r$, to be easily converted into a Boolean function $\bar{f}_i$, e.g. by thresholding its I/O, e.g., with respect to $0.5$ value. Therefore, any Boolean function $\bar{f}_i$ is converted into a FOL formula $\varphi_i$ in Disjunctive Normal Form (DNF) \cite{mendelson2009introduction} by means of its truth-table, see Fig.~\ref{fig:tt2form}.
%Given $f: C \rightarrow E$, 
\sm{In order to support the following descriptions, }
we define the set $O_i = \{c\in C:\ \bar{f}_i(c)=1\}$ as the set of all the $[0,1]$-valued concept tuples that make true the $i$-th output concept/explanation, i.e., the \emph{support} of $\bar{f}_i$. %For instance, if we are interested in targeted explanations only, any $O_i$ will generally consist in the set of inputs that are classified as belonging to the $i$-th class by the LEN.
% \paragraph{Local Explanation}
% \paragraph{Example-Level Explanation}

%\sm{Each output concept $i$ is associated to one of more explanations $\varphi_i,\cdot$, depending on its granularity level. In what follows, we described the case }

\textsc{Example-level explanations. }
Given $c\in O_i$, the booleanization of its continuous features may provide a natural way to get a logical explanation at example-level $\varphi_{i,c}$ as a FOL formula. In particular, \sm{if we indicate with $c_j,\ j=1,\ldots,k$ the human understandable name of the $j$-th input concept}, for any $c\in O_i$, we can consider the following as the \emph{local explanation} of the $i$-th output $f_i$ on example $c$,
\begin{equation}
    \varphi_{i,c} = \tilde{c}_1\wedge\ldots\wedge\tilde{c}_k \qquad\mbox{where } \tilde{c}_j:= 
    \begin{cases}
        \bar{c}_j, & \mbox{if }c_j \geq 0.5\\
        \neg \bar{c}_j, &\mbox{if } c_j < 0.5\\
    \end{cases}\ ,    
    \mbox{ for $j=1,\ldots,k$.}
    \label{eq:locexp}
\end{equation}
\begin{figure}[t]
\centering
    \includegraphics[width=0.8\textwidth]{figs/truth-table.png}
    \caption{Extracting a logic formula from the truth-table of a binary boolean function $\bar{f}$.}
    \label{fig:tt2form}
\end{figure}
% \paragraph{Aggregated Explanation}
%\textsc{Aggregated explanation. }


%By considering Eq. \ref{eq:locexp} for any $c\in S$, and aggregating all the example-level explanations, we may easily provide a \emph{Cluster Explanation} $\varphi_{i,S}$ for a subset of samples $S \subseteq C_i$ as
\begin{equation}
    \varphi_{i,S} = \displaystyle\bigvee_{c \in S}\varphi_{i,c} = \displaystyle\bigvee_{c \in S}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_k
\label{eq:agg_exp}
\end{equation}
%Any formula $\varphi_{i,S}$ can be thought of as a $\{0,1\}$-valued mapping defined on $C$, that is equal to 1 exactly on a cluster $S \subseteq C_i\subseteq C$. We may also get an explicit explanation relating $\varphi_{i,S}$ and the $i$-th output $f_i$ by the FOL formula:
%\[
%\forall c\in S:\ \varphi_{i,S}(c)\rightarrow \bar{f}_i(c)
%\]
% \paragraph{Global Explanation}
% \paragraph{Class-Level Explanation}

\textsc{Class-level explanation. }
We can aggregate local explanations associated to data belonging to a set $S \subseteq O_i$, yielding $\varphi_{i,S}$,
By considering Eq. \ref{eq:agg_exp} with $S=O_i$, i.e., aggregating all the example-level \sm{explanations of class $i$}, we get an overall explanation $\varphi_i$ for the \sm{LEN} output $f_i$.
\begin{equation}
    \varphi_i = \displaystyle\bigvee_{c \in C_i}\varphi_{i,c} = \displaystyle\bigvee_{c \in C_i}\tilde{c}_1\wedge\ldots\wedge\tilde{c}_k.
\label{eq:glo_exp}
\end{equation}
Also in this case, any formula $\varphi_i$ can be thought of as a $\{0,1\}$-valued mapping, that is equal to 1 exactly on $O_i\subseteq C$. We may get as \emph{global explanation} a FOL formula relating $\varphi_i$ and the $i$-th output $f_i$ by means of
\[
\forall c\in C:\ \bar{f}_i(c)\leftrightarrow\varphi_i(c).
\]
% RECURSION\_STEP
% \paragraph{Compounding Explanations}
%\textsc{Compounding explanations. }

Both example-level, aggregated and class-level explanations can be recursively applied in case a cascading LENs or a single LEN with multiple $[0,1]$-valued layers are considered. For instance, given a cascading LEN as \sm{the one of Fig.~\ref{fig:CascadeExplainer}}, we may get both local and global explanation of the concepts in \sm{$E_1 = C_2$ with respect to the ones in $C_1$, so as the concepts in $E_2$ with respect to the ones in $C_2$ and, in turn, in $C_1$}. The modularity of FOL formulas allows the composition of concepts at different levels that may express arbitrary complex relationships among them.

% \paragraph{Aggregation of Cluster-Level Explanations}
\textsc{Cluster-level explanations. }
In the case in which the maximum MI criterion (Eq. \ref{eq:MI}) is used to drive the learning problem, each $\varphi_i$ will generally hold on a sub-portion of the concept space $O_i\subseteq C$. {\color{red}[This is also true for the supervised case, what is the difference?]} However, we may get a FOL providing a global explanation by means of the disjunction
$\varphi = \varphi_1\vee\ldots\vee\varphi_r$, indeed $C_1\cup\ldots\cup C_r=C$. Since the formula $\varphi$ can be very complex, if we are interested in simpler global explanations we may  convert $\varphi$ into an equivalent $\varphi'$ in \emph{Conjunctive Normal Form} (CNF). In particular, there exist $r'$ and clauses $\varphi'_1,\ldots,\varphi'_{r'}$ such that: 
\[
\varphi=\bigvee_{i=1}^r\varphi_i \equiv \bigwedge_{i=1}^{r'}\varphi'_i=\varphi'.
\]
As a result, we get the following global explanations for $i=1,\ldots,r':
\forall c\in C:\ \varphi'_i(c)$.
Unfortunately, converting a boolean formula into CNF can lead to an exponential explosion of the formula; in the following, we will see how to address this problem. 
% However, after having converted each $\varphi_i$ in CNF, the conversion can be computed in polynomial time with respect to the number of minterms in each $\varphi_i$ \cite{russell2016artificial}.

\begin{example}
\label{ex:xor}
Let's consider the boolean $xor$ function, defined by $xor(0,0)=xor(1,1)=0$, $xor(1,0)=xor(0,1)=1$. 
Let $f$ be a LEN that has been trained to approximate the $xor$ function in the input space $C=[0,1]^2$. Then, if we consider e.g. the inputs $c^1=(0.2,0.7)$, $c^2=(0.6, 0.3)$, we get $\bar{c}^1=(0,1)$, $\bar{c}^2=(1,0)$, and therefore $\bar{f}_1(c^1)=\bar{f}_1(c^2)=1$. These examples yield respectively the local explanations $\varphi_{1,c^1}=\neg \bar{c}_1\wedge \bar{c}_2$ and $\varphi_{1,c^2}=\bar{c}_1\wedge\neg \bar{c}_2$, and the class-level explanation for $f_1$ is given by $\varphi_i=(\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)$. In the same way, we may get the class-level explanation for the output $f_0$. In the end, the following formulas represent the supervised explanations of the false and true classes, respectively:
\[
\forall c:\ \bar{f}_0(c)\leftrightarrow (\neg \bar{c}_1\wedge\neg \bar{c}_2)\vee(\bar{c}_1\wedge \bar{c}_2)\qquad\mbox{and}\qquad
\forall c:\ \bar{f}_1(c)\leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2)
\]
The two global explanations correctly match the truth table of the boolean $xor$ function.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/truth-table-counter.png}
    \caption{Aggregation of concept tuples with the same booleanization yields a common example-level explanation, and do not complicate the class-level explanation. For any example-level explanation, we may count how many samples it explains. Infrequent explanations may then be pruned to avoid explanation overfitting.}
    \label{fig:tt2form_freq}
\end{figure}

% If we then consider that $f$ is composed of two hidden and one output neurons, we may want to explain the behaviour of each node. In particular, we may get that the first hidden neuron is represented by $ \tilde{h}_1^1  \leftrightarrow \neg \textit{c}_1\wedge \textit{c}_2$ 
% while the second $ \tilde{h}_2^1  \leftrightarrow \textit{c}_1\wedge \neg \textit{c}_2$. The output neurons $h^2 = f$ can be also represented in terms of the hidden neurons $f \leftrightarrow h_1^1 \vee h_2^1$ which in turns can be described again in terms of input concepts $f \leftrightarrow (\neg \textit{c}_1\wedge \textit{c}_2) \vee ( \textit{c}_1\wedge \neg\textit{c}_2)$.

\end{example}

% \paragraph{Remarks}
The method described so far illustrates how logic-based explanations can be formally aggregated to produce a range of explanations, from the characterization of individual observations to formulas explaining the model predictions for all the samples of a target class.
The formula for a whole class can be obtained by aggregating all the minterms corresponding to local explanations of all the observations having the same class label.
In theory, this procedure may lead to overly long formulas as each minterm may increase the complexity of the explanation. In practice, we observe that many observations share the same logic explanation, hence their aggregation does not change the complexity of the class-level formula (Fig. \ref{fig:tt2form_freq}). In general, class-level explanations can be provided by aggregating just the most common explanations extracted from samples with the same class label, avoiding a sort of "explanation overfitting" with the inclusion of noisy minterms which may correspond to outliers. To summing up, a possible limitation of this naive approach can be the readability of the logical rules, for instance in case (i) the number of input features (the length of any minterm) $d \gg 1$, (ii) the size of the support $|C_i|$ is very large (possibly getting too many different minterms for any $f_i$). For these reasons, possible approaches to maintain an easy-to-understand set of very concise logical rules are fundamental to provide an useful explanation, e.g. as decision support. More details on how to select the most meaningful explanation terms are provided in Sec. \ref{sec:parsimony}.


\subsection{Parsimony criteria} \label{sec:parsimony}
When humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one \cite{aristotlePosterior,mackay2003information}. Over the years, researchers have proposed many approaches to integrate "\textit{the law of parsimony}" into learning machines.
Here we describe a few fundamental parsimony criteria which may help in developing and implementing a variety of Logically Explained Networks. A specific combination of the following methodologies may be adopted or ignored depending on end-user requirements on the explanations and on the classification performance.
% \subsubsection{Occam's razors}
% \paragraph{Occam's razors}
% \textsc{Occam's Razors. }
Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous techniques to put in practice the Occam's razor principles in the fields of statistics and machine learning.
Among such techniques, $L1$-regularization \cite{santosa1986linear} has been recently shown quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages weight sparsity \cite{tibshirani1996regression}:
% \begin{equation}
    $\lambda ||W||_1$.
% \end{equation}
By shrinking the less important weights %'s values 
to zero, this regularization technique completely removes some weights %altogether in the limit, 
leading to sparse configurations. This allows to ignore the associated input features and, therefore, to provide simpler explanations. For this reason, all out-of-the-box LENs presented in the next section are trained using this parsimony criterion.

\subsubsection{Pruning strategies}
\label{sec:pruning}
The action of parsimony criteria, such as regularizers or human priors, influences the learning process %of learning machines 
towards specific local minima. Once the model has finally converged to the desired region of the optimization space, the effort can be speed up and finalized by pruning the neural network \cite{lecun1989optimal,hassibi1993second}. The pruning strategy has a profound impact both on the quality of the explanations but also on the learning capacity model and, as a result, on the classification performance as well \cite{frankle2018lottery}. Here we present three effective pruning strategies specifically devised for LENs.

% \paragraph{Node-level pruning}
\textsc{Node-level pruning. }
A straightforward approach to pruning consists in defining the maximum \textit{fan-in} (number of non-pruned connections) for each neuron of a feed-forward neural network. We refer to this strategy as \textit{Node-level pruning}.
%A fan-in pruning strategy generates a feed-forward graph where each neuron has the same number of incoming non-pruned connections. 
At the end of the training process, the absolute value of the weight matrix $W_i$ is computed for each layer $i=1,\dots,L$. 
The node-level approach prunes one by one the weights with the smallest absolute value, such that each neuron in the network has a fixed number of incoming non-pruned weights $q \geq 2$. The parameter $q$ must be decided a priori and determines the learning capacity of the pruned model as well as the complexity of the logic formulas which can be extracted. To get reasonably simple explanations, the parameter $q$ may range between $2$ and $9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Recent work on explainer networks has shown how node-level pruning strategies may lead to fully explainable models  \cite{ciravegna2020constraint}. However, we will show in the experimental section that this pruning strategy strongly reduce the classification performances.

% \paragraph{Network-level pruning}
\textsc{Network-level pruning. }
In order to overcome the heavy reduction of the learning capacity of the node-level pruned models, we introduce here the \textit{Network-level pruning}. 
Indeed, the main aim of pruning is to only reduce the number of input terms involved in the final explanations. By directly limiting the number of input features considered by the network, we can achieve this result with a lighter impact on the overall model. 
Once the network has converged, the Frobenius norm of the first-layer weight matrix $W_1$ is computed: $w_1 = ||W_1||_2$. The vector $w_1$ is then re-scaled in the interval $[0,1]$:
\begin{equation}
    w_1' = \frac{w_1}{\max w_1}
\end{equation}
In this way, $w_1'$ gives a normalized score to rank input feature by importance. The \textit{Network-level strategy} consists in pruning all the input features where $w_1' < w_t$, where $w_t$ is a threshold set a priori (usually $w_t = 0.5$). Alternatively, %the $\mu$ approach may 
we can also retain the $q$ most important input features and prune the others for the entire first layer, as done in the \textit{Node-level pruning} for each single node. %The parameter $q$ is user-defined and may range between $2$ and $9$ to get sensibly compact explanations \cite{miller1956magical,cowan2001magical,ma2014changing}. 
This pruning strategy is far less stringent compared to the node-level pruning as it affects only the first layer and it does not prescribe a fixed fan-in for each neuron.

% \paragraph{ReLU pruning}
% \paragraph{Example-level Pruning}
\textsc{Example-level pruning. }
Example-level pruning is a particular strategy exploiting the well-studied local linearity property of neural networks whose activation functions in all hidden layers are Rectified Linear Units (ReLu Networks) \cite{hahnloser2000digital}. 
% \paragraph{Local Linearity}
For any input $x \in \mathbb{R}^d$, the initial Directed Acyclic Graph (DAG) ${\cal G}$ describing the structure of a ReLu Network, is reduced to ${\cal G}_{x}$,
which only keeps the units corresponding to active neurons and the corresponding arcs (firing path). 
Since all neurons operate in ``linear regime'' (affine functions), as stated in the following, 
the transformation $z: X \rightarrow Y$, which  is the composition of affine functions, corresponds to a single affine function $f^*(x) = W x + b$. 
\begin{theorem}
	Let $\{h_1,\ldots,h_L \}$ a collection of affine functions, where
% 	\[
		$h_{i}: X_{i} \mapsto Y_{i}: x \mapsto W_{i} x + b_{i}$
% 	\]
	and $\forall i=1,\ldots, L-1: \ \ X_{i+1} \subset Y_{i}$, then, 
% 	\[
		$z(x) = h_{L} \circ h_{L-1} \circ \dots \circ h_{2} \circ h_{1} x.$
% 	\]
	is affine and we have $f^*(x) = W x + b$, where
	\begin{equation}
	    W(L) = \prod_{\kappa=1}^{L} W_{\kappa}, \qquad 
		b(L) = \sum_{\kappa=0}^{L-1}  b_{L-\kappa} \prod_{h=0}^{\kappa} W_{L-h+1}  
	\end{equation}
	and $W_{L+1}:=I$.
	\label{theorem:affine}
\end{theorem}

Therefore, for a given input $x$ an affine function $f^*(x)$ can be devised. Notice that Theorem \ref{theorem:affine} only requires hidden layers node to be equipped with a ReLU activation function: nor the input nor the output nodes needs to employ it. %On the contrary, output nodes may be equipped with a sigmoid activation for binary or multi-label classification or a softmax activation function in case of multiclass.
Since the function $f^*(x)$ is affine, its interpretation is already much easier than considering the initial deep network $f(x) = h_{L} \circ h_{L-1} \circ \dots \circ h_{2} \circ h_{1} x$. Indeed, for each sample we can calculate the Frobenius norm of the corresponding weight matrix $w_L = ||W(L)||_2$. At last, similarly to what is done in the network-level pruning, we can retain the most important input features which satisfy $w'_L > w_t$, where again $w'_L = \frac{w_L}{\max w_L}$ and $w_t$ is set to 0.5. 


\section{Out-of-the-box LENs}\label{sec:outofthebox}


Crafting state-of-the-art fully interpretable models is not an easy task; rather, there is a trade-off between interpretability and performances.
The proposed framework is designed to provide the building-blocks to create a wide range of models having different interpretability-VS-accuracy
% interpretability-VS-explainability-VS-performance
trade-offs.
Here, we show how to combine the methods presented in the previous section to design three different out-of-the-box LENs (Fig. \ref{fig:out-of-the-box}): a) the $\psi$ network, as proposed in \cite{ciravegna2020constraint} which is a fully interpretable model with limited learning capacity and providing mediocre explanations; b) the $\mu$ network, a neural model providing high-quality explanations, great learning performances and modest interpretability;  c) the ReLU network, a black box model ensuring state-of-the-art learning performance and good explanations at the cost of very low interpretability. The characteristics of these three LENs are also resumed in Tab. \ref{tab:LENs}.


\begin{table}[ht]
\centering
\caption{Out-of-the-box LENs summary.}
\label{tab:LENs}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{LEN}                            & \textbf{Pruning} & \textbf{Activation}  & \textbf{Learning}  & \textbf{Explanation}   & \textbf{Interpretability}\\
\midrule

$\psi$ Network (Fig. \ref{fig:psi_net}) & Node-level        & Sigmoid                       & Low                           & Low                               & Very high     \\
$\mu$ Network (Fig. \ref{fig:mu_net})   & Network-level     & Any                           & High                          & Very high                         & High          \\
ReLU Network (Fig. \ref{fig:relu_net})  & Example-level     & ReLU                          & Very high                     & High                              & Low           \\

\bottomrule
\end{tabular}
}
\end{table}


\begin{figure}[ht]
    \centering
     
     \begin{subfigure}{1\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth]{figs/psi_nn.png}
         \caption{$\psi$ network (Subsection \ref{subsec:psi}).}
         \label{fig:psi_net}
     \end{subfigure}\\
     
     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/mu_nn.png}
         \caption{$\mu$ network (Subsection \ref{subsec:mu}).}
         \label{fig:mu_net}
     \end{subfigure}
     \qquad
     \begin{subfigure}{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figs/relu_nn.png}
         \caption{ReLU network (Subsection \ref{subsec:relu}).}
         \label{fig:relu_net}
     \end{subfigure}
     
    \caption{Out-of-the-box LENs. (a) $\psi$ networks 
    %(Subsection \ref{subsec:psi}) 
    only admit $[0,1]$-valued neurons with low fan-in, hence we can associate a boolean formula to each neuron by analysing its I/O truth-table. (b) $\mu$ networks 
    %(Subsection \ref{subsec:mu}) 
    do not have interpretable hidden neurons but the input concepts are drastically pruned which allows to provide simple network-level explanations. (c) ReLU networks 
    %(Subsection \ref{subsec:relu}) 
    supply explanations for each sample by means of the equivalent affine transformation. However, nor the nodes, nor the network can be logically interpreted.}
    \label{fig:out-of-the-box}
\end{figure}

\subsection{The $\psi$ network} \label{subsec:psi}
A $\psi$ network is a Logically Explained Network already proposed by \cite{ciravegna2020constraint,ciravegna2020human}. A $\psi$ network is based on three design principles: 
(i) all activation functions for all neurons (including hidden units) should be Sigmoid;
(ii) a strong L1-regularization is used in all layers to shrink the less important weight's values towards zero;
(iii) a Node-level pruning strategy, where each neuron of the network must have the same number of incoming non-pruned weights (suggested values are between 2 and 9). This number is directly proportional to the number of terms involved in the explanations. 
Also the number of hidden layers in the network needs to be set carefully, since the number of terms exponentially grows with the number of layers. 
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.24]{figs/psi_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
The typical use case presented in the original work is a concept-bottleneck scenario. A black-box model $g$ (e.g. a convolutional neural network) is used to predict a set of categories $C$ from an unstructured data set $X$ (e.g. images). The authors used a $\psi$ network to explain the behaviour of a classifier $g$, i.e. $C \xrightarrow[]{f} E=g(X)$. The $\psi$ network is specifically designed to be a fully interpretable neural network, therefore, here we also show its performances as a classifier in different contexts. It can provide the whole set of logic-based explanations: example-level, aggregated, class-level, and it is the only LEN providing also compounding node by node explanations. As a matter of fact, thanks to the node-level pruning strategy, the $\psi$ network allows to interpret (and extract a corresponding logic formulas) from each node. 
Recalling Example \ref{ex:xor}, a $\psi$ network with two hidden nodes may learn the logic formula 
\begin{equation}
\forall c:\ \bar{f}_1(c)\leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)\vee(\bar{c}_1\wedge\neg \bar{c}_2),
\label{eq:xor}
\end{equation}
with hidden nodes learning $h_1(c) \leftrightarrow (\neg \bar{c}_1\wedge \bar{c}_2)$, $h_2(c) \leftrightarrow ( \bar{c}_1\wedge \neg\bar{c}_2)$ and output node $f_1 \leftrightarrow h_1 \vee h_2$.
A $\psi$ network can be seen as a Cascading LEN where each layer corresponds to a new level of LEN. However, the network is always trained as a whole since no symbolic concept is provided at each level. Furthermore, also the explanations are always given in terms of input features for this reason. 
As reported in Fig. \ref{fig:psi_net}, this network provides the highest level of interpretability since the $\psi$ network provides for an explanation of the behaviour of each neuron. 
On the contrary, the strong regularization and the restrictive pruning strategy lead to poor classification accuracy making $\psi$ networks hard to train and not suitable for solving complex categorical learning problems. Besides, the provided explanations can be very expressive but they can be not outstanding as expected, due to the limited learning performance. 

\subsection{The $\mu$ network}  \label{subsec:mu}
A $\mu$ network is a LEN based on a standard multi-layer perceptron. A $\mu$ network is based on two design principles:
    (i) a strong L1-regularization is used only in the first layer of the network;
    (ii) a Network-level pruning strategy, which only prune the  neurons (features).
After the pruning step, the $\mu$ network can be fine-tuned to adjust to the new configuration. No assumption need to be made nor on the hidden layers nor on the activation functions. However, by applying a Network-level strategy, the same set of retained features is used for the whole network. On the one side, this allows to logically-interpret the network and, therefore, to provide explanations. On the other side, this may represent a severe limitations for multi-class classification since each class may rely on few features, but these may be very different between each class. Therefore, in the multi-class experiments of Sec. \ref{sec:experiments}, we train a set of light binary $\mu$ networks, one for each class. 

%This LEN can provide a wide range of logic-based explanations (i.e. local, cluster, and class-level).
%For each $\mu$ network, an explanation is provided in terms of the input concepts. 
Recalling Ex. \ref{ex:xor}, a $\mu$ network with variable number of hidden layers, may learn the logic formula in \ref{eq:xor}.
The Network-level strategy in this case should not prune any input features since both $c_1$ and $c_2$ are important for the final classification. In case instead also some redundant features are present, they are discard in favor of $c_1$ and $c_2$ as shown in Fig. \ref{fig:mu_net}. 
%As described in Sec. \ref{sec:logic_rule_extr} 
For some points the network will learn the aggregated explanations:
\begin{equation}
\forall c \in S_1: \neg c_1 \wedge c_2 \rightarrow f_1(c) \quad \text{and} \quad \forall c \in S_2: c_1 \wedge \neg c_2 \rightarrow f_1(c). 
\end{equation}
The two explanations can be then considered altogether to explain the class $C_1$: 
\begin{equation}
\forall c\in C:\ \bar{f}_1(c)\leftrightarrow\varphi_1(c) = \bigvee_{c \in C_i}\varphi_{i,c} =
 (\neg \bar{c}_1\wedge \bar{c}_2) \vee ( \bar{c}_1\wedge \neg\bar{c}_2).
 \label{eq:mu}
\end{equation}

Thanks to the permissive pruning strategy, the learning capacity of the network remains intact for the most part. As a consequence, $\mu$ networks are suitable for solving and explaining more complex categorical learning problems. The quality of the explanations provided by the $mu$ networks are among the higher between the proposed models. At last, a mild-level of interpretability is also guaranteed since it can be logically interpreted at a network-level. 

\subsection{The ReLU network}  \label{subsec:relu}
Another example of LEN which provides a different accuracy-vs-interpretability trade-off is the ReLU network. %is a special case of a $\mu$ network sharing most of its characteristics but with a few different properties. 
It is based on three design principles:
    (i) all activation functions for all \emph{hidden} neurons are rectified linear units;
    (ii) a mild L1-regularization in all layers of the network;
    (iii) an Example-level pruning strategy, i.e. a specialized pruning strategy for each sample.
The pruning employed in this LEN is an example-level pruning, which is available since it employs rectified linear units activation functions. %, i.e. a pruning strategy which is applied for each sample. 
This is not a limitations since it is one of the most widely used and efficient activation functions employed in deep learning \cite{glorot2011deep,ramachandran2017searching}.
On the contrary, this pruning strategy, does not cut the connections of the LEN $f$ as it is applied on the affine function $f^*$ directly to get a custom explanation for each observation. This means that the original capacity of the model is fully preserved, eventually leading to state-of-the-art classification performances. However, this type of pruning does not provide any insights of the model behaviour and may not always lead to optimum explanations.

Recalling again Example \ref{ex:xor}, a ReLu network with variable number of hidden layers, may learn the correct logic formula by aggregating local examples as it is done in \ref{eq:mu}. However, the local explanations of a certain point $c$ may not be as correct as the ones provided by the $\mu$ networks. Indeed, it can be demonstrated that the corresponding affine function $f*$, actually corresponds to the nearest decision boundary to the points. 
% On the other hand, an example-based pruning strategy may be provide more unstable explanations as the pruning may be negatively affected by the presence of outliers.
Therefore, the corresponding weights may miss some important features to explain $c$. A Relu network sometimes may explain the XOR problems with the wrong formula:
\begin{equation}
\forall c\in C:\ \bar{f}_1(c)\leftrightarrow\varphi_1(c) = \bigvee_{c \in C_i}\varphi_{i,c} =
 (\neg \bar{c}_1) \vee (\neg\bar{c}_2).
\end{equation}
Summing up, this LEN does provide the best performances in terms of classification accuracy thanks to the example-level pruning strategy. However, this comes at the cost of poor model interpretability and mild explanation capacity. 

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figs/relu_nn.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


\section{Benchmarking out-of-the-box LENs} \label{sec:experiments}
In this section, we quantitatively assess the quality of the explanations and the performance of Logically Explained Networks compared to state-of-the-art white-box models. Each task is uniquely defined by the tuple "pipeline / explanation style". The summary of each task is reported in Table \ref{tab:datasets}.
A brief description of each task, the corresponding dataset and all the related experimental details are exposed in Subsection \ref{sec:exp_details}. In Subsection \ref{sec:exp_metrics} six quantitative metrics are defined and used to compare LENs with state-of-the-art methods.

\begin{table}[ht]
\centering
\caption{Experiments.}
\label{tab:datasets}
\resizebox{\textwidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Dataset} & \textbf{Description} & \textbf{Explanation Style} & \textbf{Pipeline}\\
\midrule

MIMIC-II (Fig. \ref{fig:E2EExplainer})                      & \small{Predict patient survival from clinical data}       & Interpretable classification  & E2E \\
MNIST E/O (Fig. \ref{fig:CMBExplainer})                         & \small{Predict parity from digit images}                  & Interpretable classification  & CB\\
CUB (Fig. \ref{fig:len})                                    & \small{Predict bird species from bird images}             & Interpretable classification  & CB\\
V-Dem (Fig. \ref{fig:CascadeExplainer})                     & \small{Predict electoral democracy from social indexes}   & Interpretable classification  & Cascading \\
MIMIC-II (EBB) (Fig. \ref{fig:explainablevsexplanation})    & \small{Predict patient survival from clinical data}       & Explaining black box       & E2E\\
MNIST E/O (IC) (Fig. \ref{fig:concept_relations})                    & \small{Cluster digit properties from digit images}        & Interpretable clustering      & CB\\
\bottomrule
\end{tabular}
}
\end{table}


% \subsection{Software tool and usability}
% \label{sec:tool}
In order to make the LENs framework accessible to the whole community, we released of a Python package\footnote{\url{https://pypi.org/project/deep-logic/}} with an extensive documentation on methods and out-of-the-box LENs. The Python code and the scripts used for the experiments, including parameter values and documentation, is freely available under Apache 2.0 Public License from a GitHub repository\footnote{\url{https://github.com/pietrobarbiero/deep-logic}}.

The Deep Logic library is designed to make out-of-the-box LENs accessible to researchers and neophytes by means of intuitive APIs requiring only a few lines of code to train and get explanations from a LEN (as shown in the code example \ref{code:example}).

\begin{lstlisting}[language=Python, label=code:example, caption=Example on how to use the Deep Logic library.]
import deep_logic as dl

# import train, validation and test data loaders
[...]

# instantiate a mu network
model = dl.models.MuNN(n_classes=n_classes, n_features=n_features,
                       hidden_neurons=[200], loss=torch.nn.CrossEntropyLoss(), 
                       l1_weight=0.001, fan_in=10)

# fit the model
model.fit(train_data, val_data, epochs=100, l_r=0.0001)

# get predictions on test samples
outputs, labels = model.predict(test_data)

# get first-order logic explanations for a specific target class
target_class = 1
formula = model.get_global_explanation(x_val, y_val, target_class)
# compute explanation accuracy
accuracy = dl.logic.test_explanation(formula, target_class, x_test, y_test)
\end{lstlisting}

% \textbf{Unless required by applicable law or agreed to in writing, software is distributed on an "as is" basis, without warranties or conditions of any kind, either express or implied.}

\subsection{Dataset and classification task details}
\label{sec:exp_details}
For the experimental analysis, we consider five categorical learning problems ranging from computer vision to medicine and democracy. Some datasets (e.g. CUB) were already annotated with high-level concepts (e.g. bird attributes) which can be exploited to train a concept bottleneck pipeline. For datasets without annotations for high-level concepts, we transform the input space into a predicate space (i.e. $\mathbb{R}^d \rightarrow [0,1]^d$) to make it suitable for training LENs. According to the considered data type, we evaluate and discuss the usage of  different LEN pipeline, classification and explanation style (see Tab. \ref{tab:datasets}).
For the sake of consistency, in all supervised experiments LENs were trained by optimizing Eq. \ref{eq:IFF}, therefore extracting IFF rules. However also Eq. \ref{eq:IF} \ref{eq.IF2} could be optimized, above all when explaining a black-box model.


\textsc{MIMIC-II - E2E Interpretable classification. }
The Multiparameter Intelligent Monitoring in Intensive Care II (MIMIC-II, \cite{saeed2011multiparameter,goldberger2000physiobank}) is a public-access intensive care unit (ICU) database consisting of 32,536 subjects (with 40,426 ICU admissions) admitted to
%medical, surgical, cardiovascular and neonatal ICUs, surgical recovery units, and coronary care units 
ICUs at a single tertiary care hospital. The dataset contains detailed description of a variety of clinical data classes: general,
%(e.g. patient demographics, hospital admission and discharge dates, hospital death dates, etc), 
physiological, % (e.g.	nurse-verified vital signs, blood pressure, heart rate, etc), 
results of clinical laboratory tests, % (e.g. hematology, blood chemistries, urinalysis, microbiology, etc), 
records of medications, fluid balance, %(e.g. solutions, urine, estimated blood loss, etc), 
and free text notes and reports of imaging studies (e.g. x-ray, CT, MRI, etc). In our experiments, we remove the text-based input features and 
%discretize some of the continuous features into a set of categories in order to get a one-hot encoded representation. For instance, 
we discretize blood pressure (BP) into five different categories (one-hot encoded): very low BP, low BP, normal BP, high BP, and very high BP. After such preprocessing step, we obtain an input space $X=C \subset [0,1]^d$ composed of $d=90$ key features. 
The task consists in training a classifier function to identify recovering ($Y=1$) or dying ($Y=0$) patients, after 28 days from ICU admission. In particular, we consider the case of
% {\bf Interpretable classification. }
\textit{Interpretable classification} where an End-to-End LEN $X=C \rightarrow E=Y$ is employed to carry out the classification task.
But we also considered the case of 

\textsc{MIMIC-II (EBB) - {E2E Explaining a black-box model}. } On the same dataset, a second task is set up. A black-box model $g$ $X=C \rightarrow Y$ is employed to solve the classification task, with predictions $g(C) \approx Y$. The end-to-end model $f$ $X=C \rightarrow E=g(C)$ instead is trained to mimic the behaviour of the black box $g$.

% \subsubsection{Concept bottleneck explainers}
% \label{sec:exp_cbm}

% \paragraph{MNIST Even/Odd}
\textsc{MNIST Even/Odd - {CB Interpretable classifications}. }
The Modified National Institute of Standards and Technology database (MNIST, \cite{lecun1998mnist}) contains a large collection of images representing handwritten digits. The input space $X \subset \mathbb{R}^{28\times 28}$ is composed of 28x28 pixel images while the concept space $C \subset [0,1]^{10}$ is represented by digits from $0$ to $9$. 
However, the task we aim to solve is slightly different from the common digit-classification. In the case of 
% {\bf Interpretable classification}
\textit{interpretable classification}, indeed, assuming $Y \subset [0,1]^2$, we are interested in determining if a digit is either odd or even, and explain the assignment to one of these classes in terms of the high-level concepts $C$ (digits). The mapping $X \rightarrow C$ is learned by a ResNet10 classifier $g$ \cite{he2016deep}  trained from scratch, while a LEN $f$ is used to learn both the mapping and the explanation as a function $C=g(X) \rightarrow E=Y$. 

% The $\mu$ network is equipped with a single hidden layer with 10 neurons and the $L_1$ loss weight $\lambda = 10^{-2}$. 
% The $ReLU$ network is equipped with two hidden layers composed of 30, 10 hidden neurons respectively and $\lambda = 10^{-3}$. 
% The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^-3$ and fan-in = 5. 
% All networks have been trained for 200 epochs with learning rate = $10^ {-3}$.

\textsc{MNIST E/O (IC) - {CB Interpretable clustering}. }
 The same dataset has been used to perform
% {\bf Interpretable Clustering}
\textit{Interpretable clustering}.  We consider a concept space $C \subset [0,1]^{12}$ which comprise both the digits and the even/odd labels. The mapping $X \rightarrow C$ is learned again by a Resnet10 model $g$ trained as a multi-label classifier, while the LEN $f$ performs clustering from $C=g(X) \rightarrow E$, where $E \subset [0,1]^{2}$ space, in order two extract two clusters. 
% In this case, 
% the $\mu$ network is equipped with two hidden layer with 20, 10 neurons respectively and the $L_1$ loss weight $\lambda = 10^{-3}$. 
% The $ReLU$ network is equipped with two hidden layers composed of 50, 30 hidden neurons and $\lambda = 10^{-4}$. 
% The $\psi$ network at last is equipped with no hidden layers, $\lambda = 10^{-2}$ and fan-in = 2. 
% The $\mu$ and the $ReLU$ networks have been trained for 100 epochs with learning rate = $10^{-3}$ while for the $\psi$ network is equal to $10^{-2}$.

%Quantitative results are reported in Table \ref{tab:exp_metrics_mnist_cbm} while Table \ref{tab:exp_formula_mnist_cbm} shows for each fold the explanation extracted from trained explainers.
\textsc{CUB - CB Interpretable Classification .}
The Caltech-UCSD Birds-200-2011 dataset (CUB, \cite{wah2011caltech}) is a fine-grained classification dataset. It includes 11,788 images representing $r = 200$ ($Y \subset [0,1]^{200}$) different bird species. 312 binary attributes have been also collected for each image representing visual characteristics (color, pattern, shape) of particular parts (beak, wings, tail, etc.). Attributes annotations, however, is quite noisy. Similarly to \cite{koh2020concept}, we denoised attributes by considering class-level annotations, i.e. a certain attribute is set as present only if it is also present in at least 50\% of the images of the same class. Furthermore we only considered attributes present in at least 10 classes after this refinement. In the end, a total of $d = 108$ attributes ($C \subset [0,1]^{108}$) have been retained. The mapping $X \rightarrow C$ from images to attribute concepts is performed again with a ResNet10 model $g$ trained from scratch while a LEN $f$ learns the final function $C = g(X) \rightarrow E=Y$.


\textsc{V-Dem - Cascade Interpretable classification. }
Varieties of Democracy (V-Dem, \cite{pemstein2018v,coppedge2021v}) is a dataset containing a collection of indicators of latent regime characteristics over 202 countries from 1789 to 2020. The database include $d_1 = 483$ low-level indicators $C_1 \subset [0,1]^{d_1}$ (e.g. media bias, party ban, high-court independence, initiatives permitted, etc), $d_2 = 82$ mid-level indices $C_1 \subset [0,1]^{d_2}$ (e.g. freedom of expression, freedom of association, equality before the law, etc), and 5 high-level indices of democracy principles (i.e. electoral, liberal, participatory, deliberative, and egalitarian). In the experiments a binary classification problem is considered to identify electoral democracies ($Y=1$) from non-electoral democracies ($Y=0$). Cascading LENs $f_1$ and $f_2$ are trained to learn the map $C_1 \rightarrow C_2 \rightarrow E=Y$.



\subsection{Quantitative metrics for model and explanations}
\label{sec:exp_metrics}
Seven metrics are used to compare the performance of LENs with respect to state-of-the-art approaches.
While measuring classification metrics is necessary for models to be viable in practice to perform interpretable classification tasks, assessing the quality of the explanations is required to justify their use for explainability. In contrast with other kind of explanations, logic-based formulas can be evaluated quantitatively. Given a classification problem, first we extract a set of rules from a trained model and then we test each explanation on an unseen set of samples.
The results for each metric are reported in terms of the mean and the standard error of the mean, computed over a 10-fold cross validation \cite{krzywinski2013error}. Only in the CUB experiments a 5-fold cross validation is performed due to timing issues related to BRL (each training of BRL on CUB lasts about 3 hours).
For each experiment we measure: 
% (1) the test accuracy of the classifier, (2) the test accuracy of the explanation, (3) the complexity of the explanation, (4) the fidelity of the explanation with respect to the classifier, (5) the elapsed time required to extract the explanations, (6) the consistency of the explanation over different runs, and (7) the normalized mutual information (for unsupervised tasks only). 
% \cite{andrews1995survey}. 

\begin{itemize}
\item The \textsc{model accuracy} measures how well the classifier correctly identifies the target class (see Table. \ref{tab:model-accuracy}). When the model is the classifier itself (i.e. interpretable classification), this metric represents the accuracy of the model. Instead, when the model explain the predictions of a black box classifier, this metric represents the accuracy of the black box classifier.
\item The \textsc{explanation accuracy} measures how well the extracted logic formula correctly identifies the target  class (see Table. \ref{tab:explanation-accuracy}).
\item The \textsc{complexity of an explanation} measures how hard would it be for a human being to understand the logic formula (see Table. \ref{tab:complexity}). This metric is computed by standardizing the explanations in disjunctive normal form and then by counting the number of terms of the standardized formula.
\item The \textsc{fidelity of an explanation} measures how well the predictions obtained using the extracted explanation match the predictions obtained using the classifier (see Table. \ref{tab:fidelity}). When the model is the classifier itself (i.e. interpretable classification), this metric represents the match between the extracted explanation and the model. Instead, when the model is explaining the predictions of a black box classifier, this metric represents the match between the extracted explanation and the black box classifier.
\item The \textsc{rule extraction} measures the time required to obtain an explanation from scratch. It is computed as the sum of the time required to train the (see Table. \ref{tab:extraction}) model and the time required to extract the formula from a trained model. This is justified by the fact that for some models, like BRL, training and rule extraction consist of just one simultaneous process.
\item The \textsc{consistency of an explanation} measures the similarity of the extracted explanations over different runs (see Table. \ref{tab:consistency}). It is computed by counting how many times the same concepts appear in the logic formulas over different folds of a cross-validation or over different initialization seeds.
% \item The \textsc{normalized mutual information} measures the quality of the clusters obtained in the interpretable clustering experiments. It is calculated as the mutual information of Eq. \ref{eq:MI}, divided by the Entropy $H_E$ so that it reports a number always comprehended between $[0,1]$.
\end{itemize}








\subsection{Results and Discussion}
% \textsc{Interpretable classification. } 
Experiments show how LENs generalize better than decision trees on complex Boolean functions (e.g. CUB and MIMIC-II) as already observed in \cite{tavares2020understanding} (Table. \ref{tab:model-accuracy}). For most experiments the formulas extracted from LENs are either better or almost as accurate as the formulas found by decision trees or mined by BRL (Table. \ref{tab:explanation-accuracy}). The complexity of LEN explanations is usually lower than the complexity of the rules extracted from a decision tree or mined by BRL. The complexity of decision tree formulas is never below 100 terms, making them useless for quick decision making (Table. \ref{tab:complexity}). White-box models like decision trees and BRL outperform LENs in terms of fidelity. Their predictions is directly based on the explanation therefore fidelity is always 100\%. However, the fidelity of the formulas extracted by the $\mu$ and the ReLU network is often higher than $90\%$. This means that almost any prediction has been correctly explained, making these networks very close to white boxes (Table. \ref{tab:fidelity}). BRL is the slowest rule extractor over all the experiments by one order of magnitude, while the decision tree is the fastest overall (Table. \ref{tab:extraction}). In terms of consistency there is not a dominant method (Table. \ref{tab:consistency}).

Fig. \ref{fig:multi-objective} shows the Pareto frontiers \cite{marler2004survey} for each experiment in terms of the complexity of the explanation and its classification error ($100 -$ classification accuracy). The simplest and most accurate formulas are found by the LENs, whose complexity is almost always below the maximum complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}). Across all the experiments, there is at least one set of formulas extracted from out-of-the-box LEN dominating both BRL and decision trees.

For each dataset and for each method Table \ref{tab:best-rules} reports some compact FOL formula extracted. 


\textsc{Interpretable Clustering. } 
As introduced in the MNIST E/O dataset explanation we performed clustering starting from a Concept space composed of the 10 digits and the even/odd labels. The LEN are instructed two extract 2 clusters possibly respecting the even/odd division of digits. In Table \ref{tab:exp_metrics_mnist_mi} the metrics regarding this task are reported. We can see that all methods are capable to maximize the normalized mutual information. However only the $\psi$ network is capable to consistently explain the two clusters in terms of the important labels (even and odd), as we can see from the complexity of the rules (higher than 2 for the $\mu$ and ReLu net) and for the consistency of terms used in the explanation (100\% for the $\psi$ network). 
Other examples and application of Interpretable Clustering has been performed in \cite{ciravegna2020constraint, ciravegna2020human} employing the $\psi$ network only.

% \subsection{Other experiences}

% \textsc{Explanation as a defense}


\begin{table}[!h]
\centering
\caption{Model's accuracy (\%)}
\label{tab:model-accuracy}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllll}
\toprule
{} &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL & Black box \\
\midrule
\textbf{MIMIC-II     }  &  ${\bf 86.60 \pm 0.30}$ &  $85.36 \pm 0.78$ &  $84.01 \pm 0.09$ &  $79.56 \pm 0.80$ &  $86.15 \pm 0.51$ & N/A \\
\textbf{MIMIC-II (EBB)}  &  N/A &  N/A &  N/A &  N/A &  N/A  & $85.13 \pm 0.70$\\
\textbf{V-Dem         } &  $91.96 \pm 0.42$ &  $91.88 \pm 0.37$ &  $79.23 \pm 2.20$ &  $92.11 \pm 0.38$ &  ${\bf 92.23 \pm 0.38}$ & N/A \\
\textbf{MNIST}          &  $99.75 \pm 0.02$ &  $99.81 \pm 0.01$ &  $99.80 \pm 0.01$ &  ${\bf 99.96 \pm 0.01}$ &  $99.80 \pm 0.01$ & N/A \\
\textbf{CUB          }  &  ${\bf 92.26 \pm 0.28}$ &  $92.19 \pm 0.27$ &  $91.72 \pm 0.56$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ & N/A \\

\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[!h]
\centering
\caption{Explanation's accuracy (\%)}
\label{tab:explanation-accuracy}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
\midrule
\textbf{MIMIC-II     } &  $85.08 \pm 0.48$ &  $82.09 \pm 1.38$ &  $82.83 \pm 0.66$ &  $79.56 \pm 0.80$ &   ${\bf86.15 \pm 0.51}$ \\
\textbf{MIMIC-II (EBB)} &  ${\bf85.75 \pm 0.51}$ &  $81.07 \pm 3.33$ &  $83.90 \pm 1.25$ &  $85.53 \pm 0.61$ &  $85.70 \pm 0.48$ \\
\textbf{V-Dem         } &  $90.81 \pm 1.24$ & ${\bf94.65 \pm 0.32}$ &  $80.29 \pm 2.99$ &  $92.11 \pm 0.38$ &  $92.23 \pm 0.38$ \\
\textbf{MNIST}         &  $99.67 \pm 0.01$ &  $98.04 \pm 1.60$ &  $75.47 \pm 0.46$ &  ${\bf99.96 \pm 0.01}$  &  $99.80 \pm 0.01$ \\
\textbf{CUB*         } &  ${\bf96.15 \pm 0.16}$ &  $93.98 \pm 1.97$ &  $80.41 \pm 2.31$ &  $89.30 \pm 0.42$ &  $82.18 \pm 0.43$ \\


\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[!h]
\centering
\caption{Complexity}
\label{tab:complexity}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{}                     &        $\mu$ net &         ReLU net &       $\psi$ net &                 Tree &               BRL \\
\midrule
\textbf{MIMIC-II     } &  $5.10 \pm 0.35$ &  $23.40 \pm 11.20$ &  ${\bf2.60 \pm 0.16}$ &  $1342.60 \pm 16.94$ &  $20.70 \pm 4.08$ \\
\textbf{MIMIC-II (EBB)} &  $7.00 \pm 0.70$ &    $6.40 \pm 0.95$ &  ${\bf1.30 \pm 0.15}$ &   $432.10 \pm 16.46$ &  $22.90 \pm 4.13$ \\
\textbf{V-Dem         } &  $9.60 \pm 1.17$ &    $4.90 \pm 0.10$ &  ${\bf2.00 \pm 0.49}$ &    $294.10 \pm 7.88$ &   $8.70 \pm 0.97$ \\
\textbf{MNIST}         &  ${\bf22.00 \pm 4.67}$ &  $48.10 \pm 1.43$ &  $24.85 \pm 2.89$ &  $632.35 \pm 5.01$ &  $1291.05 \pm 234.40$ \\
\textbf{CUB          } &  $10.53 \pm 0.08$ &  $29.25 \pm 3.26$ &  $28.36 \pm 2.75$ &  $138.83 \pm 5.31$ &  ${\bf4.10 \pm 0.09}$ \\


\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[!h]
\centering
\caption{Fidelity (\%)}
\label{tab:fidelity}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{}                     &         $\mu$ net &          ReLU net &        $\psi$ net &              Tree &               BRL \\
\midrule
\textbf{MIMIC-II     } &  $96.23 \pm 0.81$ &  $87.84 \pm 2.12$ &  $84.63 \pm 0.67$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
\textbf{MIMIC-II (EBB)} &  $92.28 \pm 0.90$ &  $86.58 \pm 4.00$ &  $90.32 \pm 1.27$ &   $93.07 \pm 0.53$ &   ${\bf94.82 \pm 0.50}$ \\
\textbf{V-Dem         } &  $91.52 \pm 1.13$ &  $94.62 \pm 0.37$ &  $82.45 \pm 1.80$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
\textbf{MNIST}         &  $99.90 \pm 0.03$ &  $98.14 \pm 1.60$ &  $75.53 \pm 0.46$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\
\textbf{CUB*         } &  $97.82 \pm 0.15$ &  $95.37 \pm 2.06$ &  $81.89 \pm 2.35$ &  ${\bf100.00 \pm 0.00}$ &  ${\bf100.00 \pm 0.00}$ \\


\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[!h]
\centering
\caption{Rule extraction time (s)}
\label{tab:extraction}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
{} &        $\mu$ net &         ReLU net &       $\psi$ net &             Tree &              BRL \\
\midrule
\textbf{MIMIC-II     } &  $13.32 \pm 0.30$ &  $266.22 \pm 166.90$ &   $8.81 \pm 0.15$ &  ${\bf0.02 \pm 0.00}$ &  $495.59 \pm 7.13$ \\
\textbf{MIMIC-II (EBB)} &  $15.30 \pm 0.19$ &     $18.46 \pm 1.00$ &  $10.14 \pm 0.03$ &  ${\bf0.01 \pm 0.00}$ &  $543.43 \pm 3.39$ \\
\textbf{V-Dem         } &  $34.40 \pm 0.78$ &     $34.24 \pm 0.32$ &  $20.83 \pm 0.04$ &  ${\bf0.06 \pm 0.00}$ &   $53.69 \pm 0.41$ \\
\textbf{MNIST}         &  $173.24 \pm 6.77$ &  $221.07 \pm 4.06$ &  $236.71 \pm 3.36$ &  ${\bf2.04 \pm 0.04}$ &  $836.14 \pm 3.15$ \\
\textbf{CUB          } &  $726.19 \pm 2.43$ &  $660.30 \pm 121.16$ &  $2094.49 \pm 730.50$ &  ${\bf4.17 \pm 0.07}$ &  $9863.52 \pm 147.57$ \\

\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[!h]
\centering
\caption{Rule consistency (\%)}
\label{tab:consistency}
\begin{tabular}{llllll}
\toprule
{} & $\mu$ net & ReLU net & $\psi$ net &     Tree &      BRL \\
\midrule
\textbf{MIMIC-II     } &   $51.00$ &  $26.00$ &    $37.14$ &  ${\bf81.50}$ &  $28.33$ \\
\textbf{MIMIC-II (EBB)} &   $41.18$ &  $35.56$ &    $43.33$ &  ${\bf60.36}$ &  $22.22$ \\
\textbf{V-Dem         }&   $71.67$ &  ${\bf98.00}$ &    $15.83$ &  $36.86$ &  $76.25$ \\
\textbf{MNIST}         &   $60.00$ &  ${\bf100.00}$ &    $50.00$ &  $50.95$ &  ${\bf100.00}$ \\
\textbf{CUB          } &   ${\bf58.82}$ &  $58.40$ &    $43.08$ &  $21.79$ &  $30.00$ \\

\bottomrule
\end{tabular}
\end{table}



\begin{figure}[!h]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/mimic2.pdf}
    \includegraphics[width=0.49\textwidth]{figs/mimic_explain_classifier.pdf}\\
    \includegraphics[width=0.49\textwidth]{figs/mnist.pdf}
    \includegraphics[width=0.49\textwidth]{figs/cub.pdf}\\
    \includegraphics[width=0.49\textwidth]{figs/vdem_low2mid.pdf}
    \\
    \includegraphics[width=0.7\textwidth]{figs/legend.pdf}
    \caption{Pareto frontiers (dotted black line) in terms of average test error and average complexity of the explanations. Formulas out-of-the-box extracted from out-of-the-box LENs are reported as circles while BRL and decision trees as crosses. The vertical dotted red line marks the maximum explanation complexity laypeople can handle (i.e. complexity $\leq 9$ \cite{miller1956magical,cowan2001magical,ma2014changing}).}
    \label{fig:multi-objective}
\end{figure}

\begin{table}[!h]
\centering
\caption{MNIST Mutual Information}
\label{tab:exp_metrics_mnist_mi}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
     Method & Model's accuracy (\%) & Exp. accuracy (\%) &       Complexity & Extraction time (s) & Rule consistency (\%) \\
\midrule
 $\psi$  net &     $99.90 \pm 0.01$ &           $99.90 \pm 0.01$ &  $2.00 \pm 0.00$ &     $0.33 \pm 0.15$ &             $100.00$ \\
 $\mu$ net &     $94.91 \pm 4.99$ &           $95.41 \pm 4.50$ &  $2.30 \pm 0.64$ &     $2.36 \pm 0.75$ &              $35.00$ \\
   ReLU net &     $96.87 \pm 3.04$ &           $95.97 \pm 3.94$ &  $2.15 \pm 0.39$ &     $4.15 \pm 1.62$ &              $45.00$ \\
\bottomrule
\end{tabular}
}
\end{table}





% \subsection{Rules Extracted}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
{\renewcommand{\arraystretch}{2.5}
\begin{table}[!h]
\centering
\caption{A selection of some of the best rules extracted for each experiment.}
\label{tab:best-rules}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
\multicolumn{1}{l}{\textbf{Dataset}}    & \textbf{Model}  & \textbf{Rule} \\ \hline
\multirow{5}{*}{MIMIC-II}      & $\mu$ net  & $Death \leftarrow stroke \wedge age\_HIGH  \wedge \neg atrial\_fibrillation $  \\
                               & ReLU net   & $Death \leftarrow stroke \wedge age\_HIGH \wedge \neg atrial_fibrillation \wedge \neg sapsi\_first\_LOW \wedge \neg sapsi\_first\_HIGH $  \\
                               & $\psi$ net & $Death \leftarrow stroke \vee bun\_first\_NORMAL \vee sapsi\_first\_HIGH $  \\
                               & Tree       & $Death \leftarrow \quad ^*$formula is too long (1000+ terms) \\ 
                               & BRL        & $Death \leftarrow \makecell[l]{(stroke \wedge resp \wedge \neg age\_LOW \wedge \neg sapsi\_first\_LOW) \\
                               \vee (stroke  \wedge age\_HIGH \wedge \neg age\_LOW  \wedge  \neg sapsi\_first\_LOW) }$  \\ \hline
\multirow{5}{*}{MIMIC-II (EBB)} & $\mu$ net  & $Death \leftarrow atrial_fibrillation \wedge stroke \wedge \neg sapsi\_first\_HIGH \wedge \neg weight\_first\_NORMAL $  \\
                               & ReLU net   & $Death \leftarrow stroke \wedge \neg sapsi\_first\_LOW  \wedge  \neg sapsi\_first\_HIGH \wedge \neg sodium\_first\_LOW $  \\
                               & $\psi$ net & $Death \leftarrow stroke \wedge age\_HIGH $  \\
                               & Tree       & $Death \leftarrow  \quad ^*$formula is too long (100+ terms)  \\ 
                               & BRL        & $Death \leftarrow \makecell[l]{stroke \wedge age\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW) \\ \vee  (stroke \wedge platelet\_first\_HIGH \wedge weight\_first\_LOW \wedge \neg sapsi\_first\_LOW } $  \\  \hline
\multirow{5}{*}{MNIST}         & $\mu$ net  & $Even \leftarrow \neg One \wedge \neg Three \wedge \neg Five \wedge \neg Seven \wedge \neg Nine $  \\
                              & ReLU net   & $Even \leftarrow \makecell[l]{(Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\ 
                              \vee (Two \wedge \neg Zero \wedge \neg One \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\ 
                              \vee (Four \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\ 
                              \vee (Six \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Seven \wedge \neg Eight \wedge \neg Nine) \\
                              \vee (Eight \wedge \neg Zero \wedge \neg One \wedge \neg Two \wedge \neg Three \wedge \neg Four \wedge \neg Five \wedge \neg Six \wedge \neg Seven \wedge \neg Nine) } $ \\
                              & $\psi$ net & $Even \leftarrow \makecell[l]{(Six \wedge Zero \wedge \neg One \wedge \neg Seven)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Three)  \\
                              \vee (Six \wedge Zero \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge \neg One \wedge \neg Seven \wedge \neg Three) \\
                              \vee (Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)  \vee (Six \wedge Zero \wedge \neg One \wedge \neg Seven \wedge \neg Three)}$  \\
                              & Tree       & $Even \leftarrow \quad ^*$formula is too long \\
                              & BRL        & $Even \leftarrow  \makecell[l]{(Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two)) \vee (Eight \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Five \wedge \neg Two)) 
                              \\ \vee (Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Seven \wedge \neg Two)) \\ 
                              \vee (Two \wedge \neg One \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \\ \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two)) \\
                              \vee (Four \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \\ \wedge  \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One)) \\
                              \vee (Zero \wedge \neg Four \wedge \neg Nine \wedge \neg Six \wedge \neg Three \wedge \neg (Eight \wedge \neg Nine) \wedge \neg (Five \wedge \neg Two) \wedge \neg (Four \wedge \neg Nine) \\
                              \wedge \neg (Nine \wedge \neg Zero) \wedge \neg (One \wedge \neg Two) \wedge \neg (Seven \wedge \neg Nine) \wedge \neg (Seven \wedge \neg Two) \wedge \neg (Two \wedge \neg One))
                              }$  \\ \hline
\multirow{5}{*}{CUB}          & $\mu$ net  & $ Black\ foot\ albatross \leftarrow \makecell[l]{  bill \ shape \ hooked \ seabird \ \wedge \  size \ medium \wedge \ wing \ pattern \ solid \\
                              \wedge \neg wing color \ black \wedge \neg  underparts\ color\ white \wedge \neg upper\ tail\ color\ grey \\
                              \wedge \neg breast\ color\ white \wedge \neg  throat\ color\ white \wedge \neg tail\ pattern\ solid \wedge \neg  crown\ color\ white} $  \\
                              & ReLU net   & $ Black\ foot\ albatross \leftarrow  \makecell[l]{ size\  medium  \wedge \neg  bill\  shape\  allpurpose  \\ 
                              \wedge \neg  upperparts\  color\  black  \wedge \neg  head\  pattern\  plain  \wedge \neg  under\  tail\  color\  yellow \\  \wedge \neg  under\  tail\  color\  black  \wedge \neg  nape\  color\  buff  \\
                              \wedge \neg  wing\  shape\  roundedwings  \wedge \neg  shape\  perchinglike  \\
                              \wedge \neg  leg\  color\  grey  \wedge \neg  leg\  color\  black  \wedge \neg  bill\  color\  grey  \\
                              \wedge \neg  bill\  color\  black  \wedge \neg  wing\  pattern\  multicolored }$\\
                              & $\psi$ net & $ Black\ foot\ albatross \leftarrow  \makecell[l]{(bill \ shape \ hooked\ seabird \wedge tail \ pattern \ solid \wedge \neg underparts \ color \ white \\
                              \wedge ( \neg  \ breast \ color \ white \vee \neg   \ wing \ color \ grey)) }$  \\
                              & Tree       & $ Black\ foot\ albatross \leftarrow  ^*$formula is too long (1000+ terms)  \\
                              & BRL        & $ Black\ foot\ albatross \leftarrow  \makecell[l]{( bill\  shape\  hooked\  seabird \wedge forehead\ color\ blue \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white) \\
                              \vee ( bill\  shape\  hooked\  seabird \wedge  \neg  bill\  color\  black \wedge  \neg  nape\  color\  white \wedge  \neg  tail\  pattern\  solid)}$ \\ 
\hline
\multirow{5}{*}{V-Dem}         & $\mu$ net  & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & ReLU net   & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\
                               & $\psi$ net & $Elect\_ Dem \leftarrow v2x\_frassoc\_thick \wedge v2xeg\_eqaccess $  \\
                               & Tree       & $Elect\_ Dem \leftarrow \quad ^*$formula is too long (1000+ terms)  \\
                               & BRL        & $Elect\_ Dem \leftarrow v2x\_freexp\_altinf \wedge v2x\_frassoc\_thick \wedge v2xel\_frefair \wedge v2x\_elecoff \wedge v2xcl\_rol $  \\ \hline
\end{tabular}%
}
\end{table}}



% These challenging or product-oriented contexts are the actual targets of XAI research. This great research effort have produced a variety of quite interesting and efficient approaches to unveil the decision process of black-box models. Some of the most common taxonomies are based on a few discriminative criteria (intrinsic interpretability VS post-hoc, model-specific VS model-agnostic, local VS global explanations), but the most important characteristic, i.e. the \textit{form} of the explanation, is often overlooked.

% include white-box models, model-agnostic approaches \cite{ribeiro2016model} and example-based explanations \cite{aamodt1994case,kim2016examples,barbiero2020uncovering}. 


% decision trees \cite{breiman1984classification}, or decision rules: oneR \cite{holte1993very}, RIPPER \cite{cohen1995fast}, Bayesian Rule Lists \cite{letham2015interpretable}).

% \begin{itemize}
%     \item many interesting works around explainability, from fully interpretable models (LR, DT, DR), to surrogates (LIME, Anchors, SHAP, etc) to example-based
%     \item great effort on scoring/ranking features/concepts
%     \item that's NOT the whole point
%     \item what matters (even more?) is how concepts are related (PDP? mah...)
%     \item what is the effort for the end user for analyzing a pairwise dependence plot or a ranking or a decision tree with depth 5?
%     \item good explanations must be simple
%     \item simple <-> few concepts involved? well yes, but...
%     \item traditional methods tend to assume: simplicity -> simple relationships among concepts (linear, max PDP)
%     \item we argue: why??
% \end{itemize}

% % -idee generali su che tipo di bestie c'è per fare expl.. 
% % -s'è già detto che i sistemi a regole sono più utili per fare supporto a umani.. che robe c'è in giro, perchè il nostro è più fiho
% % - il survey congnitivo dice che regole buone devono essere semplici.. -> pruning! che tipi di pruning usa sta gente che fa expl?

% What Is an Explanation? An explanation is the answer to a why-question (Miller 2017).


% to mention: (Bayesian Rule Lists: \cite{letham2015interpretable} tipo decision trees)

% \begin{itemize}
%     \item taxonomy
%     \begin{itemize}
%         \item intrinsic or post-hoc? LENs support both!
%         \item result of the interpretation:
%         \begin{itemize}
%             \item Feature summary statistic (feature importance or pairwise feature interactions or rank visualization)
%             \item Model internals (weights in linear models or the learned tree structure)
%             \item Data point (counterfactual explanations or identification of prototypes of predicted classes)
%             \item Intrinsically interpretable model
%         \end{itemize}
%         \item Model-specific or model-agnostic?
%         \item Local or global?
%     \end{itemize}
%     \item Properties of Explanation Methods
%     \begin{itemize}
%         \item Expressive Power is the "language" or structure of the explanations (IF-THEN rules, decision trees, a weighted sum, natural language or something else)
%         \item Translucency describes how much the explanation method relies on looking into the machine learning model
%         \item Portability 
%         \item Algorithmic Complexity
%     \end{itemize}
%     \item Properties of Individual Explanations
%     \begin{itemize}
%         \item Accuracy: How well does an explanation predict unseen data?
%         \item Fidelity: How well does the explanation approximate the prediction of the black box model?
%         \item Consistency: How much does an explanation differ between models that have been trained on the same task and that produce similar predictions?
%         \item Stability: How similar are the explanations for similar instances?
%         \item Comprehensibility: How well do humans understand the explanations?
%         \item Certainty: Does the explanation reflect the certainty of the machine learning model?
%         \item Degree of Importance: How well does the explanation reflect the importance of features or parts of the explanation?
%         \item Novelty: Does the explanation reflect whether a data instance to be explained comes from a "new" region far removed from the distribution of training data?
%         \item Representativeness: How many instances does an explanation cover?
%     \end{itemize}
%     \item good explanations
%     \begin{itemize}
%         \item Explanations are contrastive (Lipton 1990)
%         \item Explanations are selected (simple)
%         \item Explanations are social. They are part of a conversation
%         \item Explanations focus on the abnormal. People focus more on abnormal causes to explain events (Kahnemann and Tversky, 1981).
%         \item Explanations are truthful. Good explanations prove to be true in reality
%         \item Good explanations are consistent with prior beliefs of the explainee
%         \item Good explanations are general
%     \end{itemize}
%     \item interpretable models: logistic regression, decision trees, decision rules and the RuleFit algorithm
%     \item model agnostic: 
%     \begin{itemize}
%         \item plots: Accumulated local effects, Partial Dependence Plot, Individual Conditional Expectation
%         \item surrogates: Global Surrogate, Local Surrogate (LIME), \textbf{Scoped Rules (Anchors)} (many scenarios require discretization, many calls to the ML model), \textbf{SHAP} (SHapley Additive exPlanations)
%     \end{itemize}
%     \item example based: Counterfactual explanations, Prototypes
%     \item neural networks: Feature Visualization, Concepts, Modell Distillation (How can we explain a neural network with a simpler model?)
% \end{itemize}

% \paragraph{Occam's razors}
% In his Posterior Analytics, Aristotle stated: "We may assume the superiority ceteris paribus [other things being equal] of the demonstration which derives from fewer postulates or hypotheses" \cite{aristotlePosterior}. The \textit{law of parsimony} presented by the Greek philosopher has deeply influenced researchers and scientists across the centuries. In other words, when humans compare a set of explanations outlining the same outcomes, they tend to have an implicit bias towards the simplest one. Researchers have proposed many approaches to integrate this parsimony principle into learning machines over the years. Bayesian priors \cite{wilson2020case} and weight regularization \cite{kukavcka2017regularization} are just some of the most famous approaches. Among such techniques, $L1$-regularization \cite{santosa1986linear,tibshirani1996regression} has been recently shown quite effective for neural networks providing logic-based explanations \cite{ciravegna2020human} as it encourages sparsity by shrinking the less important weight's values to zero thus removing some weights altogether in the limit. Following \cite{ciravegna2020human}, the models analyzed in this work are mainly based on $L1$-regularization. However, in future works it may also worth exploring the integration of LENs with concept-based parsimony criteria \cite{chen2020concept} or with fuzzy-logic regularizers which have recently been used to combine deductive reasoning and human priors with deep learning \cite{marra2019lyrics}.




\section{Conclusion} \label{sec:conclusion}

\subsection{Limitations and future research directions}
The extraction of a first-order logic explanation requires symbolic input and output spaces. This constraint is the main limitation of our framework, as narrows the range of applications down to symbolic I/O problems. In some contexts, such as computer vision, the use of LENs may require additional annotations and attribute labels to get a consistent symbolic layer of concepts. However, recent work on automatic concept extraction may partially solve this issue leading to more cost-effective concept annotations \cite{ghorbani2019towards,kazhdan2020now}.

Another area to focus on might be the improvement of out-of-the-box LENs. The efficiency and the classification performances of fully interpretable LENs, i.e. $\psi$ network, is still quite limited due to the extreme pruning strategy. Even more flexible approaches, like $\mu$ networks, are not as efficient as standard neural models when tackling multi-class or multi-label classification problems, as they require a bigger architecture to provide a disentangled explanation for each class.

In our vision this framework would thrive and express its full potential by interacting with the external world and especially with humans in a dynamic way. In this case, logic formulas might be rewritten as sentences to allow for a more natural interaction with end users. Moreover, a dynamic interaction may call for an extended expressivity leading to higher-order or temporal logic explanations. Finally, in some contexts different neural architectures as graph neural networks might be worth exploring as they may be more suitable to solve the classification problem.


\subsection{Broader impact}
Current legislation in US and Europe binds AI to provide explanations especially when the economical, ethical, or financial impact is significant \cite{gdpr2017,law10code}. This work contributes to a lawful and safer adoption of some of the most powerful AI technologies allowing deep neural networks to have a greater impact on society. Extracting first-order logic explanations from deep neural networks enables satisficing knowledge distillation while achieving performances comparable with the state of the art. The formal language of logic provides clear and synthetic explanations, suitable for laypeople, managers, and in general for decision makers outside the AI research field. 

The experiments show how this framework can be used to aid bias identification and to make black boxes more robust to adversarial attacks by giving an explanation for the attack itself. As out-of-the-box LENs are easy to use even for neophytes and can be effectively used to understand the behavior of an existing algorithm, our approach might be used to reverse engineer competitor products, to find vulnerabilities, or to improve system design. From a scientific perspective, formal knowledge distillation from state-of-the-art networks may enable scientific discoveries or confirmation of existing theories.


\section*{Acknowledgments and Disclosure of Funding}
We thank ... for useful feedback and suggestions.

This work was partially supported by the European Union’s Horizon 2020 research and innovation programme under grant agreement No 848077.




\bibliographystyle{apalike}  % Sry Pietro, just had to
\bibliography{references}  %%% Remove comment to use the external .bib file (using bibtex).
%%% and comment out the ``thebibliography'' section.

\end{document}


==> old_rel_work.tex <==

\section{Related work}
\label{sec:related}
%%% taxonomy:




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DALLA 4
% XAI literature can be roughly partitioned into two categories: works focusing on white-box interpretable models and those aiming at providing satisficing explanations of model behaviours which are treated as black boxes. In the first category we can find models like Bayesian Rule Lists, Decision Tree; in the latter, post-hoc explanation algorithm such as LIME, SHAP but also saliency-map fall. 
% Based on this distinction and differently from other papers in literature, we here define \textit{Interpretability} and \textit{Explainability} as two different properties of machine learning models. \fg{In che senso? Volevi dire che noi offriamo entrambe le cose come 2 estremi di un unico modello?}

% \begin{definition}[Interpretability] 
% Interpretability is the extent to which the behavior of a model can be easily comprehended by a human.
% \end{definition}

% \begin{definition}[Explainability]
% It is the capacity to provide comprehensible explanations of the decisions taken by a certain model. 
% \end{definition}
% \fg{Da dove sono prese queste definizioni? Metterei citazione} 

% It is important to notice that both definitions point their attention on the model and not on the algorithm used to train it, which in this respect can be ignored.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



In the last few years, the demand for human-comprehensible models has significantly increased in safety-critical and data-sensible contexts. This popularity is justified by the emerging need for unveiling the decision process of pitch-black models like deep neural networks. To this aim, the scientific community has developed an important variety of XAI techniques, with different properties and goals. A simple but useful taxonomy has been recently considered in \cite{Das2020OpportunitiesAC} and it will be followed also in this paper. In particular, the authors identify in the \textit{Scope}, the \textit{Usage} and in the \textit{Methodology} the key-properties to define an XAI technique, to which we add the \textit{Explanation type}.

% \paragraph{Scope}
{\bf Scope. }
A fundamental feature to distinguish among explainable methods is whether they provide \textit{local} explanations, valid for a given sample, or \textit{global} explanations, valid on the whole input space. 
% For example, in the field of loan approval, an XAI technique providing local explanations might reveal which features leads to refuse a certain request. On the contrary, global explanations may uncover which are the most important factors leading to loan approval.

% \paragraph{Usage}
{\bf Usage. }
According to how the explained model is treated, an XAI techniques can be generally categorized as \textit{Model-intrinsic} or \textit{Post-hoc} methods. In the first category, we can finds techniques intrinsically provided by the model they explain, as for the interpretable-by-design models. %In principle, these are the best methods to provide explanations since these algorithms were originally developed for decision support systems. However, their decision function often is not smooth which makes them quite sensible to data distribution shifts and impairs their generalization ability on unseen observations \cite{tavares2020understanding,molnar2020interpretable}. 
Instead, in the \textit{Post-hoc} category, we can find techniques explaining models which do not provide explanations per se. These methods are referred to as \textit{post-hoc methods} since the explanations are generally given when the training procedure is concluded. %In some cases is treated as a black-box. 
%However, the explanations extracted in this way may not live up to the expectations. The main issue is that these methodologies usually focus on scoring/ranking the input features/concepts or on providing activation maps over the input. The way concepts are interconnected is usually not explored.
\fg{anche per gli interpretabili la procedura di training deve essere conclusa no? Direi che la differenza principale è che (post-hoc) uno ne spiega un altro, (intrisic) il classificatore è interpretabile per sè.}

% \paragraph{Methodology}
{\bf Methodology. }
The algorithms employed by most XAI models can be roughly categorized into two main categories. \textit{Backpropagation}-based techniques analyze the gradients of the activation up to the input features, in order to identify the most relevant ones for the classification task. \textit{Perturbation}-based techniques, instead, observe how the machine output changes when altering a given input data. The aim of these methods is to understand which %are the most discriminative 
features (when altered) may drive the model to take different decisions. 
Nonetheless, not all algorithms belong to these two categories. In particular, \textit{Model-intrinsic} explanation methods significantly differ according to the training algorithms.

{\bf Explanation Type. }
As anticipated in the previous section, there is no consensus on what an explanation should actually be.
Most of the methods in literature usually focus on scoring input features. However, \textit{Feature-scoring} methods
%
can be of scarce utility in decision support cases, whereas a comprehensible language may bring light on the predictor behaviour by identifying concept-based correlation.
% do not consider how concepts are interconnected, therefore, these explanations may not live up to the expectations. 
FOL formulas were the most common explanations in symbolic methods, but their popularity reduced with the advent of
%machine learning
sub-symbolic models. However, due to the advantages provided by this type of explanations, several \textit{FOL}-based explanation methods have been devised also in the last few years.

Some of the most famous XAI techniques share the characteristic of being Feature-scoring, Local, Post-hoc methods.
Sometimes indeed, the easiest way to solve the explanation problem is simply to treat the model as a black-box and sample by sample determine which are the most important features for a prediction. 
Prominent examples of algorithms falling in this area %are Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should}, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} and DeConvolution Neural Network (DeConv) \cite{zeiler2014visualizing}, which
accomplish this task by perturbing the input data. 
Local Interpretable Model-agnostic Explanations (LIME) \cite{ribeiro2016should} trains a white-box model (e.g. a logistic regression) to mimic the predictions of a given model in the neighbourhood of the sample to explain. By analyzing the weights of the white-box model it identifies the most important patch of pixels (superpixel).
Differently, SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} computes the Shapley value of each feature by iteratively removing each one of them. %provides for local explanations by computing each input feature contributions in a certain prediction. In the Kernel SHAP version, the Shapley values of each feature are calculated by iteratively removing features in a similar way to what is done in LIME.
% Deconvolutional Network were initially introduce in \cite{zeiler2011adaptive} for unsupervised learning.
% Firstly introduced in \cite{zeiler2011adaptive}, DeConvolution Neural Network (DeConv) are used in \cite{zeiler2014visualizing} to %visualize the activation of a convolutional layer. In particular, they 
%visually determine pixel importance for a certain prediction by analyzing how the classification output changes when part of the input image is masked. 
Other important techniques %such as Activation Maximization \cite{erhan2010understanding}, Saliency Maps \cite{simonyan2013deep} and Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} 
provide the same type of explanations through gradient analysis. %Differently from the previous one, however, they determine feature importance  %in the context of Convolutional Neural Network (CNN). 
Authors of Activation Maximization \cite{erhan2010understanding} firstly introduced this idea as an optimization problem. They explain the behaviour of a hidden/output unit by slightly modifying a given input data such that it maximizes its activation. An easier way to identify features causing a certain output has been found with Saliency Maps \cite{simonyan2013deep}, which project the classification loss until the input image. 
% A further improvement has been introduced with Gradient Class Activation Mapping (Grad-CAM) \cite{selvaraju2017grad} which allows to identify both class-specific image area and counterfactual explanations. 
%They achieved this by modifying global average pooling with class activation mapping which allows to identify important image area with a single forward pass.


Other post-hoc methods have been devised to extract global feature-scoring explanations, often starting from local explanations. %like LIME for Global Explanations \cite{ribeiro2016should} based on perturbation and Class Model Visualization \cite{simonyan2013deep} or Testing with Class Activation Vectors \cite{kim2018interpretability} based on Backpropagation. 
A submodular-pick algorithm extends the LIME module (SP-LIME) in %LIME for Global Explanations 
\cite{ribeiro2016should} to provide global explanations. SP-LIME first finds superpixels of all input samples with the standard LIME module. Successively, it finds the minimum number of common superpixels that covers most of the images.
Starting from the idea of Activation Maximization,  Class Model Visualization \cite{simonyan2013deep} finds the input sample that maximizes a certain class probability score in the whole input space. %Differently from Activation Maximization, here the input sample is not searched in the neighbourhood of a given sample, but in the whole input space. 

Post-hoc methods, however, can also supply FOL explanations. 
LOcal Rule-based Explanations of black-box decision systems (LORE) \cite{guidotti2018local} extracts FOL explanations via tree induction. They focus on local rules extracted through input perturbation. For each sample to explain, a simple decision tree is trained to mimic the behaviour of the black-box model in the neighbourhood of the sample. Both standard and counterfactual explanations can then be extracted  following the branches of the tree. 
Again based on LIME, Anchors \cite{ribeiro2018anchors}  also provides local rules of black-box model prediction via input perturbation. In this case, rules are not extracted from a decision tree but are generated by solving a Multi-Armed-Bandit beam search problem. 
Extending the CRED algorithm \cite{sato2001rule}, DeepRED  \cite{zilke2016deepred} employs a decompositional strategy to globally explain neural networks. Starting from the output nodes, each node in a layer is explained in terms of the activations of the previous one through a decision tree. In the end, all rules for each class are merged in a single global rule in terms of input nodes only. For a single example, however, a single local rule can be extracted following the firing path.

% Historically\fg{perchè historically?}, 
Intrinsic methods are generally capable to provide both local and global explanations. These explanations may be based again on feature-scoring as in Generalized Additive Models (GAM) or on FOL rules as in Decision Tree \cite{breiman1984classification} and Bayesian Rule Lists (BRL) \cite{letham2015interpretable}. Meant to overcome the non-linearity assumptions of Linear regression, GAM learns to predict the given class for each feature via decision tree. In \cite{caruana2015intelligible}, authors proposed GA$^2$M where attribute interaction is allowed at a pair level. Recently a further extension employing neural network as non-linear function has been proposed in \cite{agarwal2020neural}, which, however, lose interpretability at feature-level.
Decision trees are a greedy learning algorithm which iteratively divides input data into smaller subsets until they only contain elements belonging to the same class. Different pruning algorithms have been also proposed to simplify the resulting structure and therefore the explanations \cite{quinlan1987simplifying}. Each path of a decision tree may be seen as a decision rule i.e. an \textit{IF-THEN} statement. Decision rule methods base their classification on a set of logic rules and therefore they are probably the most interpretable ML method.
The set of rules may be generated in different ways, either with sequential covering as in \cite{cohen1995fast} or by selecting the best rules from a pre-mined set via Bayesian statistics as in BRL. 
%original:
% The approach proposed in this paper is in some sense similar to the DeepRED algorithm. LENs can explain the behaviourof a neural network either end-to-end or layer by layer.  However, on the one-side, by employing an interpretableby-design neural network as explainer, the same explainer can be used also the classify. On the other side, relying on aneural network, LEN generalization performance is much better than standard interpretable-by-design methods. Hence,the proposed approach can be both a post-hoc and an intrinsic model. Furthermore, it provides explanations in terms of FOL rules which represents the best type of explanations. In the following sections, we will see how these explanationsare extracted with different scopes, from local rules valid on a single sample to global rules valid for an entire class.

The approach proposed in this paper is in some sense similar to the DeepRED algorithm. Indeed, LENs can explain the behaviour of a neural network both end-to-end and layer by layer. Actually, LENs can be used to explain any black-box model as far as its input and output are interpretable, as we will see in a while. Further, Logic Explainer Networks can be used to solve a learning task itself, being interpretable per se. 
Employing an interpretable by-design neural network as explainer has the advantage that the explanations will perfectly match the classifier predictions. In addition, relying on a neural network, LEN generalization performance can be much better than standard interpretable-by-design methods, that generally have a very limited representation capacity. To summing up, the proposed approach can be used both as post-hoc and intrinsic model, allowing LENs to be suitable to deal with the Interpretability-versus-Accuracy
trade-off. 
The explanation type of LENs is in terms of FOL rules and different explanation styles, corresponding to different kind of logic formulas, can be expressed. Such explanations are extracted with different scopes, from local rules valid on a single sample to global rules valid for an entire class.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|ccc}
                                    & \multicolumn{2}{c|}{Explanation Type} & \multicolumn{2}{c|}{Scope} & \multicolumn{2}{c|}{Usage} & \multicolumn{3}{c}{Methodology}       \\
                                    & Feature-scoring & FOL & Local        & Global      & Intrinsic    & Post-hoc    &  Perturbation & Back-prop & Other    \\ 
\hline
LIME \cite{ribeiro2016model}                            &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           & \faCheckCircle         &               &                  \\
SHAP \cite{lundberg2017unified}                         &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           & \faCheckCircle         &               &                  \\
% DeConv \cite{zeiler2014visualizing}                     &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           & \faCheckCircle         &               &                  \\
Activation Maximization \cite{erhan2010understanding}   &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
Saliency Maps \cite{simonyan2013deep}                   &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
% Grad-CAM \cite{selvaraju2017grad}                       &\faCheckCircle&& \faCheckCircle            &            &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
SP-LIME \cite{ribeiro2016model}                         &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle           & \faCheckCircle          &              &                  \\
Class Model Visualization \cite{simonyan2013deep}       &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
% TCAV \cite{kim2018tcav}                                 &\faCheckCircle&&              & \faCheckCircle          &              & \faCheckCircle           &              & \faCheckCircle          &                  \\
LORE \cite{guidotti2018local}                         &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle & \faCheckCircle & &   \\
Anchors \cite{ribeiro2018anchors}                         &&\faCheckCircle& \faCheckCircle & &  & \faCheckCircle & \faCheckCircle & &   \\
DeepRED \cite{zilke2016deepred}                         &&\faCheckCircle& \faCheckCircle & \faCheckCircle &  & \faCheckCircle & & & \faCheckCircle  \\
GAM \cite{caruana2015intelligible}                      &\faCheckCircle&&              & \faCheckCircle          & \faCheckCircle            &             &           &              & \faCheckCircle                 \\
Decision Trees \cite{breiman1984classification}         &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &             &           &              & \faCheckCircle                 \\
BRL \cite{letham2015interpretable}                      &&\faCheckCircle& \faCheckCircle & \faCheckCircle          & \faCheckCircle            &             &           &              & \faCheckCircle                 \\
\textbf{LENs}                                           &&\faCheckCircle& \textbf{\faCheckCircle}    & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle}  & \textbf{\faCheckCircle}  & \textbf{}  & \textbf{}    & \textbf{\faCheckCircle}       \\
\end{tabular}
}
\vspace{0.1cm}
\caption{Summary of Related work 
%\fg{Ma ci sono altri modelli che hanno sia scope locale che globale? tipo quelli che poi aggregano spiegazioni locali?} \gc{SP-LIME fa proprio questo! anche BRL fa un po questo, aggregando regole però. Se ci sono altri che vi vengono in mente aggiungeteli alla tabella che poi li sistemo in giro =)}
}
\label{tab:related_work}
\end{table}


% Many authors have tried to list the characteristics of a good explanation, but in the end what will make it good or bad depends on "the degree to which a human can understand the cause of a decision" \cite{miller2019explanation}. All quality metrics are based on human perceptions. This is why we think many standard white-box models are not suitable for providing good explanations (e.g. naive Bayes classifier \cite{harry2004optimality}, k-nearest neighbors \cite{fix1951discriminatory} or logistic regression \cite{berkson1953statistically}). They were not designed for this purpose, hence their explanations are far from being useful. How good is an explanation listing the weight values of a logistic regression? Other approaches, like example-based explanations \cite{aamodt1994case,kim2016examples}, yield more intuitive explanations but their main focus is on individual predictions rather than the entire model behavior. 

% Such limitations can partially be solved using some machine learning and data mining approaches like decision trees \cite{breiman1984classification} or decision rule mining (e.g. oneR \cite{holte1993very}, RIPPER \cite{cohen1995fast}, Bayesian Rule Lists \cite{letham2015interpretable}). Decision rules provide one of the best forms of explanations by design.  

% Sometimes the easiest way to solve a learning problem is simply a black-box. This is where model-agnostic approaches come into play \cite{ribeiro2016model}. They can provide explanations for any machine learning model. The fact that many trendy techniques fall in this area is not a coincidence (e.g. LIME \cite{ribeiro2016should}, Anchors \cite{ribeiro2018anchors}, or SHAP \cite{lundberg2017unified}, Grad-cam \cite{selvaraju2017grad}). Their popularity is justified by the pressing need for unveiling the decision process of pitch-black models like deep neural networks. However, the outlook of their explanations may not live up to the expectations. The main issue is that these methodologies usually focus on scoring/ranking the input features/concepts or on providing activation maps over the input. The way concepts are interconnected is usually not explored. If I know that the concepts "head", "arms" and "wings" are needed to determine the concept "human", what do I know about their mutual relationships? Even worse, when the problem becomes more challenging (e.g. genomics) the explanations may become incomprehensible. Which biologist can make use of a ranking of thousands or millions of features (e.g. genes)?

==> supplementary_tables.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{XOR explanations}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clllll}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multicolumn{2}{c}{\textbf{Positive explanation}} &
  \multicolumn{2}{c}{\textbf{Negative explanation}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model's accuracy}}} \\
 &
  \textbf{Formula} &
  \textbf{Accuracy (\%)} &
  \textbf{Formula} &
  \textbf{Accuracy (\%)} &
  \multicolumn{1}{c}{} \\ \hline
\multirow{10}{*}{LIME} &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\ \hline
\multirow{10}{*}{Pruning} &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\ \hline
\multirow{10}{*}{$\psi$ net} &
  $((c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1))$ &
  $100.00$ &
  $( \neg c1 \wedge  \neg c2)$ &
  $88.89$ &
  $88.89$ \\
 &
  $((c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1))$ &
  $100.00$ &
  $((c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2))$ &
  $100.00$ &
  $77.78$ \\
 &
  $((c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1))$ &
  $100.00$ &
  $((c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2))$ &
  $100.00$ &
  $100.00$ \\
 &
  $((c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1))$ &
  $100.00$ &
  $(c2 \vee  \neg c1)$ &
  $44.44$ &
  $44.44$ \\
 &
  $((c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1))$ &
  $100.00$ &
  $((c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2))$ &
  $100.00$ &
  $77.78$ \\
 &
  $(c2 \wedge  \neg c1)$ &
  $77.78$ &
  $((c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2))$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c2 \wedge  \neg c1)$ &
  $77.78$ &
  $( \neg c1 \wedge  \neg c2)$ &
  $88.89$ &
  $44.44$ \\
 &
  $(c1 \wedge  \neg c2)$ &
  $44.44$ &
  $((c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2))$ &
  $100.00$ &
  $100.00$ \\
 &
  $((c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1))$ &
  $100.00$ &
  $(c1 \wedge c2)$ &
  $88.89$ &
  $77.78$ \\
 &
  $(c1 \vee c2)$ &
  $100.00$ &
  $(c1 \vee  \neg c2)$ &
  $77.78$ &
  $77.78$ \\ \hline
\multirow{10}{*}{Decision tree} &
  $(c2  \leq  0.50 \wedge c1 > 0.50) \vee (c2 > 0.50 \wedge c1  \leq  0.50)$ &
  $100.00$ &
  $(c2  \leq  0.50 \wedge c1  \leq  0.50) \vee (c2 > 0.50 \wedge c1 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1  \leq  0.50 \wedge c2 > 0.50) \vee (c1 > 0.50 \wedge c2  \leq  0.50)$ &
  $100.00$ &
  $(c1  \leq  0.50 \wedge c2  \leq  0.50) \vee (c1 > 0.50 \wedge c2 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1  \leq  0.50 \wedge c2 > 0.50) \vee (c1 > 0.50 \wedge c2  \leq  0.50)$ &
  $100.00$ &
  $(c1  \leq  0.50 \wedge c2  \leq  0.50) \vee (c1 > 0.50 \wedge c2 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1  \leq  0.50 \wedge c2 > 0.50) \vee (c1 > 0.50 \wedge c2  \leq  0.50)$ &
  $100.00$ &
  $(c1  \leq  0.50 \wedge c2  \leq  0.50) \vee (c1 > 0.50 \wedge c2 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1  \leq  0.50 \wedge c2 > 0.50) \vee (c1 > 0.50 \wedge c2  \leq  0.50)$ &
  $100.00$ &
  $(c1  \leq  0.50 \wedge c2  \leq  0.50) \vee (c1 > 0.50 \wedge c2 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c2  \leq  0.50 \wedge c1 > 0.50) \vee (c2 > 0.50 \wedge c1  \leq  0.50)$ &
  $100.00$ &
  $(c2  \leq  0.50 \wedge c1  \leq  0.50) \vee (c2 > 0.50 \wedge c1 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1  \leq  0.50 \wedge c2 > 0.50) \vee (c1 > 0.50 \wedge c2  \leq  0.50)$ &
  $100.00$ &
  $(c1  \leq  0.50 \wedge c2  \leq  0.50) \vee (c1 > 0.50 \wedge c2 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c2  \leq  0.50 \wedge c1 > 0.50) \vee (c2 > 0.50 \wedge c1  \leq  0.50)$ &
  $100.00$ &
  $(c2  \leq  0.50 \wedge c1  \leq  0.50) \vee (c2 > 0.50 \wedge c1 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c2  \leq  0.50 \wedge c1 > 0.50) \vee (c2 > 0.50 \wedge c1  \leq  0.50)$ &
  $100.00$ &
  $(c2  \leq  0.50 \wedge c1  \leq  0.50) \vee (c2 > 0.50 \wedge c1 > 0.50)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1  \leq  0.50 \wedge c2 > 0.50) \vee (c1 > 0.50 \wedge c2  \leq  0.50)$ &
  $100.00$ &
  $(c1  \leq  0.50 \wedge c2  \leq  0.50) \vee (c1 > 0.50 \wedge c2 > 0.50)$ &
  $100.00$ &
  $100.00$ \\ \hline
\multirow{10}{*}{ReLU} &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c2$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $ \neg c1 \vee  \neg c2$ &
  $100.00$ &
  $c2 \vee  \neg c1$ &
  $44.44$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\
 &
  $(c1 \wedge  \neg c2) \vee (c2 \wedge  \neg c1)$ &
  $100.00$ &
  $(c1 \wedge c2) \vee ( \neg c1 \wedge  \neg c2)$ &
  $100.00$ &
  $100.00$ \\ \hline
\end{tabular}%
}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{MNIST explanations}
\label{tab:exp_formula_mnist_cbm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|p{10cm}|l|p{10cm}|ll}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multicolumn{2}{c}{\textbf{Odd explanation}} &
  \multicolumn{2}{c}{\textbf{Even explanation}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model's accuracy}}} \\
 &
  \textbf{Formula} &
  \textbf{Accuracy (\%)} &
  \textbf{Formula} &
  \textbf{Accuracy (\%)} &
  \multicolumn{1}{c}{} \\ \hline
\multirow{10}{*}{Pruning} &
  $ \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8$ &
  $100.00$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $ \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8$ &
  $100.00$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $ \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8$ &
  $100.00$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $ \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8$ &
  $100.00$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\ \hline
\multirow{10}{*}{$\psi$ net} &
  $(c7 \wedge  \neg c4)$ &
  $59.54$ &
  $( \neg c3 \wedge  \neg c5)$ &
  $68.28$ &
  $89.91$ \\
 &
  $( \neg c4 \wedge (c1 \vee c3) \wedge (c1 \vee  \neg c8))$ &
  $49.13$ &
  $( \neg c1 \wedge (c0 \vee c6) \wedge (c0 \vee  \neg c3) \wedge (c4 \vee  \neg c5))$ &
  $58.18$ &
  $79.63$ \\
 &
  $( \neg c8 \wedge (c1 \vee  \neg c2) \wedge (c3 \vee  \neg c0) \wedge ( \neg c2 \vee  \neg c6))$ &
  $19.56$ &
  $( \neg c1 \wedge  \neg c9 \wedge (c0 \vee  \neg c7))$ &
  $59.54$ &
  $80.98$ \\
 &
  $(c7 \vee c9 \vee ( \neg c4 \wedge  \neg c8) \vee (c3 \wedge  \neg c0 \wedge  \neg c4))$ &
  $39.83$ &
  $( \neg c3 \wedge (c2 \vee c4 \vee c8) \wedge (c2 \vee c8 \vee  \neg c7))$ &
  $59.54$ &
  $80.62$ \\
 &
  $( \neg c4 \wedge  \neg c8 \wedge (c7 \vee  \neg c6) \wedge (c9 \vee  \neg c2))$ &
  $40.69$ &
  $((c0 \wedge c8) \vee (c2 \wedge c8) \vee (c0 \wedge  \neg c1) \vee (c2 \wedge  \neg c1) \vee ( \neg c5 \wedge  \neg c7))$ &
  $68.46$ &
  $90.18$ \\
 &
  $( \neg c0 \wedge  \neg c2 \wedge  \neg c6 \wedge  \neg c8)$ &
  $90.18$ &
  $( \neg c5 \wedge (c4 \vee  \neg c9))$ &
  $59.35$ &
  $68.27$ \\
 &
  $(c5 \wedge  \neg c4)$ &
  $58.18$ &
  $(c0 \vee c2 \vee c4 \vee c6)$ &
  $90.26$ &
  $90.26$ \\
 &
  $( \neg c2 \wedge  \neg c8 \wedge (c1 \vee  \neg c0) \wedge (c9 \vee  \neg c4))$ &
  $39.12$ &
  $(c0 \vee c6 \vee (c8 \wedge  \neg c7))$ &
  $79.86$ &
  $79.86$ \\
 &
  $( \neg c0 \vee  \neg c6)$ &
  $29.88$ &
  $( \neg c1 \wedge  \neg c3 \wedge (c6 \vee  \neg c9) \wedge ( \neg c7 \vee  \neg c9))$ &
  $59.35$ &
  $91.08$ \\
 &
  $( \neg c0 \wedge  \neg c2 \wedge  \neg c6 \wedge  \neg c8)$ &
  $90.18$ &
  $( \neg c1 \wedge  \neg c3 \wedge (c2 \vee  \neg c9))$ &
  $59.35$ &
  $80.80$ \\ \hline
\multirow{10}{*}{Decision tree} &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h5 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\
 &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1  \leq  0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6  \leq  0.50 \wedge h1 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8  \leq  0.50 \wedge h6 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2  \leq  0.50 \wedge h8 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7  \leq  0.50 \wedge h2 > 0.50)$ &
  $97.95$ &
  $(h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h7 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h4  \leq  0.50 \wedge h0  \leq  0.50 \wedge h9 > 0.50) \vee (h4  \leq  0.50 \wedge h0 > 0.50) \vee (h4 > 0.50)$ &
  $97.95$ &
  $97.95$ \\ \hline
\multirow{10}{*}{ReLU} &
  $c1 \vee c5 \vee c9 \vee ( \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8)$ &
  $69.64$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c3$ &
  $59.36$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $c9 \vee ( \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8)$ &
  $89.91$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $c0 \vee ( \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9)$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\
 &
  $( \neg c0 \wedge  \neg c2 \wedge  \neg c7 \wedge  \neg c8) \vee ( \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8)$ &
  $40.14$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $ \neg c0 \wedge  \neg c2 \wedge  \neg c4 \wedge  \neg c6 \wedge  \neg c8$ &
  $100.00$ &
  $c0 \vee c2 \vee c4 \vee c6 \vee c8$ &
  $100.00$ &
  $100.00$ \\
 &
  $c1 \vee c3 \vee c5 \vee c7 \vee c9$ &
  $100.00$ &
  $ \neg c1 \wedge  \neg c3 \wedge  \neg c5 \wedge  \neg c7 \wedge  \neg c9$ &
  $100.00$ &
  $100.00$ \\ \hline
\end{tabular}%
}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{MNIST (hidden) explanations}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|p{10cm}|l|p{10cm}|ll}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multicolumn{2}{c}{\textbf{Positive explanation}} &
  \multicolumn{2}{c}{\textbf{Negative explanation}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model's accuracy}}} \\
 &
  \textbf{Formula} &
  \textbf{Accuracy (\%)} &
  \textbf{Formula} &
  \textbf{Accuracy (\%)} &
  \multicolumn{1}{c}{} \\ \hline
\multirow{10}{*}{Pruning} &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\ \hline
\multirow{10}{*}{$\psi$ net} &
  $(h0 \vee h2 \vee  \neg h1)$ &
  $52.02$ &
  $( \neg h4 \wedge  \neg h5 \wedge (h6 \vee  \neg h7))$ &
  $56.63$ &
  $71.43$ \\
 &
  $((h2 \vee h5) \wedge (h2 \vee  \neg h1) \wedge (h5 \vee  \neg h3) \wedge ( \neg h1 \vee  \neg h3))$ &
  $28.47$ &
  $( \neg h4 \wedge  \neg h5 \wedge (h1 \vee h3))$ &
  $78.74$ &
  $78.74$ \\
 &
  $( \neg h1 \wedge (h2 \vee  \neg h9) \wedge (h0 \vee h7 \vee  \neg h6))$ &
  $30.72$ &
  $( \neg h0 \wedge  \neg h2 \wedge  \neg h5 \wedge  \neg h7)$ &
  $84.57$ &
  $84.57$ \\
 &
  $((h2 \wedge h5) \vee (h2 \wedge  \neg h3) \vee (h2 \wedge  \neg h9) \vee (h5 \wedge  \neg h3) \vee (h7 \wedge  \neg h6) \vee ( \neg h3 \wedge  \neg h9))$ &
  $40.02$ &
  $(h1 \vee h3 \vee h6 \vee h9)$ &
  $99.28$ &
  $99.28$ \\
 &
  $( \neg h1 \wedge  \neg h6 \wedge (h2 \vee h7))$ &
  $72.44$ &
  $(h1 \vee h9 \vee (h3 \wedge  \neg h2 \wedge  \neg h5))$ &
  $92.42$ &
  $92.42$ \\
 &
  $(h2 \wedge  \neg h6 \wedge  \neg h9)$ &
  $65.07$ &
  $(h9 \wedge  \neg h5 \wedge  \neg h7)$ &
  $64.42$ &
  $75.13$ \\
 &
  $(h0 \vee h2 \vee h5)$ &
  $77.20$ &
  $(h6 \vee (h3 \wedge  \neg h2 \wedge  \neg h4))$ &
  $64.81$ &
  $71.44$ \\
 &
  $(h2 \wedge  \neg h3)$ &
  $65.07$ &
  $(h3 \vee h6)$ &
  $64.81$ &
  $64.81$ \\
 &
  $((h2 \vee  \neg h9) \wedge (h4 \vee  \neg h6) \wedge (h5 \vee  \neg h1))$ &
  $40.92$ &
  $((h9 \vee  \neg h0) \wedge (h9 \vee  \neg h5) \wedge (h3 \vee h6 \vee h9) \wedge ( \neg h0 \vee  \neg h7) \wedge ( \neg h5 \vee  \neg h7) \wedge (h3 \vee h6 \vee  \neg h7))$ &
  $56.63$ &
  $78.49$ \\
 &
  $( \neg h1 \wedge  \neg h3 \wedge (h2 \vee  \neg h9))$ &
  $48.61$ &
  $( \neg h4)$ &
  $55.63$ &
  $75.14$ \\ \hline
\multirow{10}{*}{Decision tree} &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\
 &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7  \leq  0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2  \leq  0.50 \wedge h7 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8  \leq  0.50 \wedge h2 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6  \leq  0.50 \wedge h8 > 0.50)$ &
  $99.28$ &
  $(h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3  \leq  0.50 \wedge h6 > 0.50) \vee (h1  \leq  0.50 \wedge h9  \leq  0.50 \wedge h3 > 0.50) \vee (h1  \leq  0.50 \wedge h9 > 0.50) \vee (h1 > 0.50)$ &
  $99.28$ &
  $99.28$ \\ \hline
\multirow{10}{*}{ReLU} &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee ( \neg h0 \wedge  \neg h2 \wedge  \neg h4 \wedge  \neg h7 \wedge  \neg h8)$ &
  $90.85$ &
  $99.28$ \\
 &
  $h2 \vee  \neg h6$ &
  $41.79$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $h2 \vee h7 \vee h8 \vee ( \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9)$ &
  $67.76$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $( \neg h3 \wedge  \neg h7) \vee ( \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9)$ &
  $15.30$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $h2 \vee ( \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9)$ &
  $83.47$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $( \neg h0 \wedge  \neg h1 \wedge  \neg h2) \vee ( \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9)$ &
  $41.02$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\
 &
  $ \neg h1 \wedge  \neg h3 \wedge  \neg h6 \wedge  \neg h9$ &
  $99.28$ &
  $h1 \vee h3 \vee h6 \vee h9$ &
  $99.28$ &
  $99.28$ \\ \hline
\end{tabular}%
}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Cell differentiation explanations (* the explanation is too complex)}
\label{tab:exp_formula_celldiff}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|p{8cm}|l|p{8cm}|lll}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multicolumn{2}{c}{\textbf{Positive explanation}} &
  \multicolumn{2}{c}{\textbf{Negative explanation}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model's accuracy (\%)}}} \\
 &
  \multicolumn{1}{c}{\textbf{Formula}} &
  \multicolumn{1}{c}{\textbf{Accuracy (\%)}} &
  \multicolumn{1}{c}{\textbf{Formula}} &
  \multicolumn{1}{c}{\textbf{Accuracy (\%)}} &
  \multicolumn{1}{c}{} \\ \hline
\multirow{10}{*}{\textbf{Pruning}} &
  $pcxa \wedge nr2c2 \wedge kat6b \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg dnajc28 \wedge  \neg oraov1 \wedge  \neg igic1s1 \wedge  \neg clmn \wedge  \neg prune2$ &
  $90.91$ &
  $prune2 \wedge nr2c2 \wedge kat6b \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg dnajc28 \wedge  \neg oraov1 \wedge  \neg igic1s1 \wedge  \neg pcxa \wedge  \neg clmn$ &
  $27.97$ &
  $93.71$ \\
 &
  $anxa3b \wedge dpysl5b \wedge pcxa \wedge nr2c2 \wedge kat6b \wedge  \neg Unnamed: 168 \wedge  \neg im:7151449 \wedge  \neg oraov1 \wedge  \neg eif4g2b \wedge  \neg clmn \wedge  \neg rgs11$ &
  $89.51$ &
  $nr2c2 \wedge  \neg pcxa \wedge  \neg clmn$ &
  $45.45$ &
  $94.41$ \\
 &
  $si:ch211-132g1.1 \wedge nr2c2 \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg oraov1 \wedge  \neg Unnamed: 419 \wedge  \neg hif1al2 \wedge  \neg eif4g2b \wedge  \neg zdhhc5a \wedge  \neg clmn \wedge  \neg nanos1 \wedge  \neg adora2aa$ &
  $89.44$ &
  $eif4g2b \wedge  \neg si:ch211-132g1.1$ &
  $33.80$ &
  $92.96$ \\
 &
  $dpysl5b \wedge pcxa \wedge nr2c2 \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg si:dkey-183p4.10 \wedge  \neg lect2l \wedge  \neg im:7151449 \wedge  \neg smim14 \wedge  \neg oraov1 \wedge  \neg igic1s1 \wedge  \neg otud4.4 \wedge  \neg eif2ak1 \wedge  \neg anxa11a \wedge  \neg TMC8 \wedge  \neg zgc:158427 \wedge  \neg HHEX \wedge  \neg clmn \wedge  \neg oxsr1a \wedge  \neg lpar1$ &
  $90.14$ &
  $smim14 \wedge otud4.4 \wedge  \neg TMC8 \wedge  \neg HHEX \wedge  \neg oxsr1a \wedge  \neg lpar1$ &
  $40.85$ &
  $95.07$ \\
 &
  $nr2c2 \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg oraov1 \wedge  \neg igic1s1 \wedge  \neg eif4g2b \wedge  \neg zdhhc5a \wedge  \neg clmn$ &
  $75.35$ &
  $eif4g2b$ &
  $33.10$ &
  $91.55$ \\
 &
  $SLC16A3 \wedge pcxa \wedge nr2c2 \wedge kat6b \wedge  \neg CD37 \wedge  \neg Unnamed: 168 \wedge  \neg im:7151449 \wedge  \neg si:ch73-359m17.5 \wedge  \neg si:dkeyp-44a8.2 \wedge  \neg otud4.4 \wedge  \neg eif2ak1 \wedge  \neg anxa11a \wedge  \neg CABIN1 \wedge  \neg SBNO2 \wedge  \neg mgrn1b \wedge  \neg clmn$ &
  $85.21$ &
  $mgrn1b \wedge  \neg pcxa$ &
  $39.44$ &
  $90.14$ \\
 &
  $ap5z1 \wedge pcxa \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg si:dkey-183p4.10 \wedge  \neg si:ch73-359m17.5 \wedge  \neg si:dkeyp-44a8.2 \wedge  \neg igic1s1 \wedge  \neg hinfp \wedge  \neg zgc:154055 \wedge  \neg tbc1d25 \wedge  \neg eif2ak1 \wedge  \neg anxa11a \wedge  \neg nemp2 \wedge  \neg atxn3 \wedge  \neg eif4g2b \wedge  \neg got2a \wedge  \neg si:dkey-9i23.5 \wedge  \neg zdhhc5a \wedge  \neg clmn \wedge  \neg nanos1$ &
  $85.92$ &
  $ \neg zgc:154055 \wedge  \neg pcxa$ &
  $47.18$ &
  $92.25$ \\
 &
  $ap5z1 \wedge pcxa \wedge  \neg eif4g2b \wedge  \neg mgrn1b \wedge  \neg oxsr1a \wedge  \neg kdelc2$ &
  $91.55$ &
  $kdelc2 \wedge  \neg pcxa \wedge  \neg clmn$ &
  $43.66$ &
  $95.07$ \\
 &
  $ \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg si:dkey-183p4.10 \wedge  \neg oraov1 \wedge  \neg Unnamed: 419 \wedge  \neg igic1s1 \wedge  \neg otud4.4 \wedge  \neg anxa11a \wedge  \neg eif4g2b \wedge  \neg asap2b \wedge  \neg timm17a \wedge  \neg clmn \wedge  \neg rgs11 \wedge  \neg ADM$ &
  $88.73$ &
  $otud4.4 \wedge eif4g2b \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg si:dkey-183p4.10 \wedge  \neg oraov1 \wedge  \neg Unnamed: 419 \wedge  \neg igic1s1$ &
  $26.06$ &
  $92.96$ \\
 &
  $pcxa \wedge kat6b \wedge  \neg CD37 \wedge  \neg im:7151449 \wedge  \neg igic1s1 \wedge  \neg anxa11a \wedge  \neg eif4g2b \wedge  \neg clmn$ &
  $85.92$ &
  $ \neg CD37 \wedge  \neg im:7151449 \wedge  \neg igic1s1 \wedge  \neg pcxa \wedge  \neg clmn$ &
  $47.89$ &
  $90.85$ \\ \hline
\multirow{10}{*}{\textbf{$\psi$ net}} &
  $(False)$ &
  $0.00$ &
  $( \neg clmn \wedge (si:ch211-103n10.5 \vee oraov1))$ &
  $53.15$ &
  $83.92$ \\
 &
  $(im:7151449 \vee ( \neg si:ch211-103n10.5 \wedge  \neg anxa11a))$ &
  $32.17$ &
  $(si:ch211-103n10.5)$ &
  $30.07$ &
  $82.52$ \\
 &
  $(im:7151449 \wedge  \neg si:ch211-103n10.5)$ &
  $81.69$ &
  $(si:ch211-103n10.5 \vee  \neg im:7151449)$ &
  $81.69$ &
  $81.69$ \\
 &
  $(clmn)$ &
  $83.10$ &
  $(True)$ &
  $0.00$ &
  $83.10$ \\
 &
  $(im:7151449 \vee clmn \vee  \neg si:ch211-103n10.5)$ &
  $28.17$ &
  $(si:ch211-103n10.5)$ &
  $30.99$ &
  $83.10$ \\
 &
  $(False)$ &
  $0.00$ &
  $(si:ch211-103n10.5)$ &
  $29.58$ &
  $83.10$ \\
 &
  $(clmn \vee (im:7151449 \wedge  \neg si:ch211-103n10.5))$ &
  $84.51$ &
  $( \neg clmn)$ &
  $83.10$ &
  $81.69$ \\
 &
  $(clmn \vee (im:7151449 \wedge  \neg si:ch211-103n10.5))$ &
  $84.51$ &
  $(si:ch211-103n10.5)$ &
  $30.99$ &
  $84.51$ \\
 &
  $(pcxa \vee clmn)$ &
  $73.24$ &
  $( \neg clmn)$ &
  $83.80$ &
  $84.51$ \\
 &
  $(clmn)$ &
  $82.39$ &
  $( \neg clmn)$ &
  $82.39$ &
  $82.39$ \\ \hline
\multirow{10}{*}{\textbf{Decision tree}} &
  * &
  $88.81$ &
  * &
  $88.81$ &
  $88.81$ \\
 &
  * &
  $90.91$ &
  * &
  $90.91$ &
  $90.91$ \\
 &
  * &
  $91.55$ &
  * &
  $91.55$ &
  $91.55$ \\
 &
  * &
  $90.85$ &
  * &
  $90.85$ &
  $90.85$ \\
 &
  * &
  $94.37$ &
  * &
  $94.37$ &
  $94.37$ \\
 &
  * &
  $92.25$ &
  * &
  $92.25$ &
  $92.25$ \\
 &
  * &
  $94.37$ &
  * &
  $94.37$ &
  $94.37$ \\
 &
  * &
  $91.55$ &
  * &
  $91.55$ &
  $91.55$ \\
 &
  * &
  $91.55$ &
  * &
  $91.55$ &
  $91.55$ \\
 &
  * &
  $92.96$ &
  * &
  $92.96$ &
  $92.96$ \\ \hline
\multirow{10}{*}{\textbf{ReLU}} &
  $pcxa \wedge nr2c2 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg oraov1 \wedge  \neg clmn \wedge  \neg marcksl1b \wedge  \neg tm9sf3$ &
  $77.62$ &
  $otud4.4 \wedge  \neg pcxa \wedge  \neg clmn \wedge  \neg kdelc2$ &
  $25.17$ &
  $95.80$ \\
 &
  $pcxa \wedge  \neg si:ch211-103n10.5 \wedge  \neg kdelc2$ &
  $83.22$ &
  $pcxa \wedge  \neg si:ch211-103n10.5 \wedge  \neg kdelc2$ &
  $16.78$ &
  $94.41$ \\
 &
  $pcxa \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg otud4.4 \wedge  \neg clmn$ &
  $82.39$ &
  $ \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg otud4.4 \wedge  \neg clmn$ &
  $54.23$ &
  $96.48$ \\
 &
  $si:ch211-132g1.1 \wedge pcxa \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg otud4.4 \wedge  \neg eif2ak1 \wedge  \neg clmn \wedge  \neg marcksl1b \wedge  \neg kdelc2$ &
  $90.14$ &
  $eif2ak1 \wedge dpysl5b \wedge SLC16A3 \wedge asb12a \wedge kat6b \wedge kdelc2 \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg anxa11a \wedge  \neg mgrn1b$ &
  $32.39$ &
  $97.18$ \\
 &
  $si:ch211-132g1.1 \wedge pcxa \wedge nr2c2 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg oraov1 \wedge  \neg otud4.4 \wedge  \neg anxa11a \wedge  \neg clmn \wedge  \neg marcksl1b \wedge  \neg kdelc2$ &
  $88.73$ &
  $otud4.4 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg oraov1 \wedge  \neg anxa11a \wedge  \neg clmn \wedge  \neg kdelc2$ &
  $40.14$ &
  $98.59$ \\
 &
  $si:ch211-132g1.1 \wedge pcxa \wedge nr2c2 \wedge  \neg si:ch211-137j23.8 \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg oraov1 \wedge  \neg hinfp \wedge  \neg otud4.4 \wedge  \neg anxa11a \wedge  \neg atp2b4 \wedge  \neg clmn \wedge  \neg marcksl1b$ &
  $86.62$ &
  $oraov1 \wedge dpysl5b \wedge asb12a \wedge kat6b \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg otud4.4 \wedge  \neg anxa11a \wedge  \neg clmn \wedge  \neg marcksl1b$ &
  $32.39$ &
  $93.66$ \\
 &
  $pcxa \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg clmn \wedge  \neg kdelc2$ &
  $79.58$ &
  $ \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg clmn \wedge  \neg kdelc2$ &
  $38.73$ &
  $97.18$ \\
 &
  $si:ch211-132g1.1 \wedge pcxa \wedge nr2c2 \wedge kat6b \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg zgc:113377 \wedge  \neg otud4.4 \wedge  \neg clmn \wedge  \neg marcksl1b \wedge  \neg oxsr1a \wedge  \neg kdelc2$ &
  $90.85$ &
  $dpysl5b \wedge SLC16A3 \wedge asb12a \wedge kat6b \wedge  \neg si:ch211-103n10.5$ &
  $65.49$ &
  $95.77$ \\
 &
  $si:ch211-132g1.1 \wedge pcxa \wedge nr2c2 \wedge  \neg si:ch211-103n10.5 \wedge  \neg znf1034 \wedge  \neg smim14 \wedge  \neg oraov1 \wedge  \neg Unnamed: 419 \wedge  \neg otud4.4 \wedge  \neg anxa11a \wedge  \neg clmn \wedge  \neg marcksl1b \wedge  \neg kdelc2$ &
  $88.73$ &
  $smim14 \wedge otud4.4 \wedge pcxa \wedge nr2c2 \wedge  \neg si:ch211-137j23.8 \wedge  \neg si:ch211-103n10.5 \wedge  \neg znf1034 \wedge  \neg oraov1 \wedge  \neg Unnamed: 419 \wedge  \neg anxa11a \wedge  \neg clmn \wedge  \neg marcksl1b \wedge  \neg kdelc2$ &
  $17.61$ &
  $94.37$ \\
 &
  $pcxa \wedge  \neg si:ch211-103n10.5 \wedge  \neg im:7151449 \wedge  \neg otud4.4 \wedge  \neg CABIN1 \wedge  \neg clmn \wedge  \neg kdelc2$ &
  $83.10$ &
  $asb12a \wedge kat6b \wedge kdelc2 \wedge  \neg CD37 \wedge  \neg si:ch211-103n10.5 \wedge  \neg otud4.4 \wedge  \neg anxa11a \wedge  \neg CABIN1 \wedge  \neg pcxa \wedge  \neg clmn$ &
  $32.39$ &
  $96.48$ \\ \hline
\end{tabular}%
}
\end{table}

==> tikz/framework.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,211); %set diagram left start at 0, and has height of 211

%Shape: Rectangle [id:dp6273289469520551] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 106; blue, 159 }  ,fill opacity=1 ][line width=1.5]  (10,10) -- (560,10) -- (560,200) -- (10,200) -- cycle ;
%Shape: Rectangle [id:dp45052430143816535] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (20,60) -- (280,60) -- (280,190) -- (20,190) -- cycle ;
%Shape: Rectangle [id:dp588387099922177] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (290,60) -- (550,60) -- (550,190) -- (290,190) -- cycle ;
%Shape: Rectangle [id:dp7086572015675848] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (30.75,68.8) -- (270,68.8) -- (270,108.8) -- (30.75,108.8) -- cycle ;
%Shape: Rectangle [id:dp26433045196828997] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (300,68.8) -- (540,68.8) -- (540,108.8) -- (300,108.8) -- cycle ;

% Text Node
\draw (100,79) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textbf{{\large P}IPELINE }\large{[\ref{sec:use_cases}]}};
% Text Node
\draw (31,118.8) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{0,0.42,0.62}{- End-to-end explainer [Fig. \ref{fig:E2EExplainer}]}\\\textcolor[rgb]{0,0.42,0.62}{- Concept-bottleneck explainer [Fig. \ref{fig:CMBExplainer}]}\\\textcolor[rgb]{0,0.42,0.62}{- Cascading explainers [Fig. \ref{fig:CascadeExplainer}]}};
% Text Node
\draw (303,79) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=center] {\textbf{{\large L}EARNING \& {\large E}XPLANATIONS} \large{[\ref{sec:explanation_styles}]}};
% Text Node
\draw (301,118.8) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {
\textcolor[rgb]{0,0.42,0.62}{- Supervised explanations [Fig. \ref{fig:explainablevsexplanation}]}\\
\textcolor[rgb]{0,0.42,0.62}{\quad - \textit{Interpretable Classification}}\\
\textcolor[rgb]{0,0.42,0.62}{\quad - \textit{Explaining a Black-Box model}}\\

\textcolor[rgb]{0,0.42,0.62}{- Unsupervised explanations [Fig. \ref{fig:concept_relations}]}};
% Text Node
\hypersetup{linkcolor=white}
\draw (139, 27) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\textbf{ LENs: Logic Explainer Networks} \textcolor{white}{[{\color{white}\ref{sec:basics}}}]};
\hypersetup{linkcolor=blue}


\end{tikzpicture}


==> tikz/methods.tex <==

\resizebox{\textwidth}{!}{%
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,205); %set diagram left start at 0, and has height of 205

%Shape: Rectangle [id:dp5586184407473809] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 106; blue, 159 }  ,fill opacity=1 ][line width=1.5]  (10,10) -- (830,10) -- (830,200) -- (10,200) -- cycle ;
%Shape: Rectangle [id:dp09671327261989882] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (20,59.4) -- (280,59.4) -- (280,190) -- (20,190) -- cycle ;
%Shape: Rectangle [id:dp14940644485572818] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (290,59.4) -- (550,59.4) -- (550,190) -- (290,190) -- cycle ;
%Shape: Rectangle [id:dp7527437777291323] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (560,59.4) -- (820,59.4) -- (820,190) -- (560,190) -- cycle ;
%Shape: Rectangle [id:dp6959026208112672] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (30.75,68.8) -- (270,68.8) -- (270,108.8) -- (30.75,108.8) -- cycle ;
%Shape: Rectangle [id:dp4021455240767876] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (300,68.8) -- (540,68.8) -- (540,108.8) -- (300,108.8) -- cycle ;
%Shape: Rectangle [id:dp9828854452944691] 
\draw  [color={rgb, 255:red, 0; green, 106; blue, 159 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (570,68.8) -- (810,68.8) -- (810,108.8) -- (570,108.8) -- cycle ;

% Text Node
\draw (58,79) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textbf{{\large L}ERNING CRITERIA {\large [\ref{sec:learncrit}]}}};
% Text Node
\draw (31,118.8) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{0,0.42,0.62}{- Supervised criteria}\\\textcolor[rgb]{0,0.42,0.62}{- Unsupervised criteria}};
% Text Node
\draw (305,78) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textbf{{\large FOL }RULE EXTRACTION {\large [\ref{sec:logic_rule_extr}]}}};
% Text Node
\draw (583,78.8) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textbf{{\large P}ARSIMONY CRITERIA {\large [\ref{sec:parsimony}]}}};
% Text Node
\draw (303,119) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{0,0.42,0.62}{- Example-level explanation}\\\textcolor[rgb]{0,0.42,0.62}{- Cluster-level explanation}\\\textcolor[rgb]{0,0.42,0.62}{- Class-level explanation}};
% Text Node
\draw (571,118) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 106; blue, 159 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{0,0.42,0.62}{- L1 regularization}\\\textcolor[rgb]{0,0.42,0.62}{- Pruning strategies}};
% Text Node
\hypersetup{linkcolor=white}
\draw (317,22) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\textbf{LENs M{\small ETHODS } [\ref{sec:methods}]}};
\hypersetup{linkcolor=blue}


\end{tikzpicture}

}%
